Two Sides of the Same Coin: Heterophily and Oversmoothing in Graph Convolutional Neural Networks

In node classification tasks, graph convolutional neural networks (GCNs) have demonstrated competitive performance over traditional methods on diverse graph data. However, it is known that the performance of GCNs degrades with increasing number of layers (oversmoothing problem) and recent studies have also shown that GCNs may perform worse in heterophilous graphs, where neighboring nodes tend to belong to different classes (heterophily problem). These two problems are usually viewed as unrelated, and thus are studied independently, often at the graph filter level from a spectral perspective. We are the first to take a unified perspective to jointly explain the oversmoothing and heterophily problems at the node level. Specifically, we profile the nodes via two quantitative metrics: the relative degree of a node (compared to its neighbors) and the node-level heterophily. Our theory shows that the interplay of these two profiling metrics defines three cases of node behaviors, which explain the oversmoothing and heterophily problems jointly and can predict the performance of GCNs. Based on insights from our theory, we show theoretically and empirically the effectiveness of two strategies: structure-based edge correction, which learns corrected edge weights from structural properties (i.e., degrees), and feature-based edge correction, which learns signed edge weights from node features. Compared to other approaches, which tend to handle well either heterophily or oversmoothing, we show that {our model, GGCN}, which incorporates the two strategies performs well in both problems.

==> sections/introduction.tex <==
\vspace{-1cm}
\section{Introduction}
% \yy{Reminder to check notations: 1. we use features to represent 0-th layer representations. 2. $\rvf_i$ needs to specify layers 3. we say movements of (node) representations instead of movements of nodes 4. We use GCN in all places and say vanilla GCN to refer to the kipf's model 5. do not mention linear separability 6. check if there is overlapping of letters 7. labels of nodes have changed, check if missing anything}
\label{section: introduction}
\vspace{-0.25cm}
% \begin{itemize}
%     \item Bring up the two problems: limitations in heterophilous graphs; over-smoothing problem
%     \item Some works (ICML, NeurIPS), one is trying to solve heterophily, but accidentally quite good in oversmoothing; one aims to solve oversmoothing, but decent performance in heterophilous graphs (compared vanilla GCN).  Whether two problems are inherently correlated. 
%     \item No papers are trying to bridge the two problems from a theoretical perspective. Intuition of theoretic analysis. Study a simple synthetic case. Study the message passing. Sign \& Degree leads to the two problems
%     \item Contributions: Theoretical + empirical validation
% \end{itemize}

% \reminder{Check for consistency: "homophilous / heterophilous" graphs}
In recent years, GCNs~\citep{defferrard2016convolutional, kipf2016semi, velivckovic2017graph} have been widely used in %gained attention due to their 
applications ranging from social science~\citep{li2019encoding} and biology~\citep{yan2019groupinn} to program understanding~\citep{allamanis2018learning,shi2019learning}. A typical GCN architecture~\citep{gilmer2017neural} for the node classification task can be decomposed into two {main components}: propagation/aggregation, and combination. 
% Messages are first sent out by the neighborhood nodes, then aggregated. 
Messages are first exchanged between neighboring nodes, then aggregated. 
Afterwards, the messages are combined with the self-representations (a.k.a., the current node representations) to update the node representations. %The representations of the final layers are used to compute the losses. 
Though GCNs are effective, %~\citep{defferrard2016convolutional}, 
they have some key limitations.
%researchers have also identified limitations.

The first limitation is the ``oversmoothing" problem~\citep{li2018deeper}: the performance of GCNs degrade when stacking many layers. Recent work has found that oversmoothing could be caused by GCNs exponentially losing expressive power in the node classification task~\citep{oono2019graph} and that the node representations converge to a stationary state which is decided by the degree of the nodes and the input features~\citep{chen2020simple, wang2019improving, rong2019dropedge,RossiJSAKL2020}. These works focus on the analysis of the steady state in the limit of infinite layers, but they do not explore the dynamics on how oversmoothing is triggered, or which nodes tend to cause it. 
Other works like~\citep{xu2018representation, wang2019improving, chen2020simple} focus 
%To date, 
on heuristic-based model designs to alleviate the oversmoothing problem. 
To fill this gap, we seek to theoretically analyze the dynamics around oversmoothing.
%Our focus is to examine the dynamics around oversmoothing in this paper.
{In our  empirical analysis, by dividing the nodes in real graphs into several degree groups  
and tracking their average accuracy while increasing the layers of GCN~\citep{kipf2016semi}, we observe two phases (Fig.~\ref{fig:phase_transition}): the initial stage when higher-degree nodes have higher accuracy and the developing stage when the accuracy of higher-degree nodes decreases more sharply (cf.\ \S~\ref{exp:case study} for details). As we will show theoretically and empirically, the low-degree nodes are the ones that trigger oversmoothing. %\yy{The definition of effective homophily and more discussion of
% We discuss 
% Fig.~\ref{fig:phase_transition} %are given in \S~\ref{sec:developing-stage} and 
% in more detail in \S~\ref{exp:case study}.
Though~\cite{chen2020simple} provide some explanations for the developing stage by analyzing the convergence rate, their theory fails to characterize the initial stage. In fact, we find that the analysis of initial stage provides valuable insights about oversmoothing.} 
% These dynamics, revealed by our experiments (\S~\ref{exp:case study}), are not well-supported by existing theories.}

\begin{wrapfigure}{r}{0.49\textwidth}
\centering
\vspace{1.6cm}
\includegraphics[scale=0.15,bb=900 300 380 180]{Figs/real_plot_2_new.png}
\vspace{1.2cm}
\caption{\small Accuracy of nodes grouped by degree $d_i$ on Citeseer. Initial stage: when mean effective homophily $\heterophilyil$ (ratio of a node's neighbors in the same class--\S~\ref{sec:developing-stage}) is high, the accuracy increases as the degree increases. %as the degree increases. 
Developing stage: when $\heterophilyil$ is low, the accuracy of high-degree nodes drops more sharply. %We use logarithmic binning to obtain different degree ranges.
}
\label{fig:phase_transition}
\vspace{-0.4cm}
\end{wrapfigure}
The second limitation of GCNs is their poor performance %that they perform poorly 
on heterophilous graphs~\citep{pei2019geom, lim2021large}, 
which---unlike homophilous graphs---have 
many neighboring nodes that belong to different classes~\citep{newman2002assortative}.
% nodes large portions of neighbors from other classes~\citep{newman2002assortative}. 
%In the real world, there are many heterophilous graphs. 
For instance,
in protein networks, amino acids of different types tend to form links~\citep{zhu2020beyond}, and in transaction networks, fraudsters are more likely to connect to accomplices than to other fraudsters~\citep{pandit2007netprobe}. Most GCNs~\citep{kipf2016semi, velivckovic2017graph} fail to effectively capture heterophily, so {emerging works have proposed some effective designs~\citep{pei2019geom, zhu2020beyond}, including signed messages (positive and negative interactions between nodes) proposed by concurrent works~\citep{chien2021adaptive, bo2021beyond}. 
% not enough theoretical understanding has been provided. 
% In this work, we identify the common causes of oversmoothing and heterophily problems, and theoretically show that under certain conditions, they lead to a higher misclassification rate. 
% For instance, some concurrent works~\citep{chien2021adaptive, bo2021beyond} use signed messages (positive and negative interactions between nodes). 
{Though these works justify signed messages from a spectral perspective, they focus on asymptotic results, requiring an infinite number of filters. Our work does not make this assumption, and our theory works in more practical scenarios (\S~\ref{subsec: sign_theory}).}}
% However, the latter do not provide theoretical justifications. In this work, we theoretically justify why and under what conditions, signed messages can help alleviate the heterophily and oversmoothing problems (\S~\ref{subsec: sign_theory}).}
% it remains an under-explored area.


These two limitations have mostly been studied independently, but recent work on oversmoothing~\citep{chen2020simple} was shown empirically to address heterophily, and vice versa~\citep{chien2021adaptive}. 
Motivated by this empirical observation, we set out to understand the theoretical connection between {the oversmoothing and heterophily problems} by studying the change in node representations during message passing. 
Specifically, we make the following contributions:
\setlist{leftmargin=*}
\begin{itemize*}
    \vspace{-0.25cm}
    \item \textbf{Theory:} We introduce \ul{the first theory that explains the connections between heterophily and oversmoothing} {which opens up the possibility of jointly studying the two problems.} %that the two problems can be jointly studied.}
    % by exploring the causes that increase the misclassification rate of node labels.
    % that make node representations less separable.
    %\yy{We are the \textit{first} to unveil the connections of heterophily and oversmoothing under a unified theoretical framework. The framework explains the problems by showing the factors (e.g., degree, heterophily) that make the node representations less separable.}
%We investigate the dynamics of the node representations in the first and deeper layers. We model node features as {random} vectors and theoretically analyze the factors (e.g., degree, heterophily) that make the representations of nodes from different classes indistinguishable (oversmoothing).
    %\item \textbf{Insights:} We find that (i) Nodes with high heterophily always become less separable after graph convolutions. (ii) Even with low heterophily, a degree disparity between nodes can influence the dynamics of the network during training, explaining oversmoothing. (iii) Allowing signed messages between neighbors can alleviate both the heterophily and oversmoothing problems.
    \item \textbf{Insights:} We find that under conditions, the relative degree of a node (compared to its neighbors) and its heterophily level affect the {misclassification rate of node labels} in the oversmoothing and heterophily problems. {We further prove that signed messages can mitigate their negative impact.}
    % Representations of nodes with high heterophily and nodes with low heterophily \& low relative degrees (degree discrepancy) \yy{tend to be misclassified} after graph convolution.%and (ii) allowing signed messages between neighbors can alleviate both the heterophily and oversmoothing problems.
    \item \textbf{{Improved  model \& empirical analysis:}}  Based on these insights, we design a generalized GCN model, \method, that allows negative interactions between nodes and compensates for the effect of low-degree nodes through a learned rescaling scheme. {Our empirical results show that our model is robust to oversmoothing, achieves state-of-the-art performance on datasets with high levels of heterophily, and achieves competitive performance on homophilous datasets.} 
    % Moreover, \method alleviates the oversmoothing problem.
\end{itemize*}
%  Through the analysis, we find that (i) nodes with high heterophily and nodes with low heterophily \& low degrees compared to their neighbors (degree discrepancy) trigger the oversmoothing problem (ii) allowing `negative' messages between neighbors can decouple the heterophily and oversmoothing problems. 


%This prompts us to think whether the two problems are inherently correlated: whether solving one problem will lead to alleviating the other and whether the two problems have common causes. Up till now, to the best of our knowledge, no prior works are trying to reveal the connections between the two problems theoretically. Beyond proposing designs that are effective for both problems, the main purpose of this paper is to explain how homophily level interact with the oversmoothing problem and on node-level, which nodes are responsible for triggering both problems. 
% \ks{While I like bullet point contribution summaries, this seems to reiterate what we just said above, so perhaps it's redundant and we can save the space.}
% To summarize, this paper makes the following contributions:
% \begin{itemize*}
%     \item We are the first to theoretically analyze the connections between the oversmoothing problem and GCNs' low performance in  heterophilous graphs.
%     \item We find that (i) nodes with high heterophily and nodes with moderate heterophily but low degrees compared to their neighbors (degree discrepancy) trigger the oversmoothing problem (ii) allowing `negative' messages between neighbors can decouple the heterophily and oversmoothing problems. 
%     \item We propose a new model \method based on the insights from our analysis. The model, \method, achieves state-of-the-art performances on heterophilous graphs and comparable performances on homophilous graphs. It is also robust to oversmoothing.
% \end{itemize*}

 


==> sections/numerics.tex <==
\subsection{Number representations}


==> sections/reproducibility_statements.tex <==
\section{Reproducibility Statement}
To reproduce our experimental results, we provide the references to the datasets and baselines in \S~\ref{section: experiments}. For the baselines, we use code provided by the authors and set the hyperparameters as the authors suggest. In App.~\S~\ref{app:hyperparameter}, we provide detailed hyperparameter setting for \method. We also provide our code in the supplementary material and we will share the link to our code upon acceptance.

==> sections/sup.tex <==
\newpage
\counterwithin{figure}{section}
\counterwithin{table}{section}
% \section{Appendix}
% \subsection{Definitions \& Theorems}
% We consider a binary node classification task on an unweighted loop-free graph with adjacency matrix $\rmA$. 
% We denote the set of nodes in the first class and the second class as $\gV_1$ and $\gV_2$, respectively.
% The $i$-th node $v_i$ has a feature vector $\rvf_i$.
% When $v_i \in \gV_1$, $\rvf_i$ follows the Gaussian distribution $G(\rvmu, \rvSigma)$, and when $v_i \in \gV_2$, $\rvf_i$ follows $G(-\rvmu, \rvSigma)$.

% We denote the degree of node $v_i$ by $d_i$, and the degree matrix by $\rmD$ which is a diagonal matrix whose elements are degrees. 
% Denote $\gN_i$ as the set of nodes directly connected to $v_i$, i.e., its neighbors. We further denote $\gN^s_i$ the set of nodes that are in $\gN_i$ and have the same class as $v_i$. 
% We use a concept called homophily to represent the tendency of a node to have the same class as its neighbor. 
% Specifically, for the $i$-th node $v_i$, its homophily $h_i$ is defined as $h_i = \E(\frac{|\gN^s_i|}{|\gN_i|})$, where the expectation is taken over the randomness of the node labels. 
% %We further assume that the heterophily is a constant across all nodes, i.e., $h_i=h, \forall i$.

% Recall that, based on the GCN formulation in the Section ???, the $(l+1)$-th output is given by: $\rmF^{l+1} = \sigma(\tilde{\rmA}\rmF^{l}\rmW^{(L)})$, where $\tilde{\rmA} = \tilde{\rmD}^{-1/2}(\rmI+\rmA)\tilde{\rmD}^{-1/2}$, and $\tilde{\rmD}$ is the degree matrix of $\rmI+\rmA$ and $\sigma$ is ReLU. 
% Compared to MLP, the main difference in the GCN operation is the ``propagation and aggregation step'' done by multiplying the adjacency matrix $\tilde{\rmA}$ with the feature matrix $\rmF^{l}$. We will thoroughly discuss its effect in node classification and how it is related to the homophily of the nodes. 



% \begin{theorem}
% Different nodes have different susceptibility to oversmoothing. The \textbf{lower} the homophily $h_i$ is, and the \textbf{smaller} the degree $d_i$ is, the more the node $v_i$ will suffer from oversmoothing. Specifically, the expectation of feature $\rvf_i$ after the operation $\tilde{\rmA}\rmF^{0}$ is changed to $ (\frac{1}{(d_i+1)}+\frac{(2h-1)\sum_{j \in \gN_i}{\frac{1}{\sqrt{d_j+1}}}}{(d_i+1){\frac{1}{2}}})\E(\rvf^0_i)$ and is bounded by $\frac{1}{2}\E(\rvf^0_i)$ when $h\leq0.5$. The variance of each node is also reduced to $\frac{1}{(d_i+1)}(\frac{1}{(d_i+1)}+\sum_{j \in \gN_i}{\frac{1}{(d_j+1)}})\rvSigma$, which is bounded by $\frac{1}{2}\rvSigma$. For a model trained with a high-homophily graph and fewer layers, the increased mean distances between the large-degree nodes of different classes and the reduction in the variance lead to performance gain. On the other hand, when the model is trained with a low-homophily graph or more layers, the reduced mean distances between low-degree nodes lead to degenerated performances.
% \end{theorem}

\section{Detailed Proofs of Theorems in \S~\ref{section: analysis}}
\label{app:proof}
\subsection{Proof of Lemma 1}
\label{app:lemma_1}
\begin{proof}
\yy{The loss function for SGC is: \texttt{CrossEntropy}(\texttt{Softmax}($\rmF^{(L)}\rmW^{(L)}+\rvb^{(L)}$), $y_i$). Rewrite $\rmW^{(L)}$ into an array of column vectors: $\rmW^{(L)}=[\rvw_0^{(L)}, \rvw_1^{(L)}, \dots \rvw_{|\gL|}^{(L)}]$, $\rvb^{(L)}$ into an array of scalars: $\rvb^{(L)}=[b_0^{(L)}, b_1^{(L)}, \dots b_{|\gL|}^{(L)}]$, and $\rmF^{(L)}$ into an array of row vectors: $\rmF^{(L)}=[\rvf_0^{(L)}; \rvf_1^{(L)}; \dots \rvf_{|\gV|}^{(L)}]$ ($[\cdot ; \cdot]$ means stacking vertically). Let $p_{i,c} \equiv \frac{e^{\rvf_i^{(L)}\rvw_c^{(L)}+b_c^{(L)}}}{\sum_j e^{\rvf_i^{(L)}\rvw_j^{(L)}+b_j^{(L)}}}$ and let $y_{i,c} \equiv \begin{cases} 1, & \text{iff } y_i=c \\ 0, & \text{otherwise} \end{cases}$
% $\left\{\def\arraystretch{1.2}\begin{tabular}{@{}l@{\quad}l@{}}
%   $1$ & iff \chi(x_i)=c \\
%   $0$ & else
% \end{tabular}\right$, 
then we rewrite the loss function as:
\begin{equation}
    -\frac{1}{n}\sum_{i=1}^n{\sum_{c=1}^{|\gL|}y_{i,c}\cdot\text{log}(p_{i,c})},
\end{equation}
$n$ is the number of nodes used for training. To predict that the node $v_i$ belongs to class $c$, we require: $\forall c'\neq c$, $p_{i,c} > p_{i,c'}$. Thus, we have: 
\begin{equation}
    \frac{e^{\rvf_i^{(L)}\rvw_c^{(L)}+b_c^{(L)}}}{\sum_j e^{\rvf_i^{(L)}\rvw_j^{(L)}+b_j^{(L)}}}>\frac{e^{\rvf_i^{(L)}\rvw_{c'}^{(L)}+b_{c'}^{(L)}}}{\sum_j e^{\rvf_i^{(L)}\rvw_{j}^{(L)}+b_j^{(L)}}}.
\end{equation} 
It is equivalent to: 
\begin{equation}
    {\rvf_i^{(L)}\rvw_c^{(L)}+b_c^{(L)}}>\rvf_i^{(L)}\rvw_{c'}^{(L)}+b_{c'}^{(L)}.
\end{equation} 
It shows that the decision region of class $c$ is decided by a set of hyper-planes: 
\begin{equation}
    \rvx(\rvw_c^{(L)}-\rvw_{c'}^{(L)})+(b_c^{(L)}-b_{c'}^{(L)})>0.
\end{equation}}
\end{proof}
\subsection{Proof of Lemma 2}
\label{app:lemma_2}
\begin{proof}
\yy{We prove it by contradiction and suppose that after the movements, the total misclassification rate is lowered. For conciseness, we "overload" the symbol $f_1(\rvx)$ and $f_2(\rvx)$ to represent the distribution of $\{\rvf_i^{(L)}\}$ from class 1 and class 2, respectively (before the movements). To note that, the distributions of different layers are different.} 

\yy{After the movements, the representations from class 1 become: $\{\rvf_i^{(L)}-t{\rvw^*}^T\}$, which causes a corresponding change in the PDF of class 1: $f_1(\rvx+t{\rvw^*}^T)$. The new misclassification rate of class 1 is: 
\begin{equation}
   M_t'=\int_{\rvx{\rvw^*}'+{b^*}'<0}{f_1(\rvx+t{\rvw^*}^T)d\rvx}=\int_{(\rvx-t{\rvw^*}^T){\rvw^*}'+{b^*}'<0}{f_1(\rvx)d\rvx}. 
\end{equation}}
\yy{The new misclassification rate of class 2 is: 
\begin{equation}
    M_r'=\int_{\rvx{\rvw^*}'+{b^*}'>0}{f_2(\rvx)d\rvx}.
\end{equation}
The new total misclassification rate is:
\begin{equation}
\label{lemma2:total}
    M'=\frac{\rho}{\rho+1}M_t'+\frac{1}{\rho+1}M_r'.
\end{equation}} 
% Because the total misclassification is lowered, we have: $m'<m$. 
\yy{Next, we will prove that if the total misclassification is lowered, $\rvx\rvw^*+b^*=0$ is not the optimal hyper-plane before the movements which should achieve the lowest total misclassification rate.} 

\yy{Consider a hyper-plane $\rvx{\rvw^*}'+{b^*}'-\frac{t{{\rvw^*}^T}{\rvw^*}'}{2}=0$.}
\yy{Given that ${{\rvw^*}^T}{\rvw^*}'>0$ and $t>0$, for $\forall \rvx,$ s.t. $\rvx{\rvw^*}'+{b^*}'-\frac{t{{\rvw^*}^T}{\rvw^*}'}{2}<0$, we have: $(\rvx-t{\rvw^*}^T){\rvw^*}'+{b^*}'= \rvx{\rvw^*}'+{b^*}'-\frac{t{{\rvw^*}^T}{\rvw^*}'}{2}-\frac{t{{\rvw^*}^T}{\rvw^*}'}{2}<0$. It means: 
\begin{equation}
    \{\rvx|(\rvx-t{\rvw^*}^T){\rvw^*}'+{b^*}'<0\} \supseteq	\{\rvx|\rvx{\rvw^*}'+{b^*}'-\frac{t{{\rvw^*}^T}{\rvw^*}'}{2}<0\}.
\end{equation}}
\yy{Because $f_1(\rvx)$ is a PDF which is a nonnegative function, 
\begin{equation}
\label{lemma2:ineq_1}
    \int_{(\rvx-t{\rvw^*}^T){\rvw^*}'+{b^*}'<0}{f_1(\rvx)d\rvx}\geq \int_{\rvx{\rvw^*}'+{b^*}'-\frac{t{{\rvw^*}^T}{\rvw^*}'}{2}<0}{f_1(\rvx)d\rvx}.
\end{equation}} 
\yy{Similarly, we can obtain
\begin{equation}
    \{\rvx|\rvx{\rvw^*}'+{b^*}'>0\} \supseteq	\{\rvx|\rvx{\rvw^*}'+{b^*}'-\frac{t{{\rvw^*}^T}{\rvw^*}'}{2}>0\}.
\end{equation}
Thus, 
\begin{equation}
\label{lemma2:ineq_2}
    \int_{\rvx{\rvw^*}'+{b^*}'>0}{f_2(\rvx)d\rvx} \geq \int_{\rvx{\rvw^*}'+{b^*}'-\frac{t{{\rvw^*}^T}{\rvw^*}'}{2}>0}{f_2(\rvx)d\rvx}.
\end{equation} 
Define 
\begin{equation}
    M_{f} \equiv \frac{\rho}{\rho+1}\int_{\rvx{\rvw^*}'+{b^*}'-\frac{t{{\rvw^*}^T}{\rvw^*}'}{2}<0}{f_1(\rvx)d\rvx}+\frac{1}{\rho+1}\int_{\rvx{\rvw^*}'+{b^*}'-\frac{t{{\rvw^*}^T}{\rvw^*}'}{2}>0}{f_2(\rvx)d\rvx}.
\end{equation} 
The quantity $M_{f}$ represents the total misclassification rate before the movements if the decision boundary is $\rvx{\rvw^*}'+{b^*}'-\frac{t{{\rvw^*}^T}{\rvw^*}'}{2}=0$.
Given Eq.~\ref{lemma2:total}, \ref{lemma2:ineq_1} and \ref{lemma2:ineq_2}, we have: 
\begin{equation}
    M' \geq M_{f}. 
\end{equation} 
Let $M$ denotes the total classification rate before the movements. Based on the assumption that the total misclassification rate is lowered after the movements ($M > M'$), we have:
\begin{equation}
\label{lemma2:conclusion}
    M > M_{f}. 
\end{equation}
Eq.~\ref{lemma2:conclusion} indicates that we find a hyper-plane $\rvx{\rvw^*}'+{b^*}'-\frac{t{{\rvw^*}^T}{\rvw^*}'}{2}=0$, which yields smaller total misclassification rate than $\rvx{\rvw^*}+{b^*}=0$ before the movements. This contradicts to the fact that $\rvx{\rvw^*}+{b^*}=0$ is the optimal hyper-plane before the movements.}
\end{proof}
\subsection{Proof of Theorem~\ref{theorem: initial_stage}}
\label{app:proof1}
\begin{proof}
% Before the operation of $\tilde{\rmA}\rmF^{0}$, the distance between the mean vectors of the two classes is:
% $(1+\rho)||\rvmu||$.
%$2||\rvmu||$ and the variance within each class is $\rvSigma$. 
%and the variance of each class is $\rvSigma$ and $\rvSigma'$.
% The smaller the distance between the two classes is, the less distinguishable the node features of the two classes are.

% After this operation, the node representation of any node $v_i$ is given by:
\yy{The first layer node representations are given by:}
% \vspace{-1cm}
\begin{equation}
\rvf_i^{(1)}=\frac{\rvf_i^{(0)}}{d_i+1} + \sum_{j \in \gN_i}{\frac{\rvf_j^{(0)}}{\sqrt{d_i+1} \cdot \sqrt{d_j+1}}}.
\label{eq:1}
% \vspace{-1cm}
\end{equation}

Without loss of generality, we assume node $v_i$ is in the first class $\gV_1$ and denote $\frac{|\gN^s_i|}{|\gN_i|}$ as $k_i$. Then, we can express the expectation of $\rvf_i^{(1)}$ as:
% \vspace{-1.5cm}
\begin{equation}
\E(\rvf_i^{(1)}) = \E(\E(\rvf_i^{(1)}|k_i))
\label{eq:2}
%\vspace{-2cm}
\end{equation}
\begin{equation}
\begin{split}
\E(\rvf_i^{(1)}|k_i) =& \E\left (\frac{\rvf_i^{(0)}}{d_i+1}|k_i \right ) + \sum_{j \in \gN_i}\E\left (\frac{\rvf_j^{(0)}}{\sqrt{d_i+1} \cdot \sqrt{d_j+1}}|k_i \right ) \\
%
=& \frac{\rvmu}{d_i+1} + \sum_{j \in \gN_i} \Bigg(\E\left(\frac{\rvf_j^{(0)}}{\sqrt{d_i+1} \cdot \sqrt{d_j+1}}|k_i, v_j \in \gV_1\right)\cdot \sP(v_j \in \gV_1|k_i)\\
%
+& \E\left(\frac{\rvf_j^{(0)}}{\sqrt{d_i+1} \cdot \sqrt{d_j+1}}|k_i, v_j \in \gV_2\right)\cdot \sP(v_j \in \gV_2|k_i)\Bigg)\\
%
%=& \frac{\rvmu}{d_i+1} + \sum_{j \in \gN_i}\left(\frac{k_i}{\sqrt{d_i+1} \cdot \sqrt{d_j+1}}\rvmu-\frac{(1-k_i)}{\sqrt{d_i+1} \cdot \sqrt{d_j+1}}\rvmu\right)\\
=& \frac{\rvmu}{d_i+1} + \sum_{j \in \gN_i}\left(\frac{k_i}{\sqrt{d_i+1} \cdot \sqrt{d_j+1}}\rvmu-\frac{(1-k_i)}{\sqrt{d_i+1} \cdot \sqrt{d_j+1}}\rho\rvmu\right)\\
%
%=& \frac{\rvmu}{d_i+1} + \frac{(2k_i-1)\rvmu}{\sqrt{d_i+1}}\sum_{j \in \gN_i}{\frac{1}{\sqrt{d_j+1}}}.
=& \frac{\rvmu}{d_i+1} + \frac{((1+\rho)k_i-\rho)\rvmu}{\sqrt{d_i+1}}\sum_{j \in \gN_i}{\frac{1}{\sqrt{d_j+1}}}.
\end{split}
\label{eq:3}
\end{equation}
%\vspace{-1cm}
Given $\E(k_i)=h_i$, Equation~(\ref{eq:2}) and Equation~(\eqref{eq:3}), we have:
\begin{equation}
%\vspace{-2cm}
\begin{split}
%\E(\rvf_i^{1}) =& \E\left(\frac{\rvmu}{d_i+1} + \frac{(2k_i-1)\rvmu}{\sqrt{d_i+1}}\sum_{j \in \gN_i}{\frac{1}{\sqrt{d_j+1}}}\right) \\
\E(\rvf_i^{(1)}) =& \E\left(\frac{\rvmu}{d_i+1} + \frac{((1+\rho)k_i-\rho)\rvmu}{\sqrt{d_i+1}}\sum_{j \in \gN_i}{\frac{1}{\sqrt{d_j+1}}}\right) \\
%
%=& \frac{\rvmu}{d_i+1} + \frac{(2h_i-1)\rvmu}{\sqrt{d_i+1}}\sum_{j \in \gN_i}{\frac{1}{\sqrt{d_j+1}}} \\
=& \frac{\rvmu}{d_i+1} + \frac{((1+\rho)h_i-\rho)\rvmu}{\sqrt{d_i+1}}\sum_{j \in \gN_i}{\frac{1}{\sqrt{d_j+1}}} \\
%
%=& \left(\frac{1}{d_i+1}+\frac{\sum_{j \in \gN_i}{\frac{1}{\sqrt{d_j+1}}}}{\sqrt{d_i+1}}(2h_i-1)\right)\rvmu \\
=& \left(\frac{1}{d_i+1}+\frac{\sum_{j \in \gN_i}{\frac{1}{\sqrt{d_j+1}}}}{\sqrt{d_i+1}}((1+\rho)h_i-\rho)\right)\rvmu \\
%
%=& \left(\frac{1}{d_i+1}+\frac{\sum_{j \in \gN_i}{\frac{\sqrt{d_i + 1}}{\sqrt{d_j+1}}}}{d_i+1}(2h_i-1)\right)\rvmu \\
=& \left(\frac{1}{d_i+1}+\frac{\sum_{j \in \gN_i}{\frac{\sqrt{d_i + 1}}{\sqrt{d_j+1}}}}{d_i+1}((1+\rho)h_i-\rho)\right)\rvmu \\
%
%=& \left(\frac{1 + (2h_i - 1)d_i\ratioi}{d_i+1} \right)\rvmu \equiv \gamma_i^1 \rvmu.
=& \left(\frac{1 + ((1+\rho)h_i-\rho)d_i\ratioi}{d_i+1} \right)\rvmu \equiv \gamma_i^1 \rvmu.
\label{eq:4}
\end{split}
\end{equation}
Where $\ratioi \equiv \frac{1}{d_i} \sum_{j \in \gN_i} \frac{\sqrt{d_i + 1}}{\sqrt{d_j + 1}}$. 

\vspace{0.2cm}
% \reminder{bring about 3 cases to expect}
%Next, we consider three cases: \textbf{(1)} $h_i\leq0.5$, \textbf{(2)} $h_i > 0.5 \ \mathbf{\&} \  \ratioi \leq \frac{1}{\epsilon}$, and \textbf{(3)} $h_i > 0.5 \ \mathbf{\&} \  \ratioi > \frac{1}{\epsilon}$.
Define $\epsilon \equiv (1+\rho)h_i-\rho$, and we consider three cases: \textbf{(1)} $h_i\leq\frac{\rho}{1+\rho}$, \textbf{(2)} $h_i > \frac{\rho}{1+\rho} \ \mathbf{\&} \  \ratioi \leq \frac{1}{\epsilon}$, and \textbf{(3)} $h_i > \frac{\rho}{1+\rho} \ \mathbf{\&} \  \ratioi > \frac{1}{\epsilon}$.
% \begin{itemize*}
%     \item $h_i\leq0.5$
%     \item $h_i > 0.5 \ \mathbf{\&} \  \ratioi \leq \frac{1}{\epsilon}$ and 
%     \item $h_i > 0.5 \ \mathbf{\&} \  \ratioi > \frac{1}{\epsilon}$. 
% \end{itemize*}

% \newpage

\begin{itemize}
    \item 
\colorbox{gray!30}{\textbf{CASE 1: $\pmb{h_i\leq\frac{\rho}{1+\rho}}$}}

$\bullet$ \textbf{Upper Bound}

We have:
\begin{equation}
%\vspace{-1cm}
\gamma_i^1 \leq \frac{1}{d_i+1} \leq \frac{1}{2}.
\label{eq:5}
\end{equation}
$\bullet$  \textbf{Lower Bound}

To see if there exists a lower bound, we first show that when $h_i \leq \frac{\rho}{1+\rho}$, $\frac{1 + ((1+\rho)h_i-\rho)d_i\ratioi}{d_i+1} $ is a decreasing function of $d_i$ given that $d_i \geq 1$.

When $h_i \leq \frac{\rho}{1+\rho}$, we have:
\begin{enumerate}
    \item $((1+\rho)h_i-\rho) \leq 0$
    \item $\frac{d_i}{d_i+1}$ is an increasing non-negative function of $d_i$
    \item $\ratioi$ is an increasing non-negative function of $d_i$
    \item $\frac{1}{d_i+1}$ is a decreasing function of $d_i$ 
\end{enumerate}
Thus $\frac{1 + ((1+\rho)h_i-\rho)d_i\ratioi}{d_i+1}$ is a decreasing function of $d_i$.

When $h_i=\frac{\rho}{1+\rho}$, $\frac{1 + ((1+\rho)h_i-\rho)d_i\ratioi}{d_i+1} = \frac{1}{d_i+1}$ and $0 < \frac{1}{d_i+1} \leq \frac{1}{2}$.

When $h_i<\frac{\rho}{1+\rho}$,
\begin{equation}
\begin{split}
    \frac{1 + ((1+\rho)h_i-\rho)d_i\ratioi}{d_i+1} &\leq \frac{((1+\rho)h_i-\rho)d_i\ratioi}{d_i+1}+\frac{1}{2} \\&\leq \frac{((1+\rho)h_i-\rho)\ratioi}{2}+\frac{1}{2}.
\end{split}
\end{equation}
And we know that when $h_i<\frac{\rho}{1+\rho}$:
\begin{equation}
\lim_{d_i \to \infty}{\frac{((1+\rho)h_i-\rho)\ratioi}{2}+\frac{1}{2}}=-\infty.
\end{equation}
Thus,
\begin{equation}
\begin{split}
\lim_{d_i \to \infty}{\frac{1 + ((1+\rho)h_i-\rho)d_i\ratioi}{d_i+1}}=-\infty.
\end{split}
\label{eq:lower_bound}
\end{equation}
% If $h_i > 0.5$,
% denote $M_i$ by $\frac{1}{M_i} \equiv \frac{1}{d_i}\sum_{j \in \gN_i}{\frac{1}{\sqrt{d_j+1}}}$

% \vspace{0.2cm}
% \textbf{[OTHER CASES: $\pmb{h_i > 0.5}$]}

% Let $\epsilon=2h_i - 1$ and $0 < \epsilon \leq 1$. We have:
% \begin{equation}
% %\vspace{-1cm}
% \begin{split}
%     % \E(\rvf_i^{1}) = (\frac{1}{(d_i+1)}+(2h_i-1)\cdot \frac{d_i}{M_i \cdot \sqrt{d_i+1}})\rvmu
%     \E(\rvf_i^{1}) = \left (\frac{1 + \epsilon d_i \ratioi}{d_i+1}\right )\rvmu.
% \end{split}
% \label{eq:6}
% \end{equation}

\vspace{0.2cm}
\item \colorbox{gray!30}{\textbf{CASE 2: $\pmb{h_i > \frac{\rho}{1+\rho} \;\;\; \mathbf{\&} \;\;\;  \ratioi \leq \frac{1}{\epsilon}}$}}

If $h_i >\frac{\rho}{1+\rho}$, $0 < \epsilon \leq 1$; if $\ratioi \leq \frac{1}{\epsilon}$, $0 < \epsilon \ratioi \leq 1$. Given %$\E(\rvf_i^{1}) = \left (\frac{1 + \epsilon d_i \ratioi}{d_i+1}\right )\rvmu$
\begin{equation}
%\vspace{-1cm}
\begin{split}
    % \E(\rvf_i^{1}) = (\frac{1}{(d_i+1)}+(2h_i-1)\cdot \frac{d_i}{M_i \cdot \sqrt{d_i+1}})\rvmu
    \E(\rvf_i^{1}) = \left (\frac{1 + \epsilon d_i \ratioi}{d_i+1}\right )\rvmu.
\end{split}
\label{eq:6}
\end{equation}
we have \yy{$0<\frac{1}{d_i+1} < \gamma_i^1 \leq 1$}.
%if $\ratioi \leq \frac{1}{\epsilon}$, then $0 < \epsilon \ratioi \leq 1$, so $\frac{1}{2} < \gamma_i^1 \leq 1$. 

\vspace{0.2cm}
\item \colorbox{gray!30}{\textbf{CASE 3: $\pmb{h_i > \frac{\rho}{1+\rho} \;\;\; \mathbf{\&} \;\;\;  \ratioi > \frac{1}{\epsilon}}$}}

In this case, Equation~(\ref{eq:6}) still holds, since $h_i>\frac{\rho}{1+\rho}$.

$\bullet$  \textbf{Lower Bound}

If $\ratioi > \frac{1}{\epsilon}$, then $\epsilon \ratioi > 1$ and therefore $\gamma_i^1 > 1$.

$\bullet$  \textbf{Upper Bound}

When $\epsilon>0$,
\begin{equation}
\begin{split}
    \frac{1 + \epsilon d_i\ratioi}{d_i+1} &> \frac{\epsilon d_i\ratioi}{d_i+1}\\&\geq \frac{\epsilon\ratioi}{2}.
\end{split}
\end{equation}
Because
\begin{equation}
    \lim_{d_i \to \infty}{\frac{\epsilon\ratioi}{2}}=\infty,
\end{equation}
we have:
\begin{equation}
    \lim_{d_i \to \infty}{\frac{1 + \epsilon d_i \ratioi}{d_i+1}}=\infty.
\end{equation}

To sum it up, 
\begin{equation}
\gamma_i^1 \in 
\begin{cases}
  (-\infty, \frac{1}{2}], & \text{if}\ h_i\leq\frac{\rho}{1+\rho} \\
  (\yy{\frac{1}{d_i+1}, 1]}, & \text{if}\ h_i>\frac{\rho}{1+\rho} \ \mathrm{\&}\  \ratioi \leq \frac{1}{(1+\rho)h_i-\rho}\\
  (1, \infty), & \mathrm{otherwise}.
\end{cases}
\end{equation}

\end{itemize}


\vspace{0.5cm}
\textbf{Remarks: Special cases}

For different types of graphs and different nodes in the graph, $d_i\ratioi$ might be different. For a \textbf{d-regular graph} whose nodes have constant degree or a graph whose adjacency matrix is \textbf{row-normalized}, we will have:
\begin{equation}
\begin{split}
    \gamma_i^1 =& \left (\frac{1 + ((1+\rho)h_i-\rho)d_i\ratioi}{d_i+1}\right ) \\\leq & (\frac{1}{(d_i+1)}+\frac{d_i}{(d_i+1)}) = 1
\end{split}
\label{eq:7}
\end{equation}
Equality is achieved if and only if $h_i=1$. To note that, $h_i=1$ is not achievable for every node as long as there are more than one class. \textbf{Boundary nodes} will suffer most.  

% %In a more general case, if $\frac{1}{M_i} \ll \frac{1}{(d_i+1)^{\frac{1}{2}}}$, then the 
% In a more general case, when $d_i \geq (\frac{M_i}{2h_i-1})^2-1$, $\E(\rvf_i^{1}) \geq \rvmu$ and when $d_i < (\frac{M_i}{2h_i-1})^2-1$, $\E(\rvf_i^{1}) < \rvmu$. It suggests that a node with significantly smaller degree than its neighbors is easier to suffer from oversmoothing.




% From the above derivations, we can have the following conclusions:
% \begin{enumerate}
%     \item After "propagation and aggregation", the expectation of $\rvf_i^{1}$ changes to  $(\frac{1}{(d_i+1)}+\frac{(2h-1)\sum_{j \in \gN_i}{\frac{1}{\sqrt{d_j+1}}}}{(d_i+1)^{\frac{1}{2}}})\rvmu$. It indicates that the lower homophily of the graph, the less distinguishable of the features after $\tilde{\rmA}\rmF^{0}$. When $h_i \leq 0.5$, the node feature moves towards the origin by at least half of the original distances.
%     \item The smaller the degree of the node, the more it will suffer from oversmoothing.
%     \item The derivation can be extended to the case where the neighborhood nodes are weighted differently. In that case, the larger positive weight on the nodes that have a different class, the less distinguishable of features. 
% \end{enumerate}
% Then, we will take a look at the variance within class 1. If we assume that the feature vectors are independent of each other, then we will have:
% \begin{equation}
% \begin{split}
% \sV(\rvf_t^{1}|k_i) =& \sV\left(\frac{\rvf_i^{0}}{d_i+1}|k_i\right) + \sum_{j \in \gN_i}{\sV\left(\frac{\rvf_j^{0}}{\sqrt{d_i+1} \cdot \sqrt{d_j+1}}|k_i\right)} \\
% %
% %=& \left(\frac{1}{(d_i+1)^2} + \sum_{j \in \gN_i}{\frac{1}{(d_i+1)(d_j+1)}}\right)\rvSigma \\
% =& \frac{\rvSigma}{(d_i+1)^2} + \sum_{j \in \gN_i}{\frac{1}{(d_i+1)(d_j+1)}}\sV(\rvf_j^{0}|k_i)\\
% %
% =& \frac{\rvSigma}{(d_i+1)^2} + \sum_{j \in \gN_i}{\frac{1}{(d_i+1)(d_j+1)}}(\E(\sV(\rvf_j^{0}|k_i,\mathbbm{1}\{v_j \in \gV_1\}))+\sV(\E(\rvf_j^{0}|k_i, \mathbbm{1}\{v_j \in \gV_1\})))\\
% =& \frac{\rvSigma}{(d_i+1)^2} + \sum_{j \in \gN_i}{\frac{1}{(d_i+1)(d_j+1)}}(k_i\rvSigma+(1-k_i)\rvSigma'+k_i(1-k_i)(1+\rho)^2\rvmu^T\rvmu)
% %= & \frac{1}{d_i+1}\left(\frac{1}{d_i+1}+\sum_{j \in \gN_i}{\frac{1}{d_j+1}}\right)\rvSigma
% %
% \end{split}
% \label{eq:8}
% \end{equation}

% \begin{equation}
%     \frac{1}{d_i+1}\left(\frac{1}{d_i+1}+\sum_{j \in \gN_i}{\frac{1}{d_j+1}}\right)
% \leq \frac{1}{2}
% \end{equation}

% Note that we can derive similar results for any node $v_t$ in the second class.

% From Equation~\ref{eq:8}, we can have the following conclusion:
% \item $\tilde{\rmA}\rmF^{0}$ will reduce the variance of the node feature distribution and the reduction is irrelevant to the homophily $h_i$. The larger degree of the node, the greater the reduction will be in the variance. Note that the reduction of the variance of each node does not mean the reduction of the variance of the class as a whole. When the degree and the homophily of the nodes are diverse, the variance of the class can increase.
%This explains the gain of GCN when using fewer layers and the performance gain is a result of variance reduction.
\end{proof}

% Next, we will consider an extended scenario: we let the "messages" sent by the neighbors from the other class to be multiplied by a negative sign and the neighbors from the same class to send the "messages" as they are. For the node $v_i$, we define $m_i$ as the ratio of neighbors that do not send the "messages" correctly, i.e., neighbors from the other class send messages without being multiplied by a negative sign and neighbors from the same class send the messages multiplied by a negative sign. And we define the error rate as $e_i=\E(m_i)$, the expectation is taken over the randomness of the neighbors that wrongly send the messages. %We assume the expectation is the same for all the nodes.

% We have the following assumptions:
% \begin{enumerate}
%     \item Conditioned on $m_i$, whether the neighbor will wrongly send the information is independent of the class it belongs to.
%     \item The variable $m_i$ is independent of the class that any node $v_j$ belongs to.
% \end{enumerate}

% \begin{theorem}
% With the independence assumptions and by allowing the messages to be optionally multiplied by a negative sign, the mean distance between the nodes in different classes will \textbf{not be affected} by the homophily level $h_i$, but will be reduced for \textbf{bigger error rate} $e_i$. 
% \end{theorem}
\subsection{Proof of Theorem~\ref{theorem: developing stage}}
\label{app:proof2}
\begin{proof}
% The derivation is similar to that of Theorem~\ref{theorem: initial_stage} except that we replace the ground truth heterophily $h_i$ with the effective heterophily $\heterophilyil$, $\ratioi$ with $\ratioi'$, and $\E(\rvf_i^{l})$ with $\gamma^l_i\E(\rvf_i^{0})\rmW^{e}$. 
\yy{We derive the equation for nodes which are from class 1 and its expected representation does not cross the origin (the other cases can be derived similarly):}

\yy{Rewrite the $\E(\rvf_i^{(l)})$ in \S~\ref{sec:developing-stage}:
$$\E(\rvf_i^{(l)}) = \begin{cases}\xi^l_i\E(\rvf_i^{(0)}) & \text{if node }v_i\text{'s expected representation does not cross the origin.} \\
-\rho\xi^l_i\E(\rvf_i^{(0)}) & \text{if node }v_i\text{ is from class 1 and its expected representation moves across the origin.} \\
-\frac{1}{\rho}\xi^l_i\E(\rvf_i^{(0)}) & \text{if node }v_i\text{ is from class 2 and its expected representation moves across the origin.}
\end{cases}$$
}

\yy{Let $\hat{\mathcal{N}_i^s} \equiv \{v_j|\E(\rvf_i^{(0)})\cdot\E({\rvf_j^{(l)}}^T)>0, v_j \in \gN_i\}$. Recall that $\mathcal{N}_i^s$ is the set of neighbors that have the same label as node $v_i$, so we have: $\hat{\mathcal{N}_i^s} = \{v_j|v_j \in \mathcal{N}_i^s \;\&\;\E(\rvf_j^{(l)})\text{ does not cross the origin}\} \cup \{v_j|v_j \not\in \mathcal{N}_i^s, v_j \in \mathcal{N}_i \; \& \; \E(\rvf_j^{(l)})\text{ crosses the origin}\}$. Define $k_i=\frac{|\hat{\mathcal{N}_i^s}|}{|\mathcal{N}_i|}$ and $\mathbb{E}(k_i)=\heterophilyil$. The expectation is taken over possible distributions of ground truth labels in $v_i$'s neighborhood. From the definition of $\xi_i^l$, we have: if $v_j \in \hat{\mathcal{N}_i^s}$, $\mathbb{E}(\mathbf{f}_j^{(l)})=\xi_j^l\rvmu$; if $v_j \not\in \hat{\mathcal{N}_i^s}, v_j \in \mathcal{N}_i$, $\mathbb{E}(\mathbf{f}_j^{(l)})=-\rho\xi_j^l\rvmu$. 
The representations at $(l+1)$-th layer:
\begin{equation}
    \mathbf{f}_i^{(l+1)}=\frac{\mathbf{f}_i^{(l)}}{d_i+1} + \sum_{j \in \mathcal{N}_i}{\frac{\mathbf{f}_i^{(l)}}{\sqrt{d_i+1} \cdot \sqrt{d_j+1}}}
\end{equation}
\begin{equation}
    \mathbb{E}(\mathbf{f}_i^{(l+1)}) = \mathbb{E}(\mathbb{E}(\mathbf{f}_i^{(l+1)}|k_i))
\end{equation}
\begin{eqnarray}\mathbb{E}(\mathbf{f}_i^{(l+1)}|k_i) &=& \mathbb{E}\left (\frac{\mathbf{f}_i^{(l)}}{d_i+1}|k_i \right ) + \sum_{j \in \mathcal{N}_i}\mathbb{E}\left (\frac{\mathbf{f}_j^{(l)}}{\sqrt{d_i+1} \cdot \sqrt{d_j+1}}|k_i \right) \\ &=& \frac{\xi_i^l\rvmu}{d_i+1} + \sum_{j \in \mathcal{N}_i} \Bigg(\mathbb{E}\left(\frac{\mathbf{f}_j^{(l)}}{\sqrt{d_i+1} \cdot \sqrt{d_j+1}}|k_i, v_j \in \hat{\mathcal{N}_i^s}\right)\cdot \mathbb{P}(v_j \in \hat{\mathcal{N}_i^s}|k_i) \\ &+& \mathbb{E}\left(\frac{\mathbf{f}_j^{(l)}}{\sqrt{d_i+1} \cdot \sqrt{d_j+1}}|k_i, v_j \not\in \hat{\mathcal{N}_i^s}\right)\cdot \mathbb{P}(v_j \not\in \hat{\mathcal{N}_i^s}|k_i)\Bigg)\\ &=& \frac{\xi_i^l\rvmu}{d_i+1} + \sum_{j \in \mathcal{N}_i}\left(\frac{k_i}{\sqrt{d_i+1} \cdot \sqrt{d_j+1}}\xi_j^l\rvmu-\frac{(1-k_i)}{\sqrt{d_i+1} \cdot \sqrt{d_j+1}}\rho\xi_j^l\rvmu\right)\\ &=& \frac{\xi_i^l\rvmu}{d_i+1} + \sum_{j \in \mathcal{N}_i}\left(\frac{\frac{\xi_j^l}{\xi_i^l}k_i\xi_i^l\rvmu}{\sqrt{d_i+1} \cdot \sqrt{d_j+1}}-\frac{\frac{\xi_j^l}{\xi_i^l}(1-k_i)\rho\xi_i^l\rvmu}{\sqrt{d_i+1} \cdot \sqrt{d_j+1}}\right)
\end{eqnarray}
In Thm~\ref{theorem: developing stage}, we define $r_{ij}'\equiv r_{ij}\frac{\xi_j^l}{\xi_i^l}$ and $\overline{r_{i}'} \equiv \frac{1}{d_i}\sum_{j \in \mathcal{N}_i}{r_{ij}'}$, thus
\begin{equation}
    \mathbb{E}(\mathbf{f}_i^{(l+1)}|k_i) = \frac{\xi_i^l\rvmu}{d_i+1} + \sum_{j \in \mathcal{N}_i}(r_{ij}'((1+\rho)k_i-\rho)\xi_i^l\rvmu)=\left(\frac{1 + ((1+\rho)k_i-\rho)d_i\overline{r_{i}'}}{d_i+1} \right)\xi_i^l\rvmu
\end{equation}
\begin{equation}
    \mathbb{E}(\mathbf{f}_i^{(l+1)})=\mathbb{E}(\mathbb{E}(\mathbf{f}_i^{(l+1)}|k_i))=\left(\frac{1 + ((1+\rho)\heterophilyil-\rho)d_i\overline{r_{i}'}}{d_i+1} \right)\xi_i^l\mathbb{E}(\mathbf{f}_i^{(0)})
\end{equation}}

Next, we prove that $\left (\frac{((1+\rho)\heterophilyil-\rho) d_i \ratioi' + 1}{d_i+1}\right )$ is a decreasing function of $d_i$. Since graph $\gG$ is connected, the node degrees $d_i \geq 1$; thus, $\frac{d_i}{d_i+1}$ and $\ratioi'$ are increasing functions of $d_i$, while $\frac{1}{d_i+1}$ is a decreasing function of $d_i$. When $\heterophilyil \leq \frac{\rho}{1+\rho}$, we have $((1+\rho)\heterophilyil-\rho) \leq 0$, so $((1+\rho)\heterophilyil-\rho) \cdot \frac{d_i}{d_i+1} \cdot \ratioi + \frac{1}{d_i+1}$ is a decreasing function of $d_i$). This suggests that the higher-degree nodes move towards the opposing class more and "under non-swapping condition", the accuracy of higher-degree nodes drops more sharply.
\end{proof}
\subsection{Proof of Theorem~\ref{theorem: signed_messages}}
\label{app:proof3}
\begin{proof}
Similar to Equation~\ref{eq:2}, we can express the expectation of $\rvf_i^{(1)}$ as:
\begin{equation}
\begin{split}
\E(\rvf_i^{(1)}) =& \E(\E(\rvf_i^{(1)}|m_i^0))  \\
%
=& \E\left(\E\left(\frac{\rvf_i^{(0)}}{d_i+1}|m_i^0\right) + \sum_{j \in \gN_i}\E\left(\frac{\rvf_j^{(0)}}{\sqrt{d_i+1} \cdot \sqrt{d_j+1}}|m_i^0\right)\right) \\
%
=& \E\Bigg(\frac{\rvmu}{d_i+1} + \sum_{j \in \gN_i}\Bigg(\E\left(\frac{\rvf_j^{(0)}}{\sqrt{d_i+1} \cdot \sqrt{d_j+1}}|m_i^0, v_j \in \gV_1\right)\sP(v_j \in \gV_1|m_i^0) \\
%
+& \E\left(\frac{\rvf_j^{(0)}}{\sqrt{d_i+1} \cdot \sqrt{d_j+1}}|m_i^0, v_j \in \gV_2\right)\sP(v_j \in \gV_2|m_i^0)\Bigg)\Bigg).
\end{split}
\label{eq:9}  
\end{equation}

Next, we will show how to compute the conditional expectation and conditional probability in the summand.
\begin{equation}
\begin{split}
\E\left(\frac{\rvf_j^{(0)}}{\sqrt{d_i+1} \cdot \sqrt{d_j+1}}|m_i^0, v_j \in \gV_1\right) =& \E\left(\frac{\rvf_j^{(0)}}{\sqrt{d_i+1} \cdot \sqrt{d_j+1}}|m_i^0, v_j \in \gV_1, v_j \text{wrongly send information}\right) \\
%
& \cdot \sP(v_j \text{wrongly send information}|m_i^0, v_j \in \gV_1) \\
%
+& \E\left(\frac{\rvf_j^{(0)}}{\sqrt{d_i+1} \cdot \sqrt{d_j+1}}|m_i^0, v_j \in \gV_1, v_j \text{correctly send information}\right) \\
%
& \cdot \sP(v_j \text{correctly send information}|m_i^0, v_j \in \gV_1).
\end{split}
\label{eq:10}
\end{equation}
Combined with the conditional independence assumption, we have:
\begin{equation}
\begin{split}
\sP(v_j \text{wrongly send information}|m_i^0, v_j \in \gV_1) =& \frac{\sP(v_j \text{wrongly send information}, v_j \in \gV_1|m_i^0)}{\sP(v_j \in \gV_1|m_i^0)} \\
%
=& \frac{\sP(v_j \text{wrongly send information}|m_i^0)\cdot \sP(v_j \in \gV_1|m_i^0)}{\sP(v_j \in \gV_1)|m_i^0)} \\
%
=& \sP(v_j \text{ wrongly send information}|m_i^0)=m_i^0.
\end{split}
\label{eq:11}
\end{equation}
Similarly, we obtain:
\begin{equation}
\sP(v_j \text{ correctly send information}|m_i^0, v_j \in \gV_1) = 1-m_i^0.
\label{eq:12}
\end{equation}
Then Equation~(\ref{eq:10}) can be rewritten as:
\begin{equation}
\begin{split}
\E\left(\frac{\rvf_j^{(0)}}{\sqrt{d_i+1} \cdot \sqrt{d_j+1}}|m_i^0, v_j \in \gV_1\right) =& \E\left(\frac{\rvf_j^{(0)}}{\sqrt{d_i+1} \cdot \sqrt{d_j+1}}|m_i^0, v_j \in \gV_1, v_j \text{wrongly send information}\right)\cdot m_i^0 \\
%
+& \E\left(\frac{\rvf_j^{(0)}}{\sqrt{d_i+1} \cdot \sqrt{d_j+1}}|m_i^0, v_j \in \gV_1, v_j \text{correctly send information}\right)\cdot (1-m_i^0) \\
%
=& -\frac{m_i^0\rvmu}{\sqrt{d_i+1} \cdot \sqrt{d_j+1}} + \frac{(1-m_i^0)\rvmu}{\sqrt{d_i+1} \cdot \sqrt{d_j+1}} \\
%
=&
\frac{(1-2m_i^0)\rvmu}{\sqrt{d_i+1} \cdot \sqrt{d_j+1}}.
\end{split}
\label{eq:13}
\end{equation}
Similarly, we have:
\begin{equation}
\E\left(\frac{\rvf_j^{(0)}}{\sqrt{d_i+1} \cdot \sqrt{d_j+1}}|m_i^0, v_j \in \gV_2\right) = \frac{(1-2m_i^0)\rho\rvmu}{\sqrt{d_i+1}. \cdot \sqrt{d_j+1}}.
\label{eq:14}
\end{equation}
Consider the independence between $m_i^0$ and node class, and insert Equation~(\ref{eq:13}) and Equation~(\ref{eq:14}) into Equation~(\ref{eq:9}), we will have:
\begin{equation}
\begin{split}
\E(\rvf_i^{(1)}) =& \E\left(\frac{\rvmu}{d_i+1} + \sum_{j \in \gN_i}(\frac{(1-2m_i^0)k_i\rvmu}{\sqrt{d_i+1} \cdot \sqrt{d_j+1}}+\frac{(1-2m_i^0)(1-k_i)\rho\rvmu}{\sqrt{d_i+1} \cdot \sqrt{d_j+1}})\right) \\
%
=& \E\left(\frac{\rvmu}{d_i+1} + \sum_{j \in \gN_i}\frac{(1-2m_i^0)(\rho+(1-\rho)k_i)\rvmu}{\sqrt{d_i+1} \cdot \sqrt{d_j+1}}\right) \\
%
=& \frac{\rvmu}{d_i+1} + \sum_{j \in \gN_i}\frac{(1-2e_i^0)(\rho+(1-\rho)h_i)\rvmu}{\sqrt{d_i+1} \cdot \sqrt{d_j+1}} \\
%
=& \left(\frac{1 + (1 - 2e_i^0)(\rho+(1-\rho)h_i)d_i\ratioi}{d_i+1}\right)\rvmu \equiv \gamma_i^1 \E(\rvf^{(0)}_i).
\end{split}
\label{eq:15}
\end{equation}
% From Equation~\ref{eq:15}, we can conclude that:
% \begin{enumerate}
%     \item If we allow the neighbors of a different class to send the information but be multiplied with a negative sign, then low homophily will not degenerate the performance.
%     \item If the model does not work well in the heterophily setting, i.e., they have a higher error rate $e_i$ in identifying neighbors from another class, the model will also suffer from oversmoothing problem. 
% \end{enumerate}
When $h_i \leq 1$, $\rho+(1-\rho)h_i=(1-h_i)\rho+h_i>0.$ Define $\epsilon' \equiv (1 - 2e_i^0)(\rho+(1-\rho)h_i)$. To obtain the ranges of $\gamma_i^1$, when $e_i^0 \geq 0.5$, $\epsilon' \leq 0$, it resembles the derivations of CASE 1 in Proof~\ref{app:proof1}; when $e_i^0 < 0.5$, $0 < \epsilon \ratioi \leq 1$, it resembles the derivations of CASE 2; when $e_i^0 < 0.5$, $\epsilon \ratioi > 1$, it resembles the derivations of CASE 3.
% The ranges of $\gamma_i^1$ under different conditions of $e_i^0$ and $\ratioi$ can be derived similarly as shown by the Proof~\ref{app:proof1}.
\end{proof}

\section{Additional Experiments}
\vspace{-0.3cm}
\subsection{Ablation study}
\label{subsec:ablation}
\setlength{\tabcolsep}{3pt}
\begin{table*}[h]
\centering
\vspace{-0.5cm}
\caption{Ablation study: degree correction has consistent benefits (robust to oversmoothing \& ability to handle heterophily) in different datasets while signed information has more benefits in heterophilous datasets. Best performance of each model is highlighted in gray.}
\label{tab:ablation}
\begin{adjustbox}{width=1\linewidth}
{\footnotesize
\begin{tabular}{ccccccccccccccc}
\toprule
                                         %\multirow{2}{*}{\backslashbox{\textbf{Model}}{\textbf{Layers}}}    
                                \multicolumn{1}{r}{\textbf{Layers}} 
                                      && \textbf{2}           & \multicolumn{1}{c}{\textbf{4}} & \multicolumn{1}{c}{\textbf{8}} & \multicolumn{1}{c}{\textbf{16}} & \multicolumn{1}{c}{\textbf{32}} & \multicolumn{1}{c}{\textbf{64}} &&  \multicolumn{1}{c}{\textbf{2}}           & \multicolumn{1}{c}{\textbf{4}} & \multicolumn{1}{c}{\textbf{8}} & \multicolumn{1}{c}{\textbf{16}} & \multicolumn{1}{c}{\textbf{32}} & \multicolumn{1}{c}{\textbf{64}}  \\ \cmidrule{1-1} \cmidrule{3-8} \cmidrule{10-15} %cline{2-8}
%\multirow{10}{*}{\rotatebox[origin=c]{90}{\textbf{Homophily datasets}}}   
%\textbf{Model} 
&& \multicolumn{6}{c}{\textbf{Cora} ($h$=0.81)}     & & \multicolumn{6}{c}{\textbf{Citeseer} ($h$=0.74)}                                                                         \\ %\cline{1-1} 
\cline{3-8} \cline{10-15}
                                    
                                        \multicolumn{1}{c}{Base}    &&   
                                        %cora results
                                        \cellcolor{gray!15}$ 86.56{\scriptstyle\pm1.21}$         & \multicolumn{1}{c}{$ 86.04{\scriptstyle\pm0.72}$}    &        \multicolumn{1}{c}{$ 85.51{\scriptstyle\pm1.51}$}     &       \multicolumn{1}{c}{$ 85.33{\scriptstyle\pm0.72}$}      &     \multicolumn{1}{c}{$ 85.37{\scriptstyle\pm1.58}$}       &    \multicolumn{1}{c}{$ 72.17{\scriptstyle\pm8.89}$}   & &  
                                        % citeseer results
                                        \cellcolor{gray!15}$76.51{\scriptstyle\pm1.63}$ & $75.03{\scriptstyle\pm1.67}$ & $73.96{\scriptstyle\pm1.52}$ & $73.59{\scriptstyle\pm1.51}$& $71.91{\scriptstyle\pm1.94}$ & $32.08{\scriptstyle\pm15.74}$                                         \\ 
                                        
                                      \multicolumn{1}{c}{\texttt{+deg}}    &&  
                                      %cora results
                                      \cellcolor{gray!15}$86.72{\scriptstyle\pm1.29}$      &          \multicolumn{1}{c}{$86.02{\scriptstyle\pm0.97}$}           & \multicolumn{1}{c}{$85.49{\scriptstyle\pm1.32}$}           & \multicolumn{1}{c}{$85.27{\scriptstyle\pm1.59}$}            & \multicolumn{1}{c}{$85.27{\scriptstyle\pm1.51}$}            & \multicolumn{1}{c}{$84.21{\scriptstyle\pm1.22}$}   &   &                   % citeseer results
                                      \cellcolor{gray!15}$76.63{\scriptstyle\pm1.38}$  & $74.64{\scriptstyle\pm1.97}$&  $74.15{\scriptstyle\pm1.61}$&  $73.73{\scriptstyle\pm1.31}$&  $73.61{\scriptstyle\pm1.84}$&  $70.56{\scriptstyle\pm2.27}$
                                      \\  \multicolumn{1}{c}{\texttt{+sign}} &&  
                                      %cora results
                                      $84.81{\scriptstyle\pm1.63}$&   \cellcolor{gray!15}$86.06{\scriptstyle\pm1.7}$&   $85.67{\scriptstyle\pm1.26}$&   $85.39{\scriptstyle\pm0.97}$&   $84.85{\scriptstyle\pm0.98}$&   $78.57{\scriptstyle\pm6.73}$   & &    % citeseer results
                                      \cellcolor{gray!15}$77.13{\scriptstyle\pm1.69}$&  $74.56{\scriptstyle\pm2.02}$&   $73.64{\scriptstyle\pm1.65}$&   $72.31{\scriptstyle\pm2.32}$&   $71.98{\scriptstyle\pm3.44}$&   $68.68{\scriptstyle\pm6.72}$
                        \\  \multicolumn{1}{c}{\texttt{+deg,sign}} &&
                         % cora results
                        \cellcolor{gray!15}$86.96{\scriptstyle\pm1.38}$ & $86.20{\scriptstyle\pm0.89}$ & $85.63{\scriptstyle\pm0.78}$ &
                              $85.47{\scriptstyle\pm1.18}$ & $85.55{\scriptstyle\pm1.66}$ & $77.81{\scriptstyle\pm7.95}$     &  & 
                              % citeseer results 
                              \cellcolor{gray!15}$76.81{\scriptstyle\pm1.71}$ & $74.68{\scriptstyle\pm1.97}$ & $74.69{\scriptstyle\pm2.35}$ &
                              $73.28{\scriptstyle\pm1.45}$ & $71.81{\scriptstyle\pm2.28}$ & $69.91{\scriptstyle\pm3.97}$ 
                              \\ \midrule %\cmidrule{1-1} \cmidrule{3-8} \cmidrule{10-15} 
                                    %   & \multicolumn{6}{c}{\textbf{Citeseer ($h$=0.74)}}                                                            \\ \hline 
                                        % \multicolumn{1}{c}{Base}    & \cellcolor{gray!15}$76.51{\scriptstyle\pm1.63}$ & $75.03{\scriptstyle\pm1.67}$ & $73.96{\scriptstyle\pm1.52}$ & $73.59{\scriptstyle\pm1.51}$& $71.91{\scriptstyle\pm1.94}$ & $32.08{\scriptstyle\pm15.74}$                                         \\  
                                    %   \multicolumn{1}{c}{+deg}    &  \cellcolor{gray!15}$76.63{\scriptstyle\pm1.38}$  & $74.64{\scriptstyle\pm1.97}$&  $74.15{\scriptstyle\pm1.61}$&  $73.73{\scriptstyle\pm1.31}$&  $73.61{\scriptstyle\pm1.84}$&  $70.56{\scriptstyle\pm2.27}$                     \\  
                                    %   \multicolumn{1}{c}{+sign} &   \cellcolor{gray!15}$77.13{\scriptstyle\pm1.69}$&  $74.56{\scriptstyle\pm2.02}$&   $73.64{\scriptstyle\pm1.65}$&   $72.31{\scriptstyle\pm2.32}$&   $71.98{\scriptstyle\pm3.44}$&   $68.68{\scriptstyle\pm6.72}$                                                                     \\ 
                            %           \multicolumn{1}{c}{+deg,sign}   & \cellcolor{gray!15}$76.81{\scriptstyle\pm1.71}$ & $74.68{\scriptstyle\pm1.97}$ & $74.69{\scriptstyle\pm2.35}$ &
                            %   $73.28{\scriptstyle\pm1.45}$ & $71.81{\scriptstyle\pm2.28}$ & $69.91{\scriptstyle\pm3.97}$                                              \\ \hline
&& \multicolumn{6}{c}{\textbf{Cornell ($h$=0.3)}} && \multicolumn{6}{c}{\textbf{Chameleon ($h$=0.23)}}                                                                                                                                                                                                                               \\ %\cline{1-1} 
\cline{3-8} \cline{10-15} 
                                      \multicolumn{1}{c}{Base}    && \cellcolor{gray!15}$61.89{\scriptstyle\pm3.72}$ & $60.00{\scriptstyle\pm5.24}$ & $58.92{\scriptstyle\pm5.24}$ &
                              $56.49{\scriptstyle\pm5.73}$ & $58.92{\scriptstyle\pm3.15}$ & $49.19{\scriptstyle\pm16.70}$          &&
% Chameleon results
\cellcolor{gray!15}$64.98{\scriptstyle\pm1.84}$ & $62.65{\scriptstyle\pm3.09}$ & $62.43{\scriptstyle\pm3.28}$ & $54.69{\scriptstyle\pm2.58}$& $47.68{\scriptstyle\pm2.63}$ & $29.74{\scriptstyle\pm5.21}$
\\  
                                      \multicolumn{1}{c}{\texttt{+deg}}    && \cellcolor{gray!15}$63.78{\scriptstyle\pm5.57}$ & $62.70{\scriptstyle\pm5.90}$ & $59.46{\scriptstyle\pm4.52}$ &
                              $56.49{\scriptstyle\pm5.73}$ & $57.57{\scriptstyle\pm4.20}$ & $58.92{\scriptstyle\pm3.15}$    &&
% Chameleon results
$66.54{\scriptstyle\pm2.19}$ & $68.31{\scriptstyle\pm2.70}$ & \cellcolor{gray!15}$68.99{\scriptstyle\pm2.38}$ & $67.68{\scriptstyle\pm3.70}$& $56.86{\scriptstyle\pm8.80}$ & $41.95{\scriptstyle\pm9.56}$
\\  
                                      \multicolumn{1}{c}{\texttt{+sign}} && \cellcolor{gray!15}$85.41{\scriptstyle\pm7.27}$&  $76.76{\scriptstyle\pm7.07}$& $70.00{\scriptstyle\pm5.19}$&  $67.57{\scriptstyle\pm9.44}$&  $63.24{\scriptstyle\pm6.07}$&  $63.24{\scriptstyle\pm6.53}$    && 
% Chameleon results
\cellcolor{gray!15}$65.31{\scriptstyle\pm3.20}$&  $53.55{\scriptstyle\pm6.35}$& $53.05{\scriptstyle\pm2.28}$&  $51.93{\scriptstyle\pm4.00}$&  $57.17{\scriptstyle\pm3.39}$&  $51.93{\scriptstyle\pm8.95}$
\\  
                                      \multicolumn{1}{c}{\texttt{+deg,sign}}            && \cellcolor{gray!15}$84.32{\scriptstyle\pm6.37}$&  $78.92{\scriptstyle\pm8.09}$& $73.51{\scriptstyle\pm5.90}$&  $70.81{\scriptstyle\pm5.64}$&  $68.11{\scriptstyle\pm5.14}$&  $62.43{\scriptstyle\pm6.67}$ &&
% Chameleon results
\cellcolor{gray!15}$65.75{\scriptstyle\pm1.81}$ & $61.49{\scriptstyle\pm7.38}$ & $53.73{\scriptstyle\pm7.79}$ &
                               $52.43{\scriptstyle\pm5.37}$ & $55.92{\scriptstyle\pm5.14}$ & $56.95{\scriptstyle\pm3.93}$ 
%                                       \\ \hline
% %\multirow{10}{*}{\rotatebox[origin=c]{90}{\textbf{Heterophily datasets}}} 
% & \multicolumn{6}{c}{\textbf{Chameleon ($h$=0.23)}}                                                                                                                                                                                                                                       \\  \hline
%                                       \multicolumn{1}{c}{Base}    & \cellcolor{gray!15}$64.98{\scriptstyle\pm1.84}$ & $62.65{\scriptstyle\pm3.09}$ & $62.43{\scriptstyle\pm3.28}$ & $54.69{\scriptstyle\pm2.58}$& $47.68{\scriptstyle\pm2.63}$ & $29.74{\scriptstyle\pm5.21}$                 \\ 
%                                       \multicolumn{1}{c}{+deg}    & $66.54{\scriptstyle\pm2.19}$ & $68.31{\scriptstyle\pm2.70}$ & \cellcolor{gray!15}$68.99{\scriptstyle\pm2.38}$ & $67.68{\scriptstyle\pm3.7}$& $56.86{\scriptstyle\pm8.8}$ & $41.95{\scriptstyle\pm9.56}$                                                        \\  
%                                       \multicolumn{1}{c}{+sign} & \cellcolor{gray!15}$65.31{\scriptstyle\pm3.2}$&  $53.55{\scriptstyle\pm6.35}$& $53.05{\scriptstyle\pm2.28}$&  $51.93{\scriptstyle\pm4.00}$&  $57.17{\scriptstyle\pm3.39}$&  $51.93{\scriptstyle\pm8.95}$                                            \\  
%                                       \multicolumn{1}{c}{+deg,sign}            &  \cellcolor{gray!15}$65.75{\scriptstyle\pm1.81}$ & $61.49{\scriptstyle\pm7.38}$ & $53.73{\scriptstyle\pm7.79}$ &
%                               $52.43{\scriptstyle\pm5.37}$ & $55.92{\scriptstyle\pm5.14}$ & $56.95{\scriptstyle\pm3.93}$               
                               
                              \\ \bottomrule

\end{tabular}
}
\end{adjustbox}
\vspace{-0.5cm}
\end{table*}
We now study the impact of two proposed mechanisms (signed messages and degree correction, \S~\ref{section: model_design}). To better show their effects, we  add each design choice to a base model and track the changes in the node classification performance. As the base model, we choose a GCN variant that uses the message passing mechanism \citep{kipf2016semi} with weight bias, a residual connection (but \textit{not decaying aggregation}) for robustness to oversmoothing, and Elu non-linearity $\sigma$. 
We denote the model that replaces the message passing with our signed messages mechanism as \texttt{+sign}, and the model that incorporates the degree correction as \texttt{+deg}. The model that uses both designs is denoted as \texttt{+sign,deg}. 
Table~\ref{tab:ablation} gives the accuracy of the models in the supervised node classification task for different layers. 

We observe that both mechanisms alleviate the oversmoothing problem. Specifically, the base model has a sharp performance decrease after 32 layers, while the other models have significantly higher performance. 
In general, the \texttt{+deg} model is better than \texttt{+sign} in alleviating oversmoothing, and has a consistent performance gain across different data. For Chameleon, we observe increase in accuracy as we stack more layers; the large performance gain of \method results from the degree correction.
In Cora and Cornell, \texttt{+sign,deg} consistently performs better across different layers than the model with only one design, demonstrating the constructive effect from our two proposed mechanisms.

The signed message design has an advantage in heterophilous datasets. In the Cornell dataset, using signed information rather than plain message passing  results in over 20\% gain, which explains the strong performance of \method. However, in homophilous datasets, the benefit from signed messages is  limited, as these datasets have few different-class neighbors. % from different classes. %This is understandable, because in homophily datasets, there are not many neighbors from other classes. 
%As we pointed out in Thm.~\ref{theorem: signed_messages},  when signs are included, the error rate affects the performance. For the models that do not include signed messages, Thms.~\ref{theorem: initial_stage} and~\ref{theorem: developing stage} indicate that the effective homophily level affects the performance. 
{This is because when the effective homophily $\heterophilyil$ is high and error rate $e_i^0$ is low, $\lim_{\heterophilyil \to 1, e_i^0 \to 0} \frac{(1+\rho)\heterophilyil-\rho}{(1 - 2e_i^0)(\rho+(1-\rho)\heterophilyil)}=1$, so using signed messages is less beneficial in homophilous datasets.}



\subsection{Batch norm \& Layer norm}
\label{app:batchnorm_layernorm}
In \S~\ref{section: model_design}, we use decaying aggregation instead of other normalizing mechanisms. Other mechanisms, such as batch or layer norm, may be seen as solutions to the heterophily and oversmoothing problems. 
However, batch norm cannot compensate for the dispersion of the mean vectors (\S~\ref{section: analysis}) due to different degrees and homophily levels of the nodes. Although, to some extent, it reduces the speed by which the representations of the susceptible nodes (case 1 \& 2) move towards the other class (good for oversmoothing), it also prevents the representations of the nodes that could benefit from the propagation (case 3) from increasing the distances (drop in accuracy). 
%In our experiments , we find that, in general, adding batch norm significantly decreases the accuracy in heterophily datasets, but helps alleviate oversmoothing. 
%Layer norm is a better option~\cite{zhou2020understanding} for oversmoothing and leads to a smaller decrease in accuracy than batch norm in most datasets. However, %in our experiments (App.~\ref{app:batchnorm_layernorm}), 
Layer norm is better at overcoming the dispersion effect but may lead to a significant accuracy drop in some datsets when a subset of features are more important than the others. Thus, we \textbf{do not} use any of these normalizations. 

%In this section, we verify this conjecture by comparing the prediction accuracy of the base model with  models that use either batch norm or layer norm. % in the supervised node classification tasks on real datasets.
Next, we provide experiments to show the effects of batch norm and layer norm. We use the following base model (the same model used in \S \ref{subsec:ablation}): a GCN~\cite{kipf2016semi} with weight bias, Elu non-linearity and residual connection. We do \textbf{not} include any of our designs so as to exclude any other factors that can affect the performance. The models we compare against are \texttt{+BN} and \texttt{+LN}, which %. \texttt{+BN} and \texttt{+LN} 
represent the models that add batch norm and layer norm right before the non-linear activation, respectively. 

\setlength{\tabcolsep}{3pt}
\begin{table*}[h]
\vspace{-0.2cm}
\centering
\caption{Effects of using batch norm \& layer norm: decrease in accuracy but improvement in oversmoothing. Best performance of each model across different layers is highlighted in gray.}
\label{tab:bn_ln}
\begin{adjustbox}{width=\linewidth}
{\footnotesize
\begin{tabular}{ccccccccccccccc}
\toprule
                                         %\multirow{2}{*}{\backslashbox{\textbf{Model}}{\textbf{Layers}}}    
                                \multicolumn{1}{r}{\textbf{Layers}} 
                                      && \textbf{2}           & \multicolumn{1}{c}{\textbf{4}} & \multicolumn{1}{c}{\textbf{8}} & \multicolumn{1}{c}{\textbf{16}} & \multicolumn{1}{c}{\textbf{32}} & \multicolumn{1}{c}{\textbf{64}} &&  \multicolumn{1}{c}{\textbf{2}}           & \multicolumn{1}{c}{\textbf{4}} & \multicolumn{1}{c}{\textbf{8}} & \multicolumn{1}{c}{\textbf{16}} & \multicolumn{1}{c}{\textbf{32}} & \multicolumn{1}{c}{\textbf{64}}  \\ \cmidrule{1-1} \cmidrule{3-8} \cmidrule{10-15} %cline{2-8}
%\multirow{10}{*}{\rotatebox[origin=c]{90}{\textbf{Homophily datasets}}}   
%\textbf{Model} 
&& \multicolumn{6}{c}{\textbf{Cora} ($h$=0.81)}     & & \multicolumn{6}{c}{\textbf{Citeseer} ($h$=0.74)}                                                                         \\ %\cline{1-1} 
\cline{3-8} \cline{10-15}
                                    
                                        \multicolumn{1}{c}{Base}    &&   
                                        %cora results
                                        \cellcolor{gray!15}$ 86.56{\scriptstyle\pm1.21}$         & \multicolumn{1}{c}{$ 86.04{\scriptstyle\pm0.72}$}    &        \multicolumn{1}{c}{$ 85.51{\scriptstyle\pm1.51}$}     &       \multicolumn{1}{c}{$ 85.33{\scriptstyle\pm0.72}$}      &     \multicolumn{1}{c}{$ 85.37{\scriptstyle\pm1.58}$}       &    \multicolumn{1}{c}{$ 72.17{\scriptstyle\pm8.89}$}   & &  
                                        % citeseer results
                                        \cellcolor{gray!15}$76.51{\scriptstyle\pm1.63}$ & $75.03{\scriptstyle\pm1.67}$ & $73.96{\scriptstyle\pm1.52}$ & $73.59{\scriptstyle\pm1.51}$& $71.91{\scriptstyle\pm1.94}$ & $32.08{\scriptstyle\pm15.74}$                                         \\ 
                                        
                                      \multicolumn{1}{c}{\texttt{+BN}}    &&  
                                      %cora results
                                      $84.73{\scriptstyle\pm1.10}$      &          \multicolumn{1}{c}{$83.76{\scriptstyle\pm1.61}$}           & \multicolumn{1}{c}{$83.94{\scriptstyle\pm1.51}$}           & \multicolumn{1}{c}{$84.57{\scriptstyle\pm1.22}$}            & \multicolumn{1}{c}{$84.63{\scriptstyle\pm1.58}$}            & \cellcolor{gray!15}{$85.17{\scriptstyle\pm1.18}$}   &   &                   % citeseer results
                                      $71.62{\scriptstyle\pm1.48}$  & $71.58{\scriptstyle\pm1.00}$&  $72.18{\scriptstyle\pm1.39}$&  $72.45{\scriptstyle\pm1.42}$&  \cellcolor{gray!15}$72.76{\scriptstyle\pm1.31}$&  $72.61{\scriptstyle\pm1.41}$
                                      \\  \multicolumn{1}{c}{\texttt{+LN}} &&  
                                      %cora results
                                      $84.73{\scriptstyle\pm1.63}$&   $86.60{\scriptstyle\pm1.01}$&   \cellcolor{gray!15}$86.72{\scriptstyle\pm1.36}$&   $86.08{\scriptstyle\pm1.16}$&   $85.67{\scriptstyle\pm1.23}$&   $85.13{\scriptstyle\pm1.20}$   & &    % citeseer results
                                      \cellcolor{gray!15}$76.11{\scriptstyle\pm1.80}$&  $74.02{\scriptstyle\pm2.77}$&   $75.00{\scriptstyle\pm1.95}$&   $74.50{\scriptstyle\pm0.96}$&   $74.49{\scriptstyle\pm2.10}$&   $73.94{\scriptstyle\pm2.03}$
                        \\   \midrule %\cmidrule{1-1} \cmidrule{3-8} \cmidrule{10-15} 
                                    %   & \multicolumn{6}{c}{\textbf{Citeseer ($h$=0.74)}}                                                            \\ \hline 
                                        % \multicolumn{1}{c}{Base}    & \cellcolor{gray!15}$76.51{\scriptstyle\pm1.63}$ & $75.03{\scriptstyle\pm1.67}$ & $73.96{\scriptstyle\pm1.52}$ & $73.59{\scriptstyle\pm1.51}$& $71.91{\scriptstyle\pm1.94}$ & $32.08{\scriptstyle\pm15.74}$                                         \\  
                                    %   \multicolumn{1}{c}{+deg}    &  \cellcolor{gray!15}$76.63{\scriptstyle\pm1.38}$  & $74.64{\scriptstyle\pm1.97}$&  $74.15{\scriptstyle\pm1.61}$&  $73.73{\scriptstyle\pm1.31}$&  $73.61{\scriptstyle\pm1.84}$&  $70.56{\scriptstyle\pm2.27}$                     \\  
                                    %   \multicolumn{1}{c}{+sign} &   \cellcolor{gray!15}$77.13{\scriptstyle\pm1.69}$&  $74.56{\scriptstyle\pm2.02}$&   $73.64{\scriptstyle\pm1.65}$&   $72.31{\scriptstyle\pm2.32}$&   $71.98{\scriptstyle\pm3.44}$&   $68.68{\scriptstyle\pm6.72}$                                                                     \\ 
                            %           \multicolumn{1}{c}{+deg,sign}   & \cellcolor{gray!15}$76.81{\scriptstyle\pm1.71}$ & $74.68{\scriptstyle\pm1.97}$ & $74.69{\scriptstyle\pm2.35}$ &
                            %   $73.28{\scriptstyle\pm1.45}$ & $71.81{\scriptstyle\pm2.28}$ & $69.91{\scriptstyle\pm3.97}$                                              \\ \hline
&& \multicolumn{6}{c}{\textbf{Cornell ($h$=0.3)}} && \multicolumn{6}{c}{\textbf{Chameleon ($h$=0.23)}}                                                                                                                                                                                                                               \\ %\cline{1-1} 
\cline{3-8} \cline{10-15} 
                                      \multicolumn{1}{c}{Base}    && \cellcolor{gray!15}$61.89{\scriptstyle\pm3.72}$ & $60.00{\scriptstyle\pm5.24}$ & $58.92{\scriptstyle\pm5.24}$ &
                              $56.49{\scriptstyle\pm5.73}$ & $58.92{\scriptstyle\pm3.15}$ & $49.19{\scriptstyle\pm16.70}$          &&
% Chameleon results
\cellcolor{gray!15}$64.98{\scriptstyle\pm1.84}$ & $62.65{\scriptstyle\pm3.09}$ & $62.43{\scriptstyle\pm3.28}$ & $54.69{\scriptstyle\pm2.58}$& $47.68{\scriptstyle\pm2.63}$ & $29.74{\scriptstyle\pm5.21}$
\\  
                                      \multicolumn{1}{c}{\texttt{+BN}}    && $58.38{\scriptstyle\pm6.42}$ & \cellcolor{gray!15}$59.19{\scriptstyle\pm4.59}$ & $55.41{\scriptstyle\pm6.65}$ &
                              $57.30{\scriptstyle\pm3.15}$ & $57.57{\scriptstyle\pm6.29}$ & $57.02{\scriptstyle\pm6.19}$    &&
% Chameleon results
$60.88{\scriptstyle\pm2.24}$ & $61.38{\scriptstyle\pm2.17}$ & $61.84{\scriptstyle\pm4.08}$ & \cellcolor{gray!15}$61.97{\scriptstyle\pm3.01}$& $59.04{\scriptstyle\pm3.79}$ & $57.84{\scriptstyle\pm3.67}$
\\  
                                      \multicolumn{1}{c}{\texttt{+LN}} && $58.11{\scriptstyle\pm6.19}$&  $55.68{\scriptstyle\pm6.19}$& $58.92{\scriptstyle\pm7.63}$&  \cellcolor{gray!15}$59.19{\scriptstyle\pm3.07}$&  $58.92{\scriptstyle\pm3.15}$&  $58.00{\scriptstyle\pm3.03}$    && 
% Chameleon results
$61.86{\scriptstyle\pm1.73}$&  $62.17{\scriptstyle\pm2.48}$& \cellcolor{gray!15}$62.41{\scriptstyle\pm2.99}$&  $60.37{\scriptstyle\pm2.36}$&  $58.25{\scriptstyle\pm3.03}$&  $58.92{\scriptstyle\pm3.15}$
\\  
                                      
%                                       \\ \hline
% %\multirow{10}{*}{\rotatebox[origin=c]{90}{\textbf{Heterophily datasets}}} 
% & \multicolumn{6}{c}{\textbf{Chameleon ($h$=0.23)}}                                                                                                                                                                                                                                       \\  \hline
%                                       \multicolumn{1}{c}{Base}    & \cellcolor{gray!15}$64.98{\scriptstyle\pm1.84}$ & $62.65{\scriptstyle\pm3.09}$ & $62.43{\scriptstyle\pm3.28}$ & $54.69{\scriptstyle\pm2.58}$& $47.68{\scriptstyle\pm2.63}$ & $29.74{\scriptstyle\pm5.21}$                 \\ 
%                                       \multicolumn{1}{c}{+deg}    & $66.54{\scriptstyle\pm2.19}$ & $68.31{\scriptstyle\pm2.70}$ & \cellcolor{gray!15}$68.99{\scriptstyle\pm2.38}$ & $67.68{\scriptstyle\pm3.7}$& $56.86{\scriptstyle\pm8.8}$ & $41.95{\scriptstyle\pm9.56}$                                                        \\  
%                                       \multicolumn{1}{c}{+sign} & \cellcolor{gray!15}$65.31{\scriptstyle\pm3.2}$&  $53.55{\scriptstyle\pm6.35}$& $53.05{\scriptstyle\pm2.28}$&  $51.93{\scriptstyle\pm4.00}$&  $57.17{\scriptstyle\pm3.39}$&  $51.93{\scriptstyle\pm8.95}$                                            \\  
%                                       \multicolumn{1}{c}{+deg,sign}            &  \cellcolor{gray!15}$65.75{\scriptstyle\pm1.81}$ & $61.49{\scriptstyle\pm7.38}$ & $53.73{\scriptstyle\pm7.79}$ &
%                               $52.43{\scriptstyle\pm5.37}$ & $55.92{\scriptstyle\pm5.14}$ & $56.95{\scriptstyle\pm3.93}$               
                               
                               \bottomrule

\end{tabular}
}
\end{adjustbox}
\vspace{-0.1cm}
\end{table*}

Table~\ref{tab:bn_ln} shows that both batch norm and layer norm can help with oversmoothing. Moreover, adding layer norm is in general better than adding batch norm. This is expected because the scaling effect caused by the propagation can be alleviated by normalizing across the node representations. Thus, the dispersion of the expected representations can be mitigated. On the other hand, batch norm normalizes across all the nodes, so it requires sacrificing the nodes that benefit (case 3) to compensate for the nodes that are prone to moving towards the other classes (case 1 \& case 2). As a result, batch norm is less effective in mitigating oversmoothing and leads to a bigger decrease in accuracy. 

Another finding is that both layer norm and batch norm lead to a significant accuracy decrease (2\%-3\%) in the heterophilous datasets. \texttt{+BN} has a clear accuracy drop even in the homophilous datasets. As Thm.~\ref{theorem: initial_stage} points out: higher heterophily level may result in sign flip ($\gamma_i^l<0$). If the representations flip the sign, using batch norm or layer norm will not revert the sign, but they may instead encourage the representations to move towards the other class more.

Given the limitations shown above, we \textbf{do not} use either batch norm or layer norm in our proposed model, \method.

\subsection{More on the Initial \& Developing Stages}
\label{app:2stages}
Section \ref{exp:case study} shows how the node classification accuracy changes for nodes of different degrees with the number of layers on Citeseer. Here, we provide more details of this experiment and give the results on another dataset,  Cora.

\textbf{Datasets.} According to Thm.~\ref{theorem: initial_stage} and~\ref{theorem: developing stage}, in order to see both the initial and the developing stage, we need to use homophilous datasets. In  heterophilous datasets, most nodes satisfy case 1, so the initial stage does not exist. %There are no three cases as in the initial stage and only case 2 exists.

\textbf{Measurement of effective homophily $\pmb{\heterophilyil}$.} %To align this with our theorems---which apply to binary classification---, the decision boundary is defined as the curve that maximizes the margins between the initial features in different classes. In binary classification, the decision boundary is the origin. 
To estimate the effective homophily $\heterophilyil$, we measure the portion of neighbors that have the same ground truth label as $v_i$ and are correctly classified. 
% We use this ratio to approximate the neighbors whose features are still inside the decision boundary of class $y_i$.  
%Our goal is to estimate the effective homophily $\hat{h_i}$ before the last propagation takes place and analyze its impact on the accuracy of the final layer. 
% \reminder{thenext sentence is not clear -- do you mean before performing the linear transformation too?}
Following our theory, we estimate $\heterophilyil$ \textbf{before} the last propagation takes place and analyze its impact on the accuracy of the final layer. 
In more detail, we obtain the node representations before the last propagation from a trained vanilla GCN~\cite{kipf2016semi} and then perform a linear transformation using the weight matrix and bias vector from the last layer. Then, we use the transformed representations to classify the neighbors of node $v_i$ and compute $\heterophilyil$. We note that we leverage the intermediate representations only for the estimation of $\heterophilyil$; the accuracy of the final layer is still measured using the outputs from the final layer. 
% The reason for using the features before the last propagation is that we would like to estimate the effective homophily $\hat{h_i}$ before the last propagation takes place and analyze $\hat{h_i}$'s impact on the accuracy of the final layer. 

\setlength{\tabcolsep}{4pt}
\begin{wraptable}{r}{8.2cm}
    \centering
    \vspace{-0.5cm}
    \caption{Citeseer: Accuracy (Acc) and average effective homophily ($\Bar{\heterophilyil}$) for nodes with different degrees across various layers. Last layer of initial stage marked in gray.} %The last layer in the initial stage ($\Bar{\hat{h_i}} > 0.5$ for all degrees) are marked in grey.}
    \vspace{0.1cm}
    % \begin{adjustbox}{width=0.5\textwidth}
    % {\footnotesize
    \resizebox{!}{.38\linewidth}{%\footnotesize
    \begin{tabular}{ccccccc} 
    \toprule
          & & \multicolumn{5}{c}{\bf Degrees} \\ \cline{3-7}
      \multicolumn{1}{c}{\bf  Layers} & %\backslashbox{Acc, $\Bar{\hat{h_i}}$}{Degrees} 
      &   $[1,2]$           &   $[3,6]$            &   $[7,15]$   &   $[16,39]$ & $[40,99]$  \\
    \midrule
       \multirow{2}{*}{\bf 2}& Acc & $74.44$ & $78.51$ & $84.04$
        & $96.00$ & $100.00$  \\ & $\Bar{\heterophilyil}$ & $0.65$ & $0.67$ & $0.72$
        & $0.83$ & $0.91$  \\
        \midrule
       \multirow{2}{*}{\bf 3}& Acc & $70.92$ & $77.59$ & $83.03$
        & $92.75$ & $100.00$  \\& $\Bar{\heterophilyil}$  & $0.63$ & $0.66$ & $0.71$
        & $0.84$ & $0.92$  \\
        \midrule
       \multirow{2}{*}{\bf 4}& Acc & $60.54$ & $68.56$ & $77.63$
        & $94.00$ & $100.00$  \\& $\Bar{\heterophilyil}$  & \cellcolor{gray!15}$0.54$ & \cellcolor{gray!15}$0.58$ & \cellcolor{gray!15}$0.66$
        & \cellcolor{gray!15}$0.79$ & \cellcolor{gray!15}$0.84$  \\
        \midrule
       \multirow{2}{*}{\bf 5}& Acc & $41.66$ & $48.70$ & $56.97$
        & $61.33$ & $11.11$  \\& $\Bar{\heterophilyil}$  & $0.36$ & $0.38$ & $0.45$
        & $0.48$ & $0.11$  \\
        \midrule
       \multirow{2}{*}{\bf 6}& Acc & $23.61$ & $28.87$ & $41.17$
        & $31.83$ & $0.00$  \\& $\Bar{\heterophilyil}$  & $0.18$ & $0.19$ & $0.27$
        & $0.22$ & $0.00$  \\
	   \bottomrule
    \end{tabular}}
    % \end{adjustbox}
    %}  
    % \vspace{-0.3cm}
    \label{tab:case_study_citeseer}
\end{wraptable}

\textbf{Degree intervals.} To investigate the change in GCN accuracy with different layers for nodes with different degrees, we categorize the nodes in $n$ degree intervals. For the degree intervals, we use logarithmic binning (base 2). In detail, we denote the highest and lowest degree by $d_{max}$ and $d_{min}$, respectively, and let $\Omega \equiv \frac{\log_2{d_{max}}-\log_2{d_{min}}}{n}$. Then, we divide the nodes into $n$ intervals, where the $j$-th interval is defined as: $[d_{min}\cdot 2^{(j-1)\Omega}, d_{min}\cdot 2^{j\Omega})$.

% Then we will show the accuracy of GCNs with different layers for nodes with different degrees. 

\textbf{Dataset: Citeseer.}
Figure~\ref{fig:phase_transition} and Table~\ref{tab:case_study_citeseer} show how the accuracy changes with the number of layers for different node degree intervals. We observe that in the initial stage, the accuracy increases as the degree and $\Bar{\heterophilyil}$ increase. However, in the developing stage, the accuracy of high-degree nodes drops more sharply than that of low-degree nodes. 

\textbf{Dataset: Cora.}  The results for Cora are shown in 
% As can be seen in 
Figure~\ref{fig:case_study_cora} and Table~\ref{tab:case_study_cora}.  
In the initial stage, the nodes with lower 

% \vspace{0.3cm}
\begin{minipage}{\textwidth}
\begin{minipage}[c]{0.55\textwidth}
\centering
\includegraphics[scale=0.18, bb=800 400 450 200]{Figs/transition_plot_cora_new.png}
\captionsetup{type=figure}
\vspace{2.5cm}
\captionof{figure}{Cora: Accuracy per (logarithmic) degree bin.}
\label{fig:case_study_cora}
\end{minipage}
% \begin{adjustbox}{width=0.38\textwidth}
\begin{minipage}[c]{0.45\textwidth}
\setlength{\tabcolsep}{5pt}
    \centering
    \captionsetup{type=table}
    \captionof{table}{Cora: Accuracy and average effective homophily ($\Bar{\heterophilyil}$) for nodes with different degrees across different layers. Last layer of initial stage marked in gray.}
    \resizebox{!}{.45\linewidth}{%\footnotesize
    \begin{tabular}{ccccccc} 
    \toprule
      & & \multicolumn{5}{c}{\bf Degrees} \\ \cline{3-7}
      \multicolumn{1}{c}{\bf Layers} & %\backslashbox{Acc, $\Bar{\hat{h_i}}$}{Degrees} 
      &   $[1,2]$           &   $[3,7]$            &   $[8,21]$   &   $[22,60]$ & $[61,168]$  \\
    \midrule
       \multirow{2}{*}{\bf 2}& Acc & $85.14$ & $88.52$ & $83.78$
        & $90.00$ & $100.00$  \\ & $\Bar{\heterophilyil}$ & $0.77$ & $0.77$ & $0.72$
        & $0.63$ & $0.81$  \\
        \midrule
       \multirow{2}{*}{\bf 3}& Acc & $82.28$ & $87.26$ & $84.42$
        & $85.00$ & $100.00$  \\& $\Bar{\heterophilyil}$  & $0.77$ & $0.78$ & $0.73$
        & $0.64$ & $0.84$  \\
        \midrule
       \multirow{2}{*}{\bf 4}& Acc & $79.57$ & $85.52$ & $83.26$
        & $85.00$ & $100.00$  \\& $\Bar{\heterophilyil}$  & $0.75$ & $0.76$ & $0.71$
        & $0.63$ & $0.80$  \\
        \midrule
        \multirow{2}{*}{\bf 5}& Acc & $77.38$ & $83.75$ & $82.83$
        & $85.00$ & $96.19$  \\& $\Bar{\heterophilyil}$  & $0.72$ & $0.73$ & $0.68$
        & $0.56$ & $0.83$  \\
        \midrule
        \multirow{2}{*}{\bf 6}& Acc & $63.35$ & $68.20$ & $66.01$
        & $70.00$ & $78.57$  \\& $\Bar{\heterophilyil}$  & \cellcolor{gray!15}$0.57$ & \cellcolor{gray!15}$0.60$ & \cellcolor{gray!15}$0.54$
        & \cellcolor{gray!15}$0.52$ & \cellcolor{gray!15}$0.67$  \\
        \midrule
       \multirow{2}{*}{\bf 7}& Acc & $30.91$ & $30.62$ & $29.12$
        & $17.50$ & $21.43$  \\& $\Bar{\heterophilyil}$  & $0.25$ & $0.26$ & $0.21$
        & $0.26$ & $0.23$  \\
        \midrule
       \multirow{2}{*}{\bf 8}& Acc & $31.48$ & $31.02$ & $28.44$
        & $32.50$ & $25.24$  \\& $\Bar{\heterophilyil}$  & $0.24$ & $0.26$ & $0.20$
        & $0.28$ & $0.24$  \\
	   \bottomrule
    \end{tabular}
        \vspace{-1cm}
    }
\label{tab:case_study_cora}
\end{minipage}
% \end{adjustbox}
    \vspace{-0.3cm}
\end{minipage}

\clearpage
% In the initial stage, the nodes with lower  
degrees usually have lower accuracy. One exception is the nodes with degrees in the 
range $[3, 7]$. These nodes have higher accuracy because the average effective homophily $\Bar{\heterophilyil}$ of that degree group is the second highest. In the developing stage, the accuracy of the high-degree nodes drops more than the accuracy of the remaining node groups. 

GCN's behavior on both Citesser and Cora datasets verifies our conjecture based on our theorems in \S~\ref{subsec: heterophily_oversmoothing}.



% \begin{wrapfigure}{r}{0.56\textwidth}
% \centering
% \includegraphics[width=.54\textwidth]{Figs/transition_cora_plot.png}
% \vspace{-0.5cm}
% \caption{Accuracy per (logarithmic) degree bin on Cora.}
% \label{fig:phase_transition_cora}
% \vspace{-0.6cm}
% \end{wrapfigure}
% \setlength{\tabcolsep}{4pt}
% \begin{wraptable}{r}{7cm}
%     \centering
%     \vspace{-0.9cm}
%     \caption{Accuracy (Acc) and average effective homophily ($\Bar{\hat{h_i}}$) for nodes with different degrees across various layers on Citeseer dataset. The last layer in the initial stage ($\Bar{\hat{h_i}} > 0.5$ for all degrees) are marked in grey.}
%     \label{tab:case_study_citeseer}
%     \begin{adjustbox}{width=0.4\textwidth}
%     {\footnotesize
%     \begin{tabular}{c|c|ccccc} 
%     \toprule
%       \multicolumn{1}{c|}{Layers} & \backslashbox{Acc, $\Bar{\hat{h_i}}$}{Degrees} &   $[1,2]$           &   $[3,6]$            &   $[7,15]$   &   $[16,39]$ & $[40,99]$  \\
%     \midrule
%       \multirow{2}{*}{2}& Acc & $74.44$ & $78.51$ & $84.04$
%         & $96.00$ & $100.00$  \\ & $\Bar{\hat{h_i}}$ & $0.65$ & $0.67$ & $0.72$
%         & $0.83$ & $0.91$  \\
%         \midrule
%       \multirow{2}{*}{3}& Acc & $70.92$ & $77.59$ & $83.03$
%         & $92.75$ & $100.00$  \\& $\Bar{\hat{h_i}}$  & $0.63$ & $0.66$ & $0.71$
%         & $0.84$ & $0.92$  \\
%         \midrule
%       \multirow{2}{*}{4}& Acc & $60.54$ & $68.56$ & $77.63$
%         & $94.00$ & $100.00$  \\& $\Bar{\hat{h_i}}$  & \cellcolor{gray!15}$0.54$ & \cellcolor{gray!15}$0.58$ & \cellcolor{gray!15}$0.66$
%         & \cellcolor{gray!15}$0.79$ & \cellcolor{gray!15}$0.84$  \\
%         \midrule
%       \multirow{2}{*}{5}& Acc & $41.66$ & $48.70$ & $56.97$
%         & $61.33$ & $11.11$  \\& $\Bar{\hat{h_i}}$  & $0.36$ & $0.38$ & $0.45$
%         & $0.48$ & $0.11$  \\
%         \midrule
%       \multirow{2}{*}{6}& Acc & $23.61$ & $28.87$ & $41.17$
%         & $31.83$ & $0.00$  \\& $\Bar{\hat{h_i}}$  & $0.18$ & $0.19$ & $0.27$
%         & $0.22$ & $0.00$  \\
% 	   \bottomrule
%     \end{tabular}}
%     \end{adjustbox}
%     %}  
%     \vspace{-0.5cm}
% \end{wraptable}
% As can be seen in Figure~\ref{fig:case_study_cora} and Table~\ref{tab:case_study_cora}, in the initial stage, the nodes with lower degrees usually have lower accuracy. One exception is the nodes whose degrees are in the range $[3, 7]$. They have higher accuracy because the average effective homophily $\Bar{\hat{h_i}}$ of that group is the second highest. In the developing stage, the large degree nodes drop more. 

% GCN's behavior on both Citesser and Cora datasets have verified the conjecture we made based on the theorems in \S \ref{subsec: heterophily_oversmoothing}.
% \subsection{Additional baselines}
% \label{app:additional baselines}
% Due to limited space, we only provide representative baselines in \S~\ref{section: experiments}. Here we provide another two baselines from recent works. PairNorm~\cite{zhao2019pairnorm} is proposed to address the oversmoothing problem and GPRGNN~\cite{chien2021adaptive} is proposed to address both oversmoothing and heterophily problems. We use their original model files and train their models with the datasets and splits we use for every GCN models. We adopt the same hyperperameters as they do. Note that in ~\cite{chien2021adaptive}, the authors use balanced training sets (same number of nodes from different classes), so their reported results for GPRGNN and other baselines (e.g, MLP) are different from the reported results in ours and other papers [36, 37]. \yy{change the citations}

% As shown in Tab.~\ref{tab:real-results} and Tab.~\ref{tab:additional_baselines_performance}, GPRGNN has good performance in homophily datasets such as Citeseer and Cora. For heterophily datasets, though they show improvements over GCNII* and Geom-GCN*, the performance of GPRGNN is close to the performance of MLP and is worse than \method(ours) and H2GCN*. PN is proposed to address oversmoothing so it does not have very competitive results in heterophily datasets. 
% \begin{table*}[h]%[t!]
%     \centering
%     \vspace{-0.2cm}
%     \caption{%Statistics of real datasets for different homophily levels $h$, 
%     Real data: mean accuracy $\pm$ stdev over different data splits. Per GCN model, we report the best performance  across different layers. 
%     }
%     \label{tab:additional_baselines_performance}
%     %\resizebox{0.97\textwidth}{!}{
%     \vspace{-0.15cm}
%     \begin{adjustbox}{width=.9\textwidth}
%     % \hskip-1.15cm
%     \begin{tabular}{lcccccc  ccc c } % Removed vertical rule due to NIPS requirement
%     \toprule
%       %\multirow{2}{*}{\backslashbox{\textbf{Models}}{\textbf{Data, h}}} 
%       &  \texttt{\bf Texas}           &   \texttt{\bf Wisconsin}           &   \texttt{\bf Actor}            &   \texttt{\bf Squirrel}   &   \texttt{\bf Chameleon} & \texttt{\bf Cornell}        &   \texttt{\bf Citeseer}           &   \texttt{\bf Pubmed}            &   \texttt{\bf Cora} \\
%         % & $h=0.11$ & $h=0.21$ & $h=0.22$ & $h=0.22$ & $h=0.23$ & $h=0.3$ & $h=0.57$ & $h=0.74$ & $h=0.8$ & $h=0.81$  \\
%         % \midrule 
%           \textbf{Hom.\ level} $h$ & \textbf{0.11} & \textbf{0.21} & \textbf{0.22} & \textbf{0.22} & \textbf{0.23} & \textbf{0.3} & \textbf{0.74} & \textbf{0.8} & \textbf{0.81} \\
% 		\textbf{\#Nodes} & 183 & 251 & 7,600 & 5,201 & 2,277 & 183 & 3,327 & 19,717 & 2,708 \\
% 		\textbf{\#Edges} & 295 & 466 & 26,752 & 198,493 & 31,421 & 280 & 4,676 & 44,327 & 5,278 \\
% 		\textbf{\#Classes} & 5 & 5 & 5 & 5 & 5 & 5 & 7 & 3 & 6 \\ 
%     \midrule
%     % \midrule
%       % HistFNN --network_setup M64-R-G-V-MO --hist_nhood 0 1 2
%       {PN} & $60.27{\scriptstyle\pm4.34}$ & $48.43{\scriptstyle\pm6.14}$ &
%       $27.40{\scriptstyle\pm1.24}$ & $50.44{\scriptstyle\pm2.04}$ & $62.74{\scriptstyle\pm2.82}$ &  $58.92{\scriptstyle\pm3.15}$ &  $73.59{\scriptstyle\pm1.47}$ & $87.53{\scriptstyle\pm0.44}$ & $85.79{\scriptstyle\pm1.01}$ \\
%       % HistFNN --network_setup M64-R-G-V-G-V-MO --hist_nhood 0 1 2
%       {GPRGNN} & $78.38{\scriptstyle\pm4.36}$ & $82.94{\scriptstyle\pm4.21}$ & $34.63{\scriptstyle\pm1.22}$ & $31.61{\scriptstyle\pm1.24}$ & $46.58{\scriptstyle\pm1.71}$ & $80.27{\scriptstyle\pm8.11}$ &  $77.13{\scriptstyle\pm1.67}$ & $87.54{\scriptstyle\pm0.38}$ & $87.95{\scriptstyle\pm1.18}$ \\
%       \bottomrule
%     \end{tabular}
%     \end{adjustbox}
%     %}  
%     \vspace{-0.3cm}
% \end{table*}

% From Tab.~\ref{tab:oversmoothing} and Tab.~\ref{tab:more_baselines_oversmoothing}, we can see that both GPRGNN and PN are effective in alleviating oversmoothing compared to the vanilla GCN~\cite{kipf2016semi}. PN suffers from performance drop after 32 layers. Both our model \method (Tab.~\ref{tab:oversmoothing}) and GPRGNN maintain good performance after 32 layers.
% \begin{table*}[h]
% \centering
% \caption{Model performance for different layers: mean accuracy $\pm$ stdev over different data splits.}
% \label{tab:more_baselines_oversmoothing}
% \begin{adjustbox}{width=\linewidth}
% {\footnotesize
% \begin{tabular}{ccccccccccccccc}
% \toprule
%                                          %\multirow{2}{*}{\backslashbox{\textbf{Model}}{\textbf{Layers}}}    
%                                 \multicolumn{1}{r}{\textbf{Layers}} 
%                                       && \textbf{2}           & \multicolumn{1}{c}{\textbf{4}} & \multicolumn{1}{c}{\textbf{8}} & \multicolumn{1}{c}{\textbf{16}} & \multicolumn{1}{c}{\textbf{32}} & \multicolumn{1}{c}{\textbf{64}} &&  \multicolumn{1}{c}{\textbf{2}}           & \multicolumn{1}{c}{\textbf{4}} & \multicolumn{1}{c}{\textbf{8}} & \multicolumn{1}{c}{\textbf{16}} & \multicolumn{1}{c}{\textbf{32}} & \multicolumn{1}{c}{\textbf{64}}  \\ \cmidrule{1-1} \cmidrule{3-8} \cmidrule{10-15} %cline{2-8}
% %\multirow{10}{*}{\rotatebox[origin=c]{90}{\textbf{Homophily datasets}}}   
% %\textbf{Model} 
% && \multicolumn{6}{c}{\textbf{Cora} ($h$=0.81)}     & & \multicolumn{6}{c}{\textbf{Citeseer} ($h$=0.74)}                                                                         \\ %\cline{1-1} 
% \cline{3-8} \cline{10-15}
                                    
%                                         \multicolumn{1}{c}{PN}    &&   
%                                         %cora results
%                                         \cellcolor{gray!15}$ 85.79{\scriptstyle\pm1.01}$         & \multicolumn{1}{c}{$ 85.07{\scriptstyle\pm0.91}$}    &        \multicolumn{1}{c}{$ 84.65{\scriptstyle\pm1.09}$}     &       \multicolumn{1}{c}{$ 82.21{\scriptstyle\pm2.84}$}      &     \multicolumn{1}{c}{$ 60.32{\scriptstyle\pm8.28}$}       &    \multicolumn{1}{c}{$ 44.39{\scriptstyle\pm5.60}$}   & &  
%                                         % citeseer results
%                                         \cellcolor{gray!15}$73.59{\scriptstyle\pm1.47}$ & $72.62{\scriptstyle\pm1.97}$ & $72.32{\scriptstyle\pm1.58}$ & $59.71{\scriptstyle\pm15.97}$& $27.21{\scriptstyle\pm10.95}$ & $23.82{\scriptstyle\pm6.64}$                                         \\ 
                                        
%                                       \multicolumn{1}{c}{GPRGNN}    &&  
%                                       %cora results
%                                       \multicolumn{1}{c}{$87.93{\scriptstyle\pm1.11}$}      &        \cellcolor{gray!15}$87.95{\scriptstyle\pm1.18}$           & \multicolumn{1}{c}{$87.87{\scriptstyle\pm1.41}$}           & \multicolumn{1}{c}{$87.26{\scriptstyle\pm1.51}$}            & \multicolumn{1}{c}{$87.18{\scriptstyle\pm1.29}$}            & \multicolumn{1}{c}{$87.32{\scriptstyle\pm1.21}$}   &   &                   % citeseer results
%                                       \cellcolor{gray!15}$77.13{\scriptstyle\pm1.67}$  & $77.05{\scriptstyle\pm1.43}$&  $77.09{\scriptstyle\pm1.62}$&  $76.00{\scriptstyle\pm1.64}$&  $74.97{\scriptstyle\pm1.47}$&  $74.41{\scriptstyle\pm1.65}$
                                
%                               \\ \midrule %\cmidrule{1-1} \cmidrule{3-8} \cmidrule{10-15} 
%                                     %   & \multicolumn{6}{c}{\textbf{Citeseer ($h$=0.74)}}                                                            \\ \hline 
%                                         % \multicolumn{1}{c}{Base}    & \cellcolor{gray!15}$76.51{\scriptstyle\pm1.63}$ & $75.03{\scriptstyle\pm1.67}$ & $73.96{\scriptstyle\pm1.52}$ & $73.59{\scriptstyle\pm1.51}$& $71.91{\scriptstyle\pm1.94}$ & $32.08{\scriptstyle\pm15.74}$                                         \\  
%                                     %   \multicolumn{1}{c}{+deg}    &  \cellcolor{gray!15}$76.63{\scriptstyle\pm1.38}$  & $74.64{\scriptstyle\pm1.97}$&  $74.15{\scriptstyle\pm1.61}$&  $73.73{\scriptstyle\pm1.31}$&  $73.61{\scriptstyle\pm1.84}$&  $70.56{\scriptstyle\pm2.27}$                     \\  
%                                     %   \multicolumn{1}{c}{+sign} &   \cellcolor{gray!15}$77.13{\scriptstyle\pm1.69}$&  $74.56{\scriptstyle\pm2.02}$&   $73.64{\scriptstyle\pm1.65}$&   $72.31{\scriptstyle\pm2.32}$&   $71.98{\scriptstyle\pm3.44}$&   $68.68{\scriptstyle\pm6.72}$                                                                     \\ 
%                             %           \multicolumn{1}{c}{+deg,sign}   & \cellcolor{gray!15}$76.81{\scriptstyle\pm1.71}$ & $74.68{\scriptstyle\pm1.97}$ & $74.69{\scriptstyle\pm2.35}$ &
%                             %   $73.28{\scriptstyle\pm1.45}$ & $71.81{\scriptstyle\pm2.28}$ & $69.91{\scriptstyle\pm3.97}$                                              \\ \hline
% && \multicolumn{6}{c}{\textbf{Cornell ($h$=0.3)}} && \multicolumn{6}{c}{\textbf{Chameleon ($h$=0.23)}}                                                                                                                                                                                                                               \\ %\cline{1-1} 
% \cline{3-8} \cline{10-15} 
%                                       \multicolumn{1}{c}{PN}    && $50.27{\scriptstyle\pm7.17}$ & $53.51{\scriptstyle\pm8.00}$ & $58.38{\scriptstyle\pm5.01}$ &
%                               $58.38{\scriptstyle\pm3.01}$ & \cellcolor{gray!15}$58.92{\scriptstyle\pm3.15}$ & $58.92{\scriptstyle\pm3.15}$          &&
% % Chameleon results
% \cellcolor{gray!15}$62.74{\scriptstyle\pm2.82}$ & $59.01{\scriptstyle\pm2.80}$ & $54.12{\scriptstyle\pm2.24}$ & $46.38{\scriptstyle\pm2.23}$& $46.78{\scriptstyle\pm2.26}$ & $46.27{\scriptstyle\pm3.24}$
% \\  
%                                       \multicolumn{1}{c}{GPRGNN}    && $76.76{\scriptstyle\pm8.22}$ & $77.57{\scriptstyle\pm7.46}$ & $\cellcolor{gray!15}80.27{\scriptstyle\pm8.11}$ &
%                               $78.38{\scriptstyle\pm6.04}$ & $74.59{\scriptstyle\pm7.66}$ & $70.00{\scriptstyle\pm5.73}$    &&
% % Chameleon results
% $\cellcolor{gray!15}46.58{\scriptstyle\pm1.771}$ & $45.72{\scriptstyle\pm3.45}$ & $41.16{\scriptstyle\pm5.79}$ & $39.58{\scriptstyle\pm7.85}$& $35.42{\scriptstyle\pm8.52}$ & $36.38{\scriptstyle\pm2.40}$

% %                                       \\ \hline
% % %\multirow{10}{*}{\rotatebox[origin=c]{90}{\textbf{Heterophily datasets}}} 
% % & \multicolumn{6}{c}{\textbf{Chameleon ($h$=0.23)}}                                                                                                                                                                                                                                       \\  \hline
% %                                       \multicolumn{1}{c}{Base}    & \cellcolor{gray!15}$64.98{\scriptstyle\pm1.84}$ & $62.65{\scriptstyle\pm3.09}$ & $62.43{\scriptstyle\pm3.28}$ & $54.69{\scriptstyle\pm2.58}$& $47.68{\scriptstyle\pm2.63}$ & $29.74{\scriptstyle\pm5.21}$                 \\ 
% %                                       \multicolumn{1}{c}{+deg}    & $66.54{\scriptstyle\pm2.19}$ & $68.31{\scriptstyle\pm2.70}$ & \cellcolor{gray!15}$68.99{\scriptstyle\pm2.38}$ & $67.68{\scriptstyle\pm3.7}$& $56.86{\scriptstyle\pm8.8}$ & $41.95{\scriptstyle\pm9.56}$                                                        \\  
% %                                       \multicolumn{1}{c}{+sign} & \cellcolor{gray!15}$65.31{\scriptstyle\pm3.2}$&  $53.55{\scriptstyle\pm6.35}$& $53.05{\scriptstyle\pm2.28}$&  $51.93{\scriptstyle\pm4.00}$&  $57.17{\scriptstyle\pm3.39}$&  $51.93{\scriptstyle\pm8.95}$                                            \\  
% %                                       \multicolumn{1}{c}{+deg,sign}            &  \cellcolor{gray!15}$65.75{\scriptstyle\pm1.81}$ & $61.49{\scriptstyle\pm7.38}$ & $53.73{\scriptstyle\pm7.79}$ &
% %                               $52.43{\scriptstyle\pm5.37}$ & $55.92{\scriptstyle\pm5.14}$ & $56.95{\scriptstyle\pm3.93}$               
                               
%                               \\ \bottomrule

% \end{tabular}
% }
% \end{adjustbox}
% \vspace{-0.7cm}
% \end{table*}
\textcolor{blue}{\subsection{Evaluation Metric}
In Table~\ref{tab:real-results}, we provide the graph's homophily level $h$, which is the average of the node's homophily level. In our theoretical analysis~\S~\ref{section: analysis}, we use the node's homophily level and relative degree to characterize three cases (Fig.~\ref{fig:concept} and Thm.~\ref{theorem: initial_stage}).
To better align with our theoretical analysis, we provide below the proportion of nodes in each case.}

\setlength{\tabcolsep}{4pt}
\begin{table*}[h]%[t!]
    \centering
    \vspace{-0.2cm}
    \caption{%Statistics of real datasets for different homophily levels $h$, 
    The percentage (\%) of nodes in each case (Fig.~\ref{fig:concept} and Thm.~\ref{theorem: initial_stage}): case 1: $h_i\leq \frac{\rho}{1+\rho}$, case 2: $h_i>\frac{\rho}{1+\rho} \ \mathrm{\&}\  \ratioi \leq \frac{1}{(1+\rho)h_i-\rho}$ and case 3: otherwise. The dominate case for each dataset is colored in grey.
    }
    \label{tab:ratios}
    %\resizebox{0.97\textwidth}{!}{
    \vspace{-0.15cm}
    \begin{adjustbox}{width=.9\textwidth}
    % \hskip-1.15cm
    \begin{tabular}{lcccccc  ccc c} % Removed vertical rule due to NIPS requirement
    \toprule
       %\multirow{2}{*}{\backslashbox{\textbf{Models}}{\textbf{Data, h}}} 
       &  \texttt{\bf Texas}           &   \texttt{\bf Wisconsin}           &   \texttt{\bf Actor}            &   \texttt{\bf Squirrel}   &   \texttt{\bf Chameleon} & \texttt{\bf Cornell}        &   \texttt{\bf Citeseer}           &   \texttt{\bf Pubmed}            &   \texttt{\bf Cora} \\
        % & $h=0.11$ & $h=0.21$ & $h=0.22$ & $h=0.22$ & $h=0.23$ & $h=0.3$ & $h=0.57$ & $h=0.74$ & $h=0.8$ & $h=0.81$  \\
        % \midrule 
          \textbf{Hom.\ level} $h$ & \textbf{0.11} & \textbf{0.21} & \textbf{0.22} & \textbf{0.22} & \textbf{0.23} & \textbf{0.3} & \textbf{0.74} & \textbf{0.8} & \textbf{0.81} \\
		\textbf{\#Nodes} & 183 & 251 & 7,600 & 5,201 & 2,277 & 183 & 3,327 & 19,717 & 2,708 \\
		\textbf{\#Edges} & 295 & 466 & 26,752 & 198,493 & 31,421 & 280 & 4,676 & 44,327 & 5,278 \\
		\textbf{\#Classes} & 5 & 5 & 5 & 5 & 5 & 5 & 7 & 3 & 6 \\ 
    \midrule
    % \midrule
       % HistFNN --network_setup M64-R-G-V-MO --hist_nhood 0 1 2
       {Case 1} & \cellcolor{gray!15}$87.43$ & \cellcolor{gray!15}$78.49$ & \cellcolor{gray!15}
       $63.49$ & \cellcolor{gray!15}$47.74$ & \cellcolor{gray!15}$48.48$ &  \cellcolor{gray!15}$79.23$ &  $18.33$ & $14.80$ & $6.50$ \\
       % HistFNN --network_setup M64-R-G-V-G-V-MO --hist_nhood 0 1 2
       {Case 2} & $8.74$ & $15.93$ & $29.53$ & \cellcolor{gray!15}$50.14$ & \cellcolor{gray!15} $48.84$ & $6.01$ &  $25.58$ & $33.75$ & $32.98$ \\
       {Case 3} & $3.83$ & $5.58$ & $6.99$ & $2.11$ & $2.68$ & $14.75$ & \cellcolor{gray!15} $56.09$ & \cellcolor{gray!15}$51.45$ & \cellcolor{gray!15}$60.52$ \\
    %   \textbf{\method-Hist**} \\
    %   \textbf{\method-Avg-1} & $82.70{\scriptstyle \pm 6.52$ & $84.31{\scriptstyle \pm 4.34$ & $34.31{\scriptstyle \pm 1.31$ & $28.98{\scriptstyle \pm 1.97$ & $50.88{\scriptstyle \pm 1.78$ \\
    %   % HistFNN --network_setup M64-R-G-V-G-V-MO --hist_nhood 0 1 2
    %   \textbf{\method-Avg-2} &$80.54{\scriptstyle \pm 6.84$ & $83.14{\scriptstyle \pm 4.26$ & $34.49{\scriptstyle \pm 1.63$ & $31.83{\scriptstyle \pm 2.25$ & $56.47{\scriptstyle \pm 1.58$ \\
	   \bottomrule
    \end{tabular}
    \end{adjustbox}
    %}  
    \vspace{-0.3cm}
\end{table*}
\textcolor{blue}{It can be seen that in general, a low graph's homophily level indicates that case 1 is the dominate case and a high graph's homophily level indicates that case 3 is the dominate case. As we stated in Thm~\ref{theorem: initial_stage}, under "non-swapping" condition, case 3 is the only case to have a benefit. Thus, in the common homophilous datasets we use (Citeseer, Pubmed and Cora), case 3 dominates and enjoys the benefits from graph convolution. In the Texas, Wisconsin and Actor datasets, only case 1 dominates and case 1 hurts the performance most, this explains why GCN performs worse than most methods in Table~\ref{tab:real-results}. In the Squirrel and Chameleon datasets, both case 1 and case 2 dominate, GCN yields acceptable results.}

\section{Hyperparameters and Parameters}
\label{app:hyperparameter}
\subsection{Hyperparameter settings}
\textbf{Experiments for Table~\ref{tab:real-results} \& Table~\ref{tab:oversmoothing}}

For the baselines, we set the same hyperparameters that are provided by the original papers or the authors’ github repositories, and we match the results they reported in their respective papers. In our experiments, we find that the original hyperparameters set by the authors are already well-tuned. 

All the models use Adam as the optimizer. GAT sets the initial learning rate as 0.005 and Geom-GCN uses a custom learning scheduler. All the other models (include \method) use the initial learning rate 0.01.

For \method, we use the following hyperparameters:
\begin{itemize}
    \item $k$ in the decaying aggregation: 3
\end{itemize}

We tune the parameters in the following ranges:
\begin{itemize}
    \item Dropout rate:  [0.0, 0.7]
    \item Weight decay:  [1e-7, 1e-2]
    \item Hidden units: \{8, 16, 32, 64, 80\}
    \item Decay rate $\eta$: [0.0, 1.5]
\end{itemize}

\textbf{Experiments for Table~\ref{tab:ablation} and Table~\ref{tab:bn_ln}}

The hyperparameters that are used in all the models (Base, \texttt{+deg}, \texttt{+sign}, \texttt{+deg,sign}, \texttt{+BN}, \texttt{+LN}) are set to be the same and they are tuned for every dataset. Those common hyperparameters are:
\begin{itemize}
    \item Dropout rate: [0.0, 0.7]
    \item Weight decay: [1e-7, 1e-2]
    \item Hidden units: \{8, 16, 32, 64, 80\}
\end{itemize}
% For models that use signed messages, we tune the following hyperparameter:
% \begin{itemize}
%     \item Initialization of $\alpha^l$: [0.2, 1.0] (same in every layer)
% \end{itemize}
% For models that use degree correction, we tune the following hyperparameter:
% \begin{itemize}
%     \item Initialization of $\lambda_0^l$: [0.2, 1.5] (same in every layer)
% \end{itemize}
\subsection{Initialization of parameters}
\textbf{Initialization}

For \method, we adopt the following parameter initialization in the experiments for Table~\ref{tab:real-results} \& Table~\ref{tab:oversmoothing}
\begin{itemize}
    \item Initialization of $\lambda_0^l$ and $\lambda_1^l$: 0.5 and 0, respectively
    \item Initialization of $\alpha^l$, $\beta_0^l$, $\beta_1^l$ and $\beta_2^l$: 2, 0, 0, 0, respectively.
\end{itemize}
We initialize %$\beta_0^l$, 
{\small $\beta_{\{0,1,2\}}^l=0$} %and $\beta_2^l$ 
in Eq.\ (6) because, after applying softmax, 
{\small $\hat{\beta}^l_{\{0,1,2\}}=1/3$}; 
%$\hat{\beta_0^l}$, $\hat{\beta_1^l}$ and $\hat{\beta_2^l}$ 
%will all be 1/3, %$\frac{1}{3}$, 
this ensures \ul{equal contributions} from positive and negative neighbors and themselves (and sum=1).
% so that the contributions from positive and negative neighbors and themselves will be equal (sum=1). 
We initialize $\lambda_1^l=0$ in Eq.\ (9) following the common practice for initializing the bias. 
We set $\alpha^l=2$ and $\lambda_0^l=0.5$ in Eq.\ (6) and Eq.\ (9), because when $r_{ij} \to +\infty$, the degree correction (including global scaling) is: {\small $\hat{\alpha^l}\tau_{ij}^l=\text{softplus}(2) \cdot \text{softplus}(0.5 \cdot (0-1) + 0) \approx 1$}. As we mention in Thm. 1, when the homophily level is high, nodes with large $\overline{r_i}$ may benefit (case 3), thus we \ul{do not want to compensate for these nodes and would like to keep {\small $\hat{\alpha^l}\tau_{ij}^l$} close to 1}. 
\subsection{Parameters after training}
\begin{wrapfigure}{r}{0.5\textwidth}
  \begin{center}
    %\vspace{-0.8cm}
    \includegraphics[scale=0.06,bb=3000 1000 380 180]{Figs/hyp1.png}
  \end{center}
  \vspace{1.8cm}
  \caption{Original $\overline{r_{ij}}$ (avg. $r_{ij}$) %$\overline{r_{ij}}$ 
  and corrected (pre- and post-training).} %before and after the training.}
  \label{fig:parameters}
\end{wrapfigure}
Figure~\ref{fig:parameters} shows the original and corrected $\overline{r_{ij}}$ (avg $r_{ij}$). Corrected $r_{ij}$ are given by {\small $\hat{\alpha^l}\tau_{ij}^lr_{ij}$}, which are a combination of global scaling and local degree correction. Because {\small $\beta_{\{0,1,2\}}^l$} sum to 1 and do not change global scaling, they are not considered in the corrected $r_{ij}$.
As can be seen in Fig.~\ref{fig:parameters}, after the training, \ul{GGCN learns to increase $r_{ij}$}, which satisfies our theorems. 

\section{Table 2 with larger fonts}
\label{app:table 2}
\begin{sidewaystable}[h]
\centering
\caption{Model performance for different layers: mean accuracy $\pm$ stdev over different data splits. Per dataset and GNN model, we also report the layer at which the best performance (given in Table~\ref{tab:real-results}) is achieved. `OOM': out of memory; `INS': numerical instability. }
\label{app-tab:table 2}
\begin{adjustbox}{width=1\linewidth}
{\footnotesize
\begin{tabular}{r c ccccccccccccccc}
\toprule
                                         %\multirow{2}{*}{\backslashbox{\textbf{Model}}{\textbf{Layers}}}    
                                      \textbf{Layers} 
                                      && \textbf{2}           & \multicolumn{1}{c}{\textbf{4}} & \multicolumn{1}{c}{\textbf{8}} & \multicolumn{1}{c}{\textbf{16}} & \multicolumn{1}{c}{\textbf{32}} & \multicolumn{1}{c}{\textbf{64}} &
                                      \multicolumn{1}{c}{\textbf{Best}}
                                      &&  \multicolumn{1}{c}{\textbf{2}}           & \multicolumn{1}{c}{\textbf{4}} & \multicolumn{1}{c}{\textbf{8}} & \multicolumn{1}{c}{\textbf{16}} & \multicolumn{1}{c}{\textbf{32}} & \multicolumn{1}{c}{\textbf{64}}  &
                                      \multicolumn{1}{c}{\textbf{Best}} \\ \cmidrule{1-1} \cmidrule{3-9} \cmidrule{11-17} %cline{2-8}
%\multirow{10}{*}{\rotatebox[origin=c]{90}{\textbf{Homophily datasets}}}   
%\textbf{Model} 
&& \multicolumn{7}{c}{\textbf{Cora} ($h$=0.81)}     & & \multicolumn{7}{c}{\textbf{Citeseer} ($h$=0.74)}                                                                         \\ %\cline{1-1} 
\cline{3-9} \cline{11-17}
                                    
                                        \multicolumn{1}{l}{GGCN (\textbf{ours})}    &&   
                                        %cora results
                                        $87.00{\scriptstyle\pm1.15}$         & {$ 87.48{\scriptstyle\pm1.32}$}           & {$ 87.63{\scriptstyle\pm1.33}$}           & {$ 87.51{\scriptstyle\pm1.19}$}            & 
                                        {$ 87.95{\scriptstyle\pm1.05}$}            & {$ 87.28{\scriptstyle\pm1.41}$}            & 
                                        32
                                           & &  
                                        % citeseer results
                                        $76.83{\scriptstyle\pm1.82}$ & $76.77{\scriptstyle\pm1.48}$ & $76.91{\scriptstyle\pm1.56}$ & $76.88{\scriptstyle\pm1.56}$& $76.97{\scriptstyle\pm1.52}$ & $76.65{\scriptstyle\pm1.38}$ & 
                                        10 \\ 
                                        
                            \multicolumn{1}{l}{GPRGNN}    &&  
                                      %cora results
                                      \multicolumn{1}{c}{$87.93{\scriptstyle\pm1.11}$}      &        $87.95{\scriptstyle\pm1.18}$           & \multicolumn{1}{c}{$87.87{\scriptstyle\pm1.41}$}           & \multicolumn{1}{c}{$87.26{\scriptstyle\pm1.51}$}            & \multicolumn{1}{c}{$87.18{\scriptstyle\pm1.29}$}            & \multicolumn{1}{c}{$87.32{\scriptstyle\pm1.21}$} & 4 &   &                   % citeseer results
                                      $77.13{\scriptstyle\pm1.67}$  & $77.05{\scriptstyle\pm1.43}$&  $77.09{\scriptstyle\pm1.62}$&  $76.00{\scriptstyle\pm1.64}$&  $74.97{\scriptstyle\pm1.47}$&  $74.41{\scriptstyle\pm1.65}$
                            & 2
                            \\
                            \multicolumn{1}{l}{H2GCN*} &&  
                                      %cora results
                                      $87.87{\scriptstyle\pm1.20}$  &   $86.10{\scriptstyle\pm1.51}$&   $86.18{\scriptstyle\pm2.10}$&    OOM                    &       OOM                     &      OOM                      &     2
                                      & &    
                                     % citeseer results
                                    $76.90{\scriptstyle\pm1.80}$  & 
                                      $76.09{\scriptstyle\pm1.54}$  & 
                                      $74.10{\scriptstyle\pm1.83}$  &  
                                      OOM     &  
                                      OOM     &  
                                      OOM     &     1
                                      
                        \\      
                                     \multicolumn{1}{l}{GCNII*}    &&  
                                      %cora results
                                      $85.35{\scriptstyle\pm1.56}$                & {$85.35{\scriptstyle\pm1.48}$}           & {$86.38{\scriptstyle\pm0.98}$}           & {$87.12{\scriptstyle\pm1.11}$}            & {$87.95{\scriptstyle\pm1.23}$}            & {$88.37{\scriptstyle\pm1.25}$}      &       
                                      64  & &
                                      % citeseer results
                                      $75.42{\scriptstyle\pm1.78}$  & $75.29{\scriptstyle\pm1.90}$&  $76.00{\scriptstyle\pm1.66}$&  $76.96{\scriptstyle\pm1.38}$&  $77.33{\scriptstyle\pm1.48}$&  $77.18{\scriptstyle\pm1.47}$ & 32
                                      \\  
                                      
                        \multicolumn{1}{l}{PairNorm}    &&   
                                        %cora results
                                        $ 85.79{\scriptstyle\pm1.01}$         & \multicolumn{1}{c}{$ 85.07{\scriptstyle\pm0.91}$}    &        \multicolumn{1}{c}{$ 84.65{\scriptstyle\pm1.09}$}     &       \multicolumn{1}{c}{$ 82.21{\scriptstyle\pm2.84}$}      &     \multicolumn{1}{c}{$ 60.32{\scriptstyle\pm8.28}$}       &    \multicolumn{1}{c}{$ 44.39{\scriptstyle\pm5.60}$}   & 2 & & 
                                        % citeseer results
                                        $73.59{\scriptstyle\pm1.47}$ & $72.62{\scriptstyle\pm1.97}$ & $72.32{\scriptstyle\pm1.58}$ & $59.71{\scriptstyle\pm15.97}$& $27.21{\scriptstyle\pm10.95}$ & $23.82{\scriptstyle\pm6.64}$ & 2                                        \\               
                        \multicolumn{1}{l}{Geom-GCN*} &&
                         % cora results
                          $85.35{\scriptstyle\pm1.57}$&   $21.01{\scriptstyle\pm2.61}$&   $13.98{\scriptstyle\pm1.48}$&   $13.98{\scriptstyle\pm1.48}$&   $13.98{\scriptstyle\pm1.48}$&   $13.98{\scriptstyle\pm1.48}$&   
                          2
                         &  & 
                        % citeseer results 
                         $78.02{\scriptstyle\pm1.15}$&  $23.01{\scriptstyle\pm1.95}$&   $7.23{\scriptstyle\pm0.87}$&   $7.23{\scriptstyle\pm0.87}$&   $7.23{\scriptstyle\pm0.87}$&   $7.23{\scriptstyle\pm0.87}$
                         &   2 
                         \\ 
                        \multicolumn{1}{l}{GCN} &&
                         % cora results
                        $86.98{\scriptstyle\pm1.27}$ & $83.24{\scriptstyle\pm1.56}$ & $31.03{\scriptstyle\pm3.08}$ &
                        $31.05{\scriptstyle\pm2.36}$ & $30.76{\scriptstyle\pm3.43}$ & $31.89{\scriptstyle\pm2.08}$ & 2
                         &  & 
                        % citeseer results 
                        $76.50{\scriptstyle\pm1.36}$ & $64.33{\scriptstyle\pm8.27}$ & $24.18{\scriptstyle\pm1.71}$ &
                               $23.07{\scriptstyle\pm2.95}$ & $25.3{\scriptstyle\pm1.77}$ & $24.73{\scriptstyle\pm1.66}$ & 2  
                         \\              
                        
                         \multicolumn{1}{l}{GAT} &&
                         % cora results
                         $87.30{\scriptstyle\pm1.10}$ & $86.50{\scriptstyle\pm1.20}$ & $84.97{\scriptstyle\pm1.24}$ &
                              INS  & INS & INS & 2
                         &  & 
                        % citeseer results 
                        $76.55{\scriptstyle\pm1.23}$ &$75.33{\scriptstyle\pm1.39}$&    $66.57{\scriptstyle\pm5.08}$         &    INS                             &    INS                             &       INS                          & 2  
                         \\
                         
                         \midrule 
&& \multicolumn{7}{c}{\textbf{Cornell ($h$=0.3)}} && \multicolumn{7}{c}{\textbf{Chameleon ($h$=0.23)}}                                                                         \\ %\cline{1-1} 
\cline{3-9} \cline{11-17}
                                    
                        \multicolumn{1}{l}{GGCN (\textbf{ours})}    &&   
                        %cornell results
                        $83.78{\scriptstyle\pm6.73}$ & $83.78{\scriptstyle\pm6.16}$ & $84.86{\scriptstyle\pm5.69}$ &
                        $83.78{\scriptstyle\pm6.73}$ & 
                        $83.78{\scriptstyle\pm6.51}$ & 
                        $84.32{\scriptstyle\pm5.90}$ & 
                               6
                        & &  
                        % Chameleon results
                        $70.77{\scriptstyle\pm1.42}$ & $69.58{\scriptstyle\pm2.68}$ & $70.33{\scriptstyle\pm1.70}$ & $70.44{\scriptstyle\pm1.82}$& $70.29{\scriptstyle\pm1.62}$ & $70.20{\scriptstyle\pm1.95}$ & 
                        5                
                        \\ 
            \multicolumn{1}{l}{GPRGNN}    && $76.76{\scriptstyle\pm8.22}$ & $77.57{\scriptstyle\pm7.46}$ & $80.27{\scriptstyle\pm8.11}$ &
                              $78.38{\scriptstyle\pm6.04}$ & $74.59{\scriptstyle\pm7.66}$ & $70.00{\scriptstyle\pm5.73}$    & 8 & &
% Chameleon results
$46.58{\scriptstyle\pm1.771}$ & $45.72{\scriptstyle\pm3.45}$ & $41.16{\scriptstyle\pm5.79}$ & $39.58{\scriptstyle\pm7.85}$& $35.42{\scriptstyle\pm8.52}$ & $36.38{\scriptstyle\pm2.40}$ & 2
            \\
            \multicolumn{1}{l}{H2GCN*} &&  
                        %cornell results
                        $81.89{\scriptstyle\pm5.98}$ & $82.70{\scriptstyle\pm6.27}$ & $80.27{\scriptstyle\pm6.63}$ &
                               OOM & OOM & OOM & 1  
                        & &    
                        % Chameleon results
                        $59.06{\scriptstyle\pm1.85}$ & $60.11{\scriptstyle\pm2.15}$ & OOM &                          OOM &                          OOM &                          OOM &                          4            
                        \\  
            
                        \multicolumn{1}{l}{GCNII*} && 
                        %cornell results
                        $67.57{\scriptstyle\pm11.34}$ & $64.59{\scriptstyle\pm9.63}$ & $73.24{\scriptstyle\pm5.91}$ &
                               $77.84{\scriptstyle\pm3.97}$ & $75.41{\scriptstyle\pm5.47}$ & $73.78{\scriptstyle\pm4.37}$ & 16   
                        & &
                        % Chameleon results
                        $61.07{\scriptstyle\pm4.10}$ & $63.86{\scriptstyle\pm3.04}$ & $62.89{\scriptstyle\pm1.18}$ & $60.20{\scriptstyle\pm2.10}$& $56.97{\scriptstyle\pm1.81}$ & $55.99{\scriptstyle\pm2.27}$ & 4  
                        \\ 
                        \multicolumn{1}{l}{PairNorm}    && $50.27{\scriptstyle\pm7.17}$ & $53.51{\scriptstyle\pm8.00}$ & $58.38{\scriptstyle\pm5.01}$ &
                              $58.38{\scriptstyle\pm3.01}$ & $58.92{\scriptstyle\pm3.15}$ & $58.92{\scriptstyle\pm3.15}$          & 32 & &
% Chameleon results
$62.74{\scriptstyle\pm2.82}$ & $59.01{\scriptstyle\pm2.80}$ & $54.12{\scriptstyle\pm2.24}$ & $46.38{\scriptstyle\pm2.23}$& $46.78{\scriptstyle\pm2.26}$ & $46.27{\scriptstyle\pm3.24}$ & 2
\\  
                        
                        \multicolumn{1}{l}{Geom-GCN*} &&
                         % cornell results
                        $60.54{\scriptstyle\pm3.67}$&  $23.78{\scriptstyle\pm11.64}$& $12.97{\scriptstyle\pm2.91}$&  $12.97{\scriptstyle\pm2.91}$&  $12.97{\scriptstyle\pm2.91}$&  $12.97{\scriptstyle\pm2.91}$&  
                        2  
                         &  & 
                        % Chameleon results 
                        $60.00{\scriptstyle\pm2.81}$&  $19.17{\scriptstyle\pm1.66}$& $19.58{\scriptstyle\pm1.73}$&  $19.58{\scriptstyle\pm1.73}$&  $19.58{\scriptstyle\pm1.73}$&  $19.58{\scriptstyle\pm1.73}$
                        &  2 
                        \\
                         \multicolumn{1}{l}{GCN} &&
                         % cornell results
                        $60.54{\scriptstyle\pm5.30}$ & $59.19{\scriptstyle\pm3.30}$ & $58.92{\scriptstyle\pm3.15}$ &
                        $58.92{\scriptstyle\pm3.15}$ & 
                        $58.92{\scriptstyle\pm3.15}$ & 
                        $58.92{\scriptstyle\pm3.15}$ & 2
                               &  & 
                        % Chameleon results 
                        $64.82{\scriptstyle\pm2.24}$ & $53.11{\scriptstyle\pm4.44}$ & $35.15{\scriptstyle\pm3.14}$ &
                               $35.39{\scriptstyle\pm3.23}$ & $35.20{\scriptstyle\pm3.25}$ & $35.50{\scriptstyle\pm3.08}$ & 2 
                         \\ 
                         \multicolumn{1}{l}{GAT} &&
                         % cornell results
                        $61.89{\scriptstyle\pm5.05}$ &      $58.38{\scriptstyle\pm4.05}$ &     $58.38{\scriptstyle\pm3.86}$                           
                        &   INS                    
                        &   INS                         
                        &   INS &  
                        2 
                         &  & 
                        % Chameleon results 
                        $60.26{\scriptstyle\pm2.50}$ &   $48.71{\scriptstyle\pm2.96}$                             &  $35.09{\scriptstyle\pm3.55}$                              &      INS                           &    INS                             &   INS                              &  2 
                         
                        \\ \bottomrule
\end{tabular}
}
\end{adjustbox}
\end{sidewaystable}


==> sections/sup_back_up.tex <==
\newpage
\counterwithin{figure}{section}
\counterwithin{table}{section}
% \section{Appendix}
% \subsection{Definitions \& Theorems}
% We consider a binary node classification task on an unweighted loop-free graph with adjacency matrix $\rmA$. 
% We denote the set of nodes in the first class and the second class as $\gV_1$ and $\gV_2$, respectively.
% The $i$-th node $v_i$ has a feature vector $\rvf_i$.
% When $v_i \in \gV_1$, $\rvf_i$ follows the Gaussian distribution $G(\rvmu, \rvSigma)$, and when $v_i \in \gV_2$, $\rvf_i$ follows $G(-\rvmu, \rvSigma)$.

% We denote the degree of node $v_i$ by $d_i$, and the degree matrix by $\rmD$ which is a diagonal matrix whose elements are degrees. 
% Denote $\gN_i$ as the set of nodes directly connected to $v_i$, i.e., its neighbors. We further denote $\gN^s_i$ the set of nodes that are in $\gN_i$ and have the same class as $v_i$. 
% We use a concept called homophily to represent the tendency of a node to have the same class as its neighbor. 
% Specifically, for the $i$-th node $v_i$, its homophily $h_i$ is defined as $h_i = \E(\frac{|\gN^s_i|}{|\gN_i|})$, where the expectation is taken over the randomness of the node labels. 
% %We further assume that the heterophily is a constant across all nodes, i.e., $h_i=h, \forall i$.

% Recall that, based on the GCN formulation in the Section ???, the $(l+1)$-th output is given by: $\rmF^{l+1} = \sigma(\tilde{\rmA}\rmF^{l}\rmW^{(L)})$, where $\tilde{\rmA} = \tilde{\rmD}^{-1/2}(\rmI+\rmA)\tilde{\rmD}^{-1/2}$, and $\tilde{\rmD}$ is the degree matrix of $\rmI+\rmA$ and $\sigma$ is ReLU. 
% Compared to MLP, the main difference in the GCN operation is the ``propagation and aggregation step'' done by multiplying the adjacency matrix $\tilde{\rmA}$ with the feature matrix $\rmF^{l}$. We will thoroughly discuss its effect in node classification and how it is related to the homophily of the nodes. 



% \begin{theorem}
% Different nodes have different susceptibility to oversmoothing. The \textbf{lower} the homophily $h_i$ is, and the \textbf{smaller} the degree $d_i$ is, the more the node $v_i$ will suffer from oversmoothing. Specifically, the expectation of feature $\rvf_i$ after the operation $\tilde{\rmA}\rmF^{0}$ is changed to $ (\frac{1}{(d_i+1)}+\frac{(2h-1)\sum_{j \in \gN_i}{\frac{1}{\sqrt{d_j+1}}}}{(d_i+1){\frac{1}{2}}})\E(\rvf^0_i)$ and is bounded by $\frac{1}{2}\E(\rvf^0_i)$ when $h\leq0.5$. The variance of each node is also reduced to $\frac{1}{(d_i+1)}(\frac{1}{(d_i+1)}+\sum_{j \in \gN_i}{\frac{1}{(d_j+1)}})\rvSigma$, which is bounded by $\frac{1}{2}\rvSigma$. For a model trained with a high-homophily graph and fewer layers, the increased mean distances between the large-degree nodes of different classes and the reduction in the variance lead to performance gain. On the other hand, when the model is trained with a low-homophily graph or more layers, the reduced mean distances between low-degree nodes lead to degenerated performances.
% \end{theorem}

\section{Detailed Proofs of Theorems in \S~\ref{section: analysis}}
\label{app:proof}
\subsection{Proof of Lemma 1}
\label{app:lemma_1}
\begin{proof}
\yy{The loss function for SGC is: \texttt{CrossEntropy}(\texttt{Softmax}($\rmF^{(L)}\rmW^{(L)}+\rvb^{(L)}$), $y_i$). Rewrite $\rmW^{(L)}$ into an array of column vectors: $\rmW^{(L)}=[\rvw_0^{(L)}, \rvw_1^{(L)}, \dots \rvw_{|\gL|}^{(L)}]$, $\rvb^{(L)}$ into an array of scalars: $\rvb^{(L)}=[b_0^{(L)}, b_1^{(L)}, \dots b_{|\gL|}^{(L)}]$, and $\rmF^{(L)}$ into an array of row vectors: $\rmF^{(L)}=[\rvf_0^{(L)}; \rvf_1^{(L)}; \dots \rvf_{|\gV|}^{(L)}]$ ($[\cdot ; \cdot]$ means stacking vertically). Let $p_{i,c} \equiv \frac{e^{\rvf_i^{(L)}\rvw_c^{(L)}+b_c^{(L)}}}{\sum_j e^{\rvf_i^{(L)}\rvw_j^{(L)}+b_j^{(L)}}}$ and let $y_{i,c} \equiv \begin{cases} 1, & \text{iff } y_i=c \\ 0, & \text{otherwise} \end{cases}$
% $\left\{\def\arraystretch{1.2}\begin{tabular}{@{}l@{\quad}l@{}}
%   $1$ & iff \chi(x_i)=c \\
%   $0$ & else
% \end{tabular}\right$, 
then we rewrite the loss function as:
\begin{equation}
    -\frac{1}{n}\sum_{i=1}^n{\sum_{c=1}^{|\gL|}y_{i,c}\cdot\text{log}(p_{i,c})},
\end{equation}
$n$ is the number of nodes used for training. To predict that the node $v_i$ belongs to class $c$, we require: $\forall c'\neq c$, $p_{i,c} > p_{i,c'}$. Thus, we have: 
\begin{equation}
    \frac{e^{\rvf_i^{(L)}\rvw_c^{(L)}+b_c^{(L)}}}{\sum_j e^{\rvf_i^{(L)}\rvw_j^{(L)}+b_j^{(L)}}}>\frac{e^{\rvf_i^{(L)}\rvw_{c'}^{(L)}+b_{c'}^{(L)}}}{\sum_j e^{\rvf_i^{(L)}\rvw_{j}^{(L)}+b_j^{(L)}}}.
\end{equation} 
It is equivalent to: 
\begin{equation}
    {\rvf_i^{(L)}\rvw_c^{(L)}+b_c^{(L)}}>\rvf_i^{(L)}\rvw_{c'}^{(L)}+b_{c'}^{(L)}.
\end{equation} 
It shows that the decision region of class $c$ is decided by a set of hyper-planes: 
\begin{equation}
    \rvx(\rvw_c^{(L)}-\rvw_{c'}^{(L)})+(b_c^{(L)}-b_{c'}^{(L)})>0.
\end{equation}}
\end{proof}
\textcolor{blue}{$\rvx$ is the vector variable that describes the plane. Any vectors that satisfy the equation are on this plane. We note that for binary classification, there is one hyper-plane.}
\subsection{Proof of Lemma 2}
\label{app:lemma_2}

\textcolor{blue}{Before giving the proof, we first explain the meaning of the Lemma. As we point out in~\S~\ref{section: analysis}, the misclassification rate of an $L$-layer SGC can be studied through its last logistic-regression layer, the input to which is $\{\rvf_i^{(L)}\}$. To study the misclassification rate of an $(L+1)$-layer SGC, we can view the input to the last layer  $\{\rvf_i^{(L+1)}\}$ as being moved from $\{\rvf_i^{(L)}\}$. The misclassification rate is closely related to the decision boundary and will be our tool for studying the change of the misclassification rate. This Lemma studies the movements that bring the node representations closer to the original decision boundary; we will prove that moving towards the original decision boundary by a non-zero step is not beneficial (i.e., harmful) to the SGC's performance.}

\begin{proof}
We prove it by contradiction and suppose that after the movements, the total misclassification rate is lowered. 
\textcolor{blue}{We denote the conditional distribution of $\{\rvf_i^{(L)}\}$ as $f_1^{L}(\rvx)$ conditioned on that they are from class 1 and $f_2^{L}(\rvx)$ conditioned on that they are from class 1 or class 2, respectively.} 
% \reminder{I cannot parse this sentence -- given whether?}
% For conciseness, we "overload" the symbol $f_1(\rvx)$ and $f_2(\rvx)$ to represent the distribution of $\{\rvf_i^{(L)}\}$ from class 1 and class 2, respectively (before the movements). 
To note that, the distributions of different layers are different. 

{After the movements, the representations from class 1 become: $\{\rvf_i^{(L)}-t{\rvw^*}^T\}, t>0$. \textcolor{blue}{$t{\rvw^*}^T$ represents moving towards the original decision boundary along the norm direction by a non-zero step.} This causes a corresponding change in the conditional PDF given that they are from class 1: $f_1^L(\rvx+t{\rvw^*}^T)$. 

\textcolor{blue}{Recall that in \S~\ref{section: analysis}, the parameters for the original optimal hyperplane ${\rvw^*}$ and ${b^*}$, and the parameters for the later optimal hyperplane ${\rvw^*}'$ and ${b^*}'$ are normalized such that when $\rvx{\rvw^*}+{b^*}>0$ and $\rvx{\rvw^*}'+{b^*}'>0$, we predict class 1.} 
% \reminder{revisit this sentence, something is off}

The new misclassification rate conditioned on class 1 is: 
\begin{equation}
   M_t'=\int_{\rvx{\rvw^*}'+{b^*}'<0}{f_1^L(\rvx+t{\rvw^*}^T)d\rvx}=\int_{(\rvx-t{\rvw^*}^T){\rvw^*}'+{b^*}'<0}{f_1^L(\rvx)d\rvx}. 
\end{equation}}
\yy{The new misclassification rate conditioned on class 2 is: 
\begin{equation}
    M_r'=\int_{\rvx{\rvw^*}'+{b^*}'>0}{f_2^L(\rvx)d\rvx}.
\end{equation}
The new total misclassification rate is:
\textcolor{blue}{
\begin{equation}
\label{lemma2:total}
\begin{split}
    M' &= M_t'\sP(v_i \in \gV_1)+M_r'\sP(v_i \in \gV_2)\\ &= M_t'\frac{\sP(v_i \in \gV_1)}{\sP(v_i \in \gV_1)+\sP(v_i \in \gV_2)}+M_r'\frac{\sP(v_i \in \gV_2)}{\sP(v_i \in \gV_1)+\sP(v_i \in \gV_2)}\\ &=\frac{\rho}{\rho+1}M_t'+\frac{1}{\rho+1}M_r'.
\end{split}
\end{equation}}} 
% Because the total misclassification is lowered, we have: $m'<m$. 
\yy{Next, we will prove that if the total misclassification is lowered, $\rvx\rvw^*+b^*=0$ is not the optimal hyper-plane before the movements which should achieve the lowest total misclassification rate.} 

\yy{Consider a hyper-plane $\rvx{\rvw^*}'+{b^*}'-\frac{t{{\rvw^*}^T}{\rvw^*}'}{2}=0$.}
\yy{Given that ${{\rvw^*}^T}{\rvw^*}'>0$ and $t>0$, for $\forall \rvx,$ s.t. $\rvx{\rvw^*}'+{b^*}'-\frac{t{{\rvw^*}^T}{\rvw^*}'}{2}<0$, we have: $(\rvx-t{\rvw^*}^T){\rvw^*}'+{b^*}'= \rvx{\rvw^*}'+{b^*}'-\frac{t{{\rvw^*}^T}{\rvw^*}'}{2}-\frac{t{{\rvw^*}^T}{\rvw^*}'}{2}<0$. It means: 
\begin{equation}
    \{\rvx|(\rvx-t{\rvw^*}^T){\rvw^*}'+{b^*}'<0\} \supseteq	\{\rvx|\rvx{\rvw^*}'+{b^*}'-\frac{t{{\rvw^*}^T}{\rvw^*}'}{2}<0\}.
\end{equation}}
\yy{Because $f_1^L(\rvx)$ is a PDF which is a nonnegative function, 
\begin{equation}
\label{lemma2:ineq_1}
    \int_{(\rvx-t{\rvw^*}^T){\rvw^*}'+{b^*}'<0}{f_1^L(\rvx)d\rvx}\geq \int_{\rvx{\rvw^*}'+{b^*}'-\frac{t{{\rvw^*}^T}{\rvw^*}'}{2}<0}{f_1^L(\rvx)d\rvx}.
\end{equation}} 
\yy{Similarly, we can obtain
\begin{equation}
    \{\rvx|\rvx{\rvw^*}'+{b^*}'>0\} \supseteq	\{\rvx|\rvx{\rvw^*}'+{b^*}'-\frac{t{{\rvw^*}^T}{\rvw^*}'}{2}>0\}.
\end{equation}
Thus, 
\begin{equation}
\label{lemma2:ineq_2}
    \int_{\rvx{\rvw^*}'+{b^*}'>0}{f_2^L(\rvx)d\rvx} \geq \int_{\rvx{\rvw^*}'+{b^*}'-\frac{t{{\rvw^*}^T}{\rvw^*}'}{2}>0}{f_2^L(\rvx)d\rvx}.
\end{equation} 
Define 
\begin{equation}
    M_{f} \equiv \frac{\rho}{\rho+1}\int_{\rvx{\rvw^*}'+{b^*}'-\frac{t{{\rvw^*}^T}{\rvw^*}'}{2}<0}{f_1^L(\rvx)d\rvx}+\frac{1}{\rho+1}\int_{\rvx{\rvw^*}'+{b^*}'-\frac{t{{\rvw^*}^T}{\rvw^*}'}{2}>0}{f_2^L(\rvx)d\rvx}.
\end{equation} 
The quantity $M_{f}$ represents the total misclassification rate before the movements if the decision boundary is $\rvx{\rvw^*}'+{b^*}'-\frac{t{{\rvw^*}^T}{\rvw^*}'}{2}=0$.
Given Eq.~\ref{lemma2:total}, \ref{lemma2:ineq_1} and \ref{lemma2:ineq_2}, we have: 
\begin{equation}
    M' \geq M_{f}. 
\end{equation} 
Let $M$ denotes the total classification rate before the movements. Based on the assumption that the total misclassification rate is lowered after the movements ($M > M'$), we have:
\begin{equation}
\label{lemma2:conclusion}
    M > M_{f}. 
\end{equation}
Eq.~\ref{lemma2:conclusion} indicates that we find a hyper-plane $\rvx{\rvw^*}'+{b^*}'-\frac{t{{\rvw^*}^T}{\rvw^*}'}{2}=0$, which yields smaller total misclassification rate than $\rvx{\rvw^*}+{b^*}=0$ before the movements. This contradicts to the fact that $\rvx{\rvw^*}+{b^*}=0$ is the optimal hyper-plane before the movements.}
\end{proof}
\subsection{Proof of Theorem~\ref{theorem: initial_stage}}
\label{app:proof1}
\begin{proof}
% Before the operation of $\tilde{\rmA}\rmF^{0}$, the distance between the mean vectors of the two classes is:
% $(1+\rho)||\rvmu||$.
%$2||\rvmu||$ and the variance within each class is $\rvSigma$. 
%and the variance of each class is $\rvSigma$ and $\rvSigma'$.
% The smaller the distance between the two classes is, the less distinguishable the node features of the two classes are.

% After this operation, the node representation of any node $v_i$ is given by:
\yy{The node representations of first layer are given by:}
% \vspace{-1cm}
\begin{equation}
\rvf_i^{(1)}=\frac{\rvf_i^{(0)}}{d_i+1} + \sum_{j \in \gN_i}{\frac{\rvf_j^{(0)}}{\sqrt{d_i+1} \cdot \sqrt{d_j+1}}}.
\label{eq:1}
% \vspace{-1cm}
\end{equation}

Without loss of generality, we assume node $v_i$ is in the first class $\gV_1$.
Then, we can express the conditional expectation of
  $\rvf_i^{(1)}$ as:
% \vspace{-1.5cm}
\begin{equation}
\E_{\rmA, \{y_i\}, \{\rvf_i^{(0)}\}|d_i, v_i \in \gV_1}(\rvf_i^{(1)}|v_i \in \gV_1, d_i) = \E_{\rmA|d_i, v_i \in \gV_1}(\E_{\{y_i\}, \{\rvf_i^{(0)}\}|\rmA,v_i \in \gV_1}(\rvf_i^{(1)}|v_i \in \gV_1, \rmA))
\label{eq:2}
%\vspace{-2cm}
\end{equation}
\textcolor{blue}{Recall that $\rmA$ is the graph adjacency matrix; the first expectation is taken over the randomness of ground truth labels and initial input features, and the second expectation is taken over the randomness of graph structure ($\rmA$) given the degree of node $v_i$ and its label.} Denote $k_i=\E_{\{y_i\}, \{\rvf_i^{(0)}\}|\rmA,v_i \in \gV_1}(\frac{|\gN^s_i|}{|\gN_i|})$ and $h_i=\E_{\rmA,\{y_i\}, \{\rvf_i^{(0)}\}|v_i \in \gV_1, d_i}(\frac{|\gN^s_i|}{|\gN_i|})$.
\begin{equation}
\begin{split}
& \E_{\{y_i\}, \{\rvf_i^{(0)}\}|\rmA,v_i \in \gV_1}(\rvf_i^{(1)}|v_i \in \gV_1, \rmA) \\=& \E_{\{y_i\}, \{\rvf_i^{(0)}\}|\rmA,v_i \in \gV_1}\left (\frac{\rvf_i^{(0)}}{d_i+1}|v_i \in \gV_1, \rmA \right ) + \sum_{j \in \gN_i}\E_{\{y_i\}, \{\rvf_i^{(0)}\}|\rmA,v_i \in \gV_1}\Bigg (\frac{\rvf_j^{(0)}}{\sqrt{d_i+1} \cdot \sqrt{d_j+1}}|v_i \in \gV_1, \rmA \Bigg) \\
%
=& \frac{\rvmu}{d_i+1} + \sum_{j \in \gN_i} \Bigg(\E_{\{y_i\}, \{\rvf_i^{(0)}\}|\rmA,v_i, v_j \in \gV_1}\left(\frac{\rvf_j^{(0)}}{\sqrt{d_i+1} \cdot \sqrt{d_j+1}}|\rmA, v_i, v_j \in \gV_1\right) \cdot \sP(v_j \in \gV_1|\rmA, v_i \in \gV_1)\\
%
+& \E_{\{y_i\}, \{\rvf_i^{(0)}\}|\rmA,v_i \in \gV_1,v_j \in \gV_2}\left(\frac{\rvf_j^{(0)}}{\sqrt{d_i+1} \cdot \sqrt{d_j+1}}|\rmA, v_i \in \gV_1, v_j \in \gV_2\right) \cdot \sP(v_j \in \gV_2|\rmA, v_i \in \gV_1)\Bigg)
\end{split}
\end{equation}
\textcolor{blue}{Let $\s1\{\cdot\}$ represent the indicator function: it equals 1 if and only if the event in the bracket holds. 
% Due to the independence of $\rmA$ and $\{y_i\}$, we can have:
\begin{equation}
\begin{split}
    \E_{\{y_i\}, \{\rvf_i^{(0)}\}|\rmA, v_i \in \gV_1}(\sum_{j \in \gN_i}\s1\{v_j \in \gV_1|\rmA, v_i \in \gV_1\}) &=\sum_{j \in \gN_i}\sP(v_j \in \gV_1|\rmA, v_i \in \gV_1)=d_ik_i.
\end{split}
\end{equation}
Due to our assumptions in~\S~\ref{section: analysis}, though the labels of nodes are dependent, they share the same marginal distribution and their joint distribution is a permutation-invariant function. Thus, given $v_i \in \gV_1 (y_i=1)$, the conditional joint distribution of $\{y_t|t \neq i\}$ is also permutation invariant---i.e., $\forall j, j' \in \gN_i, \sP(v_j \in \gV_1|v_i \in \gV_1)=\sP(v_j' \in \gV_1|v_i \in \gV_1)$. Then for $\forall j \in \gN_i$, we have:
$d_i\sP(v_j \in \gV_1|v_i \in \gV_1)=d_ik_i
$
and $\sP(v_j \in \gV_1|v_i \in \gV_1)=k_i$. Due to the independence of $\rmA$ and $\{y_i\}$, $\sP(v_j \in \gV_1|\rmA, v_i \in \gV_1)=k_i$.}
\begin{equation}
\begin{split}
%
%=& \frac{\rvmu}{d_i+1} + \sum_{j \in \gN_i}\left(\frac{k_i}{\sqrt{d_i+1} \cdot \sqrt{d_j+1}}\rvmu-\frac{(1-k_i)}{\sqrt{d_i+1} \cdot \sqrt{d_j+1}}\rvmu\right)\\
\E_{\{y_i\}, \{\rvf_i^{(0)}\}|v_i \in \gV_1, \rmA}(\rvf_i^{(1)}|v_i \in \gV_1, \rmA) =& \frac{\rvmu}{d_i+1} + \sum_{j \in \gN_i}\left(\frac{k_i}{\sqrt{d_i+1} \cdot \sqrt{d_j+1}}\rvmu-\frac{(1-k_i)}{\sqrt{d_i+1} \cdot \sqrt{d_j+1}}\rho\rvmu\right)\\
%
%=& \frac{\rvmu}{d_i+1} + \frac{(2k_i-1)\rvmu}{\sqrt{d_i+1}}\sum_{j \in \gN_i}{\frac{1}{\sqrt{d_j+1}}}.
=& \frac{\rvmu}{d_i+1} + \frac{((1+\rho)k_i-\rho)\rvmu}{\sqrt{d_i+1}}\sum_{j \in \gN_i}{\frac{1}{\sqrt{d_j+1}}}\\
=& \left(\frac{1}{d_i+1}+\frac{\sum_{j \in \gN_i}{\frac{1}{\sqrt{d_j+1}}}}{\sqrt{d_i+1}}((1+\rho)k_i-\rho)\right)\rvmu \\
=& \left(\frac{1}{d_i+1}+\frac{\sum_{j \in \gN_i}{\frac{\sqrt{d_i + 1}}{\sqrt{d_j+1}}}}{d_i+1}((1+\rho)k_i-\rho)\right)\rvmu \\
=& \left(\frac{1}{d_i+1}+\frac{d_i}{d_i+1}\frac{\sum_{j \in \gN_i}r_{ij}}{d_i}((1+\rho)k_i-\rho)\right)\rvmu.
\end{split}
\label{eq:3}
\end{equation}
%\vspace{-1cm}
Combining Equation~(\ref{eq:2}) and Equation~(\ref{eq:3}) and given the independence of $r_{ij}$ and $k_i$, we have:
\begin{equation}
%\vspace{-2cm}
\begin{split}
%\E(\rvf_i^{1}) =& \E\left(\frac{\rvmu}{d_i+1} + \frac{(2k_i-1)\rvmu}{\sqrt{d_i+1}}\sum_{j \in \gN_i}{\frac{1}{\sqrt{d_j+1}}}\right) \\
\E_{\rmA, \{y_i\}, \{\rvf_i^{(0)}\}|d_i, v_i \in \gV_1}(\rvf_i^{(1)}|v_i \in \gV_1, d_i) &= \frac{1}{d_i+1}+\frac{d_i}{d_i+1}\E_{\rmA|d_i, v_i \in \gV_1}\left(\frac{\sum_{j \in \gN_i}r_{ij}}{d_i}\right)\E_{\rmA|d_i, v_i \in \gV_1}\left((1+\rho)k_i-\rho)\right)\rvmu  \\
&=\left(\frac{1 + ((1+\rho)h_i-\rho)d_i\ratioi}{d_i+1} \right)\rvmu \equiv \gamma_i^1 \rvmu.
\end{split}
\end{equation}
%
%=& \frac{\rvmu}{d_i+1} + \frac{(2h_i-1)\rvmu}{\sqrt{d_i+1}}\sum_{j \in \gN_i}{\frac{1}{\sqrt{d_j+1}}} \\
% =& \frac{\rvmu}{d_i+1} + \frac{((1+\rho)h_i-\rho)\rvmu}{\sqrt{d_i+1}}\sum_{j \in \gN_i}{\frac{1}{\sqrt{d_j+1}}} \\
%
%=& \left(\frac{1}{d_i+1}+\frac{\sum_{j \in \gN_i}{\frac{1}{\sqrt{d_j+1}}}}{\sqrt{d_i+1}}(2h_i-1)\right)\rvmu \\
% =& \left(\frac{1}{d_i+1}+\frac{\sum_{j \in \gN_i}{\frac{1}{\sqrt{d_j+1}}}}{\sqrt{d_i+1}}((1+\rho)h_i-\rho)\right)\rvmu \\
%
%=& \left(\frac{1}{d_i+1}+\frac{\sum_{j \in \gN_i}{\frac{\sqrt{d_i + 1}}{\sqrt{d_j+1}}}}{d_i+1}(2h_i-1)\right)\rvmu \\
% =& \left(\frac{1}{d_i+1}+\frac{\sum_{j \in \gN_i}{\frac{\sqrt{d_i + 1}}{\sqrt{d_j+1}}}}{d_i+1}((1+\rho)h_i-\rho)\right)\rvmu \\
%
%=& \left(\frac{1 + (2h_i - 1)d_i\ratioi}{d_i+1} \right)\rvmu \equiv \gamma_i^1 \rvmu.
% =& \left(\frac{1 + ((1+\rho)h_i-\rho)d_i\ratioi}{d_i+1} \right)\rvmu \equiv \gamma_i^1 \rvmu.
Define $\epsilon \equiv (1+\rho)h_i-\rho$, and we consider three cases: \textbf{(1)} $h_i\leq\frac{\rho}{1+\rho}$, \textbf{(2)} $h_i > \frac{\rho}{1+\rho} \ \mathbf{\&} \  \ratioi \leq \frac{1}{\epsilon}$, and \textbf{(3)} $h_i > \frac{\rho}{1+\rho} \ \mathbf{\&} \  \ratioi > \frac{1}{\epsilon}$.
% \begin{itemize*}
%     \item $h_i\leq0.5$
%     \item $h_i > 0.5 \ \mathbf{\&} \  \ratioi \leq \frac{1}{\epsilon}$ and 
%     \item $h_i > 0.5 \ \mathbf{\&} \  \ratioi > \frac{1}{\epsilon}$. 
% \end{itemize*}

% \newpage

\begin{itemize}
    \item 
\colorbox{gray!30}{\textbf{CASE 1: $\pmb{h_i\leq\frac{\rho}{1+\rho}}$}}

$\bullet$ \textbf{Upper Bound}

We have:
\begin{equation}
%\vspace{-1cm}
\gamma_i^1 \leq \frac{1}{d_i+1} \leq \frac{1}{2}.
\label{eq:5}
\end{equation}
$\bullet$  \textbf{Lower Bound}

To see if there exists a lower bound, we first show that when $h_i \leq \frac{\rho}{1+\rho}$, $\frac{1 + ((1+\rho)h_i-\rho)d_i\ratioi}{d_i+1} $ is a decreasing function of $d_i$ given that $d_i \geq 1$.

When $h_i \leq \frac{\rho}{1+\rho}$, we have:
\begin{enumerate}
    \item $((1+\rho)h_i-\rho) \leq 0$
    \item $\frac{d_i}{d_i+1}$ is an increasing non-negative function of $d_i$
    \item $\ratioi$ is an increasing non-negative function of $d_i$
    \item $\frac{1}{d_i+1}$ is a decreasing function of $d_i$ 
\end{enumerate}
Thus $\frac{1 + ((1+\rho)h_i-\rho)d_i\ratioi}{d_i+1}$ is a decreasing function of $d_i$.

When $h_i=\frac{\rho}{1+\rho}$, $\frac{1 + ((1+\rho)h_i-\rho)d_i\ratioi}{d_i+1} = \frac{1}{d_i+1}$ and $0 < \frac{1}{d_i+1} \leq \frac{1}{2}$.

When $h_i<\frac{\rho}{1+\rho}$,
\begin{equation}
\begin{split}
    \frac{1 + ((1+\rho)h_i-\rho)d_i\ratioi}{d_i+1} &\leq \frac{((1+\rho)h_i-\rho)d_i\ratioi}{d_i+1}+\frac{1}{2} \\&\leq \frac{((1+\rho)h_i-\rho)\ratioi}{2}+\frac{1}{2}.
\end{split}
\end{equation}
And we know that when $h_i<\frac{\rho}{1+\rho}$:
\begin{equation}
\lim_{\ratioi \to \infty}{\frac{((1+\rho)h_i-\rho)\ratioi}{2}+\frac{1}{2}}=-\infty.
\end{equation}
Thus,
\begin{equation}
\begin{split}
\lim_{\ratioi \to \infty}{\frac{1 + ((1+\rho)h_i-\rho)d_i\ratioi}{d_i+1}}=-\infty.
\end{split}
\label{eq:lower_bound}
\end{equation}
% If $h_i > 0.5$,
% denote $M_i$ by $\frac{1}{M_i} \equiv \frac{1}{d_i}\sum_{j \in \gN_i}{\frac{1}{\sqrt{d_j+1}}}$

% \vspace{0.2cm}
% \textbf{[OTHER CASES: $\pmb{h_i > 0.5}$]}

% Let $\epsilon=2h_i - 1$ and $0 < \epsilon \leq 1$. We have:
% \begin{equation}
% %\vspace{-1cm}
% \begin{split}
%     % \E(\rvf_i^{1}) = (\frac{1}{(d_i+1)}+(2h_i-1)\cdot \frac{d_i}{M_i \cdot \sqrt{d_i+1}})\rvmu
%     \E(\rvf_i^{1}) = \left (\frac{1 + \epsilon d_i \ratioi}{d_i+1}\right )\rvmu.
% \end{split}
% \label{eq:6}
% \end{equation}

\vspace{0.2cm}
\item \colorbox{gray!30}{\textbf{CASE 2: $\pmb{h_i > \frac{\rho}{1+\rho} \;\;\; \mathbf{\&} \;\;\;  \ratioi \leq \frac{1}{\epsilon}}$}}

If $h_i >\frac{\rho}{1+\rho}$, $0 < \epsilon \leq 1$; if $\ratioi \leq \frac{1}{\epsilon}$, $0 < \epsilon \ratioi \leq 1$. Given %$\E(\rvf_i^{1}) = \left (\frac{1 + \epsilon d_i \ratioi}{d_i+1}\right )\rvmu$
\begin{equation}
%\vspace{-1cm}
\begin{split}
    % \E(\rvf_i^{1}) = (\frac{1}{(d_i+1)}+(2h_i-1)\cdot \frac{d_i}{M_i \cdot \sqrt{d_i+1}})\rvmu
    \E(\rvf_i^{1}) = \left (\frac{1 + \epsilon d_i \ratioi}{d_i+1}\right )\rvmu.
\end{split}
\label{eq:6}
\end{equation}
we have \yy{$0<\frac{1}{d_i+1} < \gamma_i^1 \leq 1$}.
%if $\ratioi \leq \frac{1}{\epsilon}$, then $0 < \epsilon \ratioi \leq 1$, so $\frac{1}{2} < \gamma_i^1 \leq 1$. 

\vspace{0.2cm}
\item \colorbox{gray!30}{\textbf{CASE 3: $\pmb{h_i > \frac{\rho}{1+\rho} \;\;\; \mathbf{\&} \;\;\;  \ratioi > \frac{1}{\epsilon}}$}}

In this case, Equation~(\ref{eq:6}) still holds, since $h_i>\frac{\rho}{1+\rho}$.

$\bullet$  \textbf{Lower Bound}

If $\ratioi > \frac{1}{\epsilon}$, then $\epsilon \ratioi > 1$ and therefore $\gamma_i^1 > 1$.

$\bullet$  \textbf{Upper Bound}

When $\epsilon>0$,
\begin{equation}
\begin{split}
    \frac{1 + \epsilon d_i\ratioi}{d_i+1} &> \frac{\epsilon d_i\ratioi}{d_i+1}\\&\geq \frac{\epsilon\ratioi}{2}.
\end{split}
\end{equation}
Because
\begin{equation}
    \lim_{\ratioi \to \infty}{\frac{\epsilon\ratioi}{2}}=\infty,
\end{equation}
we have:
\begin{equation}
    \lim_{\ratioi \to \infty}{\frac{1 + \epsilon d_i \ratioi}{d_i+1}}=\infty.
\end{equation}

To sum it up, 
\begin{equation}
\gamma_i^1 \in 
\begin{cases}
  (-\infty, \frac{1}{2}], & \text{if}\ h_i\leq\frac{\rho}{1+\rho} \\
  (0, 1], & \text{if}\ h_i>\frac{\rho}{1+\rho} \ \mathrm{\&}\  \ratioi \leq \frac{1}{(1+\rho)h_i-\rho}\\
  (1, \infty), & \mathrm{otherwise}.
\end{cases}
\end{equation}

\end{itemize}


\vspace{0.5cm}
\textbf{Remarks: Special cases}

For different types of graphs and different nodes in the graph, $d_i\ratioi$ might be different. For a \textbf{d-regular graph} whose nodes have constant degree or a graph whose adjacency matrix is \textbf{row-normalized}, we will have:
\begin{equation}
\begin{split}
    \gamma_i^1 =& \left (\frac{1 + ((1+\rho)h_i-\rho)d_i\ratioi}{d_i+1}\right ) \\\leq & (\frac{1}{(d_i+1)}+\frac{d_i}{(d_i+1)}) = 1
\end{split}
\label{eq:7}
\end{equation}
Equality is achieved if and only if $h_i=1$. To note that, $h_i=1$ is not achievable for every node as long as there are more than one class. \textbf{Boundary nodes} will suffer most.  

% %In a more general case, if $\frac{1}{M_i} \ll \frac{1}{(d_i+1)^{\frac{1}{2}}}$, then the 
% In a more general case, when $d_i \geq (\frac{M_i}{2h_i-1})^2-1$, $\E(\rvf_i^{1}) \geq \rvmu$ and when $d_i < (\frac{M_i}{2h_i-1})^2-1$, $\E(\rvf_i^{1}) < \rvmu$. It suggests that a node with significantly smaller degree than its neighbors is easier to suffer from oversmoothing.




% From the above derivations, we can have the following conclusions:
% \begin{enumerate}
%     \item After "propagation and aggregation", the expectation of $\rvf_i^{1}$ changes to  $(\frac{1}{(d_i+1)}+\frac{(2h-1)\sum_{j \in \gN_i}{\frac{1}{\sqrt{d_j+1}}}}{(d_i+1)^{\frac{1}{2}}})\rvmu$. It indicates that the lower homophily of the graph, the less distinguishable of the features after $\tilde{\rmA}\rmF^{0}$. When $h_i \leq 0.5$, the node feature moves towards the origin by at least half of the original distances.
%     \item The smaller the degree of the node, the more it will suffer from oversmoothing.
%     \item The derivation can be extended to the case where the neighborhood nodes are weighted differently. In that case, the larger positive weight on the nodes that have a different class, the less distinguishable of features. 
% \end{enumerate}
% Then, we will take a look at the variance within class 1. If we assume that the feature vectors are independent of each other, then we will have:
% \begin{equation}
% \begin{split}
% \sV(\rvf_t^{1}|k_i) =& \sV\left(\frac{\rvf_i^{0}}{d_i+1}|k_i\right) + \sum_{j \in \gN_i}{\sV\left(\frac{\rvf_j^{0}}{\sqrt{d_i+1} \cdot \sqrt{d_j+1}}|k_i\right)} \\
% %
% %=& \left(\frac{1}{(d_i+1)^2} + \sum_{j \in \gN_i}{\frac{1}{(d_i+1)(d_j+1)}}\right)\rvSigma \\
% =& \frac{\rvSigma}{(d_i+1)^2} + \sum_{j \in \gN_i}{\frac{1}{(d_i+1)(d_j+1)}}\sV(\rvf_j^{0}|k_i)\\
% %
% =& \frac{\rvSigma}{(d_i+1)^2} + \sum_{j \in \gN_i}{\frac{1}{(d_i+1)(d_j+1)}}(\E(\sV(\rvf_j^{0}|k_i,\mathbbm{1}\{v_j \in \gV_1\}))+\sV(\E(\rvf_j^{0}|k_i, \mathbbm{1}\{v_j \in \gV_1\})))\\
% =& \frac{\rvSigma}{(d_i+1)^2} + \sum_{j \in \gN_i}{\frac{1}{(d_i+1)(d_j+1)}}(k_i\rvSigma+(1-k_i)\rvSigma'+k_i(1-k_i)(1+\rho)^2\rvmu^T\rvmu)
% %= & \frac{1}{d_i+1}\left(\frac{1}{d_i+1}+\sum_{j \in \gN_i}{\frac{1}{d_j+1}}\right)\rvSigma
% %
% \end{split}
% \label{eq:8}
% \end{equation}

% \begin{equation}
%     \frac{1}{d_i+1}\left(\frac{1}{d_i+1}+\sum_{j \in \gN_i}{\frac{1}{d_j+1}}\right)
% \leq \frac{1}{2}
% \end{equation}

% Note that we can derive similar results for any node $v_t$ in the second class.

% From Equation~\ref{eq:8}, we can have the following conclusion:
% \item $\tilde{\rmA}\rmF^{0}$ will reduce the variance of the node feature distribution and the reduction is irrelevant to the homophily $h_i$. The larger degree of the node, the greater the reduction will be in the variance. Note that the reduction of the variance of each node does not mean the reduction of the variance of the class as a whole. When the degree and the homophily of the nodes are diverse, the variance of the class can increase.
%This explains the gain of GCN when using fewer layers and the performance gain is a result of variance reduction.
\end{proof}


% Next, we will consider an extended scenario: we let the "messages" sent by the neighbors from the other class to be multiplied by a negative sign and the neighbors from the same class to send the "messages" as they are. For the node $v_i$, we define $m_i$ as the ratio of neighbors that do not send the "messages" correctly, i.e., neighbors from the other class send messages without being multiplied by a negative sign and neighbors from the same class send the messages multiplied by a negative sign. And we define the error rate as $e_i=\E(m_i)$, the expectation is taken over the randomness of the neighbors that wrongly send the messages. %We assume the expectation is the same for all the nodes.

% We have the following assumptions:
% \begin{enumerate}
%     \item Conditioned on $m_i$, whether the neighbor will wrongly send the information is independent of the class it belongs to.
%     \item The variable $m_i$ is independent of the class that any node $v_j$ belongs to.
% \end{enumerate}

% \begin{theorem}
% With the independence assumptions and by allowing the messages to be optionally multiplied by a negative sign, the mean distance between the nodes in different classes will \textbf{not be affected} by the homophily level $h_i$, but will be reduced for \textbf{bigger error rate} $e_i$. 
% \end{theorem}
\subsection{Proof of Theorem~\ref{theorem: developing stage}}
\label{app:proof2}
\begin{proof}
% The derivation is similar to that of Theorem~\ref{theorem: initial_stage} except that we replace the ground truth heterophily $h_i$ with the effective heterophily $\heterophilyil$, $\ratioi$ with $\ratioi'$, and $\E(\rvf_i^{l})$ with $\gamma^l_i\E(\rvf_i^{0})\rmW^{e}$. 
% \yy{We derive the equation for nodes which are from class 1 and its expected representation does not cross the origin (the other cases can be derived similarly):}

% \yy{Rewrite the $\E(\rvf_i^{(l)})$ in \S~\ref{sec:developing-stage}:
% $$\E(\rvf_i^{(l)}) = \begin{cases}\xi^l_i\E(\rvf_i^{(0)}) & \text{if node }v_i\text{'s expected representation does not cross the origin.} \\
% -\rho\xi^l_i\E(\rvf_i^{(0)}) & \text{if node }v_i\text{ is from class 1 and its expected representation moves across the origin.} \\
% -\frac{1}{\rho}\xi^l_i\E(\rvf_i^{(0)}) & \text{if node }v_i\text{ is from class 2 and its expected representation moves across the origin.}
% \end{cases}$$
% }

% Let $\hat{\mathcal{N}_i^s} \equiv \{v_j|\E(\rvf_i^{(0)})\cdot\E({\rvf_j^{(l)}}^T)>0, v_j \in \gN_i\}$. Recall that $\mathcal{N}_i^s$ is the set of neighbors that have the same label as node $v_i$, so we have: $\hat{\mathcal{N}_i^s} = \{v_j|v_j \in \mathcal{N}_i^s \;\&\;\E(\rvf_j^{(l)})\text{ does not cross the origin}\} \cup \{v_j|v_j \not\in \mathcal{N}_i^s, v_j \in \mathcal{N}_i \; \& \; \E(\rvf_j^{(l)})\text{ crosses the origin}\}$. Define $k_i=\frac{|\hat{\mathcal{N}_i^s}|}{|\mathcal{N}_i|}$ and $\mathbb{E}(k_i)=\heterophilyil$. The expectation is taken over possible distributions of ground truth labels in $v_i$'s neighborhood. From the definition of $\xi_i^l$, we have: if $v_j \in \hat{\mathcal{N}_i^s}$, $\mathbb{E}(\mathbf{f}_j^{(l)})=\xi_j^l\rvmu$; if $v_j \not\in \hat{\mathcal{N}_i^s}, v_j \in \mathcal{N}_i$, $\mathbb{E}(\mathbf{f}_j^{(l)})=-\rho\xi_j^l\rvmu$
\textcolor{blue}{ 
After propagating over multiple layers, we use $\xi_{i}^l$ to account for the accumulated scaling effects ($\gamma_i^{l}$). That is, $\mathbb{E}_{\rmA,\{y_i\},\{\rvf_i^{(0)}\}|d_i}\left (\frac{\mathbf{f}_i^{(l)}}{d_i+1}|d_i \right)=\xi_{i}^l\rvmu$.
Furthermore, conditioned on $\rmA$ and $\xi_{i}^l$, the set of nodes contributing positively to node $v_i$ is defined as:\\ $\hat{\mathcal{N}_i^s}(\rmA, \xi_{i}^l) \equiv 
% \{v_j|\E_{\{y_i\},\{\rvf_i^{(0)}\}|\mathbf{f}_i^{(l)}, \rmA, v_j \in \gN_i}\left(\rvf_i^{(l)}|\mathbf{f}_i^{(l)}, \rmA, v_j \in \gN_i\right)
\{v_j|v_j \in \gN_i \text{ and } (\xi_{i}^l\rvmu) \cdot \E_{\{y_i\},\{\rvf_i^{(0)}\}|\xi_{i}^l, \rmA}\left({\rvf_j^{(l)}}^T|\xi_{i}^l, \rmA\right)>0\}$.\\
$\mathbb{E}_{\rmA,\{y_i\},\{\rvf_i^{(0)}\}|d_i,\xi_{i}^l, v_j \in \gN_i}\Bigg(\mathbf{f}_j^{(l)}r_{ij}|d_i, \xi_{i}^l, v_j \in \gN_i\Bigg)=\begin{cases}
{\xi_{i}^{l}}'\rvmu & v_j \in   \hat{\mathcal{N}_i^s}(\rmA, \xi_{i}^l) \\
-\rho_{i}^{l}{\xi_{i}^{l}}'\rvmu & v_j \not\in   \hat{\mathcal{N}_i^s}(\rmA, \xi_{i}^l)
\end{cases}$}

In the following proof, we use $\hat{\mathcal{N}_i^s}$ to refer to $\hat{\mathcal{N}_i^s}(\rmA, \xi_{i}^l)$ for conciseness.

The representations at $(l+1)$-th layer:
\begin{equation}
    \mathbf{f}_i^{(l+1)}=\frac{\mathbf{f}_i^{(l)}}{d_i+1} + \sum_{j \in \mathcal{N}_i}{\frac{\mathbf{f}_i^{(l)}}{\sqrt{d_i+1} \cdot \sqrt{d_j+1}}}
\end{equation}
% \begin{equation}
%     \mathbb{E}(\mathbf{f}_i^{(l+1)}|\mathbf{f}_i^{(l)}) = \mathbb{E}_{d_i|\mathbf{f}_i^{(l)}}\Bigg(\mathbb{E}_{\rmA,\{y_i\},\{\rvf_i^{(0)}\}|d_i,\mathbf{f}_i^{(l)}}\Bigg(\mathbf{f}_i^{(l+1)}|d_i,\mathbf{f}_i^{(l)}\Bigg)\Bigg)
% \end{equation}
\begin{eqnarray}
& & \mathbb{E}_{\rmA,\{y_i\},\{\rvf_i^{(0)}\}|d_i,\xi_{i}^l}\Bigg(\mathbf{f}_i^{(l+1)}|d_i,\xi_{i}^l\Bigg) \\&=& \mathbb{E}_{\rmA,\{y_i\},\{\rvf_i^{(0)}\}|d_i,\xi_{i}^l}\left (\frac{\mathbf{f}_i^{(l)}}{d_i+1}|d_i,\xi_{i}^l \right ) + \mathbb{E}_{\rmA,\{y_i\},\{\rvf_i^{(0)}\}|d_i,\xi_{i}^l}\left(\sum_{j \in \mathcal{N}_i}\frac{\mathbf{f}_j^{(l)}}{\sqrt{d_i+1} \cdot \sqrt{d_j+1}}|d_i,\xi_{i}^l \right) \\ &=& \frac{\xi_i^l\rvmu}{d_i+1} + \frac{1}{d_i+1}\mathbb{E}_{\rmA,\{y_i\},\{\rvf_i^{(0)}\}|d_i,\xi_{i}^l}\Bigg(\sum_{j \in \mathcal{N}_i}\frac{\mathbf{f}_j^{(l)}\sqrt{d_i+1}}{\sqrt{d_j+1}}|d_i, \xi_{i}^l\Bigg) 
\label{eq:44}
\end{eqnarray}
\textcolor{blue}{In ~\S~\ref{section: analysis}, we assume that $\{d_j\}$ follow the same distribution and their joint distribution function is permutation-invariant, and $\{y_j\}$ and $\{\rvf_j^{l}\}$ also have this property. Thus, conditioned on $d_i$, $\xi_{i}^l$ and $\gN_i$,
the distribution of $\frac{\mathbf{f}_j^{(l)}\sqrt{d_i+1}}{\sqrt{d_j+1}}$  is the same for $\forall j \in \mathcal{N}_i$ (neighbors are indistinguishable) and we obtain:
\begin{eqnarray}
& &\mathbb{E}_{\rmA,\{y_i\},\{\rvf_i^{(0)}\}|d_i,\xi_{i}^l, \gN_i}\Bigg(\sum_{j \in \mathcal{N}_i}\frac{\mathbf{f}_j^{(l)}\sqrt{d_i+1}}{\sqrt{d_j+1}}|d_i, \xi_{i}^l, \gN_i\Bigg) \\&=& d_i\mathbb{E}_{\rmA,\{y_i\},\{\rvf_i^{(0)}\}|d_i,\xi_{i}^l, \gN_i, v_j \in \gN_i}\Bigg(\frac{\mathbf{f}_j^{(l)}\sqrt{d_i+1}}{\sqrt{d_j+1}}|d_i, \xi_{i}^l, \gN_i, v_j \in \gN_i\Bigg)\end{eqnarray}
Given that the joint distribution of $\{d_j\}$, the joint distribution of $\{y_j\}$ and the joint distribution of $\{\rvf_j^{l}\}$ are permutation-invariant functions, for any $\gN_i$, $\mathbb{E}_{\rmA,\{y_i\},\{\rvf_i^{(0)}\}|d_i,\xi_{i}^l, \gN_i}\Bigg(\sum_{j \in \mathcal{N}_i}\frac{\mathbf{f}_j^{(l)}\sqrt{d_i+1}}{\sqrt{d_j+1}}|d_i, \xi_{i}^l, \gN_i\Bigg)$ is the same. That is:
\begin{eqnarray}
& &\mathbb{E}_{\rmA,\{y_i\},\{\rvf_i^{(0)}\}|d_i,\xi_{i}^l}\Bigg(\sum_{j \in \mathcal{N}_i}\frac{\mathbf{f}_j^{(l)}\sqrt{d_i+1}}{\sqrt{d_j+1}}|d_i, \xi_{i}^l\Bigg) 
\\ &=&\mathbb{E}_{\rmA,\{y_i\},\{\rvf_i^{(0)}\}|d_i,\xi_{i}^l, \gN_i}\Bigg(\sum_{j \in \mathcal{N}_i}\frac{\mathbf{f}_j^{(l)}\sqrt{d_i+1}}{\sqrt{d_j+1}}|d_i, \xi_{i}^l, \gN_i\Bigg) \\&=&
d_i\mathbb{E}_{\rmA,\{y_i\},\{\rvf_i^{(0)}\}|d_i,\xi_{i}^l, v_j \in \gN_i}\Bigg(\frac{\mathbf{f}_j^{(l)}\sqrt{d_i+1}}{\sqrt{d_j+1}}|d_i, \xi_{i}^l, v_j \in \gN_i\Bigg)
\label{eq:49}
\end{eqnarray}}

\textcolor{blue}{We note that $v_j$ in Equation~\ref{eq:49} can be any node except $v_i$ due to the equivalence of those nodes.}

Combining Equation~\ref{eq:44} and Equation~\ref{eq:49}, we can obtain:
\begin{eqnarray}
& &\mathbb{E}_{\rmA,\{y_i\},\{\rvf_i^{(0)}\}|d_i,\xi_{i}^l}\Bigg(\mathbf{f}_i^{(l+1)}|d_i,\xi_{i}^l\Bigg) \\&=& 
\frac{\xi_i^l\rvmu}{d_i+1} +
\frac{d_i}{d_i+1}\mathbb{E}_{\rmA,\{y_i\},\{\rvf_i^{(0)}\}|d_i,\xi_{i}^l, v_j \in \gN_i}\Bigg(\frac{\mathbf{f}_j^{(l)}\sqrt{d_i+1}}{\sqrt{d_j+1}}|d_i, \xi_{i}^l, v_j \in \gN_i \Bigg)\\&=& \frac{\xi_i^l\rvmu}{d_i+1} + \frac{d_i}{d_i+1}\Bigg(\mathbb{E}_{\rmA,\{y_i\},\{\rvf_i^{(0)}\}|d_i,\xi_{i}^l,v_j \in \hat{\mathcal{N}_i^s}, v_j \in \gN_i}\Bigg(\frac{\mathbf{f}_j^{(l)}\sqrt{d_i+1}}{\sqrt{d_j+1}}|d_i, \xi_{i}^l, v_j \in \hat{\mathcal{N}_i^s}, v_j \in \gN_i\Bigg) \\
&\cdot& \sP\Bigg(v_j \in \hat{\mathcal{N}_i^s}|v_j \in \gN_i, d_i, \xi_{i}^l\Bigg)
+ \mathbb{E}_{\rmA,\{y_i\},\{\rvf_i^{(0)}\}|d_i,\xi_{i}^l,v_j \not\in \hat{\mathcal{N}_i^s}, v_i \in \gN_i}\Bigg(\frac{\mathbf{f}_j^{(l)}\sqrt{d_i+1}}{\sqrt{d_j+1}}|d_i, \xi_{i}^l, v_j \not\in \hat{\mathcal{N}_i^s}, v_j \in \gN_i\Bigg)
\\ &\cdot& \sP\Bigg(v_j \not\in \hat{\mathcal{N}_i^s}, |d_i, \xi_{i}^l, v_j \in \gN_i\Bigg)\Bigg)\\ &=& \frac{\xi_i^l\rvmu}{d_i+1} + \Bigg(\frac{d_i\sP(v_j \in \hat{\mathcal{N}_i^s}|d_i, \xi_{i}^l, v_j \in \gN_i)}{{d_i+1} }{\xi_{i}^{l}}'\rvmu- \frac{d_i(1-\sP(v_j \in \hat{\mathcal{N}_i^s}|d_i, \xi_{i}^l, v_j \in \gN_i))}{ {d_i+1}}\rho_{i}^{l}{\xi_{i}^{l}}'\rvmu\Bigg)\\ &=& \frac{\xi_{i}^l\rvmu}{d_i+1} + \frac{d_i(\sP(v_j \in \hat{\mathcal{N}_i^s}|d_i, \xi_{i}^l, v_j \in \gN_i)(1+\rho_{i}^l)-\rho_{i}^l){\xi_{i}^{l}}'\rvmu}{d_i+1}
\label{eq:58}
\end{eqnarray}

\textcolor{blue}{Define $\bar{r_i}^{l}\equiv \frac{{\xi_{i}^{l}}'}{{\xi_{i}^{l}}}$. If we know the degree $d_i$, $\xi_{i}^l$, and that a neighbor $v_j$ is in the group $\hat{\mathcal{N}_i^s}$, $\bar{r_i}^{l}$ actually represents the ratio of expected $\rvf_j^{l}r_{i,j}$ to expected $\rvf_i^{l}$. We regard it as the effective related degree at $l$-th
layer. For the initial layer, if we know the degree $d_i$, $y_i$, and that a neighbor $v_j$ is in the group $\mathcal{N}_i^s$, the ratio of  $\rvf_j^{0}r_{i,j}$ to $\rvf_i^{0}$ is $r_{ij}$.
 Recall that the related degree $\ratioi$ at the initial layer is the expected average of $r_{ij}$ in the neighborhood. Thus $\bar{r_i}^{l}$ is an extension of $\ratioi$.
Moreover, let $\hat{h_i^{l}}=\sP(v_j \in \hat{\mathcal{N}_i^s}|v_j \in \gN_i, d_i, \xi_{i}^l)$ represent the probability of a neighbor whose representation has a positive contribution in expectation. This naturally extends the meaning of homophily in deeper layers. Thus, we regard it as the effective homophily of node $v_i$ at $l$-th layer. Given the degree $d_i$, $\xi_{i}^l$, $\rho_{i}^l$ represents the ratio of the probability that a neighbor will have a positive  rather than a negative contribution to $v_i$. This naturally extends the meaning of $\rho$.}

We further write Equation~\ref{eq:58} as:
$$\frac{\xi_{i}^l}{d_i+1}\Bigg(1+\Bigg((\hat{h_i^{l}}(1+\rho_{i}^l)-\rho_{i}^l)d_i\bar{r_i}^{l})\Bigg)\rvmu$$ and it will have three cases similar to Thm.~\ref{theorem: initial_stage}.


% In Thm~\ref{theorem: developing stage}, we define $r_{ij}'\equiv r_{ij}\frac{\xi_j^l}{\xi_i^l}$ and $\overline{r_{i}'} \equiv \frac{1}{d_i}\sum_{j \in \mathcal{N}_i}{r_{ij}'}$, thus
% \begin{equation}
%     \mathbb{E}(\mathbf{f}_i^{(l+1)}|k_i) = \frac{\xi_i^l\rvmu}{d_i+1} + \sum_{j \in \mathcal{N}_i}(r_{ij}'((1+\rho)k_i-\rho)\xi_i^l\rvmu)=\left(\frac{1 + ((1+\rho)k_i-\rho)d_i\overline{r_{i}'}}{d_i+1} \right)\xi_i^l\rvmu
% \end{equation}
% \begin{equation}
%     \mathbb{E}(\mathbf{f}_i^{(l+1)})=\mathbb{E}(\mathbb{E}(\mathbf{f}_i^{(l+1)}|d_i,\mathbf{f}_i^{(l)}))=\left(\frac{1 + ((1+\rho)\heterophilyil-\rho)d_i\overline{r_{i}'}}{d_i+1} \right)\xi_i^l\mathbb{E}(\mathbf{f}_i^{(0)})
% \end{equation}
% }

% Next, we prove that $\left (\frac{((1+\rho)\heterophilyil-\rho) d_i \ratioi' + 1}{d_i+1}\right )$ is a decreasing function of $d_i$. Since graph $\gG$ is connected, the node degrees $d_i \geq 1$; thus, $\frac{d_i}{d_i+1}$ and $\ratioi'$ are increasing functions of $d_i$, while $\frac{1}{d_i+1}$ is a decreasing function of $d_i$. When $\heterophilyil \leq \frac{\rho}{1+\rho}$, we have $((1+\rho)\heterophilyil-\rho) \leq 0$, so $((1+\rho)\heterophilyil-\rho) \cdot \frac{d_i}{d_i+1} \cdot \ratioi + \frac{1}{d_i+1}$ is a decreasing function of $d_i$). This suggests that the higher-degree nodes move towards the opposing class more and "under non-swapping condition", the accuracy of higher-degree nodes drops more sharply.
\end{proof}
\subsection{Proof of Theorem~\ref{theorem: signed_messages}}
\label{app:proof3}
\begin{proof}
Similar to Equation~\ref{eq:2}, we can express the conditional expectation of $\rvf_i^{(1)}$ as:
\begin{equation}
\begin{split}
% \E_{\rmA, \{y_i\}, \{\rvf_i^{(0)}\}|d_i, v_i \in \gV_1}(\rvf_i^{(1)}|v_i \in \gV_1, d_i) = \E_{\rmA|d_i, v_i \in \gV_1}(\E_{\{y_i\}, \{\rvf_i^{(0)}\}|\rmA,v_i \in \gV_1}(\rvf_i^{(1)}|v_i \in \gV_1, \rmA))\\
& \E_{\rmA, \{y_i\}, \{\rvf_i^{(0)}\}|d_i, v_i \in \gV_1}\left(\rvf_i^{(1)}|v_i \in \gV_1, d_i\right) \\=& \E_{m_i^0|v_i \in \gV_1, d_i}\left(\E_{\rmA, \{y_i\}, \{\rvf_i^{(0)}\}|d_i, v_i \in \gV_1, m_i^0}\left(\rvf_i^{(1)}|v_i \in \gV_1, d_i, m_i^0\right)\right)  \\
%
=& \E_{m_i^0|v_i \in \gV_1, d_i}\left(\E_{\rmA, \{y_i\}, \{\rvf_i^{(0)}\}|v_i \in \gV_1, d_i, m_i^0}\Bigg(\frac{\rvf_i^{(0)}}{d_i+1}|v_i \in \gV_1, d_i, m_i^0\right) \\+& \E_{\rmA, \{y_i\}, \{\rvf_i^{(0)}\}|v_i \in \gV_1, d_i, m_i^0}\left(\sum_{j \in \gN_i}\frac{\rvf_j^{(0)}}{\sqrt{d_i+1} \cdot \sqrt{d_j+1}}|v_i \in \gV_1, d_i, m_i^0\right)\Bigg) \\
%
=& \frac{\rvmu}{d_i+1}\\+& \E_{m_i^0|v_i \in \gV_1, d_i}\Bigg(\E_{\rmA|d_i, v_i \in \gV_1, m_i^0}\Bigg(\sum_{j \in \gN_i}\Bigg(\E_{\{y_i\}, \{\rvf_i^{(0)}\}|\rmA,v_i,v_j \in \gV_1, m_i^0}\left(\frac{\rvf_j^{(0)}}{\sqrt{d_i+1} \cdot \sqrt{d_j+1}}|\rmA, m_i^0, v_j \in \gV_1, v_i \in \gV_1 \right)\\ \cdot& \sP(v_j \in \gV_1|m_i^0, v_i \in \gV_1, \rmA) \\
%
+& \E_{\{y_i\}, \{\rvf_i^{(0)}\}|\rmA,v_i \in \gV_1, v_j \in \gV_2, m_i^0}\left(\frac{\rvf_j^{(0)}}{\sqrt{d_i+1} \cdot \sqrt{d_j+1}}|\rmA, m_i^0, v_i \in \gV_1, v_j \in \gV_2\right)\cdot \sP(v_j \in \gV_2|m_i^0)\Bigg)\Bigg)\Bigg).
\end{split}
\label{eq:9}  
\end{equation}

Next, we will show how to compute the conditional expectation and conditional probability in the summand.
\begin{equation}
\begin{split}
&\E_{\{y_i\}, \{\rvf_i^{(0)}\}|\rmA,v_i,v_j \in \gV_1, m_i^0}\left(\frac{\rvf_j^{(0)}}{\sqrt{d_i+1} \cdot \sqrt{d_j+1}}|m_i^0, v_i, v_j \in \gV_1,\rmA\right) \\=& \E_{\{y_i\}, \{\rvf_i^{(0)}\}|\rmA,v_i \in \gV_1, m_i^0, v_j}\left(\frac{\rvf_j^{(0)}}{\sqrt{d_i+1} \cdot \sqrt{d_j+1}}|\rmA, m_i^0, v_i \in \gV_1, v_j \in \gV_1, v_j \text{wrongly send information}\right) \\
%
& \cdot \sP(v_j \text{wrongly send information}|\rmA, m_i^0, v_i \in \gV_1, v_j \in \gV_1) \\
%
+& \E_{\{y_i\}, \{\rvf_i^{(0)}\}|\rmA,v_i \in \gV_1, m_i^0, v_j}\left(\frac{\rvf_j^{(0)}}{\sqrt{d_i+1} \cdot \sqrt{d_j+1}}|\rmA, m_i^0, v_i \in \gV_1, v_j \in \gV_1, v_j \text{correctly send information}\right) \\
%
& \cdot \sP(v_j \text{correctly send information}|\rmA, m_i^0, v_i \in \gV_1, v_j \in \gV_1).
\end{split}
\label{eq:10}
\end{equation}
Combined with the independence assumption, we have:
\begin{equation}
\begin{split}
\sP(v_j \text{wrongly send information}|\rmA, m_i^0, v_i \in \gV_1, v_j \in \gV_1) =
% & \frac{\sP(v_j \text{wrongly send information}, v_j \in \gV_1|m_i^0)}{\sP(v_j \in \gV_1|m_i^0)} \\
%
% =& \frac{\sP(v_j \text{wrongly send information}|m_i^0)\cdot \sP(v_j \in \gV_1|m_i^0)}{\sP(v_j \in \gV_1)|m_i^0)} \\
%
% =& \sP(v_j \text{ wrongly send information}|m_i^0)=
m_i^0.
\end{split}
\label{eq:11}
\end{equation}
Similarly, we obtain:
\begin{equation}
\sP(v_j \text{correctly send information}|\rmA, m_i^0, v_i \in \gV_1, v_j \in \gV_1) = 1-m_i^0.
\label{eq:12}
\end{equation}
Then Equation~(\ref{eq:10}) can be rewritten as:
\begin{equation}
\begin{split}
&\E_{\{y_i\}, \{\rvf_i^{(0)}\}|\rmA,v_i,v_j \in \gV_1, m_i^0}\left(\frac{\rvf_j^{(0)}}{\sqrt{d_i+1} \cdot \sqrt{d_j+1}}|m_i^0, v_i, v_j \in \gV_1,\rmA\right) \\ =& \E_{\{y_i\}, \{\rvf_i^{(0)}\}|\rmA,v_i \in \gV_1, m_i^0, v_j}\left(\frac{\rvf_j^{(0)}}{\sqrt{d_i+1} \cdot \sqrt{d_j+1}}|\rmA, m_i^0, v_i \in \gV_1, v_j \in \gV_1, v_j \text{wrongly send information}\right)\cdot m_i^0 \\
%
+& \E_{\{y_i\}, \{\rvf_i^{(0)}\}|\rmA,v_i \in \gV_1, m_i^0, v_j}\left(\frac{\rvf_j^{(0)}}{\sqrt{d_i+1} \cdot \sqrt{d_j+1}}|\rmA, m_i^0, v_i \in \gV_1, v_j \in \gV_1, v_j \text{correctly send information}\right)\cdot (1-m_i^0) \\
%
=& -\frac{m_i^0\rvmu}{\sqrt{d_i+1} \cdot \sqrt{d_j+1}} + \frac{(1-m_i^0)\rvmu}{\sqrt{d_i+1} \cdot \sqrt{d_j+1}} \\
%
=&
\frac{(1-2m_i^0)\rvmu}{\sqrt{d_i+1} \cdot \sqrt{d_j+1}}.
\end{split}
\label{eq:13}
\end{equation}
\vspace{-0.3cm}
Similarly, we have:
\vspace{-0.2cm}
\begin{equation}
\E_{\{y_i\}, \{\rvf_i^{(0)}\}|\rmA,v_i \in \gV_1, v_j \in \gV_2, m_i^0 }\left(\frac{\rvf_j^{(0)}}{\sqrt{d_i+1} \cdot \sqrt{d_j+1}}|\rmA, m_i^0, v_i \in \gV_1, v_j \in \gV_2\right) = \frac{(1-2m_i^0)\rho\rvmu}{\sqrt{d_i+1}. \cdot \sqrt{d_j+1}}.
\label{eq:14}
\end{equation}
Consider the independence between $m_i^0$ and node class \& degrees, and insert Equation~(\ref{eq:13}) and Equation~(\ref{eq:14}) into Equation~(\ref{eq:9}), we will have:
\begin{equation}
\begin{split}
& \E_{\rmA, \{y_i\}, \{\rvf_i^{(0)}\}|d_i, v_i \in \gV_1}\left(\rvf_i^{(1)}|v_i \in \gV_1, d_i\right) \\ =& \frac{\rvmu}{d_i+1} + \E_{m_i^0|v_i \in \gV_1, d_i}\Bigg(\E_{\rmA|d_i, v_i \in \gV_1, m_i^0}\left(\sum_{j \in \gN_i}(\frac{(1-2m_i^0)k_i\rvmu}{\sqrt{d_i+1} \cdot \sqrt{d_j+1}}+\frac{(1-2m_i^0)(1-k_i)\rho\rvmu}{\sqrt{d_i+1} \cdot \sqrt{d_j+1}})\right)\Bigg) \\
%
=& \frac{\rvmu}{d_i+1} + \E_{m_i^0|v_i \in \gV_1, d_i}\Bigg(\E_{\rmA|d_i, v_i \in \gV_1, m_i^0}\left( \sum_{j \in \gN_i}\frac{(1-2m_i^0)(\rho+(1-\rho)k_i)\rvmu}{\sqrt{d_i+1} \cdot \sqrt{d_j+1}}\right)\Bigg) \\
%
% =& \frac{\rvmu}{d_i+1} + \sum_{j \in \gN_i}\frac{(1-2e_i^0)(\rho+(1-\rho)h_i)\rvmu}{\sqrt{d_i+1} \cdot \sqrt{d_j+1}} \\
%
=& \frac{\rvmu}{d_i+1} + \E_{m_i^0|v_i \in \gV_1, d_i}\Bigg(\left(\frac{(1 - 2m_i^0)(\rho+(1-\rho)h_i)d_i\ratioi}{d_i+1}\right)\rvmu\Bigg)\\
=& \left(\frac{1 + (1 - 2e_i^0)(\rho+(1-\rho)h_i)d_i\ratioi}{d_i+1}\right)\rvmu \equiv \gamma_i^1 \E(\rvf^{(0)}_i).
\end{split}
\label{eq:15}
\end{equation}
% From Equation~\ref{eq:15}, we can conclude that:
% \begin{enumerate}
%     \item If we allow the neighbors of a different class to send the information but be multiplied with a negative sign, then low homophily will not degenerate the performance.
%     \item If the model does not work well in the heterophily setting, i.e., they have a higher error rate $e_i$ in identifying neighbors from another class, the model will also suffer from oversmoothing problem. 
% \end{enumerate}
When $h_i \leq 1$, $\rho+(1-\rho)h_i=(1-h_i)\rho+h_i>0.$ Define $\epsilon' \equiv (1 - 2e_i^0)(\rho+(1-\rho)h_i)$. To obtain the ranges of $\gamma_i^1$, when $e_i^0 \geq 0.5$, $\epsilon' \leq 0$, it resembles the derivations of CASE 1 in Proof~\ref{app:proof1}; when $e_i^0 < 0.5$, $0 < \epsilon \ratioi \leq 1$, it resembles the derivations of CASE 2; when $e_i^0 < 0.5$, $\epsilon \ratioi > 1$, it resembles the derivations of CASE 3.
% The ranges of $\gamma_i^1$ under different conditions of $e_i^0$ and $\ratioi$ can be derived similarly as shown by the Proof~\ref{app:proof1}.
\end{proof}

\section{Additional Experiments}
\vspace{-0.3cm}
\subsection{Ablation study}
\label{subsec:ablation}
\setlength{\tabcolsep}{3pt}
\begin{table*}[h]
\centering
\vspace{-0.5cm}
\caption{Ablation study: degree correction has consistent benefits (robust to oversmoothing \& ability to handle heterophily) in different datasets while signed information has more benefits in heterophilous datasets. Best performance of each model is highlighted in gray.}
\label{tab:ablation}
\begin{adjustbox}{width=1\linewidth}
{\footnotesize
\begin{tabular}{ccccccccccccccc}
\toprule
                                         %\multirow{2}{*}{\backslashbox{\textbf{Model}}{\textbf{Layers}}}    
                                \multicolumn{1}{r}{\textbf{Layers}} 
                                      && \textbf{2}           & \multicolumn{1}{c}{\textbf{4}} & \multicolumn{1}{c}{\textbf{8}} & \multicolumn{1}{c}{\textbf{16}} & \multicolumn{1}{c}{\textbf{32}} & \multicolumn{1}{c}{\textbf{64}} &&  \multicolumn{1}{c}{\textbf{2}}           & \multicolumn{1}{c}{\textbf{4}} & \multicolumn{1}{c}{\textbf{8}} & \multicolumn{1}{c}{\textbf{16}} & \multicolumn{1}{c}{\textbf{32}} & \multicolumn{1}{c}{\textbf{64}}  \\ \cmidrule{1-1} \cmidrule{3-8} \cmidrule{10-15} %cline{2-8}
%\multirow{10}{*}{\rotatebox[origin=c]{90}{\textbf{Homophily datasets}}}   
%\textbf{Model} 
&& \multicolumn{6}{c}{\textbf{Cora} ($h$=0.81)}     & & \multicolumn{6}{c}{\textbf{Citeseer} ($h$=0.74)}                                                                         \\ %\cline{1-1} 
\cline{3-8} \cline{10-15}
                                    
                                        \multicolumn{1}{c}{Base}    &&   
                                        %cora results
                                        \cellcolor{gray!15}$ 86.56{\scriptstyle\pm1.21}$         & \multicolumn{1}{c}{$ 86.04{\scriptstyle\pm0.72}$}    &        \multicolumn{1}{c}{$ 85.51{\scriptstyle\pm1.51}$}     &       \multicolumn{1}{c}{$ 85.33{\scriptstyle\pm0.72}$}      &     \multicolumn{1}{c}{$ 85.37{\scriptstyle\pm1.58}$}       &    \multicolumn{1}{c}{$ 72.17{\scriptstyle\pm8.89}$}   & &  
                                        % citeseer results
                                        \cellcolor{gray!15}$76.51{\scriptstyle\pm1.63}$ & $75.03{\scriptstyle\pm1.67}$ & $73.96{\scriptstyle\pm1.52}$ & $73.59{\scriptstyle\pm1.51}$& $71.91{\scriptstyle\pm1.94}$ & $32.08{\scriptstyle\pm15.74}$                                         \\ 
                                        
                                      \multicolumn{1}{c}{\texttt{+deg}}    &&  
                                      %cora results
                                      \cellcolor{gray!15}$86.72{\scriptstyle\pm1.29}$      &          \multicolumn{1}{c}{$86.02{\scriptstyle\pm0.97}$}           & \multicolumn{1}{c}{$85.49{\scriptstyle\pm1.32}$}           & \multicolumn{1}{c}{$85.27{\scriptstyle\pm1.59}$}            & \multicolumn{1}{c}{$85.27{\scriptstyle\pm1.51}$}            & \multicolumn{1}{c}{$84.21{\scriptstyle\pm1.22}$}   &   &                   % citeseer results
                                      \cellcolor{gray!15}$76.63{\scriptstyle\pm1.38}$  & $74.64{\scriptstyle\pm1.97}$&  $74.15{\scriptstyle\pm1.61}$&  $73.73{\scriptstyle\pm1.31}$&  $73.61{\scriptstyle\pm1.84}$&  $70.56{\scriptstyle\pm2.27}$
                                      \\  \multicolumn{1}{c}{\texttt{+sign}} &&  
                                      %cora results
                                      $84.81{\scriptstyle\pm1.63}$&   \cellcolor{gray!15}$86.06{\scriptstyle\pm1.7}$&   $85.67{\scriptstyle\pm1.26}$&   $85.39{\scriptstyle\pm0.97}$&   $84.85{\scriptstyle\pm0.98}$&   $78.57{\scriptstyle\pm6.73}$   & &    % citeseer results
                                      \cellcolor{gray!15}$77.13{\scriptstyle\pm1.69}$&  $74.56{\scriptstyle\pm2.02}$&   $73.64{\scriptstyle\pm1.65}$&   $72.31{\scriptstyle\pm2.32}$&   $71.98{\scriptstyle\pm3.44}$&   $68.68{\scriptstyle\pm6.72}$
                        \\  \multicolumn{1}{c}{\texttt{+deg,sign}} &&
                         % cora results
                        \cellcolor{gray!15}$86.96{\scriptstyle\pm1.38}$ & $86.20{\scriptstyle\pm0.89}$ & $85.63{\scriptstyle\pm0.78}$ &
                              $85.47{\scriptstyle\pm1.18}$ & $85.55{\scriptstyle\pm1.66}$ & $77.81{\scriptstyle\pm7.95}$     &  & 
                              % citeseer results 
                              \cellcolor{gray!15}$76.81{\scriptstyle\pm1.71}$ & $74.68{\scriptstyle\pm1.97}$ & $74.69{\scriptstyle\pm2.35}$ &
                              $73.28{\scriptstyle\pm1.45}$ & $71.81{\scriptstyle\pm2.28}$ & $69.91{\scriptstyle\pm3.97}$ 
                              \\ \midrule %\cmidrule{1-1} \cmidrule{3-8} \cmidrule{10-15} 
                                    %   & \multicolumn{6}{c}{\textbf{Citeseer ($h$=0.74)}}                                                            \\ \hline 
                                        % \multicolumn{1}{c}{Base}    & \cellcolor{gray!15}$76.51{\scriptstyle\pm1.63}$ & $75.03{\scriptstyle\pm1.67}$ & $73.96{\scriptstyle\pm1.52}$ & $73.59{\scriptstyle\pm1.51}$& $71.91{\scriptstyle\pm1.94}$ & $32.08{\scriptstyle\pm15.74}$                                         \\  
                                    %   \multicolumn{1}{c}{+deg}    &  \cellcolor{gray!15}$76.63{\scriptstyle\pm1.38}$  & $74.64{\scriptstyle\pm1.97}$&  $74.15{\scriptstyle\pm1.61}$&  $73.73{\scriptstyle\pm1.31}$&  $73.61{\scriptstyle\pm1.84}$&  $70.56{\scriptstyle\pm2.27}$                     \\  
                                    %   \multicolumn{1}{c}{+sign} &   \cellcolor{gray!15}$77.13{\scriptstyle\pm1.69}$&  $74.56{\scriptstyle\pm2.02}$&   $73.64{\scriptstyle\pm1.65}$&   $72.31{\scriptstyle\pm2.32}$&   $71.98{\scriptstyle\pm3.44}$&   $68.68{\scriptstyle\pm6.72}$                                                                     \\ 
                            %           \multicolumn{1}{c}{+deg,sign}   & \cellcolor{gray!15}$76.81{\scriptstyle\pm1.71}$ & $74.68{\scriptstyle\pm1.97}$ & $74.69{\scriptstyle\pm2.35}$ &
                            %   $73.28{\scriptstyle\pm1.45}$ & $71.81{\scriptstyle\pm2.28}$ & $69.91{\scriptstyle\pm3.97}$                                              \\ \hline
&& \multicolumn{6}{c}{\textbf{Cornell ($h$=0.3)}} && \multicolumn{6}{c}{\textbf{Chameleon ($h$=0.23)}}                                                                                                                                                                                                                               \\ %\cline{1-1} 
\cline{3-8} \cline{10-15} 
                                      \multicolumn{1}{c}{Base}    && \cellcolor{gray!15}$61.89{\scriptstyle\pm3.72}$ & $60.00{\scriptstyle\pm5.24}$ & $58.92{\scriptstyle\pm5.24}$ &
                              $56.49{\scriptstyle\pm5.73}$ & $58.92{\scriptstyle\pm3.15}$ & $49.19{\scriptstyle\pm16.70}$          &&
% Chameleon results
\cellcolor{gray!15}$64.98{\scriptstyle\pm1.84}$ & $62.65{\scriptstyle\pm3.09}$ & $62.43{\scriptstyle\pm3.28}$ & $54.69{\scriptstyle\pm2.58}$& $47.68{\scriptstyle\pm2.63}$ & $29.74{\scriptstyle\pm5.21}$
\\  
                                      \multicolumn{1}{c}{\texttt{+deg}}    && \cellcolor{gray!15}$63.78{\scriptstyle\pm5.57}$ & $62.70{\scriptstyle\pm5.90}$ & $59.46{\scriptstyle\pm4.52}$ &
                              $56.49{\scriptstyle\pm5.73}$ & $57.57{\scriptstyle\pm4.20}$ & $58.92{\scriptstyle\pm3.15}$    &&
% Chameleon results
$66.54{\scriptstyle\pm2.19}$ & $68.31{\scriptstyle\pm2.70}$ & \cellcolor{gray!15}$68.99{\scriptstyle\pm2.38}$ & $67.68{\scriptstyle\pm3.70}$& $56.86{\scriptstyle\pm8.80}$ & $41.95{\scriptstyle\pm9.56}$
\\  
                                      \multicolumn{1}{c}{\texttt{+sign}} && \cellcolor{gray!15}$85.41{\scriptstyle\pm7.27}$&  $76.76{\scriptstyle\pm7.07}$& $70.00{\scriptstyle\pm5.19}$&  $67.57{\scriptstyle\pm9.44}$&  $63.24{\scriptstyle\pm6.07}$&  $63.24{\scriptstyle\pm6.53}$    && 
% Chameleon results
\cellcolor{gray!15}$65.31{\scriptstyle\pm3.20}$&  $53.55{\scriptstyle\pm6.35}$& $53.05{\scriptstyle\pm2.28}$&  $51.93{\scriptstyle\pm4.00}$&  $57.17{\scriptstyle\pm3.39}$&  $51.93{\scriptstyle\pm8.95}$
\\  
                                      \multicolumn{1}{c}{\texttt{+deg,sign}}            && \cellcolor{gray!15}$84.32{\scriptstyle\pm6.37}$&  $78.92{\scriptstyle\pm8.09}$& $73.51{\scriptstyle\pm5.90}$&  $70.81{\scriptstyle\pm5.64}$&  $68.11{\scriptstyle\pm5.14}$&  $62.43{\scriptstyle\pm6.67}$ &&
% Chameleon results
\cellcolor{gray!15}$65.75{\scriptstyle\pm1.81}$ & $61.49{\scriptstyle\pm7.38}$ & $53.73{\scriptstyle\pm7.79}$ &
                               $52.43{\scriptstyle\pm5.37}$ & $55.92{\scriptstyle\pm5.14}$ & $56.95{\scriptstyle\pm3.93}$ 
%                                       \\ \hline
% %\multirow{10}{*}{\rotatebox[origin=c]{90}{\textbf{Heterophily datasets}}} 
% & \multicolumn{6}{c}{\textbf{Chameleon ($h$=0.23)}}                                                                                                                                                                                                                                       \\  \hline
%                                       \multicolumn{1}{c}{Base}    & \cellcolor{gray!15}$64.98{\scriptstyle\pm1.84}$ & $62.65{\scriptstyle\pm3.09}$ & $62.43{\scriptstyle\pm3.28}$ & $54.69{\scriptstyle\pm2.58}$& $47.68{\scriptstyle\pm2.63}$ & $29.74{\scriptstyle\pm5.21}$                 \\ 
%                                       \multicolumn{1}{c}{+deg}    & $66.54{\scriptstyle\pm2.19}$ & $68.31{\scriptstyle\pm2.70}$ & \cellcolor{gray!15}$68.99{\scriptstyle\pm2.38}$ & $67.68{\scriptstyle\pm3.7}$& $56.86{\scriptstyle\pm8.8}$ & $41.95{\scriptstyle\pm9.56}$                                                        \\  
%                                       \multicolumn{1}{c}{+sign} & \cellcolor{gray!15}$65.31{\scriptstyle\pm3.2}$&  $53.55{\scriptstyle\pm6.35}$& $53.05{\scriptstyle\pm2.28}$&  $51.93{\scriptstyle\pm4.00}$&  $57.17{\scriptstyle\pm3.39}$&  $51.93{\scriptstyle\pm8.95}$                                            \\  
%                                       \multicolumn{1}{c}{+deg,sign}            &  \cellcolor{gray!15}$65.75{\scriptstyle\pm1.81}$ & $61.49{\scriptstyle\pm7.38}$ & $53.73{\scriptstyle\pm7.79}$ &
%                               $52.43{\scriptstyle\pm5.37}$ & $55.92{\scriptstyle\pm5.14}$ & $56.95{\scriptstyle\pm3.93}$               
                               
                              \\ \bottomrule

\end{tabular}
}
\end{adjustbox}
\vspace{-0.5cm}
\end{table*}
We now study the impact of two proposed mechanisms (signed messages and degree correction, \S~\ref{section: model_design}). To better show their effects, we  add each design choice to a base model and track the changes in the node classification performance. As the base model, we choose a GCN variant that uses the message passing mechanism \citep{kipf2016semi} with weight bias, a residual connection (but \textit{not decaying aggregation}) for robustness to oversmoothing, and Elu non-linearity $\sigma$. 
We denote the model that replaces the message passing with our signed messages mechanism as \texttt{+sign}, and the model that incorporates the degree correction as \texttt{+deg}. The model that uses both designs is denoted as \texttt{+sign,deg}. 
Table~\ref{tab:ablation} gives the accuracy of the models in the supervised node classification task for different layers. 

We observe that both mechanisms alleviate the oversmoothing problem. Specifically, the base model has a sharp performance decrease after 32 layers, while the other models have significantly higher performance. 
In general, the \texttt{+deg} model is better than \texttt{+sign} in alleviating oversmoothing, and has a consistent performance gain across different data. For Chameleon, we observe increase in accuracy as we stack more layers; the large performance gain of \method results from the degree correction.
In Cora and Cornell, \texttt{+sign,deg} consistently performs better across different layers than the model with only one design, demonstrating the constructive effect from our two proposed mechanisms.

The signed message design has an advantage in heterophilous datasets. In the Cornell dataset, using signed information rather than plain message passing  results in over 20\% gain, which explains the strong performance of \method. However, in homophilous datasets, the benefit from signed messages is  limited, as these datasets have few different-class neighbors. % from different classes. %This is understandable, because in homophily datasets, there are not many neighbors from other classes. 
%As we pointed out in Thm.~\ref{theorem: signed_messages},  when signs are included, the error rate affects the performance. For the models that do not include signed messages, Thms.~\ref{theorem: initial_stage} and~\ref{theorem: developing stage} indicate that the effective homophily level affects the performance. 
{This is because when the effective homophily $\heterophilyil$ is high and error rate $e_i^0$ is low, $\lim_{\heterophilyil \to 1, e_i^0 \to 0} \frac{(1+\rho)\heterophilyil-\rho}{(1 - 2e_i^0)(\rho+(1-\rho)\heterophilyil)}=1$, so using signed messages is less beneficial in homophilous datasets.}



\subsection{Batch norm \& Layer norm}
\label{app:batchnorm_layernorm}
In \S~\ref{section: model_design}, we use decaying aggregation instead of other normalizing mechanisms. Other mechanisms, such as batch or layer norm, may be seen as solutions to the heterophily and oversmoothing problems. 
However, batch norm cannot compensate for the dispersion of the mean vectors (\S~\ref{section: analysis}) due to different degrees and homophily levels of the nodes. Although, to some extent, it reduces the speed by which the representations of the susceptible nodes (case 1 \& 2) move towards the other class (good for oversmoothing), it also prevents the representations of the nodes that could benefit from the propagation (case 3) from increasing the distances (drop in accuracy). 
%In our experiments , we find that, in general, adding batch norm significantly decreases the accuracy in heterophily datasets, but helps alleviate oversmoothing. 
%Layer norm is a better option~\cite{zhou2020understanding} for oversmoothing and leads to a smaller decrease in accuracy than batch norm in most datasets. However, %in our experiments (App.~\ref{app:batchnorm_layernorm}), 
Layer norm is better at overcoming the dispersion effect but may lead to a significant accuracy drop in some datsets when a subset of features are more important than the others. Thus, we \textbf{do not} use any of these normalizations. 

%In this section, we verify this conjecture by comparing the prediction accuracy of the base model with  models that use either batch norm or layer norm. % in the supervised node classification tasks on real datasets.
Next, we provide experiments to show the effects of batch norm and layer norm. We use the following base model (the same model used in \S \ref{subsec:ablation}): a GCN~\cite{kipf2016semi} with weight bias, Elu non-linearity and residual connection. We do \textbf{not} include any of our designs so as to exclude any other factors that can affect the performance. The models we compare against are \texttt{+BN} and \texttt{+LN}, which %. \texttt{+BN} and \texttt{+LN} 
represent the models that add batch norm and layer norm right before the non-linear activation, respectively. 

\setlength{\tabcolsep}{3pt}
\begin{table*}[h]
\vspace{-0.2cm}
\centering
\caption{Effects of using batch norm \& layer norm: decrease in accuracy but improvement in oversmoothing. Best performance of each model across different layers is highlighted in gray.}
\label{tab:bn_ln}
\begin{adjustbox}{width=\linewidth}
{\footnotesize
\begin{tabular}{ccccccccccccccc}
\toprule
                                         %\multirow{2}{*}{\backslashbox{\textbf{Model}}{\textbf{Layers}}}    
                                \multicolumn{1}{r}{\textbf{Layers}} 
                                      && \textbf{2}           & \multicolumn{1}{c}{\textbf{4}} & \multicolumn{1}{c}{\textbf{8}} & \multicolumn{1}{c}{\textbf{16}} & \multicolumn{1}{c}{\textbf{32}} & \multicolumn{1}{c}{\textbf{64}} &&  \multicolumn{1}{c}{\textbf{2}}           & \multicolumn{1}{c}{\textbf{4}} & \multicolumn{1}{c}{\textbf{8}} & \multicolumn{1}{c}{\textbf{16}} & \multicolumn{1}{c}{\textbf{32}} & \multicolumn{1}{c}{\textbf{64}}  \\ \cmidrule{1-1} \cmidrule{3-8} \cmidrule{10-15} %cline{2-8}
%\multirow{10}{*}{\rotatebox[origin=c]{90}{\textbf{Homophily datasets}}}   
%\textbf{Model} 
&& \multicolumn{6}{c}{\textbf{Cora} ($h$=0.81)}     & & \multicolumn{6}{c}{\textbf{Citeseer} ($h$=0.74)}                                                                         \\ %\cline{1-1} 
\cline{3-8} \cline{10-15}
                                    
                                        \multicolumn{1}{c}{Base}    &&   
                                        %cora results
                                        \cellcolor{gray!15}$ 86.56{\scriptstyle\pm1.21}$         & \multicolumn{1}{c}{$ 86.04{\scriptstyle\pm0.72}$}    &        \multicolumn{1}{c}{$ 85.51{\scriptstyle\pm1.51}$}     &       \multicolumn{1}{c}{$ 85.33{\scriptstyle\pm0.72}$}      &     \multicolumn{1}{c}{$ 85.37{\scriptstyle\pm1.58}$}       &    \multicolumn{1}{c}{$ 72.17{\scriptstyle\pm8.89}$}   & &  
                                        % citeseer results
                                        \cellcolor{gray!15}$76.51{\scriptstyle\pm1.63}$ & $75.03{\scriptstyle\pm1.67}$ & $73.96{\scriptstyle\pm1.52}$ & $73.59{\scriptstyle\pm1.51}$& $71.91{\scriptstyle\pm1.94}$ & $32.08{\scriptstyle\pm15.74}$                                         \\ 
                                        
                                      \multicolumn{1}{c}{\texttt{+BN}}    &&  
                                      %cora results
                                      $84.73{\scriptstyle\pm1.10}$      &          \multicolumn{1}{c}{$83.76{\scriptstyle\pm1.61}$}           & \multicolumn{1}{c}{$83.94{\scriptstyle\pm1.51}$}           & \multicolumn{1}{c}{$84.57{\scriptstyle\pm1.22}$}            & \multicolumn{1}{c}{$84.63{\scriptstyle\pm1.58}$}            & \cellcolor{gray!15}{$85.17{\scriptstyle\pm1.18}$}   &   &                   % citeseer results
                                      $71.62{\scriptstyle\pm1.48}$  & $71.58{\scriptstyle\pm1.00}$&  $72.18{\scriptstyle\pm1.39}$&  $72.45{\scriptstyle\pm1.42}$&  \cellcolor{gray!15}$72.76{\scriptstyle\pm1.31}$&  $72.61{\scriptstyle\pm1.41}$
                                      \\  \multicolumn{1}{c}{\texttt{+LN}} &&  
                                      %cora results
                                      $84.73{\scriptstyle\pm1.63}$&   $86.60{\scriptstyle\pm1.01}$&   \cellcolor{gray!15}$86.72{\scriptstyle\pm1.36}$&   $86.08{\scriptstyle\pm1.16}$&   $85.67{\scriptstyle\pm1.23}$&   $85.13{\scriptstyle\pm1.20}$   & &    % citeseer results
                                      \cellcolor{gray!15}$76.11{\scriptstyle\pm1.80}$&  $74.02{\scriptstyle\pm2.77}$&   $75.00{\scriptstyle\pm1.95}$&   $74.50{\scriptstyle\pm0.96}$&   $74.49{\scriptstyle\pm2.10}$&   $73.94{\scriptstyle\pm2.03}$
                        \\   \midrule %\cmidrule{1-1} \cmidrule{3-8} \cmidrule{10-15} 
                                    %   & \multicolumn{6}{c}{\textbf{Citeseer ($h$=0.74)}}                                                            \\ \hline 
                                        % \multicolumn{1}{c}{Base}    & \cellcolor{gray!15}$76.51{\scriptstyle\pm1.63}$ & $75.03{\scriptstyle\pm1.67}$ & $73.96{\scriptstyle\pm1.52}$ & $73.59{\scriptstyle\pm1.51}$& $71.91{\scriptstyle\pm1.94}$ & $32.08{\scriptstyle\pm15.74}$                                         \\  
                                    %   \multicolumn{1}{c}{+deg}    &  \cellcolor{gray!15}$76.63{\scriptstyle\pm1.38}$  & $74.64{\scriptstyle\pm1.97}$&  $74.15{\scriptstyle\pm1.61}$&  $73.73{\scriptstyle\pm1.31}$&  $73.61{\scriptstyle\pm1.84}$&  $70.56{\scriptstyle\pm2.27}$                     \\  
                                    %   \multicolumn{1}{c}{+sign} &   \cellcolor{gray!15}$77.13{\scriptstyle\pm1.69}$&  $74.56{\scriptstyle\pm2.02}$&   $73.64{\scriptstyle\pm1.65}$&   $72.31{\scriptstyle\pm2.32}$&   $71.98{\scriptstyle\pm3.44}$&   $68.68{\scriptstyle\pm6.72}$                                                                     \\ 
                            %           \multicolumn{1}{c}{+deg,sign}   & \cellcolor{gray!15}$76.81{\scriptstyle\pm1.71}$ & $74.68{\scriptstyle\pm1.97}$ & $74.69{\scriptstyle\pm2.35}$ &
                            %   $73.28{\scriptstyle\pm1.45}$ & $71.81{\scriptstyle\pm2.28}$ & $69.91{\scriptstyle\pm3.97}$                                              \\ \hline
&& \multicolumn{6}{c}{\textbf{Cornell ($h$=0.3)}} && \multicolumn{6}{c}{\textbf{Chameleon ($h$=0.23)}}                                                                                                                                                                                                                               \\ %\cline{1-1} 
\cline{3-8} \cline{10-15} 
                                      \multicolumn{1}{c}{Base}    && \cellcolor{gray!15}$61.89{\scriptstyle\pm3.72}$ & $60.00{\scriptstyle\pm5.24}$ & $58.92{\scriptstyle\pm5.24}$ &
                              $56.49{\scriptstyle\pm5.73}$ & $58.92{\scriptstyle\pm3.15}$ & $49.19{\scriptstyle\pm16.70}$          &&
% Chameleon results
\cellcolor{gray!15}$64.98{\scriptstyle\pm1.84}$ & $62.65{\scriptstyle\pm3.09}$ & $62.43{\scriptstyle\pm3.28}$ & $54.69{\scriptstyle\pm2.58}$& $47.68{\scriptstyle\pm2.63}$ & $29.74{\scriptstyle\pm5.21}$
\\  
                                      \multicolumn{1}{c}{\texttt{+BN}}    && $58.38{\scriptstyle\pm6.42}$ & \cellcolor{gray!15}$59.19{\scriptstyle\pm4.59}$ & $55.41{\scriptstyle\pm6.65}$ &
                              $57.30{\scriptstyle\pm3.15}$ & $57.57{\scriptstyle\pm6.29}$ & $57.02{\scriptstyle\pm6.19}$    &&
% Chameleon results
$60.88{\scriptstyle\pm2.24}$ & $61.38{\scriptstyle\pm2.17}$ & $61.84{\scriptstyle\pm4.08}$ & \cellcolor{gray!15}$61.97{\scriptstyle\pm3.01}$& $59.04{\scriptstyle\pm3.79}$ & $57.84{\scriptstyle\pm3.67}$
\\  
                                      \multicolumn{1}{c}{\texttt{+LN}} && $58.11{\scriptstyle\pm6.19}$&  $55.68{\scriptstyle\pm6.19}$& $58.92{\scriptstyle\pm7.63}$&  \cellcolor{gray!15}$59.19{\scriptstyle\pm3.07}$&  $58.92{\scriptstyle\pm3.15}$&  $58.00{\scriptstyle\pm3.03}$    && 
% Chameleon results
$61.86{\scriptstyle\pm1.73}$&  $62.17{\scriptstyle\pm2.48}$& \cellcolor{gray!15}$62.41{\scriptstyle\pm2.99}$&  $60.37{\scriptstyle\pm2.36}$&  $58.25{\scriptstyle\pm3.03}$&  $58.92{\scriptstyle\pm3.15}$
\\  
                                      
%                                       \\ \hline
% %\multirow{10}{*}{\rotatebox[origin=c]{90}{\textbf{Heterophily datasets}}} 
% & \multicolumn{6}{c}{\textbf{Chameleon ($h$=0.23)}}                                                                                                                                                                                                                                       \\  \hline
%                                       \multicolumn{1}{c}{Base}    & \cellcolor{gray!15}$64.98{\scriptstyle\pm1.84}$ & $62.65{\scriptstyle\pm3.09}$ & $62.43{\scriptstyle\pm3.28}$ & $54.69{\scriptstyle\pm2.58}$& $47.68{\scriptstyle\pm2.63}$ & $29.74{\scriptstyle\pm5.21}$                 \\ 
%                                       \multicolumn{1}{c}{+deg}    & $66.54{\scriptstyle\pm2.19}$ & $68.31{\scriptstyle\pm2.70}$ & \cellcolor{gray!15}$68.99{\scriptstyle\pm2.38}$ & $67.68{\scriptstyle\pm3.7}$& $56.86{\scriptstyle\pm8.8}$ & $41.95{\scriptstyle\pm9.56}$                                                        \\  
%                                       \multicolumn{1}{c}{+sign} & \cellcolor{gray!15}$65.31{\scriptstyle\pm3.2}$&  $53.55{\scriptstyle\pm6.35}$& $53.05{\scriptstyle\pm2.28}$&  $51.93{\scriptstyle\pm4.00}$&  $57.17{\scriptstyle\pm3.39}$&  $51.93{\scriptstyle\pm8.95}$                                            \\  
%                                       \multicolumn{1}{c}{+deg,sign}            &  \cellcolor{gray!15}$65.75{\scriptstyle\pm1.81}$ & $61.49{\scriptstyle\pm7.38}$ & $53.73{\scriptstyle\pm7.79}$ &
%                               $52.43{\scriptstyle\pm5.37}$ & $55.92{\scriptstyle\pm5.14}$ & $56.95{\scriptstyle\pm3.93}$               
                               
                               \bottomrule

\end{tabular}
}
\end{adjustbox}
\vspace{-0.1cm}
\end{table*}

Table~\ref{tab:bn_ln} shows that both batch norm and layer norm can help with oversmoothing. Moreover, adding layer norm is in general better than adding batch norm. This is expected because the scaling effect caused by the propagation can be alleviated by normalizing across the node representations. Thus, the dispersion of the expected representations can be mitigated. On the other hand, batch norm normalizes across all the nodes, so it requires sacrificing the nodes that benefit (case 3) to compensate for the nodes that are prone to moving towards the other classes (case 1 \& case 2). As a result, batch norm is less effective in mitigating oversmoothing and leads to a bigger decrease in accuracy. 

Another finding is that both layer norm and batch norm lead to a significant accuracy decrease (2\%-3\%) in the heterophilous datasets. \texttt{+BN} has a clear accuracy drop even in the homophilous datasets. As Thm.~\ref{theorem: initial_stage} points out: higher heterophily level may result in sign flip. If the representations flip the sign, using batch norm or layer norm will not revert the sign, but they may instead encourage the representations to move towards the other class more.

Given the limitations shown above, we \textbf{do not} use either batch norm or layer norm in our proposed model, \method.

\subsection{More on the Initial \& Developing Stages}
\label{app:2stages}
Section \ref{exp:case study} shows how the node classification accuracy changes for nodes of different degrees with the number of layers on Citeseer. Here, we provide more details of this experiment and give the results on another dataset,  Cora.

\textbf{Datasets.} According to Thm.~\ref{theorem: initial_stage} and~\ref{theorem: developing stage}, in order to see both the initial and the developing stage, we need to use homophilous datasets. In  heterophilous datasets, most nodes satisfy case 1, so the initial stage does not exist. %There are no three cases as in the initial stage and only case 2 exists.

\textbf{Measurement of effective homophily $\pmb{\heterophilyil}$.} %To align this with our theorems---which apply to binary classification---, the decision boundary is defined as the curve that maximizes the margins between the initial features in different classes. In binary classification, the decision boundary is the origin. 
To estimate the effective homophily $\heterophilyil$, we measure the portion of neighbors that have the same ground truth label as $v_i$ and are correctly classified. 
% We use this ratio to approximate the neighbors whose features are still inside the decision boundary of class $y_i$.  
%Our goal is to estimate the effective homophily $\hat{h_i}$ before the last propagation takes place and analyze its impact on the accuracy of the final layer. 
% \reminder{thenext sentence is not clear -- do you mean before performing the linear transformation too?}
Following our theory, we estimate $\heterophilyil$ \textbf{before} the last propagation takes place and analyze its impact on the accuracy of the final layer. 
In more detail, we obtain the node representations before the last propagation from a trained vanilla GCN~\cite{kipf2016semi} and then perform a linear transformation using the weight matrix and bias vector from the last layer. Then, we use the transformed representations to classify the neighbors of node $v_i$ and compute $\heterophilyil$. We note that we leverage the intermediate representations only for the estimation of $\heterophilyil$; the accuracy of the final layer is still measured using the outputs from the final layer. 
% The reason for using the features before the last propagation is that we would like to estimate the effective homophily $\hat{h_i}$ before the last propagation takes place and analyze $\hat{h_i}$'s impact on the accuracy of the final layer. 

\setlength{\tabcolsep}{4pt}
\begin{wraptable}{r}{8.2cm}
    \centering
    \vspace{-0.5cm}
    \caption{Citeseer: Accuracy (Acc) and average effective homophily ($\Bar{\heterophilyil}$) for nodes with different degrees across various layers. Last layer of initial stage marked in gray.} %The last layer in the initial stage ($\Bar{\hat{h_i}} > 0.5$ for all degrees) are marked in grey.}
    \vspace{0.1cm}
    % \begin{adjustbox}{width=0.5\textwidth}
    % {\footnotesize
    \resizebox{!}{.38\linewidth}{%\footnotesize
    \begin{tabular}{ccccccc} 
    \toprule
          & & \multicolumn{5}{c}{\bf Degrees} \\ \cline{3-7}
      \multicolumn{1}{c}{\bf  Layers} & %\backslashbox{Acc, $\Bar{\hat{h_i}}$}{Degrees} 
      &   $[1,2]$           &   $[3,6]$            &   $[7,15]$   &   $[16,39]$ & $[40,99]$  \\
    \midrule
       \multirow{2}{*}{\bf 2}& Acc & $74.44$ & $78.51$ & $84.04$
        & $96.00$ & $100.00$  \\ & $\Bar{\heterophilyil}$ & $0.65$ & $0.67$ & $0.72$
        & $0.83$ & $0.91$  \\
        \midrule
       \multirow{2}{*}{\bf 3}& Acc & $70.92$ & $77.59$ & $83.03$
        & $92.75$ & $100.00$  \\& $\Bar{\heterophilyil}$  & $0.63$ & $0.66$ & $0.71$
        & $0.84$ & $0.92$  \\
        \midrule
       \multirow{2}{*}{\bf 4}& Acc & $60.54$ & $68.56$ & $77.63$
        & $94.00$ & $100.00$  \\& $\Bar{\heterophilyil}$  & \cellcolor{gray!15}$0.54$ & \cellcolor{gray!15}$0.58$ & \cellcolor{gray!15}$0.66$
        & \cellcolor{gray!15}$0.79$ & \cellcolor{gray!15}$0.84$  \\
        \midrule
       \multirow{2}{*}{\bf 5}& Acc & $41.66$ & $48.70$ & $56.97$
        & $61.33$ & $11.11$  \\& $\Bar{\heterophilyil}$  & $0.36$ & $0.38$ & $0.45$
        & $0.48$ & $0.11$  \\
        \midrule
       \multirow{2}{*}{\bf 6}& Acc & $23.61$ & $28.87$ & $41.17$
        & $31.83$ & $0.00$  \\& $\Bar{\heterophilyil}$  & $0.18$ & $0.19$ & $0.27$
        & $0.22$ & $0.00$  \\
	   \bottomrule
    \end{tabular}}
    % \end{adjustbox}
    %}  
    % \vspace{-0.3cm}
    \label{tab:case_study_citeseer}
\end{wraptable}

\textbf{Degree intervals.} To investigate the change in GCN accuracy with different layers for nodes with different degrees, we categorize the nodes in $n$ degree intervals. For the degree intervals, we use logarithmic binning (base 2). In detail, we denote the highest and lowest degree by $d_{max}$ and $d_{min}$, respectively, and let $\Omega \equiv \frac{\log_2{d_{max}}-\log_2{d_{min}}}{n}$. Then, we divide the nodes into $n$ intervals, where the $j$-th interval is defined as: $[d_{min}\cdot 2^{(j-1)\Omega}, d_{min}\cdot 2^{j\Omega})$.

% Then we will show the accuracy of GCNs with different layers for nodes with different degrees. 

\textbf{Dataset: Citeseer.}
Figure~\ref{fig:phase_transition} and Table~\ref{tab:case_study_citeseer} show how the accuracy changes with the number of layers for different node degree intervals. We observe that in the initial stage, the accuracy increases as the degree and $\Bar{\heterophilyil}$ increase. However, in the developing stage, the accuracy of high-degree nodes drops more sharply than that of low-degree nodes. 

\textbf{Dataset: Cora.}  The results for Cora are shown in 
% As can be seen in 
Figure~\ref{fig:case_study_cora} and Table~\ref{tab:case_study_cora}.  
In the initial stage, the nodes with lower 

% \vspace{0.3cm}
\begin{minipage}{\textwidth}
\begin{minipage}[c]{0.55\textwidth}
\centering
\includegraphics[scale=0.18, bb=800 400 450 200]{Figs/transition_plot_cora_new.png}
\captionsetup{type=figure}
\vspace{2.5cm}
\captionof{figure}{Cora: Accuracy per (logarithmic) degree bin.}
\label{fig:case_study_cora}
\end{minipage}
% \begin{adjustbox}{width=0.38\textwidth}
\begin{minipage}[c]{0.45\textwidth}
\setlength{\tabcolsep}{5pt}
    \centering
    \captionsetup{type=table}
    \captionof{table}{Cora: Accuracy and average effective homophily ($\Bar{\heterophilyil}$) for nodes with different degrees across different layers. Last layer of initial stage marked in gray.}
    \resizebox{!}{.45\linewidth}{%\footnotesize
    \begin{tabular}{ccccccc} 
    \toprule
      & & \multicolumn{5}{c}{\bf Degrees} \\ \cline{3-7}
      \multicolumn{1}{c}{\bf Layers} & %\backslashbox{Acc, $\Bar{\hat{h_i}}$}{Degrees} 
      &   $[1,2]$           &   $[3,7]$            &   $[8,21]$   &   $[22,60]$ & $[61,168]$  \\
    \midrule
       \multirow{2}{*}{\bf 2}& Acc & $85.14$ & $88.52$ & $83.78$
        & $90.00$ & $100.00$  \\ & $\Bar{\heterophilyil}$ & $0.77$ & $0.77$ & $0.72$
        & $0.63$ & $0.81$  \\
        \midrule
       \multirow{2}{*}{\bf 3}& Acc & $82.28$ & $87.26$ & $84.42$
        & $85.00$ & $100.00$  \\& $\Bar{\heterophilyil}$  & $0.77$ & $0.78$ & $0.73$
        & $0.64$ & $0.84$  \\
        \midrule
       \multirow{2}{*}{\bf 4}& Acc & $79.57$ & $85.52$ & $83.26$
        & $85.00$ & $100.00$  \\& $\Bar{\heterophilyil}$  & $0.75$ & $0.76$ & $0.71$
        & $0.63$ & $0.80$  \\
        \midrule
        \multirow{2}{*}{\bf 5}& Acc & $77.38$ & $83.75$ & $82.83$
        & $85.00$ & $96.19$  \\& $\Bar{\heterophilyil}$  & $0.72$ & $0.73$ & $0.68$
        & $0.56$ & $0.83$  \\
        \midrule
        \multirow{2}{*}{\bf 6}& Acc & $63.35$ & $68.20$ & $66.01$
        & $70.00$ & $78.57$  \\& $\Bar{\heterophilyil}$  & \cellcolor{gray!15}$0.57$ & \cellcolor{gray!15}$0.60$ & \cellcolor{gray!15}$0.54$
        & \cellcolor{gray!15}$0.52$ & \cellcolor{gray!15}$0.67$  \\
        \midrule
       \multirow{2}{*}{\bf 7}& Acc & $30.91$ & $30.62$ & $29.12$
        & $17.50$ & $21.43$  \\& $\Bar{\heterophilyil}$  & $0.25$ & $0.26$ & $0.21$
        & $0.26$ & $0.23$  \\
        \midrule
       \multirow{2}{*}{\bf 8}& Acc & $31.48$ & $31.02$ & $28.44$
        & $32.50$ & $25.24$  \\& $\Bar{\heterophilyil}$  & $0.24$ & $0.26$ & $0.20$
        & $0.28$ & $0.24$  \\
	   \bottomrule
    \end{tabular}
        \vspace{-1cm}
    }
\label{tab:case_study_cora}
\end{minipage}
% \end{adjustbox}
    \vspace{-0.1cm}
\end{minipage}


% In the initial stage, the nodes with lower  
degrees usually have lower accuracy. One exception is the nodes with degrees in the 
range $[3, 7]$. These nodes have higher accuracy because the average effective homophily $\Bar{\heterophilyil}$ of that degree group is the second highest. In the developing stage, the accuracy of the high-degree nodes drops more than the accuracy of the remaining node groups. 

GCN's behavior on both Citesser and Cora datasets verifies our conjecture based on our theorems in \S~\ref{subsec: heterophily_oversmoothing}.



% \begin{wrapfigure}{r}{0.56\textwidth}
% \centering
% \includegraphics[width=.54\textwidth]{Figs/transition_cora_plot.png}
% \vspace{-0.5cm}
% \caption{Accuracy per (logarithmic) degree bin on Cora.}
% \label{fig:phase_transition_cora}
% \vspace{-0.6cm}
% \end{wrapfigure}
% \setlength{\tabcolsep}{4pt}
% \begin{wraptable}{r}{7cm}
%     \centering
%     \vspace{-0.9cm}
%     \caption{Accuracy (Acc) and average effective homophily ($\Bar{\hat{h_i}}$) for nodes with different degrees across various layers on Citeseer dataset. The last layer in the initial stage ($\Bar{\hat{h_i}} > 0.5$ for all degrees) are marked in grey.}
%     \label{tab:case_study_citeseer}
%     \begin{adjustbox}{width=0.4\textwidth}
%     {\footnotesize
%     \begin{tabular}{c|c|ccccc} 
%     \toprule
%       \multicolumn{1}{c|}{Layers} & \backslashbox{Acc, $\Bar{\hat{h_i}}$}{Degrees} &   $[1,2]$           &   $[3,6]$            &   $[7,15]$   &   $[16,39]$ & $[40,99]$  \\
%     \midrule
%       \multirow{2}{*}{2}& Acc & $74.44$ & $78.51$ & $84.04$
%         & $96.00$ & $100.00$  \\ & $\Bar{\hat{h_i}}$ & $0.65$ & $0.67$ & $0.72$
%         & $0.83$ & $0.91$  \\
%         \midrule
%       \multirow{2}{*}{3}& Acc & $70.92$ & $77.59$ & $83.03$
%         & $92.75$ & $100.00$  \\& $\Bar{\hat{h_i}}$  & $0.63$ & $0.66$ & $0.71$
%         & $0.84$ & $0.92$  \\
%         \midrule
%       \multirow{2}{*}{4}& Acc & $60.54$ & $68.56$ & $77.63$
%         & $94.00$ & $100.00$  \\& $\Bar{\hat{h_i}}$  & \cellcolor{gray!15}$0.54$ & \cellcolor{gray!15}$0.58$ & \cellcolor{gray!15}$0.66$
%         & \cellcolor{gray!15}$0.79$ & \cellcolor{gray!15}$0.84$  \\
%         \midrule
%       \multirow{2}{*}{5}& Acc & $41.66$ & $48.70$ & $56.97$
%         & $61.33$ & $11.11$  \\& $\Bar{\hat{h_i}}$  & $0.36$ & $0.38$ & $0.45$
%         & $0.48$ & $0.11$  \\
%         \midrule
%       \multirow{2}{*}{6}& Acc & $23.61$ & $28.87$ & $41.17$
%         & $31.83$ & $0.00$  \\& $\Bar{\hat{h_i}}$  & $0.18$ & $0.19$ & $0.27$
%         & $0.22$ & $0.00$  \\
% 	   \bottomrule
%     \end{tabular}}
%     \end{adjustbox}
%     %}  
%     \vspace{-0.5cm}
% \end{wraptable}
% As can be seen in Figure~\ref{fig:case_study_cora} and Table~\ref{tab:case_study_cora}, in the initial stage, the nodes with lower degrees usually have lower accuracy. One exception is the nodes whose degrees are in the range $[3, 7]$. They have higher accuracy because the average effective homophily $\Bar{\hat{h_i}}$ of that group is the second highest. In the developing stage, the large degree nodes drop more. 

% GCN's behavior on both Citesser and Cora datasets have verified the conjecture we made based on the theorems in \S \ref{subsec: heterophily_oversmoothing}.
% \subsection{Additional baselines}
% \label{app:additional baselines}
% Due to limited space, we only provide representative baselines in \S~\ref{section: experiments}. Here we provide another two baselines from recent works. PairNorm~\cite{zhao2019pairnorm} is proposed to address the oversmoothing problem and GPRGNN~\cite{chien2021adaptive} is proposed to address both oversmoothing and heterophily problems. We use their original model files and train their models with the datasets and splits we use for every GCN models. We adopt the same hyperperameters as they do. Note that in ~\cite{chien2021adaptive}, the authors use balanced training sets (same number of nodes from different classes), so their reported results for GPRGNN and other baselines (e.g, MLP) are different from the reported results in ours and other papers [36, 37]. \yy{change the citations}

% As shown in Tab.~\ref{tab:real-results} and Tab.~\ref{tab:additional_baselines_performance}, GPRGNN has good performance in homophily datasets such as Citeseer and Cora. For heterophily datasets, though they show improvements over GCNII* and Geom-GCN*, the performance of GPRGNN is close to the performance of MLP and is worse than \method(ours) and H2GCN*. PN is proposed to address oversmoothing so it does not have very competitive results in heterophily datasets. 
% \begin{table*}[h]%[t!]
%     \centering
%     \vspace{-0.2cm}
%     \caption{%Statistics of real datasets for different homophily levels $h$, 
%     Real data: mean accuracy $\pm$ stdev over different data splits. Per GCN model, we report the best performance  across different layers. 
%     }
%     \label{tab:additional_baselines_performance}
%     %\resizebox{0.97\textwidth}{!}{
%     \vspace{-0.15cm}
%     \begin{adjustbox}{width=.9\textwidth}
%     % \hskip-1.15cm
%     \begin{tabular}{lcccccc  ccc c } % Removed vertical rule due to NIPS requirement
%     \toprule
%       %\multirow{2}{*}{\backslashbox{\textbf{Models}}{\textbf{Data, h}}} 
%       &  \texttt{\bf Texas}           &   \texttt{\bf Wisconsin}           &   \texttt{\bf Actor}            &   \texttt{\bf Squirrel}   &   \texttt{\bf Chameleon} & \texttt{\bf Cornell}        &   \texttt{\bf Citeseer}           &   \texttt{\bf Pubmed}            &   \texttt{\bf Cora} \\
%         % & $h=0.11$ & $h=0.21$ & $h=0.22$ & $h=0.22$ & $h=0.23$ & $h=0.3$ & $h=0.57$ & $h=0.74$ & $h=0.8$ & $h=0.81$  \\
%         % \midrule 
%           \textbf{Hom.\ level} $h$ & \textbf{0.11} & \textbf{0.21} & \textbf{0.22} & \textbf{0.22} & \textbf{0.23} & \textbf{0.3} & \textbf{0.74} & \textbf{0.8} & \textbf{0.81} \\
% 		\textbf{\#Nodes} & 183 & 251 & 7,600 & 5,201 & 2,277 & 183 & 3,327 & 19,717 & 2,708 \\
% 		\textbf{\#Edges} & 295 & 466 & 26,752 & 198,493 & 31,421 & 280 & 4,676 & 44,327 & 5,278 \\
% 		\textbf{\#Classes} & 5 & 5 & 5 & 5 & 5 & 5 & 7 & 3 & 6 \\ 
%     \midrule
%     % \midrule
%       % HistFNN --network_setup M64-R-G-V-MO --hist_nhood 0 1 2
%       {PN} & $60.27{\scriptstyle\pm4.34}$ & $48.43{\scriptstyle\pm6.14}$ &
%       $27.40{\scriptstyle\pm1.24}$ & $50.44{\scriptstyle\pm2.04}$ & $62.74{\scriptstyle\pm2.82}$ &  $58.92{\scriptstyle\pm3.15}$ &  $73.59{\scriptstyle\pm1.47}$ & $87.53{\scriptstyle\pm0.44}$ & $85.79{\scriptstyle\pm1.01}$ \\
%       % HistFNN --network_setup M64-R-G-V-G-V-MO --hist_nhood 0 1 2
%       {GPRGNN} & $78.38{\scriptstyle\pm4.36}$ & $82.94{\scriptstyle\pm4.21}$ & $34.63{\scriptstyle\pm1.22}$ & $31.61{\scriptstyle\pm1.24}$ & $46.58{\scriptstyle\pm1.71}$ & $80.27{\scriptstyle\pm8.11}$ &  $77.13{\scriptstyle\pm1.67}$ & $87.54{\scriptstyle\pm0.38}$ & $87.95{\scriptstyle\pm1.18}$ \\
%       \bottomrule
%     \end{tabular}
%     \end{adjustbox}
%     %}  
%     \vspace{-0.3cm}
% \end{table*}

% From Tab.~\ref{tab:oversmoothing} and Tab.~\ref{tab:more_baselines_oversmoothing}, we can see that both GPRGNN and PN are effective in alleviating oversmoothing compared to the vanilla GCN~\cite{kipf2016semi}. PN suffers from performance drop after 32 layers. Both our model \method (Tab.~\ref{tab:oversmoothing}) and GPRGNN maintain good performance after 32 layers.
% \begin{table*}[h]
% \centering
% \caption{Model performance for different layers: mean accuracy $\pm$ stdev over different data splits.}
% \label{tab:more_baselines_oversmoothing}
% \begin{adjustbox}{width=\linewidth}
% {\footnotesize
% \begin{tabular}{ccccccccccccccc}
% \toprule
%                                          %\multirow{2}{*}{\backslashbox{\textbf{Model}}{\textbf{Layers}}}    
%                                 \multicolumn{1}{r}{\textbf{Layers}} 
%                                       && \textbf{2}           & \multicolumn{1}{c}{\textbf{4}} & \multicolumn{1}{c}{\textbf{8}} & \multicolumn{1}{c}{\textbf{16}} & \multicolumn{1}{c}{\textbf{32}} & \multicolumn{1}{c}{\textbf{64}} &&  \multicolumn{1}{c}{\textbf{2}}           & \multicolumn{1}{c}{\textbf{4}} & \multicolumn{1}{c}{\textbf{8}} & \multicolumn{1}{c}{\textbf{16}} & \multicolumn{1}{c}{\textbf{32}} & \multicolumn{1}{c}{\textbf{64}}  \\ \cmidrule{1-1} \cmidrule{3-8} \cmidrule{10-15} %cline{2-8}
% %\multirow{10}{*}{\rotatebox[origin=c]{90}{\textbf{Homophily datasets}}}   
% %\textbf{Model} 
% && \multicolumn{6}{c}{\textbf{Cora} ($h$=0.81)}     & & \multicolumn{6}{c}{\textbf{Citeseer} ($h$=0.74)}                                                                         \\ %\cline{1-1} 
% \cline{3-8} \cline{10-15}
                                    
%                                         \multicolumn{1}{c}{PN}    &&   
%                                         %cora results
%                                         \cellcolor{gray!15}$ 85.79{\scriptstyle\pm1.01}$         & \multicolumn{1}{c}{$ 85.07{\scriptstyle\pm0.91}$}    &        \multicolumn{1}{c}{$ 84.65{\scriptstyle\pm1.09}$}     &       \multicolumn{1}{c}{$ 82.21{\scriptstyle\pm2.84}$}      &     \multicolumn{1}{c}{$ 60.32{\scriptstyle\pm8.28}$}       &    \multicolumn{1}{c}{$ 44.39{\scriptstyle\pm5.60}$}   & &  
%                                         % citeseer results
%                                         \cellcolor{gray!15}$73.59{\scriptstyle\pm1.47}$ & $72.62{\scriptstyle\pm1.97}$ & $72.32{\scriptstyle\pm1.58}$ & $59.71{\scriptstyle\pm15.97}$& $27.21{\scriptstyle\pm10.95}$ & $23.82{\scriptstyle\pm6.64}$                                         \\ 
                                        
%                                       \multicolumn{1}{c}{GPRGNN}    &&  
%                                       %cora results
%                                       \multicolumn{1}{c}{$87.93{\scriptstyle\pm1.11}$}      &        \cellcolor{gray!15}$87.95{\scriptstyle\pm1.18}$           & \multicolumn{1}{c}{$87.87{\scriptstyle\pm1.41}$}           & \multicolumn{1}{c}{$87.26{\scriptstyle\pm1.51}$}            & \multicolumn{1}{c}{$87.18{\scriptstyle\pm1.29}$}            & \multicolumn{1}{c}{$87.32{\scriptstyle\pm1.21}$}   &   &                   % citeseer results
%                                       \cellcolor{gray!15}$77.13{\scriptstyle\pm1.67}$  & $77.05{\scriptstyle\pm1.43}$&  $77.09{\scriptstyle\pm1.62}$&  $76.00{\scriptstyle\pm1.64}$&  $74.97{\scriptstyle\pm1.47}$&  $74.41{\scriptstyle\pm1.65}$
                                
%                               \\ \midrule %\cmidrule{1-1} \cmidrule{3-8} \cmidrule{10-15} 
%                                     %   & \multicolumn{6}{c}{\textbf{Citeseer ($h$=0.74)}}                                                            \\ \hline 
%                                         % \multicolumn{1}{c}{Base}    & \cellcolor{gray!15}$76.51{\scriptstyle\pm1.63}$ & $75.03{\scriptstyle\pm1.67}$ & $73.96{\scriptstyle\pm1.52}$ & $73.59{\scriptstyle\pm1.51}$& $71.91{\scriptstyle\pm1.94}$ & $32.08{\scriptstyle\pm15.74}$                                         \\  
%                                     %   \multicolumn{1}{c}{+deg}    &  \cellcolor{gray!15}$76.63{\scriptstyle\pm1.38}$  & $74.64{\scriptstyle\pm1.97}$&  $74.15{\scriptstyle\pm1.61}$&  $73.73{\scriptstyle\pm1.31}$&  $73.61{\scriptstyle\pm1.84}$&  $70.56{\scriptstyle\pm2.27}$                     \\  
%                                     %   \multicolumn{1}{c}{+sign} &   \cellcolor{gray!15}$77.13{\scriptstyle\pm1.69}$&  $74.56{\scriptstyle\pm2.02}$&   $73.64{\scriptstyle\pm1.65}$&   $72.31{\scriptstyle\pm2.32}$&   $71.98{\scriptstyle\pm3.44}$&   $68.68{\scriptstyle\pm6.72}$                                                                     \\ 
%                             %           \multicolumn{1}{c}{+deg,sign}   & \cellcolor{gray!15}$76.81{\scriptstyle\pm1.71}$ & $74.68{\scriptstyle\pm1.97}$ & $74.69{\scriptstyle\pm2.35}$ &
%                             %   $73.28{\scriptstyle\pm1.45}$ & $71.81{\scriptstyle\pm2.28}$ & $69.91{\scriptstyle\pm3.97}$                                              \\ \hline
% && \multicolumn{6}{c}{\textbf{Cornell ($h$=0.3)}} && \multicolumn{6}{c}{\textbf{Chameleon ($h$=0.23)}}                                                                                                                                                                                                                               \\ %\cline{1-1} 
% \cline{3-8} \cline{10-15} 
%                                       \multicolumn{1}{c}{PN}    && $50.27{\scriptstyle\pm7.17}$ & $53.51{\scriptstyle\pm8.00}$ & $58.38{\scriptstyle\pm5.01}$ &
%                               $58.38{\scriptstyle\pm3.01}$ & \cellcolor{gray!15}$58.92{\scriptstyle\pm3.15}$ & $58.92{\scriptstyle\pm3.15}$          &&
% % Chameleon results
% \cellcolor{gray!15}$62.74{\scriptstyle\pm2.82}$ & $59.01{\scriptstyle\pm2.80}$ & $54.12{\scriptstyle\pm2.24}$ & $46.38{\scriptstyle\pm2.23}$& $46.78{\scriptstyle\pm2.26}$ & $46.27{\scriptstyle\pm3.24}$
% \\  
%                                       \multicolumn{1}{c}{GPRGNN}    && $76.76{\scriptstyle\pm8.22}$ & $77.57{\scriptstyle\pm7.46}$ & $\cellcolor{gray!15}80.27{\scriptstyle\pm8.11}$ &
%                               $78.38{\scriptstyle\pm6.04}$ & $74.59{\scriptstyle\pm7.66}$ & $70.00{\scriptstyle\pm5.73}$    &&
% % Chameleon results
% $\cellcolor{gray!15}46.58{\scriptstyle\pm1.771}$ & $45.72{\scriptstyle\pm3.45}$ & $41.16{\scriptstyle\pm5.79}$ & $39.58{\scriptstyle\pm7.85}$& $35.42{\scriptstyle\pm8.52}$ & $36.38{\scriptstyle\pm2.40}$

% %                                       \\ \hline
% % %\multirow{10}{*}{\rotatebox[origin=c]{90}{\textbf{Heterophily datasets}}} 
% % & \multicolumn{6}{c}{\textbf{Chameleon ($h$=0.23)}}                                                                                                                                                                                                                                       \\  \hline
% %                                       \multicolumn{1}{c}{Base}    & \cellcolor{gray!15}$64.98{\scriptstyle\pm1.84}$ & $62.65{\scriptstyle\pm3.09}$ & $62.43{\scriptstyle\pm3.28}$ & $54.69{\scriptstyle\pm2.58}$& $47.68{\scriptstyle\pm2.63}$ & $29.74{\scriptstyle\pm5.21}$                 \\ 
% %                                       \multicolumn{1}{c}{+deg}    & $66.54{\scriptstyle\pm2.19}$ & $68.31{\scriptstyle\pm2.70}$ & \cellcolor{gray!15}$68.99{\scriptstyle\pm2.38}$ & $67.68{\scriptstyle\pm3.7}$& $56.86{\scriptstyle\pm8.8}$ & $41.95{\scriptstyle\pm9.56}$                                                        \\  
% %                                       \multicolumn{1}{c}{+sign} & \cellcolor{gray!15}$65.31{\scriptstyle\pm3.2}$&  $53.55{\scriptstyle\pm6.35}$& $53.05{\scriptstyle\pm2.28}$&  $51.93{\scriptstyle\pm4.00}$&  $57.17{\scriptstyle\pm3.39}$&  $51.93{\scriptstyle\pm8.95}$                                            \\  
% %                                       \multicolumn{1}{c}{+deg,sign}            &  \cellcolor{gray!15}$65.75{\scriptstyle\pm1.81}$ & $61.49{\scriptstyle\pm7.38}$ & $53.73{\scriptstyle\pm7.79}$ &
% %                               $52.43{\scriptstyle\pm5.37}$ & $55.92{\scriptstyle\pm5.14}$ & $56.95{\scriptstyle\pm3.93}$               
                               
%                               \\ \bottomrule

% \end{tabular}
% }
% \end{adjustbox}
\vspace{-0.5cm}
% \end{table*}
\textcolor{blue}{\subsection{Homophily Metric}
\label{app:evaluation_metric}
In Table~\ref{tab:real-results}, we provide the graph homophily level $h$, which is defined as the average of the nodes' homophily levels. In our theoretical analysis in~\S~\ref{section: analysis}, we use a node's homophily level and relative degree to characterize three cases (Fig.~\ref{fig:concept} and Thm.~\ref{theorem: initial_stage}).
To better align our empirical results with our theoretical analysis, we provide below the proportion of nodes in each case.}

\setlength{\tabcolsep}{4pt}
\begin{table*}[h]%[t!]
    \centering
    \vspace{-0.2cm}
    \caption{%Statistics of real datasets for different homophily levels $h$, 
    The percentage (\%) of nodes in each case (Fig.~\ref{fig:concept} and Thm.~\ref{theorem: initial_stage}): case 1: $h_i\leq \frac{\rho}{1+\rho}$, case 2: $h_i>\frac{\rho}{1+\rho} \ \mathrm{\&}\  \ratioi \leq \frac{1}{(1+\rho)h_i-\rho}$ and case 3: otherwise. The dominant case for each dataset is colored in grey.
    }
    \label{tab:ratios}
    %\resizebox{0.97\textwidth}{!}{
    \vspace{-0.15cm}
    \begin{adjustbox}{width=.9\textwidth}
    % \hskip-1.15cm
    \begin{tabular}{lcccccc  ccc c} % Removed vertical rule due to NIPS requirement
    \toprule
       %\multirow{2}{*}{\backslashbox{\textbf{Models}}{\textbf{Data, h}}} 
       &  \texttt{\bf Texas}           &   \texttt{\bf Wisconsin}           &   \texttt{\bf Actor}            &   \texttt{\bf Squirrel}   &   \texttt{\bf Chameleon} & \texttt{\bf Cornell}        &   \texttt{\bf Citeseer}           &   \texttt{\bf Pubmed}            &   \texttt{\bf Cora} \\
        % & $h=0.11$ & $h=0.21$ & $h=0.22$ & $h=0.22$ & $h=0.23$ & $h=0.3$ & $h=0.57$ & $h=0.74$ & $h=0.8$ & $h=0.81$  \\
        % \midrule 
          \textbf{Hom.\ level} $h$ & \textbf{0.11} & \textbf{0.21} & \textbf{0.22} & \textbf{0.22} & \textbf{0.23} & \textbf{0.3} & \textbf{0.74} & \textbf{0.8} & \textbf{0.81} \\
		\textbf{\#Nodes} & 183 & 251 & 7,600 & 5,201 & 2,277 & 183 & 3,327 & 19,717 & 2,708 \\
		\textbf{\#Edges} & 295 & 466 & 26,752 & 198,493 & 31,421 & 280 & 4,676 & 44,327 & 5,278 \\
		\textbf{\#Classes} & 5 & 5 & 5 & 5 & 5 & 5 & 7 & 3 & 6 \\ 
    \midrule
    % \midrule
       % HistFNN --network_setup M64-R-G-V-MO --hist_nhood 0 1 2
       {Case 1} & \cellcolor{gray!15}$87.43$ & \cellcolor{gray!15}$78.49$ & \cellcolor{gray!15}
       $63.49$ & \cellcolor{gray!15}$47.74$ & \cellcolor{gray!15}$48.48$ &  \cellcolor{gray!15}$79.23$ &  $18.33$ & $14.80$ & $6.50$ \\
       % HistFNN --network_setup M64-R-G-V-G-V-MO --hist_nhood 0 1 2
       {Case 2} & $8.74$ & $15.93$ & $29.53$ & \cellcolor{gray!15}$50.14$ & \cellcolor{gray!15} $48.84$ & $6.01$ &  $25.58$ & $33.75$ & $32.98$ \\
       {Case 3} & $3.83$ & $5.58$ & $6.99$ & $2.11$ & $2.68$ & $14.75$ & \cellcolor{gray!15} $56.09$ & \cellcolor{gray!15}$51.45$ & \cellcolor{gray!15}$60.52$ \\
    %   \textbf{\method-Hist**} \\
    %   \textbf{\method-Avg-1} & $82.70{\scriptstyle \pm 6.52$ & $84.31{\scriptstyle \pm 4.34$ & $34.31{\scriptstyle \pm 1.31$ & $28.98{\scriptstyle \pm 1.97$ & $50.88{\scriptstyle \pm 1.78$ \\
    %   % HistFNN --network_setup M64-R-G-V-G-V-MO --hist_nhood 0 1 2
    %   \textbf{\method-Avg-2} &$80.54{\scriptstyle \pm 6.84$ & $83.14{\scriptstyle \pm 4.26$ & $34.49{\scriptstyle \pm 1.63$ & $31.83{\scriptstyle \pm 2.25$ & $56.47{\scriptstyle \pm 1.58$ \\
	   \bottomrule
    \end{tabular}
    \end{adjustbox}
    %}  
    \vspace{-0.3cm}
\end{table*}
\textcolor{blue}{We observe that a low graph homophily level indicates that case 1 is the dominant case, while a high graph homophily level indicates that case 3 is the dominant case. As we stated in Thm~\ref{theorem: initial_stage}, under "non-swapping" condition, case 3 is the only case to have a benefit. Thus, in the commonly-used homophilous datasets (Citeseer, Pubmed and Cora), case 3 dominates and enjoys the benefits from graph convolution. In the Texas, Wisconsin and Actor datasets, only case 1 dominates and case 1 hurts the performance most, this explains why GCN performs worse than most methods in Table~\ref{tab:real-results}. In the Squirrel and Chameleon datasets, both case 1 and case 2 dominate, GCN yields acceptable results. Using portions of the three cases to analyze the datasets is a better metric, because it aligns more with the GCN's performance. As shown by Table~\ref{tab:ratios}, Wisconsin, Actor, Squirrel and Chameleon have very close graph level homophily, but GCN's performance are quite different as shown in Table \ref{tab:real-results}. Our way to define homophily level does predict that GCN should perform decently in Squirrel and Chameleon datasets.}

\textcolor{blue}{
\subsection{Complexity analysis}
We first analyze the time complexity of the forward path \method. For degree correction, we need to compute the $r_{ij}$. However, we do not need to compute all of them, and we only need to compute $r_{ij}$ for node pairs who are linked. The time complexity is $O(|\gE|)$, but it is a one-time computation, the results of which can be saved. We compute $\tau_{ij}^{l}$ based on the learned weights $\lambda_0^l, \lambda_1^{l}$. The time complexity is $O(|\gE| \cdot L)$, where $L$ is the number of layers. The time complexity to compute the signed function is $O(|\gE| \cdot H \cdot L)$, where $H$ is the hidden dimension of representations, and we only compute the cosine similarity between the nodes that are linked. We also need to compute the multiplication of the propagation matrix and representation matrices. The time complexity is $O(|\gV|^2 \cdot H \cdot L)$, . Similarly, the time complexity of the multiplication of representation matrices and the weight matrices is $O(|\gV|\cdot H^2 \cdot L)$. The total time complexity would be $O(\text{max}(|\gV|^2, |\gE|)\cdot H \cdot L)$.
The complexity of \method resembles the complexity of attention-based model. Thus we compare with GAT~\citep{velivckovic2017graph} the total time to train and test on 4 larger homophilous and heterophilous datasets. We run the training and testing for 10 times.
}

\setlength{\tabcolsep}{4pt}
\begin{table*}[h]%[t!]
    \centering
    \vspace{-0.2cm}
    \caption{%Statistics of real datasets for different homophily levels $h$, 
    Training and test time (m:minutes, s:seconds) for 10 runs. Shorter time is colored in grey.
    }
    \label{tab:scalability}
    %\resizebox{0.97\textwidth}{!}{
    \vspace{-0.15cm}
    \begin{adjustbox}{width=.6\textwidth}
    % \hskip-1.15cm
    \begin{tabular}{lcccc} % Removed vertical rule due to NIPS requirement
    \toprule
       %\multirow{2}{*}{\backslashbox{\textbf{Models}}{\textbf{Data, h}}} 
       &     \texttt{\bf Actor}            &      \texttt{\bf Chameleon} &   \texttt{\bf Citeseer}                       &   \texttt{\bf Cora} \\
        % & $h=0.11$ & $h=0.21$ & $h=0.22$ & $h=0.22$ & $h=0.23$ & $h=0.3$ & $h=0.57$ & $h=0.74$ & $h=0.8$ & $h=0.81$  \\
        % \midrule 
		\textbf{\#Nodes} &  7,600 &  2,277 &  3,327  & 2,708 \\
		\textbf{\#Edges} &  26,752 &  31,421 &  4,676  & 5,278 \\
    \midrule
    % \midrule
       % HistFNN --network_setup M64-R-G-V-MO --hist_nhood 0 1 2
       {\method} & \cellcolor{gray!15}$7m24s$ & \cellcolor{gray!15}$2m29s$ & \cellcolor{gray!15}
       $2m9s$ & $5m47s$  \\
       % HistFNN --network_setup M64-R-G-V-G-V-MO --hist_nhood 0 1 2
       {GAT} & $8m14s$ & $7m34s$ & $9m39s$ & \cellcolor{gray!15}$4m11s$  \\
       
    %   \textbf{\method-Hist**} \\
    %   \textbf{\method-Avg-1} & $82.70{\scriptstyle \pm 6.52$ & $84.31{\scriptstyle \pm 4.34$ & $34.31{\scriptstyle \pm 1.31$ & $28.98{\scriptstyle \pm 1.97$ & $50.88{\scriptstyle \pm 1.78$ \\
    %   % HistFNN --network_setup M64-R-G-V-G-V-MO --hist_nhood 0 1 2
    %   \textbf{\method-Avg-2} &$80.54{\scriptstyle \pm 6.84$ & $83.14{\scriptstyle \pm 4.26$ & $34.49{\scriptstyle \pm 1.63$ & $31.83{\scriptstyle \pm 2.25$ & $56.47{\scriptstyle \pm 1.58$ \\
	   \bottomrule
    \end{tabular}
    \end{adjustbox}
    %}  
    \vspace{-0.3cm}
\end{table*}
In general, \method runs faster than GAT because degree correction and signed messages in \method learn fewer parameters.
\section{Hyperparameters and Parameters}
\label{app:hyperparameter}
\subsection{Hyperparameter settings}
\textbf{Experiments for Table~\ref{tab:real-results} \& Table~\ref{tab:oversmoothing}}

For the baselines, we set the same hyperparameters that are provided by the original papers or the authors’ github repositories, and we match the results they reported in their respective papers. In our experiments, we find that the original hyperparameters set by the authors are already well-tuned. 

All the models use Adam as the optimizer. GAT sets the initial learning rate as 0.005 and Geom-GCN uses a custom learning scheduler. All the other models (include \method) use the initial learning rate 0.01.

For \method, we use the following hyperparameters:
\begin{itemize}
    \item $k$ in the decaying aggregation: 3
\end{itemize}

We tune the parameters in the following ranges:
\begin{itemize}
    \item Dropout rate:  [0.0, 0.7]
    \item Weight decay:  [1e-7, 1e-2]
    \item Hidden units: \{8, 16, 32, 64, 80\}
    \item Decay rate $\eta$: [0.0, 1.5]
\end{itemize}

\textbf{Experiments for Table~\ref{tab:ablation} and Table~\ref{tab:bn_ln}}

The hyperparameters that are used in all the models (Base, \texttt{+deg}, \texttt{+sign}, \texttt{+deg,sign}, \texttt{+BN}, \texttt{+LN}) are set to be the same and they are tuned for every dataset. Those common hyperparameters are:
\begin{itemize}
    \item Dropout rate: [0.0, 0.7]
    \item Weight decay: [1e-7, 1e-2]
    \item Hidden units: \{8, 16, 32, 64, 80\}
\end{itemize}
% For models that use signed messages, we tune the following hyperparameter:
% \begin{itemize}
%     \item Initialization of $\alpha^l$: [0.2, 1.0] (same in every layer)
% \end{itemize}
% For models that use degree correction, we tune the following hyperparameter:
% \begin{itemize}
%     \item Initialization of $\lambda_0^l$: [0.2, 1.5] (same in every layer)
% \end{itemize}
\subsection{Initialization of parameters}
\textbf{Initialization}

For \method, we adopt the following parameter initialization in the experiments for Table~\ref{tab:real-results} \& Table~\ref{tab:oversmoothing}
\begin{itemize}
    \item Initialization of $\lambda_0^l$ and $\lambda_1^l$: 0.5 and 0, respectively
    \item Initialization of $\alpha^l$, $\beta_0^l$, $\beta_1^l$ and $\beta_2^l$: 2, 0, 0, 0, respectively.
\end{itemize}
We initialize %$\beta_0^l$, 
{\small $\beta_{\{0,1,2\}}^l=0$} %and $\beta_2^l$ 
in Eq.\ (6) because, after applying softmax, 
{\small $\hat{\beta}^l_{\{0,1,2\}}=1/3$}; 
%$\hat{\beta_0^l}$, $\hat{\beta_1^l}$ and $\hat{\beta_2^l}$ 
%will all be 1/3, %$\frac{1}{3}$, 
this ensures \ul{equal contributions} from positive and negative neighbors and themselves (and sum=1).
% so that the contributions from positive and negative neighbors and themselves will be equal (sum=1). 
We initialize $\lambda_1^l=0$ in Eq.\ (9) following the common practice for initializing the bias. 
We set $\alpha^l=2$ and $\lambda_0^l=0.5$ in Eq.\ (6) and Eq.\ (9), because when $r_{ij} \to +\infty$, the degree correction (including global scaling) is: {\small $\hat{\alpha^l}\tau_{ij}^l=\text{softplus}(2) \cdot \text{softplus}(0.5 \cdot (0-1) + 0) \approx 1$}. As we mention in Thm. 1, when the homophily level is high, nodes with large $\overline{r_i}$ may benefit (case 3), thus we \ul{do not want to compensate for these nodes and would like to keep {\small $\hat{\alpha^l}\tau_{ij}^l$} close to 1}. 
\subsection{Parameters after training}
\begin{wrapfigure}{r}{0.5\textwidth}
  \begin{center}
    %\vspace{-0.8cm}
    \includegraphics[scale=0.06,bb=3000 1000 380 180]{Figs/hyp1.png}
  \end{center}
  \vspace{1.8cm}
  \caption{Original $\overline{r_{ij}}$ (avg. $r_{ij}$) %$\overline{r_{ij}}$ 
  and corrected (pre- and post-training).} %before and after the training.}
  \label{fig:parameters}
\end{wrapfigure}
Figure~\ref{fig:parameters} shows the original and corrected $\overline{r_{ij}}$ (avg $r_{ij}$). Corrected $r_{ij}$ are given by {\small $\hat{\alpha^l}\tau_{ij}^lr_{ij}$}, which are a combination of global scaling and local degree correction. Because {\small $\beta_{\{0,1,2\}}^l$} sum to 1 and do not change global scaling, they are not considered in the corrected $r_{ij}$.
As can be seen in Fig.~\ref{fig:parameters}, after the training, \ul{GGCN learns to increase $r_{ij}$}, which satisfies our theorems. 


\section{Table 2 with larger fonts}
\label{app:table 2}
\begin{sidewaystable}[h]
\centering
\caption{Model performance for different layers: mean accuracy $\pm$ stdev over different data splits. Per dataset and GNN model, we also report the layer at which the best performance (given in Table~\ref{tab:real-results}) is achieved. `OOM': out of memory; `INS': numerical instability. }
\label{app-tab:table 2}
\begin{adjustbox}{width=1\linewidth}
{\footnotesize
\begin{tabular}{r c ccccccccccccccc}
\toprule
                                         %\multirow{2}{*}{\backslashbox{\textbf{Model}}{\textbf{Layers}}}    
                                      \textbf{Layers} 
                                      && \textbf{2}           & \multicolumn{1}{c}{\textbf{4}} & \multicolumn{1}{c}{\textbf{8}} & \multicolumn{1}{c}{\textbf{16}} & \multicolumn{1}{c}{\textbf{32}} & \multicolumn{1}{c}{\textbf{64}} &
                                      \multicolumn{1}{c}{\textbf{Best}}
                                      &&  \multicolumn{1}{c}{\textbf{2}}           & \multicolumn{1}{c}{\textbf{4}} & \multicolumn{1}{c}{\textbf{8}} & \multicolumn{1}{c}{\textbf{16}} & \multicolumn{1}{c}{\textbf{32}} & \multicolumn{1}{c}{\textbf{64}}  &
                                      \multicolumn{1}{c}{\textbf{Best}} \\ \cmidrule{1-1} \cmidrule{3-9} \cmidrule{11-17} %cline{2-8}
%\multirow{10}{*}{\rotatebox[origin=c]{90}{\textbf{Homophily datasets}}}   
%\textbf{Model} 
&& \multicolumn{7}{c}{\textbf{Cora} ($h$=0.81)}     & & \multicolumn{7}{c}{\textbf{Citeseer} ($h$=0.74)}                                                                         \\ %\cline{1-1} 
\cline{3-9} \cline{11-17}
                                    
                                        \multicolumn{1}{l}{GGCN (\textbf{ours})}    &&   
                                        %cora results
                                        $87.00{\scriptstyle\pm1.15}$         & {$ 87.48{\scriptstyle\pm1.32}$}           & {$ 87.63{\scriptstyle\pm1.33}$}           & {$ 87.51{\scriptstyle\pm1.19}$}            & 
                                        {$ 87.95{\scriptstyle\pm1.05}$}            & {$ 87.28{\scriptstyle\pm1.41}$}            & 
                                        32
                                           & &  
                                        % citeseer results
                                        $76.83{\scriptstyle\pm1.82}$ & $76.77{\scriptstyle\pm1.48}$ & $76.91{\scriptstyle\pm1.56}$ & $76.88{\scriptstyle\pm1.56}$& $76.97{\scriptstyle\pm1.52}$ & $76.65{\scriptstyle\pm1.38}$ & 
                                        10 \\ 
                                        
                            \multicolumn{1}{l}{GPRGNN}    &&  
                                      %cora results
                                      \multicolumn{1}{c}{$87.93{\scriptstyle\pm1.11}$}      &        $87.95{\scriptstyle\pm1.18}$           & \multicolumn{1}{c}{$87.87{\scriptstyle\pm1.41}$}           & \multicolumn{1}{c}{$87.26{\scriptstyle\pm1.51}$}            & \multicolumn{1}{c}{$87.18{\scriptstyle\pm1.29}$}            & \multicolumn{1}{c}{$87.32{\scriptstyle\pm1.21}$} & 4 &   &                   % citeseer results
                                      $77.13{\scriptstyle\pm1.67}$  & $77.05{\scriptstyle\pm1.43}$&  $77.09{\scriptstyle\pm1.62}$&  $76.00{\scriptstyle\pm1.64}$&  $74.97{\scriptstyle\pm1.47}$&  $74.41{\scriptstyle\pm1.65}$
                            & 2
                            \\
                            \multicolumn{1}{l}{H2GCN*} &&  
                                      %cora results
                                      $87.87{\scriptstyle\pm1.20}$  &   $86.10{\scriptstyle\pm1.51}$&   $86.18{\scriptstyle\pm2.10}$&    OOM                    &       OOM                     &      OOM                      &     2
                                      & &    
                                     % citeseer results
                                    $76.90{\scriptstyle\pm1.80}$  & 
                                      $76.09{\scriptstyle\pm1.54}$  & 
                                      $74.10{\scriptstyle\pm1.83}$  &  
                                      OOM     &  
                                      OOM     &  
                                      OOM     &     1
                                      
                        \\      
                                     \multicolumn{1}{l}{GCNII*}    &&  
                                      %cora results
                                      $85.35{\scriptstyle\pm1.56}$                & {$85.35{\scriptstyle\pm1.48}$}           & {$86.38{\scriptstyle\pm0.98}$}           & {$87.12{\scriptstyle\pm1.11}$}            & {$87.95{\scriptstyle\pm1.23}$}            & {$88.37{\scriptstyle\pm1.25}$}      &       
                                      64  & &
                                      % citeseer results
                                      $75.42{\scriptstyle\pm1.78}$  & $75.29{\scriptstyle\pm1.90}$&  $76.00{\scriptstyle\pm1.66}$&  $76.96{\scriptstyle\pm1.38}$&  $77.33{\scriptstyle\pm1.48}$&  $77.18{\scriptstyle\pm1.47}$ & 32
                                      \\  
                                      
                        \multicolumn{1}{l}{PairNorm}    &&   
                                        %cora results
                                        $ 85.79{\scriptstyle\pm1.01}$         & \multicolumn{1}{c}{$ 85.07{\scriptstyle\pm0.91}$}    &        \multicolumn{1}{c}{$ 84.65{\scriptstyle\pm1.09}$}     &       \multicolumn{1}{c}{$ 82.21{\scriptstyle\pm2.84}$}      &     \multicolumn{1}{c}{$ 60.32{\scriptstyle\pm8.28}$}       &    \multicolumn{1}{c}{$ 44.39{\scriptstyle\pm5.60}$}   & 2 & & 
                                        % citeseer results
                                        $73.59{\scriptstyle\pm1.47}$ & $72.62{\scriptstyle\pm1.97}$ & $72.32{\scriptstyle\pm1.58}$ & $59.71{\scriptstyle\pm15.97}$& $27.21{\scriptstyle\pm10.95}$ & $23.82{\scriptstyle\pm6.64}$ & 2                                        \\               
                        \multicolumn{1}{l}{Geom-GCN*} &&
                         % cora results
                          $85.35{\scriptstyle\pm1.57}$&   $21.01{\scriptstyle\pm2.61}$&   $13.98{\scriptstyle\pm1.48}$&   $13.98{\scriptstyle\pm1.48}$&   $13.98{\scriptstyle\pm1.48}$&   $13.98{\scriptstyle\pm1.48}$&   
                          2
                         &  & 
                        % citeseer results 
                         $78.02{\scriptstyle\pm1.15}$&  $23.01{\scriptstyle\pm1.95}$&   $7.23{\scriptstyle\pm0.87}$&   $7.23{\scriptstyle\pm0.87}$&   $7.23{\scriptstyle\pm0.87}$&   $7.23{\scriptstyle\pm0.87}$
                         &   2 
                         \\ 
                        \multicolumn{1}{l}{GCN} &&
                         % cora results
                        $86.98{\scriptstyle\pm1.27}$ & $83.24{\scriptstyle\pm1.56}$ & $31.03{\scriptstyle\pm3.08}$ &
                        $31.05{\scriptstyle\pm2.36}$ & $30.76{\scriptstyle\pm3.43}$ & $31.89{\scriptstyle\pm2.08}$ & 2
                         &  & 
                        % citeseer results 
                        $76.50{\scriptstyle\pm1.36}$ & $64.33{\scriptstyle\pm8.27}$ & $24.18{\scriptstyle\pm1.71}$ &
                               $23.07{\scriptstyle\pm2.95}$ & $25.3{\scriptstyle\pm1.77}$ & $24.73{\scriptstyle\pm1.66}$ & 2  
                         \\              
                        
                         \multicolumn{1}{l}{GAT} &&
                         % cora results
                         $87.30{\scriptstyle\pm1.10}$ & $86.50{\scriptstyle\pm1.20}$ & $84.97{\scriptstyle\pm1.24}$ &
                              INS  & INS & INS & 2
                         &  & 
                        % citeseer results 
                        $76.55{\scriptstyle\pm1.23}$ &$75.33{\scriptstyle\pm1.39}$&    $66.57{\scriptstyle\pm5.08}$         &    INS                             &    INS                             &       INS                          & 2  
                         \\
                         
                         \midrule 
&& \multicolumn{7}{c}{\textbf{Cornell ($h$=0.3)}} && \multicolumn{7}{c}{\textbf{Chameleon ($h$=0.23)}}                                                                         \\ %\cline{1-1} 
\cline{3-9} \cline{11-17}
                                    
                        \multicolumn{1}{l}{GGCN (\textbf{ours})}    &&   
                        %cornell results
                        $83.78{\scriptstyle\pm6.73}$ & $83.78{\scriptstyle\pm6.16}$ & $84.86{\scriptstyle\pm5.69}$ &
                        $83.78{\scriptstyle\pm6.73}$ & 
                        $83.78{\scriptstyle\pm6.51}$ & 
                        $84.32{\scriptstyle\pm5.90}$ & 
                               6
                        & &  
                        % Chameleon results
                        $70.77{\scriptstyle\pm1.42}$ & $69.58{\scriptstyle\pm2.68}$ & $70.33{\scriptstyle\pm1.70}$ & $70.44{\scriptstyle\pm1.82}$& $70.29{\scriptstyle\pm1.62}$ & $70.20{\scriptstyle\pm1.95}$ & 
                        5                
                        \\ 
            \multicolumn{1}{l}{GPRGNN}    && $76.76{\scriptstyle\pm8.22}$ & $77.57{\scriptstyle\pm7.46}$ & $80.27{\scriptstyle\pm8.11}$ &
                              $78.38{\scriptstyle\pm6.04}$ & $74.59{\scriptstyle\pm7.66}$ & $70.00{\scriptstyle\pm5.73}$    & 8 & &
% Chameleon results
$46.58{\scriptstyle\pm1.771}$ & $45.72{\scriptstyle\pm3.45}$ & $41.16{\scriptstyle\pm5.79}$ & $39.58{\scriptstyle\pm7.85}$& $35.42{\scriptstyle\pm8.52}$ & $36.38{\scriptstyle\pm2.40}$ & 2
            \\
            \multicolumn{1}{l}{H2GCN*} &&  
                        %cornell results
                        $81.89{\scriptstyle\pm5.98}$ & $82.70{\scriptstyle\pm6.27}$ & $80.27{\scriptstyle\pm6.63}$ &
                               OOM & OOM & OOM & 1  
                        & &    
                        % Chameleon results
                        $59.06{\scriptstyle\pm1.85}$ & $60.11{\scriptstyle\pm2.15}$ & OOM &                          OOM &                          OOM &                          OOM &                          4            
                        \\  
            
                        \multicolumn{1}{l}{GCNII*} && 
                        %cornell results
                        $67.57{\scriptstyle\pm11.34}$ & $64.59{\scriptstyle\pm9.63}$ & $73.24{\scriptstyle\pm5.91}$ &
                               $77.84{\scriptstyle\pm3.97}$ & $75.41{\scriptstyle\pm5.47}$ & $73.78{\scriptstyle\pm4.37}$ & 16   
                        & &
                        % Chameleon results
                        $61.07{\scriptstyle\pm4.10}$ & $63.86{\scriptstyle\pm3.04}$ & $62.89{\scriptstyle\pm1.18}$ & $60.20{\scriptstyle\pm2.10}$& $56.97{\scriptstyle\pm1.81}$ & $55.99{\scriptstyle\pm2.27}$ & 4  
                        \\ 
                        \multicolumn{1}{l}{PairNorm}    && $50.27{\scriptstyle\pm7.17}$ & $53.51{\scriptstyle\pm8.00}$ & $58.38{\scriptstyle\pm5.01}$ &
                              $58.38{\scriptstyle\pm3.01}$ & $58.92{\scriptstyle\pm3.15}$ & $58.92{\scriptstyle\pm3.15}$          & 32 & &
% Chameleon results
$62.74{\scriptstyle\pm2.82}$ & $59.01{\scriptstyle\pm2.80}$ & $54.12{\scriptstyle\pm2.24}$ & $46.38{\scriptstyle\pm2.23}$& $46.78{\scriptstyle\pm2.26}$ & $46.27{\scriptstyle\pm3.24}$ & 2
\\  
                        
                        \multicolumn{1}{l}{Geom-GCN*} &&
                         % cornell results
                        $60.54{\scriptstyle\pm3.67}$&  $23.78{\scriptstyle\pm11.64}$& $12.97{\scriptstyle\pm2.91}$&  $12.97{\scriptstyle\pm2.91}$&  $12.97{\scriptstyle\pm2.91}$&  $12.97{\scriptstyle\pm2.91}$&  
                        2  
                         &  & 
                        % Chameleon results 
                        $60.00{\scriptstyle\pm2.81}$&  $19.17{\scriptstyle\pm1.66}$& $19.58{\scriptstyle\pm1.73}$&  $19.58{\scriptstyle\pm1.73}$&  $19.58{\scriptstyle\pm1.73}$&  $19.58{\scriptstyle\pm1.73}$
                        &  2 
                        \\
                         \multicolumn{1}{l}{GCN} &&
                         % cornell results
                        $60.54{\scriptstyle\pm5.30}$ & $59.19{\scriptstyle\pm3.30}$ & $58.92{\scriptstyle\pm3.15}$ &
                        $58.92{\scriptstyle\pm3.15}$ & 
                        $58.92{\scriptstyle\pm3.15}$ & 
                        $58.92{\scriptstyle\pm3.15}$ & 2
                               &  & 
                        % Chameleon results 
                        $64.82{\scriptstyle\pm2.24}$ & $53.11{\scriptstyle\pm4.44}$ & $35.15{\scriptstyle\pm3.14}$ &
                               $35.39{\scriptstyle\pm3.23}$ & $35.20{\scriptstyle\pm3.25}$ & $35.50{\scriptstyle\pm3.08}$ & 2 
                         \\ 
                         \multicolumn{1}{l}{GAT} &&
                         % cornell results
                        $61.89{\scriptstyle\pm5.05}$ &      $58.38{\scriptstyle\pm4.05}$ &     $58.38{\scriptstyle\pm3.86}$                           
                        &   INS                    
                        &   INS                         
                        &   INS &  
                        2 
                         &  & 
                        % Chameleon results 
                        $60.26{\scriptstyle\pm2.50}$ &   $48.71{\scriptstyle\pm2.96}$                             &  $35.09{\scriptstyle\pm3.55}$                              &      INS                           &    INS                             &   INS                              &  2 
                         
                        \\ \bottomrule
\end{tabular}
}
\end{adjustbox}
\end{sidewaystable}


==> sections/theoretic_analysis.tex <==
\vspace{-0.3cm}
\section{Theoretical Analysis}
\label{section: analysis}
\vspace{-0.3cm}
% In this section, we analyze the theoretical connections between \yy{oversmoothing and heterophily problems in node classification tasks. Both problems result in degenerated GCNs'performance. We find that the movements of node representations reflect the chances of nodes to be misclassified and are a good indicator of GCNs' performance.
% Thus, we characterize in expectation how node representations move and change over the layers and use the movements of representations to explain the oversmoothing and heterophily problems. }
% {At a high level, we focus on the node classification task and we use the \textit{linear separability} of learned node representations as an indicator of GCN performance. Intuitively, linear separability is the smallest distance between node representations of opposite classes. 
% By studying the movements of node representations after propagation and aggregation in GCNs, we characterize how linear separability 
% is changed over the layers.
% We identify two causes, i.e., the level of homophily of a node and the relative degree between a node and its neighbors, which  
% \yy{determine the movements of node representations. Specifically, moving towards (away from) another class leads to higher (lower) misclassification rate and worse (better) classification performance if the movements do not swap the positions of the two classes.}
%a limited portion of nodes are allowed to cross the decision boundary.}
% the linear separability of learned representations. Specifically, the two causes determine if the node representations will tend to move towards the initial mean feature vector of the opposing class (becoming less linearly separable) or away (becoming more linearly separable). 
% Our analysis highlights that \yy{the oversmoothing and heterophily problems result from a limited portion of nodes move towards another class induced by high heterophily level and low relative degree.}

{In this section, we formalize the connection} between the oversmoothing and heterophily problems in two steps: (1) We show how the movements of node representations relate to the misclassification rate of node labels; and  (2) we identify the factors that affect the movements of representations.
{We use the SGC model to analyze binary node classification with nodes in class 1 denoted as set $\gV_{1}$ and nodes in class 2 denoted as set $\gV_{2}$. We show empirically (\S~\ref{section: experiments}) that the insights obtained in this section are effective for other non-linear models in multi-class classification. %We denote the nodes in class 1 as $\gV_{1}$ and the remaining nodes as $\gV_{2}$. 
}
%  \reminder{define $\rho$ where it comes up -- We define the size ratio $\rho$ as: $\rho\equiv\frac{|\gV_{1}|}{|\gV_{2}|}.$}


% \yaoqing{At this stage, I think the readers will be completely confused by what you are trying to say. We can probably move the last sentence after our analysis and put that as a remark.}
% both the oversmoothing problem and the heterophily problem result from \textit{less linear separability} induced by these two causes.
%Moreover, we show that signed messages help reduce the effect from the factors.


%Our analysis highlights that both the oversmoothing problem and the heterophily problem result from \textit{less linear separability} of learned representations for nodes in different classes after graph convolution.
%we analyze the impact of message propagation in the node classification task, and show how the oversmoothing  and heterophily problems are related. We also discuss the implications of our analysis, which provide valuable insights for designing our model, \method, in \S~\ref{section: model_design}. %\yy{Move using linear GCN layers to settings.}


%\subsection{Settings \& Definitions}
% \label{subsec: notations}

% We consider a binary node classification task on an unweighted self-loop-free graph with adjacency matrix $\rmA$. 
% We denote the set of nodes in the first class and the second class as $\gV_1$ and $\gV_2$, respectively.

% \yaoqing{A general comment. I think we are confusing ourselves with definitions and assumptions. There are a lot of definitions below which belong to the notation section. The assumptions, such as E(f)=0, should be separated from these.}
\vspace{-0.3cm}
\subsection{Assumptions} 
\vspace{-0.3cm}
% In 
% %$|\gL|$ balanced classes (same number of nodes in each class) in a node classification task. 
% a multi-class node classification task,
% we assume: 
{(1) Graph generation process: (1.1) Node labels $\{y_i\}$ and degrees $\{d_i\}$ are deterministic. (1.2) Node connections are randomly determined: an arbitrary node $v_i$  connects to $k_i$ neighbors randomly chosen from the same class and $(d_i-k_i)$ neighbors randomly chosen from other classes, where $k_i$ follows the discrete uniform distribution of range $[0, \text{min}(d_i, |\gV_{y_i}|)]$. $\{(\cdot)_i\}$ represents a set with $i=1, \dots, |\gV|$.}
% \yaoqing{Is there an inherent assumption that the number of nodes in each class is larger than $d_i$? Otherwise, what if one node does not have enough nodes from a class to connect?}
% (1.3) Node features of the same (different) class are drawn from the same (different) distribution(s). \yaoqing{Shall we define these distributions here?} 

{
(2) Input node features: (2.1) Input node features from the same class are drawn from the same distribution. We denote the probability density function (PDF) of class $i$ as $f_{i}({\rvx}).$
(2.2) Input node features are centered, i.e., $\E(\sum_i{\rvf_i^{(0)}})=\mathbf{0}.$ For SGC~\citep{wu2019simplifying}, no matter whether the input features are centered or not, the optimal learned parameters $\rmW^{(L)}$ will be the same. Only $\rvb^{(L)}$ will differ by a vector $\tilde{\rmA}^{L}\E(\sum{\rvf_i^{(0)}})\rmW^{(L)}.$ Thus, this assumption eases our demonstration without affecting the misclassification rate. %We define $\rvmu$ as the mean of distribution $f_{1}(\rvx)$.
Based on assumption (2.2), if $\rvmu$ is the mean of distribution $f_{1}(\rvx)$, the mean of distribution $f_2(\rvx)$ is $-\rho\rvmu,$ where $\rho$ is the size ratio defined as: $\rho\equiv\frac{|\gV_{1}|}{|\gV_{2}|}.$}
% \yaoqing{Shall we give some motivations on why these features are centered?}
% (1) The initial features are centered, i.e., $\sum{\rvf_i^0}=\mathbf{0}$; (2) Given an arbitrary node $v_i$, for any node $v_j$ s.t. $y_i\neq y_j$, the probability of connecting to $v_i$ is equal; (3) 
% (3) Following prior work~\citep{li2018deeper, oono2019graph, chen2020simple}, \yy{we analyze SGC~\citep{wu2019simplifying}} but show empirically that our results still apply to non-linearized GCNs (\S~\ref{section: experiments}). \textbf{Simplifications.} We analyze the dynamics of $\rvf_i$ in each class in a one-vs-rest fashion. \yaoqing{Shall we clarify? I don't think the readers will understand what it means by the dynamics of xxx and "one-vs-rest fashion".}
% Without loss of generality, we choose class 1 as the target class and assume $\rvf_i^0$ of class 1 follows \yy{a distribution with a probability density function (PDF) $f_1(\rvx)$ and mean $\rvmu$}. Given \yy{assumption 1.2}, $\rvf_i^0$ in the other classes can be viewed as drawing from a virtual class (`rest'). \yaoqing{What does this mean? Is this related to the so called "one-vs-rest fashion"? If what you mean is that you want to study binary classification, you probably want to just say that you study binary classification, because one-vs-rest is not the same as binary classification. If you are indeed able to study multi-class classification, you can define class 1 and the rest as $C_1$ and $\bar C_1$.}
% We denote the set of nodes in the first and the virtual class \yaoqing{Also, avoid using a word that you are not familiar with. If this word is not something written in a text book and you invented it, ML people will think this is not appropriate.} as $\gV_1$ and $\gV_2$. \yy{Given assumption (2)}, the virtual class follows a distribution with \yy{a PDF $f_2(\rvx)$ and} mean $-\rho\rvmu$, $\rho=\frac{|\gV_1|}{|\gV_2|}$. Usually, $0<\rho\leq 1$.\yaoqing{What does "usually" mean?} Thus, the analysis reduces to analyzing two classes.}
\vspace{-0.3cm}
\subsection{{{Misclassification Rate \& Movements of Node Representations}}} 
\vspace{-0.2cm}
{The following lemmas illustrate why the movements of node representations are a good indicator of SGC's performance. An $L$-layer SGC applies logistic regression to the $L$-th layer node representations $\{\rvf_i^{(L)}\}$, 
% An $L$-layer SGC applies logistic regression to the $L$-th layer representations, $\rvf_i^{(L)}$, of an arbitrary node $i$, 
so we can study its misclassification rate through the decision boundaries of $\{\rvf_i^{(L)}\}$. We view the changes of node representations across different layers as their movements in the latent space. Thus, the decision boundary of an $(L+1)$-layer SGC can be viewed as a perturbation to the decision boundary of an $L$-layer SGC due to the movements of node representations.}
% The decision boundary of an $L$-th layer SGC
% Proofs are in App.~\ref{app:lemma_1} and \ref{app:lemma_2}}.
% \yy{SGC can be viewed as applying logistic regression to the last layer features $\rvf_i^{(L)}$, so we have:}

\vspace{-0.1cm}
{\textbf{Lemma 1} In SGC, the decision boundaries w.r.t. $\{\rvf_i^{(L)}\}$ in multi-class classification are linear hyperplanes.}
\vspace{-0.4cm}
\begin{proof}
We provide the proof in App.~\ref{app:lemma_1}.
\end{proof}
\vspace{-0.4cm}
% \yaoqing{I am completely confused. I think we now have a lemma before we even defined the things in it. What does "movement" mean? What is a decision boundary? What does it mean to have a linear decision boundary? Also, avoid using things like "SGC can be viewed as applying logistic regression". People won't understand what you mean.}

% \yy{\textbf{Definition} The misclassification rate of a node set $\gV$ is: $\E(\hat{\chi}(v_i) \neq y_i)$, $v_i \in \gV$. }

% \yaoqing{What is the expectation over? The randomness in the random attachment model? The noise in SGD? The initialization of model weights? Or all of them?}

% \yy{Denote the hyperplane $\rvx\rvw+b=0$ as the decision boundary of the $\rvf_i^{l}$ that separates the nodes from the target class (predicted as the target class if $\rvx\rvw+b>0$) and the 'rest' class.
% \yaoqing{Is the following paragraph a proof?}
{Due to Lemma 1, for binary classification, we can use the hyperplane $\rvx\rvw+b=0$ to represent the decision boundary of $\{\rvf_i^{(L)}\}$, 
% that separates the nodes from class 1 and class 2, 
% \yaoqing{Do you mean "the decision boundary in the space of $\rvf_i^{l}$"? I think it is better to define the space.} 
where $\rvw$ is a unit vector, $b$ is a scalar, and the $\{\rvf_i^{(L)}\}$ are classified to class 1 if $\rvf_i^{(L)}\rvw+b>0$.
% The misclassification rate for the target class ('rest' class) is: $\int_{\rvw^T\rvx+\rvb<\mathbf{0}}{f_1(\rvx)d\rvx}$ ($\int_{\rvw^T\rvx+\rvb>\mathbf{0}}{f_2(\rvx)d\rvx}$). 
Suppose when $\rvw=\rvw^*$ and $b=b^*$, we find an optimal hyperplane $\rvx{\rvw^*}+b^*=0$ that achieves the lowest total misclassification rate (\S~\ref{section: background}) for $\{\rvf_i^{(L)}\}$. Due to the movements of node representations, the optimal hyperplane of $(L+1)$-th layer becomes: $\rvx{\rvw^*}'+{b^*}'=0$.
% $\int_{\rvw^T\rvx+\rvb<\mathbf{0}}{f_1(\rvx)d\rvx}+\int_{\rvw^T\rvx+\rvb>\mathbf{0}}{f_2(\rvx)d\rvx}$. 
% The next layer representations $\rvf_i^{l+1}$ can be viewed as being moved from $\rvf_i^{l}$. \yaoqing{One thing that confuses is me is that I thought $\rvf_i^{l}$ is a random variable. However, what you mentioned here and in the following sounds like it is a fixed vector. Also, is w* fixed? If so, it is important to state at the beginning.} Due to the movements, the optimal $\rvw^*$ and $b^*$ become ${\rvw^*}'$ and ${b^*}'$. \yaoqing{I believe you are just defining new terms. If so, say that we denote the new optimal weights and bias as xxx, instead of saying that they become xxx.} 
In Lemma 2, we show that, \ul{under constraints, moving towards the original decision boundary results in a non-decreasing total misclassification rate under the new decision boundary.}}

{\textbf{Lemma 2} Moving representations $\{\rvf_i^{(L)}\}$ from class 1 by adding $-t{\rvw^*}^T$, $t>0$, s.t. ${\rvw^*}^T{\rvw^*}'>0$, the new total misclassification rate is no less than the misclassification rate before the movements. }
% \yaoqing{Why do we add a multiple of $w*$? What if the vector added is not a multiple of that?}
\vspace{-0.35cm}
\begin{proof}
We provide the proof in App.~\ref{app:lemma_2}.
\end{proof}
\vspace{-0.3cm}
{Note that the special case where the representations of the two classes swap positions (e.g, bipartite graphs) violates the condition ${\rvw^*}^T{\rvw^*}'>0$ and leads to different conclusions. We refer to the condition ${\rvw^*}^T{\rvw^*}'>0$ as "non-swapping condition" and throughout the paper, we analyze SGC under that. Lemma 2 shows that, \ul{under the "non-swapping condition", if $\{\rvf_i^{(l)}\}$ move towards the original decision boundary (or the other class), SGC tends to perform worse.}}
% \yaoqing{Isn't this just saying that the margin will be smaller?}

%\textbf{Setup.} We consider a binary node classification task on an unweighted, self-loop-free graph $\gG$ with adjacency matrix $\rmA$. 
% \yy{[Remove Gaussian assumption]}
%We denote the set of nodes in the first and second class as $\gV_1$ and $\gV_2$, respectively. When $v_i \in \gV_1$, $\rvf_i^0$ follows a 
%Gaussian 
%distribution with mean $\rvmu$ and variance $\rvSigma$, and when $v_i \in \gV_2$, $\rvf_i^0$ follows a distribution with $-\rvmu$ and $\rvSigma$. Our analysis uses GCN layers (\S~\ref{section: background}) without nonlinearities {and focuses on binary classification}, but we demonstrate empirically that our results still apply to general settings 
%to non-linear layers and multi-class classification 
 


% We denote the degree of node $v_i$ by $d_i$, and the degree matrix by $\rmD$ which is a diagonal matrix whose elements are degrees. 
% Denote $\gN_i$ as the set of nodes directly connected to $v_i$, i.e., its neighbors. We further denote $\gN^s_i$ the set of nodes that are in $\gN_i$ and have the same class as $v_i$. 
% We use a concept called homophily to represent the tendency of a node to have the same class as its neighbor. 
% Specifically, for the $i$-th node $v_i$, its homophily $h_i$ is defined as the proportion $h_i = \E(\frac{|\gN^s_i|}{|\gN_i|})$, where $\gN^s_i$ is the set of neighboring nodes that share the same label as $v_i$, $\vert \cdot \vert$ is the cardinality operator, and the expectation is taken over the randomness of the node labels.
%We further assume that the heterophily is a constant across all nodes, i.e., $h_i=h, \forall i$.

\vspace{-0.3cm}
\subsection{{Movements of Node Representations in Shallow and Deeper Layers}}
\label{subsec: heterophily_oversmoothing}
\vspace{-0.2cm}
{In the following theorems, we will show how relative degree $r_{ij}$ and homophily level $h_i$ will affect the movement of node representations in both shallow and deeper layers. We show results for class 1 and the results for class 2 can be derived similarly.}
\vspace{-0.3cm}
\subsubsection{Initial Stage: Shallow Layers}
\label{sec:initial-stage}
\vspace{-0.2cm}
\begin{theorem}
\textbf{[Initial Stage]} {Under the "non-swapping condition", during} message passing in shallow layers, the nodes with \textbf{low} homophily $h_i \leq \frac{\rho}{1+\rho}$ and the nodes with high homophily $h_i > \frac{\rho}{1+\rho}$ but \textbf{small} degree $d_i$ (w.r.t.\ their neighbors) are prone to be misclassified.
% Denote $M_i$ by $\frac{1}{M_i} \equiv \frac{1}{d_i}\sum_{j \in \gN_i}{\frac{1}{\sqrt{(d_j+1)}}}$.
Defining $r_{ij}\equiv\sqrt{\frac{d_i + 1}{d_j + 1}}$ and $\ratioi \equiv \frac{1}{d_i} \sum_{j \in \gN_i} r_{ij}$, the expectation of representation $\rvf_i^{(1)}$ {in class 1} is given by:
% \yaoqing{I don't quite believe this. If the feature vector propagates through a matrix vector multiplication, wouldn't that change the direction of the feature vector? Do you just consider one linear matrix and all the nodes have the same mean vector? It's useful to clarify somewhere.}
% after operation $\tilde{\rmA}\rmF^{0}$ at layer 1 is:
% $\gamma_i^1 \E(\rvf^0_i)$, where $\gamma_i^l$ is a scalar and
\vspace{-0.2cm}
\begin{equation}
% \E(\rvf^1_i) =  \left (\frac{1}{(d_i+1)}+\frac{(2h_i-1)\sum_{j \in \gN_i}{\frac{1}{\sqrt{(d_j+1)}}}}{\sqrt{(d_i+1)}}\right )\E(\rvf^0_i)
% \E(\rvf^1_i) =  \left (\frac{1}{(d_i+1)}+\frac{(2h_i-1)d_i}{M_i\sqrt{(d_i+1)}}\right )\E(\rvf^0_i)
\E(\rvf^{(1)}_i) =  \left (\frac{((1+\rho)h_i-\rho) d_i \ratioi + 1}{d_i + 1}\right )\E(\rvf^{(0)}_i) \equiv \gamma_i^1 \E(\rvf^{(0)}_i), \label{eq:factor}
\end{equation}
where the multiplicative factor $\gamma_i^1$ is: %follows:
\vspace{-0.2cm}
\begin{equation}
\gamma_i^1 \in 
\begin{cases}
  (-\infty, \frac{1}{2}], & \text{if}\ h_i\leq \frac{\rho}{1+\rho} \\
  {(0, 1]}, & \text{if}\ h_i>\frac{\rho}{1+\rho} \ \mathrm{\&}\  \ratioi \leq \frac{1}{(1+\rho)h_i-\rho}\\
  (1, \infty), & \mathrm{otherwise}.
\end{cases}
% \begin{cases}
%   \gamma_i^1 \leq \frac{1}{2}, & \text{if}\ h_i\leq0.5 \\
%   \frac{1}{2} < \gamma_i^1 \leq 1, & \text{if}\ h_i>0.5 \ \mathrm{and}\  \ratioi \leq \frac{1}{2h_i-1}\\
%   \gamma_i^1 > 1, & \mathrm{otherwise}.
% \end{cases}
\label{eq:initial_stage}
\end{equation}
% Whether the mean vector moves towards or away from the origin is decided by as follows:
% \vspace{-0.2cm}
% \begin{equation}
% \begin{cases}
%   \|\E(\rvf^1_i)\| \leq \frac{||\E(\rvf^0_i)||}{2}, & \text{if}\ h_i\leq0.5 \\
%   \|\E(\rvf^1_i)\| \leq ||\E(\rvf^0_i)||, & \text{if}\ h_i>0.5\\ & \mathrm{and} \ \ratioi \leq \frac{1}{2h_i-1}\\
%   \|\E(\rvf^1_i)\| > ||\E(\rvf^0_i)||, & \text{otherwise}
% \end{cases}
% \label{eq: initial_stage}
% \end{equation}
%{For independent features $\rvf^0_i$,} the variance of each node is reduced to $\frac{1}{(d_i+1)} \left ( \frac{1}{(d_i+1)}+\sum_{j \in \gN_i}{\frac{1}{(d_j+1)}} \right )\rvSigma \leq \frac{1}{2}\rvSigma$. %, which is bounded by $\frac{1}{2}\rvSigma$. 
\label{theorem: initial_stage}
\end{theorem}
\vspace{-0.6cm}
\begin{proof}
We provide the proof in App.~\ref{app:proof1}.
\end{proof}
\vspace{-0.3cm}
% {\textbf{Effects of multiplying weight matrices.} Theorem~\ref{theorem: initial_stage} shows that after performing $\tilde{\rmA}\rmF^{0}$, $\E(\rvf^1_i)$ will remain linearly dependent and the ratio of $\E(\rvf^1_i)$ to $\E(\rvf^1_j)$ is determined by the ratio of $\gamma_i^1$ to $\gamma_j^1$. Multiplying by the same weight matrices will transform $\rvf^1_i$ and class mean at the same time, but it will not change the ratio, and thus it will not affect the linear separability of $\rvf^1_i$.}

{From Thm.~\ref{theorem: initial_stage}, we identify three types of movements of node representations, which are characterized by relative degree $r_{ij}$ and homophily level $h_i$. For illustration purposes, in Fig.~\ref{fig:concept}, we illustrate the three cases when {we apply our theorem to 1D node representations.}
% we have 1D node representations and perform binary classification. 
The bars reflect the value change of $v_i$'s node representation.} 
{Intuitively, under heterophily (case 1) or under high homophily but low degrees (case 2), the expected representations will move heavily towards the opposing class.}
% Intuitively, under heterophily (case 1), the expected feature vector will move heavily towards the opposing class.
% % the mean feature vector of the opposing class. 
% For high homophily but low degrees (case 2), it will contract towards the origin. 
Otherwise, they will move away from the opposing class (case 3). {Among the three cases, only nodes with high homophily and high relative degree  benefit from propagation and aggregation.}
% Unlike previous works~\citep{chen2020simple, wang2019improving} that focus more on the analysis of final node representations in the limit of infinite layers, we focus on the dynamic analysis of the node representations that are gradually passed to deeper layers.

\begin{figure*}[t]
\centering
\includegraphics[scale=0.21, bb=1250 0 300 250]{Figs/illustration_5.png}
\vspace{-0.2cm}
\caption{Node representation dynamics during neighborhood aggregation (in 1D for illustration purposes; `MR': misclassification rate). %{MR means misclassification rate}. 
The expectation of node representations from class 1 \& 2 are denoted by $\mu$ and $-\mu$, respectively.
The bars show the expected node representations of node $v_i$ before and after the aggregation.} 
%We list out whether the change will make the node representations more or less linearly separable (LS) in the left table. Case 1 occurs when the homophily is low and is shown in the first sub-figure; case 2 occurs when the homophily is high but relative degree is low and is shown in the second sub-figure; case 3 occurs when the homophily and relative degree are both high and is shown in the third sub-figure.
% \yaoqing{Shouldn't the expectation of node representation be a vector? Why are they scalars?}}
\label{fig:concept}
\vspace{-0.6cm}
\end{figure*}

% In this section we will demonstrate through 
%At a high level, our analysis highlights that both the oversmoothing problem and the heterophily problem result from \textit{less linear separability} of learned representations for nodes in different classes after propagation and aggregation across layers.
%Specifically, our theory demonstrates that---in expectation---the layer-wise transformation of a node's representation depends on two factors: (1) the level of homophily (proportion of neighbors with the same class label), and (2) the relative degree of the node (how many neighbors it has relative to its neighbors). These factors determine if the node representation will tend to move towards the initial mean feature vector of the opposing class (become less linearly separable) or away (become more linearly separable).  
%As shown in the left panel of Fig.~\ref{fig:concept}, in more detail:
{\textbf{Explanation of the heterophily and oversmoothing problems:}}
\begin{itemize*}
\vspace{-0.3cm}
    \item In heterophilous graphs, node representations move heavily towards the opposite class. {According to Lemma 2, under the "non-swapping" condition, it indicates higher misclassification rate (i.e., poorer performance) for SGC.}
    % The severe decrease in the linear separability causes performance drop in shallow layers (case 1).
    \item In homophilous graphs, high-degree nodes may initially benefit (case 3), leading to performance gain in shallow layers. However, the representations of low-degree nodes {tend to move towards the opposing class (case 2)
    % reduce the linear separability (case 2) 
    and eventually flip the labels. The misclassification of low-degree nodes causes a \textit{pseudo-heterophily} situation (case 1) later.}
\end{itemize*}

% in heterophily (low homophily) graphs, the decrease in the linear separability is more severe, causing  performance drop even in shallow layers (Fig.~\ref{fig:concept}, case 1). In homophily graphs, high-degree nodes might initially benefit (Fig.~\ref{fig:concept} case 3), leading to performance gain in shallow layers, but the low-degree nodes will eventually reduce the linear separability (Fig.~\ref{fig:concept} case 2).


% \yy{Through the following theorems, we would like to point out: both oversmoothing and heterophily problems result from less linear separability after neighborhood aggregation. }
% \yy{In the high heterophilic graphs, the decrease in the linear separability is more severe, causing the performance drop even in shallow layers (Figure~\ref{fig:concept}, case 1). In homophily graphs, large-degree nodes might initially benefit (Figure~\ref{fig:concept} case 3), so we may see performance gain in shallow layers, but the low-degree nodes will eventually trigger the decrease in the linear separability (Figure~\ref{fig:concept} case 2).}

%\vspace{-0.3cm}
%\textbf{Theory.} T
%In more detail, the layer-wise message propagation and aggregation in GCNs is done via the $\tilde{\rmA}\rmF^l$ operation. Thus, for simplicity, our dynamic analysis 
%of the exchanged node representations 
%investigates the impact of this operation on the node class and its relation to the level of  homophily. However, the following conclusions still hold after scaling $\tilde{\rmA}\rmF^l$ by the learnable weight matrix $\rmW^l$. 
%Next, we consider two stages: the \textit{initial stage} at shallow layers of propagation and aggregation (\S~\ref{sec:initial-stage}), and the \textit{developing stage} at deeper layers (\S~\ref{sec:developing-stage}). 

% \yy{For clarity, we analyze the impact of $\tilde{\rmA}\rmF^l$, however, the scaling effect as we will point out later still hold after multiplied by the weight matrix $\rmW^l$.}

%\reminder{incorporate here and explain clearly} Recall the GCN formulation in the Section~\ref{section: background}, the main difference between GCN and standard multilayer perceptrons (MLPs) is the ``propagation and aggregation step'' done by multiplying the adjacency matrix $\tilde{\rmA}$ with the feature matrix $\rmF^{l}$. We will thoroughly discuss its effect in node classification and how it is related to the homophily of the nodes. 
% \vspace{-0.1cm}
% \subsubsection{Initial Stage: Shallow Layers}
% \label{sec:initial-stage}
% \vspace{-0.1cm}
% \begin{theorem}
% \textbf{[Initial Stage]} During message passing in shallow layers, the nodes with \textbf{low} homophily $h_i \leq 0.5$ and the nodes with high homophily $h_i > 0.5$ but \textbf{small} degree $d_i$ (w.r.t.\ their neighbors) are prone to be misclassified.
% % Denote $M_i$ by $\frac{1}{M_i} \equiv \frac{1}{d_i}\sum_{j \in \gN_i}{\frac{1}{\sqrt{(d_j+1)}}}$.
% Defining $r_{ij}\equiv\sqrt{\frac{d_i + 1}{d_j + 1}}$ and $\ratioi \equiv \frac{1}{d_i} \sum_{j \in \gN_i} r_{ij}$, the expectation of feature $\rvf_i^1$ after operation $\tilde{\rmA}\rmF^{0}$ at layer 1 is:
% \vspace{-0.2cm}
% \begin{equation}
% % \E(\rvf^1_i) =  \left (\frac{1}{(d_i+1)}+\frac{(2h_i-1)\sum_{j \in \gN_i}{\frac{1}{\sqrt{(d_j+1)}}}}{\sqrt{(d_i+1)}}\right )\E(\rvf^0_i)
% % \E(\rvf^1_i) =  \left (\frac{1}{(d_i+1)}+\frac{(2h_i-1)d_i}{M_i\sqrt{(d_i+1)}}\right )\E(\rvf^0_i)
% \E(\rvf^1_i) =  \left (\frac{(2h_i - 1) d_i \ratioi + 1}{d_i + 1}\right )\E(\rvf^0_i) \equiv \gamma_i^1 \E(\rvf^0_i), \label{eq:factor}
% \end{equation}
% % where the multiplicative factor $\gamma_i^1$ is: %follows:
% \vspace{-0.2cm}
% \begin{equation}
% \text{where } \gamma_i^1 \in 
% \begin{cases}
%   (-\infty, \frac{1}{2}], & \text{if}\ h_i\leq0.5 \\
%   (\frac{1}{2}, 1], & \text{if}\ h_i>0.5 \ \mathrm{\&}\  \ratioi \leq \frac{1}{2h_i-1}\\
%   (1, \infty), & \mathrm{otherwise}.
% \end{cases}
% % \begin{cases}
% %   \gamma_i^1 \leq \frac{1}{2}, & \text{if}\ h_i\leq0.5 \\
% %   \frac{1}{2} < \gamma_i^1 \leq 1, & \text{if}\ h_i>0.5 \ \mathrm{and}\  \ratioi \leq \frac{1}{2h_i-1}\\
% %   \gamma_i^1 > 1, & \mathrm{otherwise}.
% % \end{cases}
% \label{eq:initial_stage}
% \end{equation}
% % Whether the mean vector moves towards or away from the origin is decided by as follows:
% % \vspace{-0.2cm}
% % \begin{equation}
% % \begin{cases}
% %   \|\E(\rvf^1_i)\| \leq \frac{||\E(\rvf^0_i)||}{2}, & \text{if}\ h_i\leq0.5 \\
% %   \|\E(\rvf^1_i)\| \leq ||\E(\rvf^0_i)||, & \text{if}\ h_i>0.5\\ & \mathrm{and} \ \ratioi \leq \frac{1}{2h_i-1}\\
% %   \|\E(\rvf^1_i)\| > ||\E(\rvf^0_i)||, & \text{otherwise}
% % \end{cases}
% % \label{eq: initial_stage}
% % \end{equation}
% {For independent features $\rvf^0_i$,} the variance of each node is reduced to $\frac{1}{(d_i+1)} \left ( \frac{1}{(d_i+1)}+\sum_{j \in \gN_i}{\frac{1}{(d_j+1)}} \right )\rvSigma \leq \frac{1}{2}\rvSigma$. %, which is bounded by $\frac{1}{2}\rvSigma$. 
% \label{theorem: initial_stage}
% \end{theorem}
% \vspace{-0.4cm}
% \begin{proof}
% We provide the proof in App.~\ref{app:proof1}.
% \end{proof}
% % Avid readers can refer to the Appendix~\ref{app:proof1} for the complete proof. 

%\vspace{-0.4cm}
 % vector.

%We note that our analysis shows that the variance of \textit{each node} is reduced in the initial stage regardless of the homophily level. 
%However, this does \textit{not} mean that the variance of the nodes in the same \textit{class} is reduced. 
%The class variance %of the class 
%is decided not only by the node variance %of each node 
%but also how dispersed their mean is. 
%\reminder{mention at the end of 3.1.1?}

% \yaoqing{I now understand what you are trying to do. I think the paper should be much clear at the beginning on the several assumptions.}
\vspace{-0.5cm}
\subsubsection{Developing Stage: Deeper Layers}
\label{sec:developing-stage}
\vspace{-0.2cm}
% Based on Eqs.~(\ref{eq:factor})-(\ref{eq:initial_stage}), after propagation in several layers, the features of low-homophily nodes, and those of high-homophily but low-degree nodes may flip their labels. 
{The following theorem analyzes the pseudo-heterophily scenario in deeper layers. Based on Thm.~\ref{theorem: initial_stage}, message passing will result in scaling the node representations ($\gamma_i^1$) and some nodes may cross the origin. To account for those, 
let $\xi^l_i>0$ be an accumulated discount factor at the $l$-th layer and
\vspace{-0.25cm}
$$\E(\rvf_i^{(l)}) = \begin{cases}\xi^l_i\E(\rvf_i^{(0)}), & \text{if node }v_i\text{'s expected representation does not cross the origin.} \\
% -\rho\xi^l_i\rvf_i^{(0)} & \text{if node }v_i\text{ is from class 1 and its representation moves across the origin.} \\
% -\frac{1}{\rho}\xi^l_i\rvf_i^{(0)} & \text{if node }v_i\text{ is from class 2 and its representation moves across the origin.}
-\frac{|\gV_{y_i}|}{|\gV \setminus \gV_{y_i}|}\xi^l_i\E(\rvf_i^{(0)}), & \text{if node }v_i\text{'s expected representation moves across the origin.}
\end{cases}
\vspace{-0.3cm}
$$}
% Assuming initial features $\rvf^0_i$, propagation through $l$ layers, and accumulated discount factor at the $l$-th layer  $\gamma^l_i > 0$, we denote the sign-flipping features as $\rvf^l_i=-\gamma^l_i \rvf^0_i\rmW^{e}$, and the remaining features as 
% $\rvf^l_i=\gamma^l_i \rvf^0_i\rmW^{e}$, {where $\rmW^{e}$ is a weight matrix that is equivalent to multiplying all of the weight matrices up to the $(l-1)$-th layer}.
% Suppose we have propagated through $l$ layers of the network, starting from initial features $\rvf^0_i$. 
% We denote sign-flipping features as $\rvf^l_i=-\gamma^l_i \rvf^0_i$, where $\gamma^l_i > 0$ is the accumulated discount factor at layer $l$ due to previous propagation. 
% Likewise, for the nodes whose features do not flip their sign, we have: $\rvf^l_i=\gamma^l_i \rvf^0_i$. 
% \vspace{-0.2cm}
{We further define the \textbf{effective homophily} of node $i$ as  $\heterophilyil=\E(\frac{|\{v_j|\E(\rvf_i^{(0)})\cdot \E({\rvf_j^{(l)}}^T)>0, v_j \in \gN_i\}|}{|\gN_i|}),$ where the expectation is taken over the randomness of the node labels. Intiuitively, even if the original graph is not heterophilous, from the perspective of message passing under this pseudo-heterophily scenario, the deeper layers will act as if the graph is more heterophilous than it truly is, which may increase the misclassification rate.}
% of node $v_i$  as the ratio of the neighbors that have the same sign as $v_i$ at the $l$-th layer.
%class and have \textit{not flipped} their sign at the  $l$-th layer. 
% Similar to the analysis in the initial stage, we have:

% For example, from $\rvf^0_i$ to $\rvf^l_i=-\gamma^l_i \rvf^0_i, \gamma^l_i>0$, $\gamma^l_i$ represents the accumulated discount factor at layer $l$ due to the propagation from previous layers. For the nodes whose features do not flip the sign, we have: $\rvf^l_i=\gamma^l_i \rvf^0_i, \gamma^l_i>0$. We denote the effective homophily $\heterophilyil$ as the ratio of the nodes that are of the same class and have \textit{not flipped} the sign at the  $l$-th layer. Then similar to the analysis in the initial stage, we have:


\begin{theorem}
\textbf{[Developing Stage]} {Under the ``non-swapping condition'', during} message passing in deeper layers, when the effective homophily $\heterophilyil$ is sufficiently \textbf{low} $(\heterophilyil \leq \frac{\rho}{1+\rho})$, the \textbf{higher}-degree nodes %$d_i$ 
(w.r.t.\ its neighbors) %nodes 
are prone to misclassification. Specifically, defining $r_{ij}'\equiv r_{ij}\frac{\xi^l_j}{\xi^l_i}$ and $\ratioi' \equiv \frac{1}{d_i} \sum_{j \in \gN_i} r_{ij}'$, when $v_i$ is from class 1 and $\E(\rvf_i^{(0)})\cdot \E({\rvf_i^{(l+1)}})^T>0$, the expectation of $\rvf_i^{(l+1)}$ is: 
% after the operation $\tilde{\rmA}\rmF^{l}$ 
% \yy{(suppose $v_i$ is from target class and $\rvf_i^{l+1} \cdot {\rvf_i^{0}}^T>0$):}
\vspace{-0.2cm}
\begin{equation}
% \E(\rvf_i^{l+1}) = \left (\frac{1}{(d_i+1)}-(1-\hat{2h_i^l})\cdot \frac{d_i\cdot \gamma^l_j}{M_i \cdot \sqrt{(d_i+1)}}\right )\E(\rvf_i^{l})
% \E(\rvf_i^{l+1}) = \left (\frac{1}{(d_i+1)}+\frac{(\hat{2h_i^l} - 1) d_i \gamma^l_j}{M_i \sqrt{(d_i+1)}}\right )\E(\rvf_i^{l})
{\E(\rvf_i^{(l+1)}) = \left (\frac{((1+\rho)\heterophilyil-\rho) d_i \ratioi' + 1}{d_i+1}\right )\xi^l_i\E(\rvf_i^{(0)}) \equiv \gamma_i^{(l+1)}\E(\rvf_i^{(0)}).}
\label{eq: developing stage}
\end{equation}
\label{theorem: developing stage}
\vspace{-0.2cm}
\end{theorem}
\vspace{-0.6cm}
\begin{proof}
We provide the proof in App.~\ref{app:proof2}. Other nodes can be derived similarly.
%The derivation is similar to that of Theorem~\ref{theorem: initial_stage} except that we replace the ground truth heterophily $h_i$ with the effective heterophily $\heterophilyil$ and $\E(\rvf_i^{l})$ with $\gamma^l_i\E(\rvf_i^{0})$. Since graph $\gG$ is connected, the node degrees $d_i \geq 1$; thus, $\frac{d_i}{d_i+1}$ and $\ratioi$ are increasing functions of $d_i$, while $\frac{1}{d_i+1}$ is a decreasing function of $d_i$. When $\heterophilyil \leq 0.5$, we have $(2\heterophilyil - 1) \leq 0$, and $(2\heterophilyil - 1) \cdot \frac{d_i}{d_i+1} \cdot \ratioi + \frac{1}{d_i+1}$ is a decreasing function of $d_i$ in Eq.~(\ref{eq: developing stage}). This suggests that the higher-degree nodes move towards the opposing class more.
\vspace{-0.2cm}
\end{proof}
\vspace{-0.25cm}
{We note that Eq.~(\ref{eq: developing stage}) holds for layers $l \geq 2$ in general. We regard layers for which $\heterophilyil > \frac{\rho}{1+\rho}$ holds for most nodes $i$ as
% up to the layer when the effective homophily $\hat{h_i^l}$ becomes smaller or equal to $\frac{\rho}{1+\rho}$ for all the nodes. 
% {We regard these layers 
part of the initial stage, as they exhibit three cases similar to Eq.~(\ref{eq:initial_stage}).}
%In those layers, we have three cases similar to Eq.~(\ref{eq:initial_stage}) and we regard them part of the initial stage.}

%Tracing how $\E(\rvf^l_i)$ and $\sV(\rvf_t^{l})$ will change after the message propagation will help us better understand whether the node features will be easier to separate. In our case where the data is drawn from two Gaussians with opposite means, moving $\E(\rvf_t^{l})$ away from the opposing mean towards the true class mean, along with a reduced $\|\sV(\rvf_t^{l})\|$, is beneficial for the node classification task. In particular, it means that they become more linearly separable. 
\vspace{-0.2cm}
% \subsubsection{Implications from Theoretical Results} 
% \label{sec:summary-theory}
% \vspace{-0.2cm}
% Three conjectures follow from Thm.~\ref{theorem: initial_stage} and~\ref{theorem: developing stage}:
% %\vspace{-0.3cm}
% %\begin{enumerate}
% % \vspace{-0.1cm}  
% \textbf{(1)} After message propagation, the mean vectors $\E(\rvf^1_i)$ will be dispersed. For a high-homophily graph, in the initial stage, the features of \textit{low}-degree nodes (where $\ratioi \ll \frac{1}{(1+\rho)h_i-\rho}$) will first move towards the opposing class mean and have relatively lower accuracy (case 2). Later, when propagating to more layers, if the accuracy of low-degree nodes drops to a level such that the $\hat{h_i^l}$ of higher degree nodes satisfies $\heterophilyil \leq \frac{\rho}{1+\rho}$, then their features begin to move towards the opposing class mean vector (case 1) because $((1+\rho)\heterophilyil-\rho) \leq 0$ in Eq.~(\ref{eq: developing stage}).
%     % Later, when propagating to more layers, the accuracy of low degree nodes drop to a level such that the effective homophily  of higher degree nodes satisfies: $\heterophilyil \leq 0.5$, then the \textit{larger} degree $d_i$ compared to $M_i$, the larger $\frac{d_i\cdot \gamma^l_j}{M_i \cdot (d_i+1)^{\frac{1}{2}}}$ is and the smaller $\|\E(\rvf_i^{l+1})\|$ is (Equation~\ref{eq: developing stage}). We will show this phenomenon in the experiments.
    
% \textbf{(2)} GCNs perform differently on graphs with different degree distributions. For homophily graphs with power-law distribution (with many low-degree nodes), the performance of low-degree nodes will degenerate fast in the initial stage and the model will quickly enter the developing stage. Then, due to few high-degree nodes, the performance will degenerate more slowly. % will be slowed down.

% \textbf{(3)} The normalization scheme of the adjacency matrix of a graph makes a difference. 
% The reason that node degrees appear in Eqs.~(\ref{eq:initial_stage})-(\ref{eq: developing stage}) is the renormalization trick on $\rmA$ in GCN (\S~\ref{section: background}). Another normalization scheme such as row-normalization makes the scenario equivalent to a $d$-regular graph where nodes have the same degree (App.~\ref{app:proof1}). 

% scheme for the graphs also makes a difference. The reason that node degrees are involved in Equations~(\ref{eq:initial_stage})-(\ref{eq: developing stage}) is due to the renormalization scheme (Section~\ref{section: background}). If another normalization scheme is used, e.g. row-normalization, then the scenario is equivalent to a d-regular graph where nodes have the same degree (Appendix~\ref{app:proof1}). 
% \end{enumerate}
% \vspace{-0.3cm}
% Based on the analysis above, we can explain the GCN behavior in various settings: when a shallow GCN model is trained with a high-homophily graph, the increased mean distances between the large-degree nodes of different classes and the reduction in the variance lead to performance gain; when the model becomes deeper or is trained with a low-homophily graph, the reduction in the mean distances between the low-degree nodes becomes dominant and leads to degenerated performances.

% \vspace{-0.3cm}
\subsection{Signed Messages \& Movements of Representations}
\label{subsec: sign_theory}
\vspace{-0.1cm}
% Attention-based GCN models~\citep{velivckovic2017graph} typically use \textit{non-negative} attention weights to discount the contribution from dissimilar neighbors. {Though some concurrent works~\citep{chien2021adaptive, bo2021beyond} use negative attention weights, they do not to provide theoretical justifications. 
{In this section, we provide theory to show that signed messages can help enhance the performance in heterophilous graphs and also alleviate oversmoothing.}
%  the oversmoothing problem. 
Due to limited space,
% space limitations, 
we only show the effect of signed messages in the initial stage; similar results can be derived in the developing stage. % can be derived similarly.

\textbf{Setup.} %Consider the following scenario: 
% Consider the scenario where 
Signed messages consist of the negated messages sent by neighbors of the opposing class (i.e., after multiplying initial messages by -1), 
%multiplied by a negative sign 
and the unchanged messages ("positive messages") sent by neighbors of the same class. {In reality, ground-truth labels are not accessible for every node, so we use approximations, which introduces errors.}
% ``messages'' as they are. 
For node $v_i$, we define $m_i^l$ as the \textit{ratio of neighbors that send incorrect messages} at the $l$-th layer (i.e., different-class neighbors that send non-negated messages %without being multiplied by a negative sign 
and same-class neighbors that send negated messages). %multiplied by a negative sign). 
We define the $l$-th layer \textit{error rate} as $e_i^l=\E(m_i^l)$, where the expectation is over the randomness of the neighbors that send incorrect messages. %We assume the expectation is the same for all the nodes.
We make two  assumptions:
% \vspace{-0.2cm}
% \begin{enumerate}
    % \item 
    (1)~Conditioned on $m_i^l$, whether the neighbor $v_j$ will wrongly send the information is independent of its class $y_j$; 
    % \item 
    (2)~The variable $m_i^l$ is independent of the classes that nodes $v_j\in\gN_i$ belong to. 
% \end{enumerate}
\begin{theorem}
\textit{\textbf{[Signed Messages]}} With the independence assumptions and {under the ``non-swapping condition'',} by allowing the messages to be optionally multiplied by a negative sign, in the initial stage, the {movements of representations} will {\textbf{be less affected} by the initial homophily level $h_i$, and will be dependent on the \textbf{error rate} $e_i^l$}. Specifically, the multiplicative factor $\gamma_i^1$ at the first layer is:
\vspace{-0.1cm}
\begin{equation}
% \E(\rvf^1_i) = (\frac{1}{(d_i+1)} + (1-2e_i^0) \frac{d_i}{M_i\cdot (d_i+1)^{\frac{1}{2}}})\E(\rvf^0_i)
\E(\rvf^{(1)}_i) = \left ( \frac{(1 - 2e_i^0)(\rho+(1-\rho)h_i)d_i\ratioi + 1}{d_i+1}\right )\E(\rvf^{(0)}_i) \\
\equiv \gamma_i^1 \E(\rvf^{(0)}_i),
\label{eq:signed_messages}
\vspace{-0.2cm}
\end{equation}
\begin{equation}
\vspace{-0.1cm}
\text{where } \gamma_i^1 \in 
\begin{cases}
  (-\infty, \frac{1}{2}], & \text{if}\ e_i^0 \geq 0.5 \\
  {(0, 1]}, & \text{if}\ e_i^0 < 0.5 \ \mathrm{\&}\  \ratioi \leq \frac{1}{(1 - 2e_i^0)(\rho+(1-\rho)h_i)}\\
  (1, \infty), & \mathrm{otherwise}.
% \begin{cases}
%   \gamma_i^1 \leq \frac{1}{2}, & \text{if}\ e_i^0 \geq 0.5 \\
%   \frac{1}{2} < \gamma_i^1 \leq 1, & \text{if}\ e_i^0 < 0.5 \ \mathrm{and}\  \ratioi \leq \frac{1}{1 - 2e_i^0}\\
%   \gamma_i^1 > 1, & \mathrm{otherwise}
%   ||\E(\rvf^1_i)|| \leq \frac{||\E(\rvf^0_i)||}{2}, & \text{if}\ e_i^0\geq0.5 \\
%   ||\E(\rvf^1_i)|| \leq ||\E(\rvf^0_i)||, & \text{if}\ (e_i^0<0.5)\\ & \& \ (d_i \leq (\frac{M_i}{1-2e_i^0})^2-1)\\
%   ||\E(\rvf^1_i)|| > ||\E(\rvf^0_i)||, & \text{otherwise}
\end{cases}
\label{eq: signed_message_initial_stage}
\end{equation}
\label{theorem: signed_messages}
\end{theorem}
\vspace{-0.7cm}
\begin{proof}
The proof is provided in App.~\ref{app:proof3}.
\end{proof}

\vspace{-0.4cm}
{
% Given $h_i \leq 1$, we have $\frac{1}{(1+\rho)h_i-\rho} \geq \frac{1}{\rho+(1-\rho)h_i}$. 
From Eq.~\ref{eq: signed_message_initial_stage}, we see that when using signed messages, to benefit from case 3 ($\gamma_i^1>1$), the minimum relative degree satisfies: $\ratioi > \frac{1}{(1 - 2e_i^0)(\rho+(1-\rho)h_i)}$. Given $h_i \leq 1$, if the error rate is low ($e_i^0 \ll 0.5$),  we get: $\frac{1}{(1 - 2e_i^0)(\rho+(1-\rho)h_i)} \leq \frac{1}{(1+\rho)h_i-\rho}$, and $\frac{1}{(1+\rho)h_i-\rho}$ is the minimum relative degree required when not using signed messages.
This implies that more nodes can benefit from using signed messages. 
We note that if low error rate cannot be guaranteed, signed messages may hurt the performance.}
% From Eq.~(\ref{eq:signed_messages}), we conclude that:
% % \vspace{-0.3cm}
% % \begin{enumerate}
%     % \item
%     \textbf{(1)} Allowing neighbors of a different class to negate their messages prevents low homophily from degenerating performance.
%     % If we allow the neighbors of a different class to send information but be multiplied with a negative sign, then low homophily will not degenerate the performance. 
%     For a model that achieves low error rate at shallow layers (i.e, $e_i^0 \ll 0.5$), the low-degree nodes ($\ratioi \ll \frac{1}{1 - 2e_i^0}$) trigger oversmoothing. 
%     % \item
%     \textbf{(2)}~If a model does not work well under heterophily (i.e., high error rate $e_i^l$ in identifying neighbors from other classes), 
%     % in the heterophily setting, i.e., they have a higher error rate $e_i^l$ in identifying neighbors from another class, the model will be 
%     it is prone to oversmoothing even  in shallow layers. 
% \end{enumerate}


% \subsection{Additional Considerations \reminder{appendix?}} 
% % \vspace{-0.3cm}
% % \begin{enumerate}

% \textbf{On Batch norm vs.\ Layer norm.} % Whether it is beneficial to use batch norm or whether the trained weights can compensate for the shrinking distances. 
% Batch norm and trained weights cannot compensate for the dispersion of the mean vectors due to different degrees and homophily levels of the nodes. Though to some extent, it reduces the speed of the feature vectors of the susceptible nodes moving towards the other class (good for oversmoothing), it also prevents the feature vectors of the nodes who were supposed to gain from the propagation from increasing the distances (drop in accuracy). We find in our experiments (\S~\ref{section: experiments}) that, in general, adding batch norm significantly decreases the accuracy in heterophily datasets, but helps alleviate oversmoothing. Layer norm is a better option~\citep{zhou2020understanding} for oversmoothing and leads to smaller accuracy drop compared to batch norm in most datasets. However, in our experiments, layer norm has a significant accuracy drop for some datsets when some features are more important than the others.

% suggestion from Google reviewer
% \textbf{Generalization.} So far we have shown theoretical results on a binary classification task. However, this approach is general and can be applied to multi-class classification as well. In the next section we show the experiments on standard multi-class classification datasets.

% \textbf{Variance reduction.} In the analysis, we show that the variance of \textit{each node} is reduced in the initial stage regardless of the homophily level. However, it does not mean that the variance of the nodes in the same \textit{class} is reduced. The variance of the class is decided not only by the variance of each node but also how dispersed their mean is. \reminder{mention at the end of 3.1.1?}
% \end{enumerate}

==> sections/theoretic_analysis_new.tex <==
\vspace{-0.3cm}
\section{Theoretical Analysis}
\label{section: analysis}
\vspace{-0.3cm}
% In this section, we analyze the theoretical connections between \yy{oversmoothing and heterophily problems in node classification tasks. Both problems result in degenerated GCNs'performance. We find that the movements of node representations reflect the chances of nodes to be misclassified and are a good indicator of GCNs' performance.
% Thus, we characterize in expectation how node representations move and change over the layers and use the movements of representations to explain the oversmoothing and heterophily problems. }
% {At a high level, we focus on the node classification task and we use the \textit{linear separability} of learned node representations as an indicator of GCN performance. Intuitively, linear separability is the smallest distance between node representations of opposite classes. 
% By studying the movements of node representations after propagation and aggregation in GCNs, we characterize how linear separability 
% is changed over the layers.
% We identify two causes, i.e., the level of homophily of a node and the relative degree between a node and its neighbors, which  
% \yy{determine the movements of node representations. Specifically, moving towards (away from) another class leads to higher (lower) misclassification rate and worse (better) classification performance if the movements do not swap the positions of the two classes.}
%a limited portion of nodes are allowed to cross the decision boundary.}
% the linear separability of learned representations. Specifically, the two causes determine if the node representations will tend to move towards the initial mean feature vector of the opposing class (becoming less linearly separable) or away (becoming more linearly separable). 
% Our analysis highlights that \yy{the oversmoothing and heterophily problems result from a limited portion of nodes move towards another class induced by high heterophily level and low relative degree.}

{In this section, we formalize the connection} between the oversmoothing and heterophily problems in two steps: (1) We show how the movements of node representations relate to the misclassification rate of node labels; and  (2) we identify the factors that affect the movements of representations.
{We use the SGC model to analyze binary node classification with nodes in class 1 denoted as set $\gV_{1}$ and nodes in class 2 denoted as set $\gV_{2}$. We show empirically (\S~\ref{section: experiments}) that the insights obtained in this section are effective for other non-linear models in multi-class classification. %We denote the nodes in class 1 as $\gV_{1}$ and the remaining nodes as $\gV_{2}$. 
}
%  \reminder{define $\rho$ where it comes up -- We define the size ratio $\rho$ as: $\rho\equiv\frac{|\gV_{1}|}{|\gV_{2}|}.$}


% \yaoqing{At this stage, I think the readers will be completely confused by what you are trying to say. We can probably move the last sentence after our analysis and put that as a remark.}
% both the oversmoothing problem and the heterophily problem result from \textit{less linear separability} induced by these two causes.
%Moreover, we show that signed messages help reduce the effect from the factors.


%Our analysis highlights that both the oversmoothing problem and the heterophily problem result from \textit{less linear separability} of learned representations for nodes in different classes after graph convolution.
%we analyze the impact of message propagation in the node classification task, and show how the oversmoothing  and heterophily problems are related. We also discuss the implications of our analysis, which provide valuable insights for designing our model, \method, in \S~\ref{section: model_design}. %\yy{Move using linear GCN layers to settings.}


%\subsection{Settings \& Definitions}
% \label{subsec: notations}

% We consider a binary node classification task on an unweighted self-loop-free graph with adjacency matrix $\rmA$. 
% We denote the set of nodes in the first class and the second class as $\gV_1$ and $\gV_2$, respectively.

% \yaoqing{A general comment. I think we are confusing ourselves with definitions and assumptions. There are a lot of definitions below which belong to the notation section. The assumptions, such as E(f)=0, should be separated from these.}
\vspace{-0.3cm}
\subsection{Assumptions} 
\vspace{-0.3cm}
% In 
% %$|\gL|$ balanced classes (same number of nodes in each class) in a node classification task. 
% a multi-class node classification task,
% we assume: 
\textcolor{blue}{We use i.d. to represent random variables/vectors who follow the same marginal distribution and their joint distribution is a permutation invariant function.}
\textcolor{blue}{(1) Random graph: Node degrees $\{d_i\}$ are i.d. random variables. Defining $r_{ij}\equiv\sqrt{\frac{d_i + 1}{d_j + 1}}$ and $\ratioi \equiv \frac{1}{d_i} \sum_{j \in \gN_i} r_{ij}$, we assume $\ratioi$ is independent of $d_i$. $\{(\cdot)_i\}$ represents a set with $i=1, \dots, |\gV|$. Denote $\bar{r} \equiv \E(\ratioi)$ and $\frac{1}{d+1} \equiv \E(\frac{1}{d_i+1})$.  D-regular graphs are an example.}
% {(1) Graph generation process: (1.1) Node labels $\{y_i\}$ and degrees $\{d_i\}$ are deterministic. (1.2) Node connections are randomly determined: an arbitrary node $v_i$  connects to $k_i$ neighbors randomly chosen from the same class and $(d_i-k_i)$ neighbors randomly chosen from other classes, where $k_i$ follows the discrete uniform distribution of range $[0, \text{min}(d_i, |\gV_{y_i}|)]$. $\{(\cdot)_i\}$ represents a set with $i=1, \dots, |\gV|$.}
% \yaoqing{Is there an inherent assumption that the number of nodes in each class is larger than $d_i$? Otherwise, what if one node does not have enough nodes from a class to connect?}
% (1.3) Node features of the same (different) class are drawn from the same (different) distribution(s). \yaoqing{Shall we define these distributions here?} 
\textcolor{blue}{(2) Inputs: (2.1) Node labels $\{y_i\}$ are i.d. Bernoulli random variables given by the ratio $\rho$: $\rho \equiv \frac{\sP(y_i=1)}{\sP(y_i=2)}, \forall i$. Thus, we have: $h_i=h$. (2.3) Initial input node features $\{\rvf_i^{(0)}\}$ are i.d. random vectors given by the probability density function (PDF) $f({\rvx})$ and $\E(\rvf_i^{(0)})=\mathbf{0}$. The PDF is expressed as: $f({\rvx})=\begin{cases}
f_1(\rvx), & \text{when } y_i=1.\\
f_2(\rvx), & \text{when } y_i=2.
\end{cases}$ and $\E(\rvf_i^{(0)}|y_i)=\begin{cases} \rvmu, & \text{when } y_i=1.\\ -\rho\rvmu, & \text{when } y_i=2.
\end{cases}$}
% (2.2) Input node features are centered, i.e., $\E(\sum_i{\rvf_i^{(0)}})=\mathbf{0}.$ For SGC~\citep{wu2019simplifying}, no matter whether the input features are centered or not, the optimal learned parameters $\rmW^{(L)}$ will be the same. Only $\rvb^{(L)}$ will differ by a vector $\tilde{\rmA}^{L}\E(\sum{\rvf_i^{(0)}})\rmW^{(L)}.$ Thus, this assumption eases our demonstration without affecting the misclassification rate. %We define $\rvmu$ as the mean of distribution $f_{1}(\rvx)$.
% Based on assumption (2.2), if $\rvmu$ is the mean of distribution $f_{1}(\rvx)$, the mean of distribution $f_2(\rvx)$ is $-\rho\rvmu,$ where $\rho$ is the size ratio defined as: $\rho\equiv\frac{|\gV_{1}|}{|\gV_{2}|}.$}
% \yaoqing{Shall we give some motivations on why these features are centered?}
% (1) The initial features are centered, i.e., $\sum{\rvf_i^0}=\mathbf{0}$; (2) Given an arbitrary node $v_i$, for any node $v_j$ s.t. $y_i\neq y_j$, the probability of connecting to $v_i$ is equal; (3) 
% (3) Following prior work~\citep{li2018deeper, oono2019graph, chen2020simple}, \yy{we analyze SGC~\citep{wu2019simplifying}} but show empirically that our results still apply to non-linearized GCNs (\S~\ref{section: experiments}). \textbf{Simplifications.} We analyze the dynamics of $\rvf_i$ in each class in a one-vs-rest fashion. \yaoqing{Shall we clarify? I don't think the readers will understand what it means by the dynamics of xxx and "one-vs-rest fashion".}
% Without loss of generality, we choose class 1 as the target class and assume $\rvf_i^0$ of class 1 follows \yy{a distribution with a probability density function (PDF) $f_1(\rvx)$ and mean $\rvmu$}. Given \yy{assumption 1.2}, $\rvf_i^0$ in the other classes can be viewed as drawing from a virtual class (`rest'). \yaoqing{What does this mean? Is this related to the so called "one-vs-rest fashion"? If what you mean is that you want to study binary classification, you probably want to just say that you study binary classification, because one-vs-rest is not the same as binary classification. If you are indeed able to study multi-class classification, you can define class 1 and the rest as $C_1$ and $\bar C_1$.}
% We denote the set of nodes in the first and the virtual class \yaoqing{Also, avoid using a word that you are not familiar with. If this word is not something written in a text book and you invented it, ML people will think this is not appropriate.} as $\gV_1$ and $\gV_2$. \yy{Given assumption (2)}, the virtual class follows a distribution with \yy{a PDF $f_2(\rvx)$ and} mean $-\rho\rvmu$, $\rho=\frac{|\gV_1|}{|\gV_2|}$. Usually, $0<\rho\leq 1$.\yaoqing{What does "usually" mean?} Thus, the analysis reduces to analyzing two classes.}
\vspace{-0.3cm}
\subsection{{{Misclassification Rate \& Movements of Node Representations}}} 
\vspace{-0.2cm}
The following lemmas illustrate why the movements of node representations are a good indicator of SGC's performance. {\textcolor{blue}{We view node representations across the layers as their movements; e.g., $\rvf_i^{(l+1)}$ are moved from $\rvf_i^{(l)}, \forall i$.}
% An $L$-layer SGC applies logistic regression to the $L$-th layer node representations $\{\rvf_i^{(L)}\}$, 
% % An $L$-layer SGC applies logistic regression to the $L$-th layer representations, $\rvf_i^{(L)}$, of an arbitrary node $i$, 
% so we can study its misclassification rate through the decision boundaries of $\{\rvf_i^{(L)}\}$. 
The misclassification rate of an $L$-layer SGC is determined by the \textcolor{blue}{\underline{input to the last regression layer ($\{\rvf_i^{(L)}\}$)} and can be studied through the decision boundary of $\rvf_i^{(L)}$.}
The decision boundary of an $(L+1)$-layer SGC can be viewed as a perturbation to the decision boundary of an $L$-layer SGC due to the movements from $\{\rvf_i^{(L)}\}$ to $\{\rvf_i^{(L+1)}\}$.}
% The decision boundary of an $L$-th layer SGC
% Proofs are in App.~\ref{app:lemma_1} and \ref{app:lemma_2}}.
% \yy{SGC can be viewed as applying logistic regression to the last layer features $\rvf_i^{(L)}$, so we have:}

\vspace{-0.1cm}
{\textbf{Lemma 1} In SGC, the decision boundaries w.r.t. $\{\rvf_i^{(L)}\}$ in multi-class classification are linear hyperplanes. \textcolor{blue}{In particular, the decision boundary is a single hyperplane for binary classification.}}
\vspace{-0.4cm}
\begin{proof}
We provide the proof in App.~\ref{app:lemma_1}.
\end{proof}
\vspace{-0.4cm}
% \yaoqing{I am completely confused. I think we now have a lemma before we even defined the things in it. What does "movement" mean? What is a decision boundary? What does it mean to have a linear decision boundary? Also, avoid using things like "SGC can be viewed as applying logistic regression". People won't understand what you mean.}

% \yy{\textbf{Definition} The misclassification rate of a node set $\gV$ is: $\E(\hat{\chi}(v_i) \neq y_i)$, $v_i \in \gV$. }

% \yaoqing{What is the expectation over? The randomness in the random attachment model? The noise in SGD? The initialization of model weights? Or all of them?}

% \yy{Denote the hyperplane $\rvx\rvw+b=0$ as the decision boundary of the $\rvf_i^{l}$ that separates the nodes from the target class (predicted as the target class if $\rvx\rvw+b>0$) and the 'rest' class.
% \yaoqing{Is the following paragraph a proof?}
{Due to Lemma 1, we can use the hyperplane $\rvx\rvw+b=0$ to represent the decision boundary of $\{\rvf_i^{(L)}\}$, 
% that separates the nodes from class 1 and class 2, 
% \yaoqing{Do you mean "the decision boundary in the space of $\rvf_i^{l}$"? I think it is better to define the space.} 
where $\rvw$ is a unit vector, $b$ is a scalar, and the $\{\rvf_i^{(L)}\}$ are classified to class 1 if $\rvf_i^{(L)}\rvw+b>0$.
% The misclassification rate for the target class ('rest' class) is: $\int_{\rvw^T\rvx+\rvb<\mathbf{0}}{f_1(\rvx)d\rvx}$ ($\int_{\rvw^T\rvx+\rvb>\mathbf{0}}{f_2(\rvx)d\rvx}$). 
Suppose when $\rvw=\rvw^*$ and $b=b^*$, we find an optimal hyperplane $\rvx{\rvw^*}+b^*=0$ that achieves the lowest total misclassification rate (\S~\ref{section: background}) for $\{\rvf_i^{(L)}\}$. Due to the movements of node representations, the optimal hyperplane of $(L+1)$-th layer becomes: $\rvx{\rvw^*}'+{b^*}'=0$.
% $\int_{\rvw^T\rvx+\rvb<\mathbf{0}}{f_1(\rvx)d\rvx}+\int_{\rvw^T\rvx+\rvb>\mathbf{0}}{f_2(\rvx)d\rvx}$. 
% The next layer representations $\rvf_i^{l+1}$ can be viewed as being moved from $\rvf_i^{l}$. \yaoqing{One thing that confuses is me is that I thought $\rvf_i^{l}$ is a random variable. However, what you mentioned here and in the following sounds like it is a fixed vector. Also, is w* fixed? If so, it is important to state at the beginning.} Due to the movements, the optimal $\rvw^*$ and $b^*$ become ${\rvw^*}'$ and ${b^*}'$. \yaoqing{I believe you are just defining new terms. If so, say that we denote the new optimal weights and bias as xxx, instead of saying that they become xxx.} 
In Lemma 2, we show that, \ul{under constraints, moving towards the original decision boundary with a non-zero step results in a non-decreasing total misclassification rate under the new decision boundary.}}

{\textbf{Lemma 2} Moving representations $\{\rvf_i^{(L)}\}$ from class 1 by adding $-t{\rvw^*}^T$, $t>0$, s.t. ${\rvw^*}^T{\rvw^*}'>0$, the new total misclassification rate is no less than the misclassification rate before the movements. }
% \yaoqing{Why do we add a multiple of $w*$? What if the vector added is not a multiple of that?}
\vspace{-0.35cm}
\begin{proof}
We provide the proof in App.~\ref{app:lemma_2}.
\end{proof}
\vspace{-0.3cm}
{Note that the special case where the representations of the two classes swap positions (e.g, bipartite graphs) violates the condition ${\rvw^*}^T{\rvw^*}'>0$ and leads to different conclusions. We refer to the condition ${\rvw^*}^T{\rvw^*}'>0$ as "non-swapping condition" and throughout the paper, we analyze SGC under that. Lemma 2 shows that, \ul{under the "non-swapping condition", if $\{\rvf_i^{(l)}\}$ move towards the original decision boundary (or the other class), SGC tends to perform worse.}}
% \yaoqing{Isn't this just saying that the margin will be smaller?}

%\textbf{Setup.} We consider a binary node classification task on an unweighted, self-loop-free graph $\gG$ with adjacency matrix $\rmA$. 
% \yy{[Remove Gaussian assumption]}
%We denote the set of nodes in the first and second class as $\gV_1$ and $\gV_2$, respectively. When $v_i \in \gV_1$, $\rvf_i^0$ follows a 
%Gaussian 
%distribution with mean $\rvmu$ and variance $\rvSigma$, and when $v_i \in \gV_2$, $\rvf_i^0$ follows a distribution with $-\rvmu$ and $\rvSigma$. Our analysis uses GCN layers (\S~\ref{section: background}) without nonlinearities {and focuses on binary classification}, but we demonstrate empirically that our results still apply to general settings 
%to non-linear layers and multi-class classification 
 


% We denote the degree of node $v_i$ by $d_i$, and the degree matrix by $\rmD$ which is a diagonal matrix whose elements are degrees. 
% Denote $\gN_i$ as the set of nodes directly connected to $v_i$, i.e., its neighbors. We further denote $\gN^s_i$ the set of nodes that are in $\gN_i$ and have the same class as $v_i$. 
% We use a concept called homophily to represent the tendency of a node to have the same class as its neighbor. 
% Specifically, for the $i$-th node $v_i$, its homophily $h_i$ is defined as the proportion $h_i = \E(\frac{|\gN^s_i|}{|\gN_i|})$, where $\gN^s_i$ is the set of neighboring nodes that share the same label as $v_i$, $\vert \cdot \vert$ is the cardinality operator, and the expectation is taken over the randomness of the node labels.
%We further assume that the heterophily is a constant across all nodes, i.e., $h_i=h, \forall i$.

\vspace{-0.3cm}
\subsection{{Movements of Node Representations in Shallow and Deeper Layers}}
\label{subsec: heterophily_oversmoothing}
\vspace{-0.2cm}
{In the following theorems, we will show how relative degree $\bar{r}$ and homophily level $h$ will affect the movement of node representations in both shallow and deeper layers. We show results given that node $v_i$ is in class 1 and the results given that node $v_i$ is in class 2 can be derived similarly.}
\vspace{-0.3cm}
\subsubsection{Initial Stage: Shallow Layers}
\label{sec:initial-stage}
\vspace{-0.2cm}
\begin{theorem}
\textbf{[Initial Stage]} {Under the "non-swapping condition", during} message passing in shallow layers, the nodes with \textbf{low} homophily $h \leq \frac{\rho}{1+\rho}$ and the nodes with high homophily $h > \frac{\rho}{1+\rho}$ but \textbf{small} relative degree $\bar{r}$ are prone to be misclassified.
% Denote $M_i$ by $\frac{1}{M_i} \equiv \frac{1}{d_i}\sum_{j \in \gN_i}{\frac{1}{\sqrt{(d_j+1)}}}$.
% Defining $r_{ij}\equiv\sqrt{\frac{d_i + 1}{d_j + 1}}$ and $\ratioi \equiv \frac{1}{d_i} \sum_{j \in \gN_i} r_{ij}$, t
The expectation of representation $\rvf_i^{(1)}$ {in class 1} is given by:
% \yaoqing{I don't quite believe this. If the feature vector propagates through a matrix vector multiplication, wouldn't that change the direction of the feature vector? Do you just consider one linear matrix and all the nodes have the same mean vector? It's useful to clarify somewhere.}
% after operation $\tilde{\rmA}\rmF^{0}$ at layer 1 is:
% $\gamma_i^1 \E(\rvf^0_i)$, where $\gamma_i^l$ is a scalar and
\vspace{-0.2cm}
\begin{equation}
% \E(\rvf^1_i) =  \left (\frac{1}{(d_i+1)}+\frac{(2h_i-1)\sum_{j \in \gN_i}{\frac{1}{\sqrt{(d_j+1)}}}}{\sqrt{(d_i+1)}}\right )\E(\rvf^0_i)
% \E(\rvf^1_i) =  \left (\frac{1}{(d_i+1)}+\frac{(2h_i-1)d_i}{M_i\sqrt{(d_i+1)}}\right )\E(\rvf^0_i)
\E(\rvf^{(1)}_i|y_i=1) =  \left (\frac{((1+\rho)h-\rho) d \bar{r} + 1}{d + 1}\right )\E(\rvf^{(0)}_i) \equiv \gamma^1 \E(\rvf^{(0)}_i), \label{eq:factor}
\end{equation}
where the multiplicative factor $\gamma^1$ is: %follows:
\vspace{-0.2cm}
\begin{equation}
\gamma^1 \in 
\begin{cases}
  (-\infty, \frac{1}{2}], & \text{if}\ h\leq \frac{\rho}{1+\rho} \\
  {(0, 1]}, & \text{if}\ h>\frac{\rho}{1+\rho} \ \mathrm{\&}\  \bar{r} \leq \frac{1}{(1+\rho)h-\rho}\\
  (1, \infty), & \mathrm{otherwise}.
\end{cases}
% \begin{cases}
%   \gamma_i^1 \leq \frac{1}{2}, & \text{if}\ h_i\leq0.5 \\
%   \frac{1}{2} < \gamma_i^1 \leq 1, & \text{if}\ h_i>0.5 \ \mathrm{and}\  \ratioi \leq \frac{1}{2h_i-1}\\
%   \gamma_i^1 > 1, & \mathrm{otherwise}.
% \end{cases}
\label{eq:initial_stage}
\end{equation}
% Whether the mean vector moves towards or away from the origin is decided by as follows:
% \vspace{-0.2cm}
% \begin{equation}
% \begin{cases}
%   \|\E(\rvf^1_i)\| \leq \frac{||\E(\rvf^0_i)||}{2}, & \text{if}\ h_i\leq0.5 \\
%   \|\E(\rvf^1_i)\| \leq ||\E(\rvf^0_i)||, & \text{if}\ h_i>0.5\\ & \mathrm{and} \ \ratioi \leq \frac{1}{2h_i-1}\\
%   \|\E(\rvf^1_i)\| > ||\E(\rvf^0_i)||, & \text{otherwise}
% \end{cases}
% \label{eq: initial_stage}
% \end{equation}
%{For independent features $\rvf^0_i$,} the variance of each node is reduced to $\frac{1}{(d_i+1)} \left ( \frac{1}{(d_i+1)}+\sum_{j \in \gN_i}{\frac{1}{(d_j+1)}} \right )\rvSigma \leq \frac{1}{2}\rvSigma$. %, which is bounded by $\frac{1}{2}\rvSigma$. 
\label{theorem: initial_stage}
\end{theorem}
\vspace{-0.6cm}
\begin{proof}
We provide the proof in App.~\ref{app:proof1}.
\end{proof}
\vspace{-0.3cm}
% {\textbf{Effects of multiplying weight matrices.} Theorem~\ref{theorem: initial_stage} shows that after performing $\tilde{\rmA}\rmF^{0}$, $\E(\rvf^1_i)$ will remain linearly dependent and the ratio of $\E(\rvf^1_i)$ to $\E(\rvf^1_j)$ is determined by the ratio of $\gamma_i^1$ to $\gamma_j^1$. Multiplying by the same weight matrices will transform $\rvf^1_i$ and class mean at the same time, but it will not change the ratio, and thus it will not affect the linear separability of $\rvf^1_i$.}

{From Thm.~\ref{theorem: initial_stage}, we identify three types of movements of node representations, which are characterized by relative degree $\bar{r}$ and homophily level $h$. For illustration purposes, in Fig.~\ref{fig:concept}, we illustrate the three cases when {we apply our theorem to 1D node representations.}
% we have 1D node representations and perform binary classification. 
The bars reflect the value change of $v_i$'s node representation.} 
{Intuitively, under heterophily (case 1) or under high homophily but low degrees (case 2), the expected representations will move heavily towards the opposing class.}
% Intuitively, under heterophily (case 1), the expected feature vector will move heavily towards the opposing class.
% % the mean feature vector of the opposing class. 
% For high homophily but low degrees (case 2), it will contract towards the origin. 
Otherwise, they will move away from the opposing class (case 3). {Among the three cases, only nodes with high homophily and high relative degree  benefit from propagation and aggregation.}
% Unlike previous works~\citep{chen2020simple, wang2019improving} that focus more on the analysis of final node representations in the limit of infinite layers, we focus on the dynamic analysis of the node representations that are gradually passed to deeper layers.

\begin{figure*}[t]
\centering
\includegraphics[scale=0.21, bb=1250 0 300 250]{Figs/illustration_5.png}
\vspace{-0.2cm}
\caption{Node representation dynamics during neighborhood aggregation (in 1D for illustration purposes; `MR': misclassification rate). %{MR means misclassification rate}. 
The expectation of node representations from class 1 \& 2 are denoted by $\mu$ and $-\mu$, respectively.
The bars show the expected node representations of node $v_i$ before and after the aggregation.} 
%We list out whether the change will make the node representations more or less linearly separable (LS) in the left table. Case 1 occurs when the homophily is low and is shown in the first sub-figure; case 2 occurs when the homophily is high but relative degree is low and is shown in the second sub-figure; case 3 occurs when the homophily and relative degree are both high and is shown in the third sub-figure.
% \yaoqing{Shouldn't the expectation of node representation be a vector? Why are they scalars?}}
\label{fig:concept}
\vspace{-0.6cm}
\end{figure*}

% In this section we will demonstrate through 
%At a high level, our analysis highlights that both the oversmoothing problem and the heterophily problem result from \textit{less linear separability} of learned representations for nodes in different classes after propagation and aggregation across layers.
%Specifically, our theory demonstrates that---in expectation---the layer-wise transformation of a node's representation depends on two factors: (1) the level of homophily (proportion of neighbors with the same class label), and (2) the relative degree of the node (how many neighbors it has relative to its neighbors). These factors determine if the node representation will tend to move towards the initial mean feature vector of the opposing class (become less linearly separable) or away (become more linearly separable).  
%As shown in the left panel of Fig.~\ref{fig:concept}, in more detail:
{\textbf{Explanation of the heterophily and oversmoothing problems:}}
\begin{itemize*}
\vspace{-0.3cm}
    \item In heterophilous graphs, node representations move heavily towards the opposite class. {According to Lemma 2, under the "non-swapping" condition, it indicates higher misclassification rate (i.e., poorer performance) for SGC.}
    % The severe decrease in the linear separability causes performance drop in shallow layers (case 1).
    \item In homophilous graphs, high-degree nodes may initially benefit (case 3), leading to performance gain in shallow layers. However, the representations of low-degree nodes {tend to move towards the opposing class (case 2)
    % reduce the linear separability (case 2) 
    and eventually flip the labels. The misclassification of low-degree nodes causes a \textit{pseudo-heterophily} situation (case 1) later.}
\end{itemize*}

% in heterophily (low homophily) graphs, the decrease in the linear separability is more severe, causing  performance drop even in shallow layers (Fig.~\ref{fig:concept}, case 1). In homophily graphs, high-degree nodes might initially benefit (Fig.~\ref{fig:concept} case 3), leading to performance gain in shallow layers, but the low-degree nodes will eventually reduce the linear separability (Fig.~\ref{fig:concept} case 2).


% \yy{Through the following theorems, we would like to point out: both oversmoothing and heterophily problems result from less linear separability after neighborhood aggregation. }
% \yy{In the high heterophilic graphs, the decrease in the linear separability is more severe, causing the performance drop even in shallow layers (Figure~\ref{fig:concept}, case 1). In homophily graphs, large-degree nodes might initially benefit (Figure~\ref{fig:concept} case 3), so we may see performance gain in shallow layers, but the low-degree nodes will eventually trigger the decrease in the linear separability (Figure~\ref{fig:concept} case 2).}

%\vspace{-0.3cm}
%\textbf{Theory.} T
%In more detail, the layer-wise message propagation and aggregation in GCNs is done via the $\tilde{\rmA}\rmF^l$ operation. Thus, for simplicity, our dynamic analysis 
%of the exchanged node representations 
%investigates the impact of this operation on the node class and its relation to the level of  homophily. However, the following conclusions still hold after scaling $\tilde{\rmA}\rmF^l$ by the learnable weight matrix $\rmW^l$. 
%Next, we consider two stages: the \textit{initial stage} at shallow layers of propagation and aggregation (\S~\ref{sec:initial-stage}), and the \textit{developing stage} at deeper layers (\S~\ref{sec:developing-stage}). 

% \yy{For clarity, we analyze the impact of $\tilde{\rmA}\rmF^l$, however, the scaling effect as we will point out later still hold after multiplied by the weight matrix $\rmW^l$.}

%\reminder{incorporate here and explain clearly} Recall the GCN formulation in the Section~\ref{section: background}, the main difference between GCN and standard multilayer perceptrons (MLPs) is the ``propagation and aggregation step'' done by multiplying the adjacency matrix $\tilde{\rmA}$ with the feature matrix $\rmF^{l}$. We will thoroughly discuss its effect in node classification and how it is related to the homophily of the nodes. 
% \vspace{-0.1cm}
% \subsubsection{Initial Stage: Shallow Layers}
% \label{sec:initial-stage}
% \vspace{-0.1cm}
% \begin{theorem}
% \textbf{[Initial Stage]} During message passing in shallow layers, the nodes with \textbf{low} homophily $h_i \leq 0.5$ and the nodes with high homophily $h_i > 0.5$ but \textbf{small} degree $d_i$ (w.r.t.\ their neighbors) are prone to be misclassified.
% % Denote $M_i$ by $\frac{1}{M_i} \equiv \frac{1}{d_i}\sum_{j \in \gN_i}{\frac{1}{\sqrt{(d_j+1)}}}$.
% Defining $r_{ij}\equiv\sqrt{\frac{d_i + 1}{d_j + 1}}$ and $\ratioi \equiv \frac{1}{d_i} \sum_{j \in \gN_i} r_{ij}$, the expectation of feature $\rvf_i^1$ after operation $\tilde{\rmA}\rmF^{0}$ at layer 1 is:
% \vspace{-0.2cm}
% \begin{equation}
% % \E(\rvf^1_i) =  \left (\frac{1}{(d_i+1)}+\frac{(2h_i-1)\sum_{j \in \gN_i}{\frac{1}{\sqrt{(d_j+1)}}}}{\sqrt{(d_i+1)}}\right )\E(\rvf^0_i)
% % \E(\rvf^1_i) =  \left (\frac{1}{(d_i+1)}+\frac{(2h_i-1)d_i}{M_i\sqrt{(d_i+1)}}\right )\E(\rvf^0_i)
% \E(\rvf^1_i) =  \left (\frac{(2h_i - 1) d_i \ratioi + 1}{d_i + 1}\right )\E(\rvf^0_i) \equiv \gamma_i^1 \E(\rvf^0_i), \label{eq:factor}
% \end{equation}
% % where the multiplicative factor $\gamma_i^1$ is: %follows:
% \vspace{-0.2cm}
% \begin{equation}
% \text{where } \gamma_i^1 \in 
% \begin{cases}
%   (-\infty, \frac{1}{2}], & \text{if}\ h_i\leq0.5 \\
%   (\frac{1}{2}, 1], & \text{if}\ h_i>0.5 \ \mathrm{\&}\  \ratioi \leq \frac{1}{2h_i-1}\\
%   (1, \infty), & \mathrm{otherwise}.
% \end{cases}
% % \begin{cases}
% %   \gamma_i^1 \leq \frac{1}{2}, & \text{if}\ h_i\leq0.5 \\
% %   \frac{1}{2} < \gamma_i^1 \leq 1, & \text{if}\ h_i>0.5 \ \mathrm{and}\  \ratioi \leq \frac{1}{2h_i-1}\\
% %   \gamma_i^1 > 1, & \mathrm{otherwise}.
% % \end{cases}
% \label{eq:initial_stage}
% \end{equation}
% % Whether the mean vector moves towards or away from the origin is decided by as follows:
% % \vspace{-0.2cm}
% % \begin{equation}
% % \begin{cases}
% %   \|\E(\rvf^1_i)\| \leq \frac{||\E(\rvf^0_i)||}{2}, & \text{if}\ h_i\leq0.5 \\
% %   \|\E(\rvf^1_i)\| \leq ||\E(\rvf^0_i)||, & \text{if}\ h_i>0.5\\ & \mathrm{and} \ \ratioi \leq \frac{1}{2h_i-1}\\
% %   \|\E(\rvf^1_i)\| > ||\E(\rvf^0_i)||, & \text{otherwise}
% % \end{cases}
% % \label{eq: initial_stage}
% % \end{equation}
% {For independent features $\rvf^0_i$,} the variance of each node is reduced to $\frac{1}{(d_i+1)} \left ( \frac{1}{(d_i+1)}+\sum_{j \in \gN_i}{\frac{1}{(d_j+1)}} \right )\rvSigma \leq \frac{1}{2}\rvSigma$. %, which is bounded by $\frac{1}{2}\rvSigma$. 
% \label{theorem: initial_stage}
% \end{theorem}
% \vspace{-0.4cm}
% \begin{proof}
% We provide the proof in App.~\ref{app:proof1}.
% \end{proof}
% % Avid readers can refer to the Appendix~\ref{app:proof1} for the complete proof. 

%\vspace{-0.4cm}
 % vector.

%We note that our analysis shows that the variance of \textit{each node} is reduced in the initial stage regardless of the homophily level. 
%However, this does \textit{not} mean that the variance of the nodes in the same \textit{class} is reduced. 
%The class variance %of the class 
%is decided not only by the node variance %of each node 
%but also how dispersed their mean is. 
%\reminder{mention at the end of 3.1.1?}

% \yaoqing{I now understand what you are trying to do. I think the paper should be much clear at the beginning on the several assumptions.}
\vspace{-0.5cm}
\subsubsection{Developing Stage: Deeper Layers}
\label{sec:developing-stage}
\vspace{-0.2cm}
% Based on Eqs.~(\ref{eq:factor})-(\ref{eq:initial_stage}), after propagation in several layers, the features of low-homophily nodes, and those of high-homophily but low-degree nodes may flip their labels. 
{The following theorem analyzes the pseudo-heterophily scenario in deeper layers. Based on Thm.~\ref{theorem: initial_stage}, message passing will result in scaling the node representations ($\gamma_i^1$) and some nodes may cross the origin. To account for those, 
let $\xi^l_i>0$ be an accumulated discount factor at the $l$-th layer and
\vspace{-0.25cm}
$$\E(\rvf_i^{(l)}) = \begin{cases}\xi^l_i\E(\rvf_i^{(0)}), & \text{if node }v_i\text{'s expected representation does not cross the origin.} \\
% -\rho\xi^l_i\rvf_i^{(0)} & \text{if node }v_i\text{ is from class 1 and its representation moves across the origin.} \\
% -\frac{1}{\rho}\xi^l_i\rvf_i^{(0)} & \text{if node }v_i\text{ is from class 2 and its representation moves across the origin.}
-\frac{|\gV_{y_i}|}{|\gV \setminus \gV_{y_i}|}\xi^l_i\E(\rvf_i^{(0)}), & \text{if node }v_i\text{'s expected representation moves across the origin.}
\end{cases}
\vspace{-0.3cm}
$$}
% Assuming initial features $\rvf^0_i$, propagation through $l$ layers, and accumulated discount factor at the $l$-th layer  $\gamma^l_i > 0$, we denote the sign-flipping features as $\rvf^l_i=-\gamma^l_i \rvf^0_i\rmW^{e}$, and the remaining features as 
% $\rvf^l_i=\gamma^l_i \rvf^0_i\rmW^{e}$, {where $\rmW^{e}$ is a weight matrix that is equivalent to multiplying all of the weight matrices up to the $(l-1)$-th layer}.
% Suppose we have propagated through $l$ layers of the network, starting from initial features $\rvf^0_i$. 
% We denote sign-flipping features as $\rvf^l_i=-\gamma^l_i \rvf^0_i$, where $\gamma^l_i > 0$ is the accumulated discount factor at layer $l$ due to previous propagation. 
% Likewise, for the nodes whose features do not flip their sign, we have: $\rvf^l_i=\gamma^l_i \rvf^0_i$. 
% \vspace{-0.2cm}
{We further define the \textbf{effective homophily} of node $i$ as  $\heterophilyil=\E(\frac{|\{v_j|\E(\rvf_i^{(0)})\cdot \E({\rvf_j^{(l)}}^T)>0, v_j \in \gN_i\}|}{|\gN_i|}),$ where the expectation is taken over the randomness of the node labels. Intiuitively, even if the original graph is not heterophilous, from the perspective of message passing under this pseudo-heterophily scenario, the deeper layers will act as if the graph is more heterophilous than it truly is, which may increase the misclassification rate.}
% of node $v_i$  as the ratio of the neighbors that have the same sign as $v_i$ at the $l$-th layer.
%class and have \textit{not flipped} their sign at the  $l$-th layer. 
% Similar to the analysis in the initial stage, we have:

% For example, from $\rvf^0_i$ to $\rvf^l_i=-\gamma^l_i \rvf^0_i, \gamma^l_i>0$, $\gamma^l_i$ represents the accumulated discount factor at layer $l$ due to the propagation from previous layers. For the nodes whose features do not flip the sign, we have: $\rvf^l_i=\gamma^l_i \rvf^0_i, \gamma^l_i>0$. We denote the effective homophily $\heterophilyil$ as the ratio of the nodes that are of the same class and have \textit{not flipped} the sign at the  $l$-th layer. Then similar to the analysis in the initial stage, we have:


\begin{theorem}
\textbf{[Developing Stage]} {Under the ``non-swapping condition'', during} message passing in deeper layers, when the effective homophily $\heterophilyil$ is sufficiently \textbf{low} $(\heterophilyil \leq \frac{\rho}{1+\rho})$, the \textbf{higher}-degree nodes %$d_i$ 
(w.r.t.\ its neighbors) %nodes 
are prone to misclassification. Specifically, defining $r_{ij}'\equiv r_{ij}\frac{\xi^l_j}{\xi^l_i}$ and $\ratioi' \equiv \frac{1}{d_i} \sum_{j \in \gN_i} r_{ij}'$, when $v_i$ is from class 1 and $\E(\rvf_i^{(0)})\cdot \E({\rvf_i^{(l+1)}})^T>0$, the expectation of $\rvf_i^{(l+1)}$ is: 
% after the operation $\tilde{\rmA}\rmF^{l}$ 
% \yy{(suppose $v_i$ is from target class and $\rvf_i^{l+1} \cdot {\rvf_i^{0}}^T>0$):}
\vspace{-0.2cm}
\begin{equation}
% \E(\rvf_i^{l+1}) = \left (\frac{1}{(d_i+1)}-(1-\hat{2h_i^l})\cdot \frac{d_i\cdot \gamma^l_j}{M_i \cdot \sqrt{(d_i+1)}}\right )\E(\rvf_i^{l})
% \E(\rvf_i^{l+1}) = \left (\frac{1}{(d_i+1)}+\frac{(\hat{2h_i^l} - 1) d_i \gamma^l_j}{M_i \sqrt{(d_i+1)}}\right )\E(\rvf_i^{l})
{\E(\rvf_i^{(l+1)}) = \left (\frac{((1+\rho)\heterophilyil-\rho) d_i \ratioi' + 1}{d_i+1}\right )\xi^l_i\E(\rvf_i^{(0)}) \equiv \gamma_i^{(l+1)}\E(\rvf_i^{(0)}).}
\label{eq: developing stage}
\end{equation}
\label{theorem: developing stage}
\vspace{-0.2cm}
\end{theorem}
\vspace{-0.6cm}
\begin{proof}
We provide the proof in App.~\ref{app:proof2}. Other nodes can be derived similarly.
%The derivation is similar to that of Theorem~\ref{theorem: initial_stage} except that we replace the ground truth heterophily $h_i$ with the effective heterophily $\heterophilyil$ and $\E(\rvf_i^{l})$ with $\gamma^l_i\E(\rvf_i^{0})$. Since graph $\gG$ is connected, the node degrees $d_i \geq 1$; thus, $\frac{d_i}{d_i+1}$ and $\ratioi$ are increasing functions of $d_i$, while $\frac{1}{d_i+1}$ is a decreasing function of $d_i$. When $\heterophilyil \leq 0.5$, we have $(2\heterophilyil - 1) \leq 0$, and $(2\heterophilyil - 1) \cdot \frac{d_i}{d_i+1} \cdot \ratioi + \frac{1}{d_i+1}$ is a decreasing function of $d_i$ in Eq.~(\ref{eq: developing stage}). This suggests that the higher-degree nodes move towards the opposing class more.
\vspace{-0.2cm}
\end{proof}
\vspace{-0.25cm}
{We note that Eq.~(\ref{eq: developing stage}) holds for layers $l \geq 2$ in general. We regard layers for which $\heterophilyil > \frac{\rho}{1+\rho}$ holds for most nodes $i$ as
% up to the layer when the effective homophily $\hat{h_i^l}$ becomes smaller or equal to $\frac{\rho}{1+\rho}$ for all the nodes. 
% {We regard these layers 
part of the initial stage, as they exhibit three cases similar to Eq.~(\ref{eq:initial_stage}).}
%In those layers, we have three cases similar to Eq.~(\ref{eq:initial_stage}) and we regard them part of the initial stage.}

%Tracing how $\E(\rvf^l_i)$ and $\sV(\rvf_t^{l})$ will change after the message propagation will help us better understand whether the node features will be easier to separate. In our case where the data is drawn from two Gaussians with opposite means, moving $\E(\rvf_t^{l})$ away from the opposing mean towards the true class mean, along with a reduced $\|\sV(\rvf_t^{l})\|$, is beneficial for the node classification task. In particular, it means that they become more linearly separable. 
\vspace{-0.2cm}
% \subsubsection{Implications from Theoretical Results} 
% \label{sec:summary-theory}
% \vspace{-0.2cm}
% Three conjectures follow from Thm.~\ref{theorem: initial_stage} and~\ref{theorem: developing stage}:
% %\vspace{-0.3cm}
% %\begin{enumerate}
% % \vspace{-0.1cm}  
% \textbf{(1)} After message propagation, the mean vectors $\E(\rvf^1_i)$ will be dispersed. For a high-homophily graph, in the initial stage, the features of \textit{low}-degree nodes (where $\ratioi \ll \frac{1}{(1+\rho)h_i-\rho}$) will first move towards the opposing class mean and have relatively lower accuracy (case 2). Later, when propagating to more layers, if the accuracy of low-degree nodes drops to a level such that the $\hat{h_i^l}$ of higher degree nodes satisfies $\heterophilyil \leq \frac{\rho}{1+\rho}$, then their features begin to move towards the opposing class mean vector (case 1) because $((1+\rho)\heterophilyil-\rho) \leq 0$ in Eq.~(\ref{eq: developing stage}).
%     % Later, when propagating to more layers, the accuracy of low degree nodes drop to a level such that the effective homophily  of higher degree nodes satisfies: $\heterophilyil \leq 0.5$, then the \textit{larger} degree $d_i$ compared to $M_i$, the larger $\frac{d_i\cdot \gamma^l_j}{M_i \cdot (d_i+1)^{\frac{1}{2}}}$ is and the smaller $\|\E(\rvf_i^{l+1})\|$ is (Equation~\ref{eq: developing stage}). We will show this phenomenon in the experiments.
    
% \textbf{(2)} GCNs perform differently on graphs with different degree distributions. For homophily graphs with power-law distribution (with many low-degree nodes), the performance of low-degree nodes will degenerate fast in the initial stage and the model will quickly enter the developing stage. Then, due to few high-degree nodes, the performance will degenerate more slowly. % will be slowed down.

% \textbf{(3)} The normalization scheme of the adjacency matrix of a graph makes a difference. 
% The reason that node degrees appear in Eqs.~(\ref{eq:initial_stage})-(\ref{eq: developing stage}) is the renormalization trick on $\rmA$ in GCN (\S~\ref{section: background}). Another normalization scheme such as row-normalization makes the scenario equivalent to a $d$-regular graph where nodes have the same degree (App.~\ref{app:proof1}). 

% scheme for the graphs also makes a difference. The reason that node degrees are involved in Equations~(\ref{eq:initial_stage})-(\ref{eq: developing stage}) is due to the renormalization scheme (Section~\ref{section: background}). If another normalization scheme is used, e.g. row-normalization, then the scenario is equivalent to a d-regular graph where nodes have the same degree (Appendix~\ref{app:proof1}). 
% \end{enumerate}
% \vspace{-0.3cm}
% Based on the analysis above, we can explain the GCN behavior in various settings: when a shallow GCN model is trained with a high-homophily graph, the increased mean distances between the large-degree nodes of different classes and the reduction in the variance lead to performance gain; when the model becomes deeper or is trained with a low-homophily graph, the reduction in the mean distances between the low-degree nodes becomes dominant and leads to degenerated performances.

% \vspace{-0.3cm}
\subsection{Signed Messages \& Movements of Representations}
\label{subsec: sign_theory}
\vspace{-0.1cm}
% Attention-based GCN models~\citep{velivckovic2017graph} typically use \textit{non-negative} attention weights to discount the contribution from dissimilar neighbors. {Though some concurrent works~\citep{chien2021adaptive, bo2021beyond} use negative attention weights, they do not to provide theoretical justifications. 
{In this section, we provide theory to show that signed messages can help enhance the performance in heterophilous graphs and also alleviate oversmoothing.}
%  the oversmoothing problem. 
Due to limited space,
% space limitations, 
we only show the effect of signed messages in the initial stage; similar results can be derived in the developing stage. % can be derived similarly.

\textbf{Setup.} %Consider the following scenario: 
% Consider the scenario where 
Signed messages consist of the negated messages sent by neighbors of the opposing class (i.e., after multiplying initial messages by -1), 
%multiplied by a negative sign 
and the unchanged messages ("positive messages") sent by neighbors of the same class. {In reality, ground-truth labels are not accessible for every node, so we use approximations, which introduces errors.}
% ``messages'' as they are. 
For node $v_i$, we define $m_i^l$ as the \textit{ratio of neighbors that send incorrect messages} at the $l$-th layer (i.e., different-class neighbors that send non-negated messages %without being multiplied by a negative sign 
and same-class neighbors that send negated messages). %multiplied by a negative sign). 
We define the $l$-th layer \textit{error rate} as $e_i^l=\E(m_i^l)$, where the expectation is over the randomness of the neighbors that send incorrect messages. %We assume the expectation is the same for all the nodes.
We make two  assumptions:
% \vspace{-0.2cm}
% \begin{enumerate}
    % \item 
    (1)~Conditioned on $m_i^l$, whether the neighbor $v_j$ will wrongly send the information is independent of its class $y_j$; 
    % \item 
    (2)~The variable $m_i^l$ is independent of the classes that nodes $v_j\in\gN_i$ belong to. 
% \end{enumerate}
\begin{theorem}
\textit{\textbf{[Signed Messages]}} With the independence assumptions and {under the ``non-swapping condition'',} by allowing the messages to be optionally multiplied by a negative sign, in the initial stage, the {movements of representations} will {\textbf{be less affected} by the initial homophily level $h_i$, and will be dependent on the \textbf{error rate} $e_i^l$}. Specifically, the multiplicative factor $\gamma_i^1$ at the first layer is:
\vspace{-0.1cm}
\begin{equation}
% \E(\rvf^1_i) = (\frac{1}{(d_i+1)} + (1-2e_i^0) \frac{d_i}{M_i\cdot (d_i+1)^{\frac{1}{2}}})\E(\rvf^0_i)
\E(\rvf^{(1)}_i) = \left ( \frac{(1 - 2e_i^0)(\rho+(1-\rho)h_i)d_i\ratioi + 1}{d_i+1}\right )\E(\rvf^{(0)}_i) \\
\equiv \gamma_i^1 \E(\rvf^{(0)}_i),
\label{eq:signed_messages}
\vspace{-0.2cm}
\end{equation}
\begin{equation}
\vspace{-0.1cm}
\text{where } \gamma_i^1 \in 
\begin{cases}
  (-\infty, \frac{1}{2}], & \text{if}\ e_i^0 \geq 0.5 \\
  {(0, 1]}, & \text{if}\ e_i^0 < 0.5 \ \mathrm{\&}\  \ratioi \leq \frac{1}{(1 - 2e_i^0)(\rho+(1-\rho)h_i)}\\
  (1, \infty), & \mathrm{otherwise}.
% \begin{cases}
%   \gamma_i^1 \leq \frac{1}{2}, & \text{if}\ e_i^0 \geq 0.5 \\
%   \frac{1}{2} < \gamma_i^1 \leq 1, & \text{if}\ e_i^0 < 0.5 \ \mathrm{and}\  \ratioi \leq \frac{1}{1 - 2e_i^0}\\
%   \gamma_i^1 > 1, & \mathrm{otherwise}
%   ||\E(\rvf^1_i)|| \leq \frac{||\E(\rvf^0_i)||}{2}, & \text{if}\ e_i^0\geq0.5 \\
%   ||\E(\rvf^1_i)|| \leq ||\E(\rvf^0_i)||, & \text{if}\ (e_i^0<0.5)\\ & \& \ (d_i \leq (\frac{M_i}{1-2e_i^0})^2-1)\\
%   ||\E(\rvf^1_i)|| > ||\E(\rvf^0_i)||, & \text{otherwise}
\end{cases}
\label{eq: signed_message_initial_stage}
\end{equation}
\label{theorem: signed_messages}
\end{theorem}
\vspace{-0.7cm}
\begin{proof}
The proof is provided in App.~\ref{app:proof3}.
\end{proof}

\vspace{-0.4cm}
{
% Given $h_i \leq 1$, we have $\frac{1}{(1+\rho)h_i-\rho} \geq \frac{1}{\rho+(1-\rho)h_i}$. 
From Eq.~\ref{eq: signed_message_initial_stage}, we see that when using signed messages, to benefit from case 3 ($\gamma_i^1>1$), the minimum relative degree satisfies: $\ratioi > \frac{1}{(1 - 2e_i^0)(\rho+(1-\rho)h_i)}$. Given $h_i \leq 1$, if the error rate is low ($e_i^0 \ll 0.5$),  we get: $\frac{1}{(1 - 2e_i^0)(\rho+(1-\rho)h_i)} \leq \frac{1}{(1+\rho)h_i-\rho}$, and $\frac{1}{(1+\rho)h_i-\rho}$ is the minimum relative degree required when not using signed messages.
This implies that more nodes can benefit from using signed messages. 
We note that if low error rate cannot be guaranteed, signed messages may hurt the performance.}
% From Eq.~(\ref{eq:signed_messages}), we conclude that:
% % \vspace{-0.3cm}
% % \begin{enumerate}
%     % \item
%     \textbf{(1)} Allowing neighbors of a different class to negate their messages prevents low homophily from degenerating performance.
%     % If we allow the neighbors of a different class to send information but be multiplied with a negative sign, then low homophily will not degenerate the performance. 
%     For a model that achieves low error rate at shallow layers (i.e, $e_i^0 \ll 0.5$), the low-degree nodes ($\ratioi \ll \frac{1}{1 - 2e_i^0}$) trigger oversmoothing. 
%     % \item
%     \textbf{(2)}~If a model does not work well under heterophily (i.e., high error rate $e_i^l$ in identifying neighbors from other classes), 
%     % in the heterophily setting, i.e., they have a higher error rate $e_i^l$ in identifying neighbors from another class, the model will be 
%     it is prone to oversmoothing even  in shallow layers. 
% \end{enumerate}


% \subsection{Additional Considerations \reminder{appendix?}} 
% % \vspace{-0.3cm}
% % \begin{enumerate}

% \textbf{On Batch norm vs.\ Layer norm.} % Whether it is beneficial to use batch norm or whether the trained weights can compensate for the shrinking distances. 
% Batch norm and trained weights cannot compensate for the dispersion of the mean vectors due to different degrees and homophily levels of the nodes. Though to some extent, it reduces the speed of the feature vectors of the susceptible nodes moving towards the other class (good for oversmoothing), it also prevents the feature vectors of the nodes who were supposed to gain from the propagation from increasing the distances (drop in accuracy). We find in our experiments (\S~\ref{section: experiments}) that, in general, adding batch norm significantly decreases the accuracy in heterophily datasets, but helps alleviate oversmoothing. Layer norm is a better option~\citep{zhou2020understanding} for oversmoothing and leads to smaller accuracy drop compared to batch norm in most datasets. However, in our experiments, layer norm has a significant accuracy drop for some datsets when some features are more important than the others.

% suggestion from Google reviewer
% \textbf{Generalization.} So far we have shown theoretical results on a binary classification task. However, this approach is general and can be applied to multi-class classification as well. In the next section we show the experiments on standard multi-class classification datasets.

% \textbf{Variance reduction.} In the analysis, we show that the variance of \textit{each node} is reduced in the initial stage regardless of the homophily level. However, it does not mean that the variance of the nodes in the same \textit{class} is reduced. The variance of the class is decided not only by the variance of each node but also how dispersed their mean is. \reminder{mention at the end of 3.1.1?}
% \end{enumerate}

==> sections/theoretic_analysis_new_3.tex <==
\vspace{-0.4cm}
\section{Theoretical Analysis}
\label{section: analysis}
\vspace{-0.3cm}
% In this section, we analyze the theoretical connections between \yy{oversmoothing and heterophily problems in node classification tasks. Both problems result in degenerated GCNs'performance. We find that the movements of node representations reflect the chances of nodes to be misclassified and are a good indicator of GCNs' performance.
% Thus, we characterize in expectation how node representations move and change over the layers and use the movements of representations to explain the oversmoothing and heterophily problems. }
% {At a high level, we focus on the node classification task and we use the \textit{linear separability} of learned node representations as an indicator of GCN performance. Intuitively, linear separability is the smallest distance between node representations of opposite classes. 
% By studying the movements of node representations after propagation and aggregation in GCNs, we characterize how linear separability 
% is changed over the layers.
% We identify two causes, i.e., the level of homophily of a node and the relative degree between a node and its neighbors, which  
% \yy{determine the movements of node representations. Specifically, moving towards (away from) another class leads to higher (lower) misclassification rate and worse (better) classification performance if the movements do not swap the positions of the two classes.}
%a limited portion of nodes are allowed to cross the decision boundary.}
% the linear separability of learned representations. Specifically, the two causes determine if the node representations will tend to move towards the initial mean feature vector of the opposing class (becoming less linearly separable) or away (becoming more linearly separable). 
% Our analysis highlights that \yy{the oversmoothing and heterophily problems result from a limited portion of nodes move towards another class induced by high heterophily level and low relative degree.}

{In this section, we formalize the connection} between the oversmoothing and heterophily problems in two steps: (1) We show how the movements of node representations relate to the misclassification rate of node labels; and  (2) we identify the factors that affect the movements of representations.
{We use the SGC model to analyze binary node classification with nodes in class 1 denoted as set $\gV_{1}$ and nodes in class 2 denoted as set $\gV_{2}$. We show empirically (\S~\ref{section: experiments}) that the insights obtained in this section are effective for other non-linear models in multi-class classification. %We denote the nodes in class 1 as $\gV_{1}$ and the remaining nodes as $\gV_{2}$. 
}
%  \reminder{define $\rho$ where it comes up -- We define the size ratio $\rho$ as: $\rho\equiv\frac{|\gV_{1}|}{|\gV_{2}|}.$}


% \yaoqing{At this stage, I think the readers will be completely confused by what you are trying to say. We can probably move the last sentence after our analysis and put that as a remark.}
% both the oversmoothing problem and the heterophily problem result from \textit{less linear separability} induced by these two causes.
%Moreover, we show that signed messages help reduce the effect from the factors.


%Our analysis highlights that both the oversmoothing problem and the heterophily problem result from \textit{less linear separability} of learned representations for nodes in different classes after graph convolution.
%we analyze the impact of message propagation in the node classification task, and show how the oversmoothing  and heterophily problems are related. We also discuss the implications of our analysis, which provide valuable insights for designing our model, \method, in \S~\ref{section: model_design}. %\yy{Move using linear GCN layers to settings.}


%\subsection{Settings \& Definitions}
% \label{subsec: notations}

% We consider a binary node classification task on an unweighted self-loop-free graph with adjacency matrix $\rmA$. 
% We denote the set of nodes in the first class and the second class as $\gV_1$ and $\gV_2$, respectively.

% \yaoqing{A general comment. I think we are confusing ourselves with definitions and assumptions. There are a lot of definitions below which belong to the notation section. The assumptions, such as E(f)=0, should be separated from these.}
\vspace{-0.3cm}
\subsection{Assumptions} 
\vspace{-0.3cm}
% In 
% %$|\gL|$ balanced classes (same number of nodes in each class) in a node classification task. 
% a multi-class node classification task,
% we assume: 
\textcolor{blue}{Next, we use ``i.d.'' %\reminder{identically distributed?} 
to represent random variables/vectors that follow the same marginal distribution and their joint probability density function (PDF) is a permutation-invariant function
$p(\rvx_1, \dots, \rvx_n)=p(\textbf{P}(\rvx_1, \dots, \rvx_n))$, where $\textbf{P}$($\cdot$) means permutation.}

\textcolor{blue}{\textbf{(1) Random graph}: Node degrees $\{d_i\}$ are i.d.\ random variables. $\{(\cdot)_i\}$ represents a set with $i=1, \dots, |\gV|$.
% Defining $r_{ij}\equiv\sqrt{\frac{d_i + 1}{d_j + 1}}$ and $\ratioi \equiv \frac{1}{d_i} \sum_{j \in \gN_i} r_{ij}$, we assume $\ratioi$ is independent of $d_i$.  Denote $\bar{r} \equiv \E(\ratioi)$ and $\frac{1}{d+1} \equiv \E(\frac{1}{d_i+1})$.  D-regular graphs are an example.
}
% {(1) Graph generation process: (1.1) Node labels $\{y_i\}$ and degrees $\{d_i\}$ are deterministic. (1.2) Node connections are randomly determined: an arbitrary node $v_i$  connects to $k_i$ neighbors randomly chosen from the same class and $(d_i-k_i)$ neighbors randomly chosen from other classes, where $k_i$ follows the discrete uniform distribution of range $[0, \text{min}(d_i, |\gV_{y_i}|)]$. $\{(\cdot)_i\}$ represents a set with $i=1, \dots, |\gV|$.}
% \yaoqing{Is there an inherent assumption that the number of nodes in each class is larger than $d_i$? Otherwise, what if one node does not have enough nodes from a class to connect?}
% (1.3) Node features of the same (different) class are drawn from the same (different) distribution(s). \yaoqing{Shall we define these distributions here?} 
\noindent \textcolor{blue}{\textbf{(2) Inputs}: (2.1) Node labels $\{y_i\}$ are i.d.\ Bernoulli random variables given by the ratio $\rho$: $\rho \equiv \frac{\sP(y_i=1)}{\sP(y_i=2)}, \forall i$. (2.2) Initial input node features $\{\rvf_i^{(0)}\}$ are i.d. random vectors given by (PDF) $f({\rvx})$, which is expressed as: $f({\rvx})=\begin{cases}
f_1(\rvx), & \text{when } y_i=1.\\
f_2(\rvx), & \text{when } y_i=2.
\end{cases}$ $\E(\rvf_i^{(0)}|y_i)=\begin{cases} \rvmu, & \text{when } y_i=1.\\ -\rho\rvmu, & \text{when } y_i=2.  
\end{cases}$ so $\E(\rvf_i^{(0)})=\mathbf{0}$. 
\noindent \textbf{(3) Independence}: $\{d_i\}$ are independent of $\{y_i\}$ and $\{\rvf_i^{(0)}\}$.}
% (2.2) Input node features are centered, i.e., $\E(\sum_i{\rvf_i^{(0)}})=\mathbf{0}.$ For SGC~\citep{wu2019simplifying}, no matter whether the input features are centered or not, the optimal learned parameters $\rmW^{(L)}$ will be the same. Only $\rvb^{(L)}$ will differ by a vector $\tilde{\rmA}^{L}\E(\sum{\rvf_i^{(0)}})\rmW^{(L)}.$ Thus, this assumption eases our demonstration without affecting the misclassification rate. %We define $\rvmu$ as the mean of distribution $f_{1}(\rvx)$.
% Based on assumption (2.2), if $\rvmu$ is the mean of distribution $f_{1}(\rvx)$, the mean of distribution $f_2(\rvx)$ is $-\rho\rvmu,$ where $\rho$ is the size ratio defined as: $\rho\equiv\frac{|\gV_{1}|}{|\gV_{2}|}.$}
% \yaoqing{Shall we give some motivations on why these features are centered?}
% (1) The initial features are centered, i.e., $\sum{\rvf_i^0}=\mathbf{0}$; (2) Given an arbitrary node $v_i$, for any node $v_j$ s.t. $y_i\neq y_j$, the probability of connecting to $v_i$ is equal; (3) 
% (3) Following prior work~\citep{li2018deeper, oono2019graph, chen2020simple}, \yy{we analyze SGC~\citep{wu2019simplifying}} but show empirically that our results still apply to non-linearized GCNs (\S~\ref{section: experiments}). \textbf{Simplifications.} We analyze the dynamics of $\rvf_i$ in each class in a one-vs-rest fashion. \yaoqing{Shall we clarify? I don't think the readers will understand what it means by the dynamics of xxx and "one-vs-rest fashion".}
% Without loss of generality, we choose class 1 as the target class and assume $\rvf_i^0$ of class 1 follows \yy{a distribution with a probability density function (PDF) $f_1(\rvx)$ and mean $\rvmu$}. Given \yy{assumption 1.2}, $\rvf_i^0$ in the other classes can be viewed as drawing from a virtual class (`rest'). \yaoqing{What does this mean? Is this related to the so called "one-vs-rest fashion"? If what you mean is that you want to study binary classification, you probably want to just say that you study binary classification, because one-vs-rest is not the same as binary classification. If you are indeed able to study multi-class classification, you can define class 1 and the rest as $C_1$ and $\bar C_1$.}
% We denote the set of nodes in the first and the virtual class \yaoqing{Also, avoid using a word that you are not familiar with. If this word is not something written in a text book and you invented it, ML people will think this is not appropriate.} as $\gV_1$ and $\gV_2$. \yy{Given assumption (2)}, the virtual class follows a distribution with \yy{a PDF $f_2(\rvx)$ and} mean $-\rho\rvmu$, $\rho=\frac{|\gV_1|}{|\gV_2|}$. Usually, $0<\rho\leq 1$.\yaoqing{What does "usually" mean?} Thus, the analysis reduces to analyzing two classes.}
\vspace{-0.3cm}
\subsection{{{Misclassification Rate \& Movements of Node Representations}}} 
\vspace{-0.2cm}
The following lemmas illustrate why the movements of node representations are a good indicator of SGC's performance. {\textcolor{blue}{We view the changes of node representations across the layers as their movements; i.e., $\rvf_i^{(l+1)}$ is moved from $\rvf_i^{(l)}, \forall i$.}
% An $L$-layer SGC applies logistic regression to the $L$-th layer node representations $\{\rvf_i^{(L)}\}$, 
% % An $L$-layer SGC applies logistic regression to the $L$-th layer representations, $\rvf_i^{(L)}$, of an arbitrary node $i$, 
% so we can study its misclassification rate through the decision boundaries of $\{\rvf_i^{(L)}\}$. 
The misclassification rate of an $L$-layer SGC is determined by \textcolor{blue}{$\{\rvf_i^{(L)}\}$, which is the input to the last regression layer, and  can be studied through the decision boundary of $\rvf_i^{(L)}$.}
}
% The decision boundary of an $L$-th layer SGC
% Proofs are in App.~\ref{app:lemma_1} and \ref{app:lemma_2}}.
% \yy{SGC can be viewed as applying logistic regression to the last layer features $\rvf_i^{(L)}$, so we have:}

\vspace{-0.1cm}
{\textbf{Lemma 1} In SGC, the decision boundaries w.r.t. $\{\rvf_i^{(L)}\}$ in multi-class classification are linear hyperplanes. \textcolor{blue}{
For binary classification, the decision boundary is a single hyperplane.}} 
% In particular, the decision boundary is a single hyperplane for binary classification.}}
\vspace{-0.4cm}
\begin{proof}
We provide the proof in App.~\ref{app:lemma_1}.
\end{proof}
\vspace{-0.4cm}
% \yaoqing{I am completely confused. I think we now have a lemma before we even defined the things in it. What does "movement" mean? What is a decision boundary? What does it mean to have a linear decision boundary? Also, avoid using things like "SGC can be viewed as applying logistic regression". People won't understand what you mean.}

% \yy{\textbf{Definition} The misclassification rate of a node set $\gV$ is: $\E(\hat{\chi}(v_i) \neq y_i)$, $v_i \in \gV$. }

% \yaoqing{What is the expectation over? The randomness in the random attachment model? The noise in SGD? The initialization of model weights? Or all of them?}

% \yy{Denote the hyperplane $\rvx\rvw+b=0$ as the decision boundary of the $\rvf_i^{l}$ that separates the nodes from the target class (predicted as the target class if $\rvx\rvw+b>0$) and the 'rest' class.
% \yaoqing{Is the following paragraph a proof?}
{\textcolor{blue}{The decision boundary of an $(L+1)$-layer SGC can be viewed as a perturbation to the decision boundary of an $L$-layer SGC due to the movements from $\{\rvf_i^{(L)}\}$ to $\{\rvf_i^{(L+1)}\}$.} Due to Lemma 1, we can use the hyperplane $\rvx\rvw+b=0$ to represent the decision boundary of $\{\rvf_i^{(L)}\}$, 
% that separates the nodes from class 1 and class 2, 
% \yaoqing{Do you mean "the decision boundary in the space of $\rvf_i^{l}$"? I think it is better to define the space.} 
where $\rvw$ is a unit vector, $b$ is a scalar, and the $\{\rvf_i^{(L)}\}$ are classified to class 1 if $\rvf_i^{(L)}\rvw+b>0$.
% The misclassification rate for the target class ('rest' class) is: $\int_{\rvw^T\rvx+\rvb<\mathbf{0}}{f_1(\rvx)d\rvx}$ ($\int_{\rvw^T\rvx+\rvb>\mathbf{0}}{f_2(\rvx)d\rvx}$). 
Suppose when $\rvw=\rvw^*$ and $b=b^*$, we find an optimal hyperplane $\rvx{\rvw^*}+b^*=0$ that achieves the lowest total misclassification rate (\S~\ref{section: background}) for $\{\rvf_i^{(L)}\}$. Due to the movements of node representations, the \textcolor{blue}{new optimal hyperplane is decided by}: $\rvx{\rvw^*}'+{b^*}'=0$.
% $\int_{\rvw^T\rvx+\rvb<\mathbf{0}}{f_1(\rvx)d\rvx}+\int_{\rvw^T\rvx+\rvb>\mathbf{0}}{f_2(\rvx)d\rvx}$. 
% The next layer representations $\rvf_i^{l+1}$ can be viewed as being moved from $\rvf_i^{l}$. \yaoqing{One thing that confuses is me is that I thought $\rvf_i^{l}$ is a random variable. However, what you mentioned here and in the following sounds like it is a fixed vector. Also, is w* fixed? If so, it is important to state at the beginning.} Due to the movements, the optimal $\rvw^*$ and $b^*$ become ${\rvw^*}'$ and ${b^*}'$. \yaoqing{I believe you are just defining new terms. If so, say that we denote the new optimal weights and bias as xxx, instead of saying that they become xxx.} 
In Lemma 2, we show that, \ul{under constraints, moving towards the original decision boundary with a non-zero step results in a non-decreasing total misclassification rate under the new decision boundary.}}

{\textbf{Lemma 2} Moving representations $\{\rvf_i^{(L)}\}$ from class 1 by adding $-t{\rvw^*}^T$, $t>0$, s.t. ${\rvw^*}^T{\rvw^*}'>0$, the new total misclassification rate is no less than the misclassification rate before the movements. }
% \yaoqing{Why do we add a multiple of $w*$? What if the vector added is not a multiple of that?}
\vspace{-0.35cm}
\begin{proof}
We provide the proof in App.~\ref{app:lemma_2}.
\end{proof}
\vspace{-0.3cm}
{Note that the special case where the representations of the two classes swap positions (e.g, bipartite graphs) violates the condition ${\rvw^*}^T{\rvw^*}'>0$ and leads to different conclusions. We refer to the condition ${\rvw^*}^T{\rvw^*}'>0$ as "non-swapping condition" and throughout the paper, we analyze SGC under that. Lemma 2 shows that, \ul{under the "non-swapping condition", if $\{\rvf_i^{(l)}\}$ move towards the original decision boundary (or the other class), SGC tends to perform worse.}}
% \yaoqing{Isn't this just saying that the margin will be smaller?}

%\textbf{Setup.} We consider a binary node classification task on an unweighted, self-loop-free graph $\gG$ with adjacency matrix $\rmA$. 
% \yy{[Remove Gaussian assumption]}
%We denote the set of nodes in the first and second class as $\gV_1$ and $\gV_2$, respectively. When $v_i \in \gV_1$, $\rvf_i^0$ follows a 
%Gaussian 
%distribution with mean $\rvmu$ and variance $\rvSigma$, and when $v_i \in \gV_2$, $\rvf_i^0$ follows a distribution with $-\rvmu$ and $\rvSigma$. Our analysis uses GCN layers (\S~\ref{section: background}) without nonlinearities {and focuses on binary classification}, but we demonstrate empirically that our results still apply to general settings 
%to non-linear layers and multi-class classification 
 


% We denote the degree of node $v_i$ by $d_i$, and the degree matrix by $\rmD$ which is a diagonal matrix whose elements are degrees. 
% Denote $\gN_i$ as the set of nodes directly connected to $v_i$, i.e., its neighbors. We further denote $\gN^s_i$ the set of nodes that are in $\gN_i$ and have the same class as $v_i$. 
% We use a concept called homophily to represent the tendency of a node to have the same class as its neighbor. 
% Specifically, for the $i$-th node $v_i$, its homophily $h_i$ is defined as the proportion $h_i = \E(\frac{|\gN^s_i|}{|\gN_i|})$, where $\gN^s_i$ is the set of neighboring nodes that share the same label as $v_i$, $\vert \cdot \vert$ is the cardinality operator, and the expectation is taken over the randomness of the node labels.
%We further assume that the heterophily is a constant across all nodes, i.e., $h_i=h, \forall i$.

\vspace{-0.3cm}
\subsection{{Movements of Node Representations in Shallow and Deeper Layers}}
\label{subsec: heterophily_oversmoothing}
\vspace{-0.2cm}
{In the following theorems, we will show how relative degree and homophily level will affect the movement of node representations in both shallow and deeper layers. 
% To better show the impact of different degrees, we condition on the degree of the target node and assume we
\textcolor{blue}{We show results given the degree, $d_i$, of node $v_i$ and assume that $v_i$ is in class 1.} The results in class 2 can be derived similarly.
}
\vspace{-0.3cm}
\subsubsection{Initial Stage: Shallow Layers}
\label{sec:initial-stage}
\vspace{-0.2cm}
\begin{theorem}
\textbf{[Initial Stage]} {Under the "non-swapping condition", during} message passing in shallow layers, the nodes with \textbf{low} homophily $h_i \leq \frac{\rho}{1+\rho}$ and the nodes with high homophily $h_i > \frac{\rho}{1+\rho}$ but \textbf{small} relative degree are prone to be misclassified. Defining $r_{ij}\equiv\sqrt{\frac{d_i + 1}{d_j + 1}}$ and the relative degree \textcolor{blue}{$\ratioi \equiv \E_{\rmA|d_i, v_i \in \gV_1}(\frac{1}{d_i} \sum_{j \in \gN_i} r_{ij})$},
% Denote $M_i$ by $\frac{1}{M_i} \equiv \frac{1}{d_i}\sum_{j \in \gN_i}{\frac{1}{\sqrt{(d_j+1)}}}$.
% Defining $r_{ij}\equiv\sqrt{\frac{d_i + 1}{d_j + 1}}$ and $\ratioi \equiv \frac{1}{d_i} \sum_{j \in \gN_i} r_{ij}$, t
the conditional expectation of representation $\rvf_i^{(1)}$ is given by:
% \yaoqing{I don't quite believe this. If the feature vector propagates through a matrix vector multiplication, wouldn't that change the direction of the feature vector? Do you just consider one linear matrix and all the nodes have the same mean vector? It's useful to clarify somewhere.}
% after operation $\tilde{\rmA}\rmF^{0}$ at layer 1 is:
% $\gamma_i^1 \E(\rvf^0_i)$, where $\gamma_i^l$ is a scalar and
\vspace{-0.2cm}
\begin{align}
% \E(\rvf^1_i) =  \left (\frac{1}{(d_i+1)}+\frac{(2h_i-1)\sum_{j \in \gN_i}{\frac{1}{\sqrt{(d_j+1)}}}}{\sqrt{(d_i+1)}}\right )\E(\rvf^0_i)
% \E(\rvf^1_i) =  \left (\frac{1}{(d_i+1)}+\frac{(2h_i-1)d_i}{M_i\sqrt{(d_i+1)}}\right )\E(\rvf^0_i)
&\E_{\rmA, \{y_i\}, \{\rvf_i^{(0)}\}|d_i, v_i \in \gV_1}(\rvf_i^{(1)}|v_i \in \gV_1, d_i) =  \nonumber \\
&  \left (\frac{((1+\rho)h_i-\rho) d_i \ratioi + 1}{d_i + 1}\right )\E(\rvf^{(0)}_i) \equiv \gamma_i^1 \E(\rvf^{(0)}_i), \label{eq:factor}
\end{align}
where the multiplicative factor $\gamma_i^1$ is: %follows:
\vspace{-0.2cm}
\begin{equation}
\gamma_i^1 \in 
\begin{cases}
  (-\infty, \frac{1}{2}], & \text{if}\ h_i\leq \frac{\rho}{1+\rho} \\
  {(0, 1]}, & \text{if}\ h_i>\frac{\rho}{1+\rho} \ \mathrm{\&}\  \ratioi \leq \frac{1}{(1+\rho)h_i-\rho}\\
  (1, \infty), & \mathrm{otherwise}.
\end{cases}
% \begin{cases}
%   \gamma_i^1 \leq \frac{1}{2}, & \text{if}\ h_i\leq0.5 \\
%   \frac{1}{2} < \gamma_i^1 \leq 1, & \text{if}\ h_i>0.5 \ \mathrm{and}\  \ratioi \leq \frac{1}{2h_i-1}\\
%   \gamma_i^1 > 1, & \mathrm{otherwise}.
% \end{cases}
\label{eq:initial_stage}
\end{equation}
% Whether the mean vector moves towards or away from the origin is decided by as follows:
% \vspace{-0.2cm}
% \begin{equation}
% \begin{cases}
%   \|\E(\rvf^1_i)\| \leq \frac{||\E(\rvf^0_i)||}{2}, & \text{if}\ h_i\leq0.5 \\
%   \|\E(\rvf^1_i)\| \leq ||\E(\rvf^0_i)||, & \text{if}\ h_i>0.5\\ & \mathrm{and} \ \ratioi \leq \frac{1}{2h_i-1}\\
%   \|\E(\rvf^1_i)\| > ||\E(\rvf^0_i)||, & \text{otherwise}
% \end{cases}
% \label{eq: initial_stage}
% \end{equation}
%{For independent features $\rvf^0_i$,} the variance of each node is reduced to $\frac{1}{(d_i+1)} \left ( \frac{1}{(d_i+1)}+\sum_{j \in \gN_i}{\frac{1}{(d_j+1)}} \right )\rvSigma \leq \frac{1}{2}\rvSigma$. %, which is bounded by $\frac{1}{2}\rvSigma$. 
\label{theorem: initial_stage}
\end{theorem}
\vspace{-0.7cm}
\begin{proof}
We provide the proof in App.~\ref{app:proof1}.
\end{proof}
\vspace{-0.3cm}
% {\textbf{Effects of multiplying weight matrices.} Theorem~\ref{theorem: initial_stage} shows that after performing $\tilde{\rmA}\rmF^{0}$, $\E(\rvf^1_i)$ will remain linearly dependent and the ratio of $\E(\rvf^1_i)$ to $\E(\rvf^1_j)$ is determined by the ratio of $\gamma_i^1$ to $\gamma_j^1$. Multiplying by the same weight matrices will transform $\rvf^1_i$ and class mean at the same time, but it will not change the ratio, and thus it will not affect the linear separability of $\rvf^1_i$.}

{From Thm.~\ref{theorem: initial_stage}, we identify three types of movements of node representations, which are characterized by relative degree $\ratioi$ and homophily level $h_i$. For illustration purposes, in Fig.~\ref{fig:concept}, we illustrate the three cases when {we apply our theorem to 1D node representations.}
% we have 1D node representations and perform binary classification. 
The bars reflect the value change of $v_i$'s node representation.} 
{Intuitively, under heterophily (case 1) or under high homophily but low degrees (case 2), the expected representations will move heavily towards the opposing class.}
% Intuitively, under heterophily (case 1), the expected feature vector will move heavily towards the opposing class.
% % the mean feature vector of the opposing class. 
% For high homophily but low degrees (case 2), it will contract towards the origin. 
Otherwise, they will move away from the opposing class (case 3). {Among the three cases, only nodes with high homophily and high relative degree  benefit from propagation and aggregation.}
% Unlike previous works~\citep{chen2020simple, wang2019improving} that focus more on the analysis of final node representations in the limit of infinite layers, we focus on the dynamic analysis of the node representations that are gradually passed to deeper layers.

\begin{figure*}[t]
\centering
\includegraphics[scale=0.21, bb=1250 0 300 250]{Figs/illustration_5.png}
\vspace{-0.2cm}
\caption{Node representation dynamics during neighborhood aggregation (in 1D for illustration purposes; `MR': misclassification rate). %{MR means misclassification rate}. 
The expectation of node representations from class 1 \& 2 are denoted by $\mu$ and $-\mu$, respectively.
The bars show the expected node representations of node $v_i$ before and after the aggregation.} 
%We list out whether the change will make the node representations more or less linearly separable (LS) in the left table. Case 1 occurs when the homophily is low and is shown in the first sub-figure; case 2 occurs when the homophily is high but relative degree is low and is shown in the second sub-figure; case 3 occurs when the homophily and relative degree are both high and is shown in the third sub-figure.
% \yaoqing{Shouldn't the expectation of node representation be a vector? Why are they scalars?}}
\label{fig:concept}
\vspace{-0.6cm}
\end{figure*}

% In this section we will demonstrate through 
%At a high level, our analysis highlights that both the oversmoothing problem and the heterophily problem result from \textit{less linear separability} of learned representations for nodes in different classes after propagation and aggregation across layers.
%Specifically, our theory demonstrates that---in expectation---the layer-wise transformation of a node's representation depends on two factors: (1) the level of homophily (proportion of neighbors with the same class label), and (2) the relative degree of the node (how many neighbors it has relative to its neighbors). These factors determine if the node representation will tend to move towards the initial mean feature vector of the opposing class (become less linearly separable) or away (become more linearly separable).  
%As shown in the left panel of Fig.~\ref{fig:concept}, in more detail:
{\textbf{Explanation for heterophily and oversmoothing:}}
\begin{itemize*}
\vspace{-0.3cm}
    \item In heterophilous graphs, node representations move heavily towards the opposite class. {According to Lemma 2, under the "non-swapping" condition, it indicates higher misclassification rate (i.e., poorer performance) for SGC.}
    % The severe decrease in the linear separability causes performance drop in shallow layers (case 1).
    \item In homophilous graphs, high-degree nodes may initially benefit (case 3), leading to performance gain in shallow layers. However, the representations of low-degree nodes {tend to move towards the opposing class (case 2)
    % reduce the linear separability (case 2) 
    and eventually flip the labels. The misclassification of low-degree nodes causes a \textit{pseudo-heterophily} situation (case 1) later.}
\end{itemize*}

% in heterophily (low homophily) graphs, the decrease in the linear separability is more severe, causing  performance drop even in shallow layers (Fig.~\ref{fig:concept}, case 1). In homophily graphs, high-degree nodes might initially benefit (Fig.~\ref{fig:concept} case 3), leading to performance gain in shallow layers, but the low-degree nodes will eventually reduce the linear separability (Fig.~\ref{fig:concept} case 2).


% \yy{Through the following theorems, we would like to point out: both oversmoothing and heterophily problems result from less linear separability after neighborhood aggregation. }
% \yy{In the high heterophilic graphs, the decrease in the linear separability is more severe, causing the performance drop even in shallow layers (Figure~\ref{fig:concept}, case 1). In homophily graphs, large-degree nodes might initially benefit (Figure~\ref{fig:concept} case 3), so we may see performance gain in shallow layers, but the low-degree nodes will eventually trigger the decrease in the linear separability (Figure~\ref{fig:concept} case 2).}

%\vspace{-0.3cm}
%\textbf{Theory.} T
%In more detail, the layer-wise message propagation and aggregation in GCNs is done via the $\tilde{\rmA}\rmF^l$ operation. Thus, for simplicity, our dynamic analysis 
%of the exchanged node representations 
%investigates the impact of this operation on the node class and its relation to the level of  homophily. However, the following conclusions still hold after scaling $\tilde{\rmA}\rmF^l$ by the learnable weight matrix $\rmW^l$. 
%Next, we consider two stages: the \textit{initial stage} at shallow layers of propagation and aggregation (\S~\ref{sec:initial-stage}), and the \textit{developing stage} at deeper layers (\S~\ref{sec:developing-stage}). 

% \yy{For clarity, we analyze the impact of $\tilde{\rmA}\rmF^l$, however, the scaling effect as we will point out later still hold after multiplied by the weight matrix $\rmW^l$.}

%\reminder{incorporate here and explain clearly} Recall the GCN formulation in the Section~\ref{section: background}, the main difference between GCN and standard multilayer perceptrons (MLPs) is the ``propagation and aggregation step'' done by multiplying the adjacency matrix $\tilde{\rmA}$ with the feature matrix $\rmF^{l}$. We will thoroughly discuss its effect in node classification and how it is related to the homophily of the nodes. 
% \vspace{-0.1cm}
% \subsubsection{Initial Stage: Shallow Layers}
% \label{sec:initial-stage}
% \vspace{-0.1cm}
% \begin{theorem}
% \textbf{[Initial Stage]} During message passing in shallow layers, the nodes with \textbf{low} homophily $h_i \leq 0.5$ and the nodes with high homophily $h_i > 0.5$ but \textbf{small} degree $d_i$ (w.r.t.\ their neighbors) are prone to be misclassified.
% % Denote $M_i$ by $\frac{1}{M_i} \equiv \frac{1}{d_i}\sum_{j \in \gN_i}{\frac{1}{\sqrt{(d_j+1)}}}$.
% Defining $r_{ij}\equiv\sqrt{\frac{d_i + 1}{d_j + 1}}$ and $\ratioi \equiv \frac{1}{d_i} \sum_{j \in \gN_i} r_{ij}$, the expectation of feature $\rvf_i^1$ after operation $\tilde{\rmA}\rmF^{0}$ at layer 1 is:
% \vspace{-0.2cm}
% \begin{equation}
% % \E(\rvf^1_i) =  \left (\frac{1}{(d_i+1)}+\frac{(2h_i-1)\sum_{j \in \gN_i}{\frac{1}{\sqrt{(d_j+1)}}}}{\sqrt{(d_i+1)}}\right )\E(\rvf^0_i)
% % \E(\rvf^1_i) =  \left (\frac{1}{(d_i+1)}+\frac{(2h_i-1)d_i}{M_i\sqrt{(d_i+1)}}\right )\E(\rvf^0_i)
% \E(\rvf^1_i) =  \left (\frac{(2h_i - 1) d_i \ratioi + 1}{d_i + 1}\right )\E(\rvf^0_i) \equiv \gamma_i^1 \E(\rvf^0_i), \label{eq:factor}
% \end{equation}
% % where the multiplicative factor $\gamma_i^1$ is: %follows:
% \vspace{-0.2cm}
% \begin{equation}
% \text{where } \gamma_i^1 \in 
% \begin{cases}
%   (-\infty, \frac{1}{2}], & \text{if}\ h_i\leq0.5 \\
%   (\frac{1}{2}, 1], & \text{if}\ h_i>0.5 \ \mathrm{\&}\  \ratioi \leq \frac{1}{2h_i-1}\\
%   (1, \infty), & \mathrm{otherwise}.
% \end{cases}
% % \begin{cases}
% %   \gamma_i^1 \leq \frac{1}{2}, & \text{if}\ h_i\leq0.5 \\
% %   \frac{1}{2} < \gamma_i^1 \leq 1, & \text{if}\ h_i>0.5 \ \mathrm{and}\  \ratioi \leq \frac{1}{2h_i-1}\\
% %   \gamma_i^1 > 1, & \mathrm{otherwise}.
% % \end{cases}
% \label{eq:initial_stage}
% \end{equation}
% % Whether the mean vector moves towards or away from the origin is decided by as follows:
% % \vspace{-0.2cm}
% % \begin{equation}
% % \begin{cases}
% %   \|\E(\rvf^1_i)\| \leq \frac{||\E(\rvf^0_i)||}{2}, & \text{if}\ h_i\leq0.5 \\
% %   \|\E(\rvf^1_i)\| \leq ||\E(\rvf^0_i)||, & \text{if}\ h_i>0.5\\ & \mathrm{and} \ \ratioi \leq \frac{1}{2h_i-1}\\
% %   \|\E(\rvf^1_i)\| > ||\E(\rvf^0_i)||, & \text{otherwise}
% % \end{cases}
% % \label{eq: initial_stage}
% % \end{equation}
% {For independent features $\rvf^0_i$,} the variance of each node is reduced to $\frac{1}{(d_i+1)} \left ( \frac{1}{(d_i+1)}+\sum_{j \in \gN_i}{\frac{1}{(d_j+1)}} \right )\rvSigma \leq \frac{1}{2}\rvSigma$. %, which is bounded by $\frac{1}{2}\rvSigma$. 
% \label{theorem: initial_stage}
% \end{theorem}
% \vspace{-0.4cm}
% \begin{proof}
% We provide the proof in App.~\ref{app:proof1}.
% \end{proof}
% % Avid readers can refer to the Appendix~\ref{app:proof1} for the complete proof. 

%\vspace{-0.4cm}
 % vector.

%We note that our analysis shows that the variance of \textit{each node} is reduced in the initial stage regardless of the homophily level. 
%However, this does \textit{not} mean that the variance of the nodes in the same \textit{class} is reduced. 
%The class variance %of the class 
%is decided not only by the node variance %of each node 
%but also how dispersed their mean is. 
%\reminder{mention at the end of 3.1.1?}

% \yaoqing{I now understand what you are trying to do. I think the paper should be much clear at the beginning on the several assumptions.}
\vspace{-0.5cm}
\subsubsection{Developing Stage: Deeper Layers}
\label{sec:developing-stage}
\vspace{-0.2cm}
% Based on Eqs.~(\ref{eq:factor})-(\ref{eq:initial_stage}), after propagation in several layers, the features of low-homophily nodes, and those of high-homophily but low-degree nodes may flip their labels. 
{The following theorem analyzes the pseudo-heterophily scenario in deeper layers. Based on Thm.~\ref{theorem: initial_stage}, message passing will result in scaling the node representations ($\gamma_i^1$) and some nodes may cross the origin. To account for those, 
let $\xi^l_i$ be an accumulated discount factor at the $l$-th layer and \textcolor{blue}{ $\mathbb{E}_{\rmA,\{y_i\},\{\rvf_i^{(0)}\}|d_i}\left (\frac{\mathbf{f}_i^{(l)}}{d_i+1}|d_i \right )=\xi_{i}^l\rvmu$.
\vspace{-0.25cm}
% $$\E(\rvf_i^{(l)}) = \begin{cases}\xi^l_i\E(\rvf_i^{(0)}), & \text{if node }v_i\text{'s expected representation does not cross the origin.} \\
% % -\rho\xi^l_i\rvf_i^{(0)} & \text{if node }v_i\text{ is from class 1 and its representation moves across the origin.} \\
% % -\frac{1}{\rho}\xi^l_i\rvf_i^{(0)} & \text{if node }v_i\text{ is from class 2 and its representation moves across the origin.}
% -\frac{|\gV_{y_i}|}{|\gV \setminus \gV_{y_i}|}\xi^l_i\E(\rvf_i^{(0)}), & \text{if node }v_i\text{'s expected representation moves across the origin.}
% \end{cases}
% \vspace{-0.3cm}
% $$}
Conditioned on $\rmA$ and $\xi_{i}^l$, the nodes contributing positively are defined as: $\hat{\mathcal{N}_i^s}(\rmA, \xi_{i}^l) \equiv 
% \{v_j|\E_{\{y_i\},\{\rvf_i^{(0)}\}|\mathbf{f}_i^{(l)}, \rmA, v_j \in \gN_i}\left(\rvf_i^{(l)}|\mathbf{f}_i^{(l)}, \rmA, v_j \in \gN_i\right)
\{v_j|v_j \in \gN_i \text{ and } (\xi_{i}^l\rvmu) \cdot \E_{\{y_i\},\{\rvf_i^{(0)}\}|\xi_{i}^l, \rmA}\left({\rvf_j^{(l)}}^T|\xi_{i}^l, \rmA\right)>0\}$.
We denote: $\mathbb{E}_{\rmA,\{y_i\},\{\rvf_i^{(0)}\}|d_i,\xi_{i}^l, v_j \in \gN_i}\Bigg(\mathbf{f}_j^{(l)}r_{ij}|d_i, \xi_{i}^l, v_j \in \gN_i\Bigg)=\begin{cases}
{\xi_{i}^{l}}'\rvmu & v_j \in   \hat{\mathcal{N}_i^s}(\rmA, \xi_{i}^l) \\
-\rho_{i}^{l}{\xi_{i}^{l}}'\rvmu & v_j \not\in   \hat{\mathcal{N}_i^s}(\rmA, \xi_{i}^l)
\end{cases}$}. ${\xi_{i}^{l}}'$ and $\rho_{i}^{l}$ characterize the neighborhood property of $v_i$.}
% Assuming initial features $\rvf^0_i$, propagation through $l$ layers, and accumulated discount factor at the $l$-th layer  $\gamma^l_i > 0$, we denote the sign-flipping features as $\rvf^l_i=-\gamma^l_i \rvf^0_i\rmW^{e}$, and the remaining features as 
% $\rvf^l_i=\gamma^l_i \rvf^0_i\rmW^{e}$, {where $\rmW^{e}$ is a weight matrix that is equivalent to multiplying all of the weight matrices up to the $(l-1)$-th layer}.
% Suppose we have propagated through $l$ layers of the network, starting from initial features $\rvf^0_i$. 
% We denote sign-flipping features as $\rvf^l_i=-\gamma^l_i \rvf^0_i$, where $\gamma^l_i > 0$ is the accumulated discount factor at layer $l$ due to previous propagation. 
% Likewise, for the nodes whose features do not flip their sign, we have: $\rvf^l_i=\gamma^l_i \rvf^0_i$. 
% \vspace{-0.2cm}
{We further define the \textbf{effective homophily} of node $i$ as  \textcolor{blue}{$\hat{h_i^{l}}=\sP(v_j \in \hat{\mathcal{N}_i^s}|v_j \in \gN_i, d_i, \xi_{i}^l)$.} 
% where the expectation is taken over the randomness of the node labels. 
Intiuitively, even if the original graph is not heterophilous, from the perspective of message passing under this pseudo-heterophily scenario, the deeper layers will act as if the graph is more heterophilous than it truly is, which may increase the misclassification rate.}
% of node $v_i$  as the ratio of the neighbors that have the same sign as $v_i$ at the $l$-th layer.
%class and have \textit{not flipped} their sign at the  $l$-th layer. 
% Similar to the analysis in the initial stage, we have:

% For example, from $\rvf^0_i$ to $\rvf^l_i=-\gamma^l_i \rvf^0_i, \gamma^l_i>0$, $\gamma^l_i$ represents the accumulated discount factor at layer $l$ due to the propagation from previous layers. For the nodes whose features do not flip the sign, we have: $\rvf^l_i=\gamma^l_i \rvf^0_i, \gamma^l_i>0$. We denote the effective homophily $\heterophilyil$ as the ratio of the nodes that are of the same class and have \textit{not flipped} the sign at the  $l$-th layer. Then similar to the analysis in the initial stage, we have:


\begin{theorem}
\textbf{[Developing Stage]} {Under the ``non-swapping condition'', during} message passing in deeper layers, when the effective homophily $\heterophilyil$ is sufficiently \textbf{low} $(\heterophilyil \leq \frac{\rho_{i}^{l}}{1+\rho_{i}^{l}})$, the nodes with \textbf{higher} effective relative degree
are prone to misclassification. \textcolor{blue}{Specifically, by defining the effective relative degree as} $\bar{r_i}^{l}\equiv \frac{{\xi_{i}^{l}}'}{{\xi_{i}^{l}}}$, the conditional expectation of $\rvf_i^{(l+1)}$ is: 
% after the operation $\tilde{\rmA}\rmF^{l}$ 
% \yy{(suppose $v_i$ is from target class and $\rvf_i^{l+1} \cdot {\rvf_i^{0}}^T>0$):}
\vspace{-0.2cm}
\begin{equation}
% \E(\rvf_i^{l+1}) = \left (\frac{1}{(d_i+1)}-(1-\hat{2h_i^l})\cdot \frac{d_i\cdot \gamma^l_j}{M_i \cdot \sqrt{(d_i+1)}}\right )\E(\rvf_i^{l})
% \E(\rvf_i^{l+1}) = \left (\frac{1}{(d_i+1)}+\frac{(\hat{2h_i^l} - 1) d_i \gamma^l_j}{M_i \sqrt{(d_i+1)}}\right )\E(\rvf_i^{l})
{\mathbb{E}_{\rmA,\{y_i\},\{\rvf_i^{(0)}\}|d_i,\xi_{i}^l)}\Bigg(\mathbf{f}_i^{(l+1)}|d_i,\xi_{i}^l)\Bigg) = \frac{\left((\hat{h_i^{l}}(1+\rho_{i}^l)-\rho_{i}^l)d_i\bar{r_i}^{l}+1\right)}{d_i+1}\xi_{i}^l\rvmu \equiv \gamma_i^{(l+1)}\E(\rvf_i^{(0)}).}
\label{eq: developing stage}
\end{equation}
\label{theorem: developing stage}
\vspace{-0.2cm}
\end{theorem}
\vspace{-0.6cm}
\begin{proof}
We provide the proof in App.~\ref{app:proof2}. Other nodes can be derived similarly.
%The derivation is similar to that of Theorem~\ref{theorem: initial_stage} except that we replace the ground truth heterophily $h_i$ with the effective heterophily $\heterophilyil$ and $\E(\rvf_i^{l})$ with $\gamma^l_i\E(\rvf_i^{0})$. Since graph $\gG$ is connected, the node degrees $d_i \geq 1$; thus, $\frac{d_i}{d_i+1}$ and $\ratioi$ are increasing functions of $d_i$, while $\frac{1}{d_i+1}$ is a decreasing function of $d_i$. When $\heterophilyil \leq 0.5$, we have $(2\heterophilyil - 1) \leq 0$, and $(2\heterophilyil - 1) \cdot \frac{d_i}{d_i+1} \cdot \ratioi + \frac{1}{d_i+1}$ is a decreasing function of $d_i$ in Eq.~(\ref{eq: developing stage}). This suggests that the higher-degree nodes move towards the opposing class more.
\vspace{-0.2cm}
\end{proof}
\vspace{-0.25cm}
{We note that Eq.~(\ref{eq: developing stage}) holds for layers $l \geq 2$ in general. We regard layers for which $\heterophilyil > \frac{\rho_{i}^{l}}{1+\rho_{i}^{l}}$ holds for most nodes $i$ as
% up to the layer when the effective homophily $\hat{h_i^l}$ becomes smaller or equal to $\frac{\rho}{1+\rho}$ for all the nodes. 
% {We regard these layers 
part of the initial stage, as they exhibit three cases similar to Eq.~(\ref{eq:initial_stage}).}
%In those layers, we have three cases similar to Eq.~(\ref{eq:initial_stage}) and we regard them part of the initial stage.}

%Tracing how $\E(\rvf^l_i)$ and $\sV(\rvf_t^{l})$ will change after the message propagation will help us better understand whether the node features will be easier to separate. In our case where the data is drawn from two Gaussians with opposite means, moving $\E(\rvf_t^{l})$ away from the opposing mean towards the true class mean, along with a reduced $\|\sV(\rvf_t^{l})\|$, is beneficial for the node classification task. In particular, it means that they become more linearly separable. 
\vspace{-0.2cm}
% \subsubsection{Implications from Theoretical Results} 
% \label{sec:summary-theory}
% \vspace{-0.2cm}
% Three conjectures follow from Thm.~\ref{theorem: initial_stage} and~\ref{theorem: developing stage}:
% %\vspace{-0.3cm}
% %\begin{enumerate}
% % \vspace{-0.1cm}  
% \textbf{(1)} After message propagation, the mean vectors $\E(\rvf^1_i)$ will be dispersed. For a high-homophily graph, in the initial stage, the features of \textit{low}-degree nodes (where $\ratioi \ll \frac{1}{(1+\rho)h_i-\rho}$) will first move towards the opposing class mean and have relatively lower accuracy (case 2). Later, when propagating to more layers, if the accuracy of low-degree nodes drops to a level such that the $\hat{h_i^l}$ of higher degree nodes satisfies $\heterophilyil \leq \frac{\rho}{1+\rho}$, then their features begin to move towards the opposing class mean vector (case 1) because $((1+\rho)\heterophilyil-\rho) \leq 0$ in Eq.~(\ref{eq: developing stage}).
%     % Later, when propagating to more layers, the accuracy of low degree nodes drop to a level such that the effective homophily  of higher degree nodes satisfies: $\heterophilyil \leq 0.5$, then the \textit{larger} degree $d_i$ compared to $M_i$, the larger $\frac{d_i\cdot \gamma^l_j}{M_i \cdot (d_i+1)^{\frac{1}{2}}}$ is and the smaller $\|\E(\rvf_i^{l+1})\|$ is (Equation~\ref{eq: developing stage}). We will show this phenomenon in the experiments.
    
% \textbf{(2)} GCNs perform differently on graphs with different degree distributions. For homophily graphs with power-law distribution (with many low-degree nodes), the performance of low-degree nodes will degenerate fast in the initial stage and the model will quickly enter the developing stage. Then, due to few high-degree nodes, the performance will degenerate more slowly. % will be slowed down.

% \textbf{(3)} The normalization scheme of the adjacency matrix of a graph makes a difference. 
% The reason that node degrees appear in Eqs.~(\ref{eq:initial_stage})-(\ref{eq: developing stage}) is the renormalization trick on $\rmA$ in GCN (\S~\ref{section: background}). Another normalization scheme such as row-normalization makes the scenario equivalent to a $d$-regular graph where nodes have the same degree (App.~\ref{app:proof1}). 

% scheme for the graphs also makes a difference. The reason that node degrees are involved in Equations~(\ref{eq:initial_stage})-(\ref{eq: developing stage}) is due to the renormalization scheme (Section~\ref{section: background}). If another normalization scheme is used, e.g. row-normalization, then the scenario is equivalent to a d-regular graph where nodes have the same degree (Appendix~\ref{app:proof1}). 
% \end{enumerate}
% \vspace{-0.3cm}
% Based on the analysis above, we can explain the GCN behavior in various settings: when a shallow GCN model is trained with a high-homophily graph, the increased mean distances between the large-degree nodes of different classes and the reduction in the variance lead to performance gain; when the model becomes deeper or is trained with a low-homophily graph, the reduction in the mean distances between the low-degree nodes becomes dominant and leads to degenerated performances.

% \vspace{-0.3cm}
\subsection{Signed Messages \& Movements of Representations}
\label{subsec: sign_theory}
\vspace{-0.1cm}
% Attention-based GCN models~\citep{velivckovic2017graph} typically use \textit{non-negative} attention weights to discount the contribution from dissimilar neighbors. {Though some concurrent works~\citep{chien2021adaptive, bo2021beyond} use negative attention weights, they do not to provide theoretical justifications. 
{In this section, we provide theory to show \reminder{when} %that 
signed messages can help enhance the performance in heterophilous graphs and  alleviate oversmoothing.}
%  the oversmoothing problem. 
Due to limited space,
% space limitations, 
we only show the effect of signed messages in the initial stage; similar results can be derived in the developing stage. % can be derived similarly.

\textbf{Setup.} %Consider the following scenario: 
% Consider the scenario where 
Signed messages consist of the negated messages sent by neighbors of the opposing class (i.e., after multiplying initial messages by -1), 
%multiplied by a negative sign 
and the unchanged messages ("positive messages") sent by neighbors of the same class. {In reality, ground-truth labels are not accessible for every node, so we use approximations, which introduces errors.}
% ``messages'' as they are. 
For node $v_i$, we define $m_i^l$ as the \textit{ratio of neighbors that send incorrect messages} at the $l$-th layer (i.e., different-class neighbors that send non-negated messages %without being multiplied by a negative sign 
and same-class neighbors that send negated messages). %multiplied by a negative sign). 
We define the $l$-th layer \textit{error rate} as $e_i^l=\E(m_i^l)$, where the expectation is over the randomness of the neighbors that send incorrect messages. We make the following assumption: $m_i^l$ is independent of $\{d_i\}$, $\{y_i\}$ and $\{\rvf_i^{0}\}$.
%We assume the expectation is the same for all the nodes.
% We make two  assumptions:
% \vspace{-0.2cm}
% \begin{enumerate}
    % \item 
    % (1)~Conditioned on $m_i^l$, whether the neighbor $v_j$ will wrongly send the information is independent of its class $y_j$; 
    % % \item 
    % (2)~The variable $m_i^l$ is independent of the classes that nodes $v_j\in\gN_i$ belong to.
% \end{enumerate}
\begin{theorem}
\textit{\textbf{[Signed Messages]}} With the independence assumptions and {under the ``non-swapping condition'',} by allowing the messages to be optionally multiplied by a negative sign, in the initial stage, the {movements of representations} will {\textbf{be less affected} by the initial homophily level $h_i$, and will be dependent on the \textbf{error rate} $e_i^l$}. Specifically, the multiplicative factor $\gamma_i^1$ at the first layer is:
\vspace{-0.1cm}
\begin{align}
% \E(\rvf^1_i) = (\frac{1}{(d_i+1)} + (1-2e_i^0) \frac{d_i}{M_i\cdot (d_i+1)^{\frac{1}{2}}})\E(\rvf^0_i)
&\E_{\rmA, \{y_i\}, \{\rvf_i^{(0)}\}|d_i, v_i \in \gV_1}(\rvf^{(1)}_i|d_i, v_i \in \gV_1) =  \\  
&\;\;\;\;\left ( \frac{(1 - 2e_i^0)(\rho+(1-\rho)h_i)d_i\ratioi + 1}{d_i+1}\right )\rvmu 
\equiv \gamma_i^1 \E(\rvf^{(0)}_i), \nonumber
\label{eq:signed_messages}
\vspace{-0.5cm}
\end{align}
\begin{equation}
\vspace{-0.1cm}
\text{where } \gamma_i^1 \in 
\begin{cases}
  (-\infty, \frac{1}{2}], & \text{if}\ e_i^0 \geq 0.5 \\
  {(0, 1]}, & \text{if}\ e_i^0 < 0.5 \ \mathrm{\&}\  \ratioi \leq \frac{1}{(1 - 2e_i^0)(\rho+(1-\rho)h_i)}\\
  (1, \infty), & \mathrm{otherwise}.
% \begin{cases}
%   \gamma_i^1 \leq \frac{1}{2}, & \text{if}\ e_i^0 \geq 0.5 \\
%   \frac{1}{2} < \gamma_i^1 \leq 1, & \text{if}\ e_i^0 < 0.5 \ \mathrm{and}\  \ratioi \leq \frac{1}{1 - 2e_i^0}\\
%   \gamma_i^1 > 1, & \mathrm{otherwise}
%   ||\E(\rvf^1_i)|| \leq \frac{||\E(\rvf^0_i)||}{2}, & \text{if}\ e_i^0\geq0.5 \\
%   ||\E(\rvf^1_i)|| \leq ||\E(\rvf^0_i)||, & \text{if}\ (e_i^0<0.5)\\ & \& \ (d_i \leq (\frac{M_i}{1-2e_i^0})^2-1)\\
%   ||\E(\rvf^1_i)|| > ||\E(\rvf^0_i)||, & \text{otherwise}
\end{cases}
\label{eq: signed_message_initial_stage}
\end{equation}
\label{theorem: signed_messages}
\end{theorem}
\vspace{-0.7cm}
\begin{proof}
The proof is provided in App.~\ref{app:proof3}.
\end{proof}

\vspace{-0.4cm}
{
% Given $h_i \leq 1$, we have $\frac{1}{(1+\rho)h_i-\rho} \geq \frac{1}{\rho+(1-\rho)h_i}$. 
From Eq.~\ref{eq: signed_message_initial_stage}, we see that when using signed messages, to benefit from case 3 ($\gamma_i^1>1$), the minimum relative degree satisfies: $\ratioi > \frac{1}{(1 - 2e_i^0)(\rho+(1-\rho)h_i)}$. Given $h_i \leq 1$, if the error rate is low ($e_i^0 \ll 0.5$),  we get: $\frac{1}{(1 - 2e_i^0)(\rho+(1-\rho)h_i)} \leq \frac{1}{(1+\rho)h_i-\rho}$, and $\frac{1}{(1+\rho)h_i-\rho}$ is the minimum relative degree required when not using signed messages.
This implies that more nodes can benefit from using signed messages. 
\ul{We note that if low error rate cannot be guaranteed, signed messages may hurt the performance.}}
% From Eq.~(\ref{eq:signed_messages}), we conclude that:
% % \vspace{-0.3cm}
% % \begin{enumerate}
%     % \item
%     \textbf{(1)} Allowing neighbors of a different class to negate their messages prevents low homophily from degenerating performance.
%     % If we allow the neighbors of a different class to send information but be multiplied with a negative sign, then low homophily will not degenerate the performance. 
%     For a model that achieves low error rate at shallow layers (i.e, $e_i^0 \ll 0.5$), the low-degree nodes ($\ratioi \ll \frac{1}{1 - 2e_i^0}$) trigger oversmoothing. 
%     % \item
%     \textbf{(2)}~If a model does not work well under heterophily (i.e., high error rate $e_i^l$ in identifying neighbors from other classes), 
%     % in the heterophily setting, i.e., they have a higher error rate $e_i^l$ in identifying neighbors from another class, the model will be 
%     it is prone to oversmoothing even  in shallow layers. 
% \end{enumerate}


% \subsection{Additional Considerations \reminder{appendix?}} 
% % \vspace{-0.3cm}
% % \begin{enumerate}

% \textbf{On Batch norm vs.\ Layer norm.} % Whether it is beneficial to use batch norm or whether the trained weights can compensate for the shrinking distances. 
% Batch norm and trained weights cannot compensate for the dispersion of the mean vectors due to different degrees and homophily levels of the nodes. Though to some extent, it reduces the speed of the feature vectors of the susceptible nodes moving towards the other class (good for oversmoothing), it also prevents the feature vectors of the nodes who were supposed to gain from the propagation from increasing the distances (drop in accuracy). We find in our experiments (\S~\ref{section: experiments}) that, in general, adding batch norm significantly decreases the accuracy in heterophily datasets, but helps alleviate oversmoothing. Layer norm is a better option~\citep{zhou2020understanding} for oversmoothing and leads to smaller accuracy drop compared to batch norm in most datasets. However, in our experiments, layer norm has a significant accuracy drop for some datsets when some features are more important than the others.

% suggestion from Google reviewer
% \textbf{Generalization.} So far we have shown theoretical results on a binary classification task. However, this approach is general and can be applied to multi-class classification as well. In the next section we show the experiments on standard multi-class classification datasets.

% \textbf{Variance reduction.} In the analysis, we show that the variance of \textit{each node} is reduced in the initial stage regardless of the homophily level. However, it does not mean that the variance of the nodes in the same \textit{class} is reduced. The variance of the class is decided not only by the variance of each node but also how dispersed their mean is. \reminder{mention at the end of 3.1.1?}
% \end{enumerate}

==> sections/theoretic_analysis_with_comments-Sep2021.tex <==
\vspace{-0.2cm}
\section{Theoretical Analysis\yy{not mention linear separability}}
\label{section: analysis}
\vspace{-0.2cm}
In this section, we analyze the theoretical connections between \yy{oversmoothing and heterophily problems in node classification tasks. Both problems result in degenerated GCNs'performance. We find that the movements of node representations reflect the chances of nodes to be misclassified and are a good indicator of GCNs' performance.
Thus, we characterize in expectation how node representations move and change over the layers and use the movements of representations to explain the oversmoothing and heterophily problems. }
% {At a high level, we focus on the node classification task and we use the \textit{linear separability} of learned node representations as an indicator of GCN performance. Intuitively, linear separability is the smallest distance between node representations of opposite classes. 
% By studying the movements of node representations after propagation and aggregation in GCNs, we characterize how linear separability 
% is changed over the layers.
We identify two causes, i.e., the level of homophily of a node and the relative degree between a node and its neighbors, which  
\yy{determine the movements of node representations. Specifically, moving towards (away from) another class leads to higher (lower) misclassification rate and worse (better) classification performance if the movements do not swap the positions of the two classes.}
%a limited portion of nodes are allowed to cross the decision boundary.}
% the linear separability of learned representations. Specifically, the two causes determine if the node representations will tend to move towards the initial mean feature vector of the opposing class (becoming less linearly separable) or away (becoming more linearly separable). 
Our analysis highlights that \yy{the oversmoothing and heterophily problems result from a limited portion of nodes move towards another class induced by high heterophily level and low relative degree.}

\yy{Version 2: In this section, we will first introduce the definitions and assumptions. Next we analyze the theoretical connections between oversmoothing and heterophily problems in two steps: (1) We show how the movements of node representations relate to the misclassification rate of node labels. (2) We identify the factors that affect the movements of representations.}

\yaoqing{At this stage, I think the readers will be completely confused by what you are trying to say. We can probably move the last sentence after our analysis and put that as a remark.}
% both the oversmoothing problem and the heterophily problem result from \textit{less linear separability} induced by these two causes.
%Moreover, we show that signed messages help reduce the effect from the factors.


%Our analysis highlights that both the oversmoothing problem and the heterophily problem result from \textit{less linear separability} of learned representations for nodes in different classes after graph convolution.
%we analyze the impact of message propagation in the node classification task, and show how the oversmoothing  and heterophily problems are related. We also discuss the implications of our analysis, which provide valuable insights for designing our model, \method, in \S~\ref{section: model_design}. %\yy{Move using linear GCN layers to settings.}


%\subsection{Settings \& Definitions}
% \label{subsec: notations}

% We consider a binary node classification task on an unweighted self-loop-free graph with adjacency matrix $\rmA$. 
% We denote the set of nodes in the first class and the second class as $\gV_1$ and $\gV_2$, respectively.

\yaoqing{A general comment. I think we are confusing ourselves with definitions and assumptions. There are a lot of definitions below which belong to the notation section. The assumptions, such as E(f)=0, should be separated from these.}

{\textbf{Assumptions.} In 
%$|\gL|$ balanced classes (same number of nodes in each class) in a node classification task. 
a multi-class node classification task,
we assume: 
\yy{(1) Graph generation process: (1.1) Node labels $\{\chi(v_i)\}$ and degrees $\{d_i\}$ are deterministic. (1.2) Node connections are randomly determined: for an arbitrary node $v_i$, it connects to $k_i$ neighbors randomly chosen from the same class and $(d_i-k_i)$ neighbors randomly chosen from other classes, where $k_i$ follows the discrete uniform distribution of range $[0, d_i]$.\yaoqing{Is there an inherent assumption that the number of nodes in each class is larger than $d_i$? Otherwise, what if one node does not have enough nodes from a class to connect?}
(1.3) Node features of the same (different) class are drawn from the same (different) distribution(s). \yaoqing{Shall we define these distributions here?} (2) The initial features are centered, i.e., $\E(\sum{\rvf_i^0})=\mathbf{0}$} \yaoqing{Shall we give some motivations on why these features are centered?}
% (1) The initial features are centered, i.e., $\sum{\rvf_i^0}=\mathbf{0}$; (2) Given an arbitrary node $v_i$, for any node $v_j$ s.t. $\chi(v_i)\neq \chi(v_j)$, the probability of connecting to $v_i$ is equal; (3) 
(3) Following prior work~\citep{li2018deeper, oono2019graph, chen2020simple}, \yy{we analyze SGC~\citep{wu2019simplifying}} but show empirically that our results still apply to non-linearized GCNs (\S~\ref{section: experiments}). \textbf{Simplifications.} We analyze the dynamics of $\rvf_i$ in each class in a one-vs-rest fashion. \yaoqing{Shall we clarify? I don't think the readers will understand what it means by the dynamics of xxx and "one-vs-rest fashion".}
Without loss of generality, we choose class 1 as the target class and assume $\rvf_i^0$ of class 1 follows \yy{a distribution with a probability density function (PDF) $f_1(\rvx)$ and mean $\rvmu$}. Given \yy{assumption 1.2}, $\rvf_i^0$ in the other classes can be viewed as drawing from a virtual class (`rest'). \yaoqing{What does this mean? Is this related to the so called "one-vs-rest fashion"? If what you mean is that you want to study binary classification, you probably want to just say that you study binary classification, because one-vs-rest is not the same as binary classification. If you are indeed able to study multi-class classification, you can define class 1 and the rest as $C_1$ and $\bar C_1$.}
We denote the set of nodes in the first and the virtual class \yaoqing{Also, avoid using a word that you are not familiar with. If this word is not something written in a text book and you invented it, ML people will think this is not appropriate.} as $\gV_1$ and $\gV_2$. \yy{Given assumption (2)}, the virtual class follows a distribution with \yy{a PDF $f_2(\rvx)$ and} mean $-\pi\rvmu$, $\pi=\frac{|\gV_1|}{|\gV_2|}$. Usually, $0<\pi\leq 1$.\yaoqing{What does "usually" mean?} Thus, the analysis reduces to analyzing two classes.}

\yy{\textbf{Misclassification rate \& movements of $\rvf_i$.} The following lemmas illustrate why movements of node representations are a good indicator of SGC' performance. Proofs are in App.~\ref{app:lemma_1} and \ref{app:lemma_2}}.
\yy{SGC can be viewed as applying logistic regression to the last layer features $\rvf_i^{L}$, so we have:}

\yy{\textbf{Lemma 1} The decision boundaries w.r.t. $\rvf_i^{L}$ of SGC are linear.}

\yaoqing{I am completely confused. I think we now have a lemma before we even defined the things in it. What does "movement" mean? What is a decision boundary? What does it mean to have a linear decision boundary? Also, avoid using things like "SGC can be viewed as applying logistic regression". People won't understand what you mean.}

\yy{\textbf{Definition} The misclassification rate of a node set $\gV$ is: $\E(\hat{\chi}(v_i) \neq \chi(v_i))$, $v_i \in \gV$. }

\yaoqing{What is the expectation over? The randomness in the random attachment model? The noise in SGD? The initialization of model weights? Or all of them?}

% \yy{Denote the hyper-plane $\rvx\rvw+b=0$ as the decision boundary of the $\rvf_i^{l}$ that separates the nodes from the target class (predicted as the target class if $\rvx\rvw+b>0$) and the 'rest' class.
\yaoqing{Is the following paragraph a proof?}
\yy{Denote the hyper-plane $\rvx\rvw+b=0$ as the decision boundary of the $\rvf_i^{l}$ that separates the nodes from the target class and the 'rest' class, \yaoqing{Do you mean "the decision boundary in the space of $\rvf_i^{l}$"? I think it is better to define the space.} where $\rvw$ is a unit vector, $b$ is a scalar and the $\rvf_i^{l}$ is classified to the target class if $\rvf_i^{l}\rvw+b>0$).
% The misclassification rate for the target class ('rest' class) is: $\int_{\rvw^T\rvx+\rvb<\mathbf{0}}{f_1(\rvx)d\rvx}$ ($\int_{\rvw^T\rvx+\rvb>\mathbf{0}}{f_2(\rvx)d\rvx}$). 
Suppose when $\rvw=\rvw^*$ and $b=b^*$, we find an optimal hyper-plane $\rvx{\rvw^*}+b^*=0$ which achieves the lowest total misclassification rate.
% $\int_{\rvw^T\rvx+\rvb<\mathbf{0}}{f_1(\rvx)d\rvx}+\int_{\rvw^T\rvx+\rvb>\mathbf{0}}{f_2(\rvx)d\rvx}$. 
The next layer representations $\rvf_i^{l+1}$ can be viewed as being moved from $\rvf_i^{l}$. \yaoqing{One thing that confuses is me is that I thought $\rvf_i^{l}$ is a random variable. However, what you mentioned here and in the following sounds like it is a fixed vector. Also, is w* fixed? If so, it is important to state at the beginning.} Due to the movements, the optimal $\rvw^*$ and $b^*$ become ${\rvw^*}'$ and ${b^*}'$. \yaoqing{I believe you are just defining new terms. If so, say that we denote the new optimal weights and bias as xxx, instead of saying that they become xxx.} In Lemma 2, we will show that \ul{under certain constraint, moving towards the original decision boundary will result in a non-decreasing total misclassification rate.}}

\yy{\textbf{Lemma 2} Moving $\rvf_i^{l}$ of the target class by adding $-t\rvw^*$, $t>0$, s.t. ${\rvw^*}^T{\rvw^*}'>0$, the new total misclassification rate is no less than the misclassification rate before the movements. }
\yaoqing{Why do we add a multiple of $w*$? What if the vector added is not a multiple of that?}

\yy{Note that the special case where the representations of the two classes swap positions (e.g, bipartite graphs \yaoqing{Why?}) violates the condition ${\rvw^*}^T{\rvw^*}'>0$ and leads to different conclusions. We refer to the condition ${\rvw^*}^T{\rvw^*}'>0$ as "non-swapping condition" and throughout the paper, we analyze SGC under the "non-swapping condition". Lemma 2 shows that \ul{under "non-swapping condition", if $\rvf_i^l$ moves towards the original decision boundary (or the other class), SGC tends to perform worse.}}\yaoqing{Isn't this just saying that the margin will be smaller?}

%\textbf{Setup.} We consider a binary node classification task on an unweighted, self-loop-free graph $\gG$ with adjacency matrix $\rmA$. 
% \yy{[Remove Gaussian assumption]}
%We denote the set of nodes in the first and second class as $\gV_1$ and $\gV_2$, respectively. When $v_i \in \gV_1$, $\rvf_i^0$ follows a 
%Gaussian 
%distribution with mean $\rvmu$ and variance $\rvSigma$, and when $v_i \in \gV_2$, $\rvf_i^0$ follows a distribution with $-\rvmu$ and $\rvSigma$. Our analysis uses GCN layers (\S~\ref{section: background}) without nonlinearities {and focuses on binary classification}, but we demonstrate empirically that our results still apply to general settings 
%to non-linear layers and multi-class classification 
 


% We denote the degree of node $v_i$ by $d_i$, and the degree matrix by $\rmD$ which is a diagonal matrix whose elements are degrees. 
% Denote $\gN_i$ as the set of nodes directly connected to $v_i$, i.e., its neighbors. We further denote $\gN^s_i$ the set of nodes that are in $\gN_i$ and have the same class as $v_i$. 
% We use a concept called homophily to represent the tendency of a node to have the same class as its neighbor. 
% Specifically, for the $i$-th node $v_i$, its homophily $h_i$ is defined as the proportion $h_i = \E(\frac{|\gN^s_i|}{|\gN_i|})$, where $\gN^s_i$ is the set of neighboring nodes that share the same label as $v_i$, $\vert \cdot \vert$ is the cardinality operator, and the expectation is taken over the randomness of the node labels.
%We further assume that the heterophily is a constant across all nodes, i.e., $h_i=h, \forall i$.

\vspace{-0.3cm}
\subsection{Heterophily \& Oversmoothing}
\label{subsec: heterophily_oversmoothing}
\vspace{-0.2cm}
{In the following theorems, we will show how relative degree $r_{ij}$ and homophily level $h_i$ will affect the movement of node representations in both shallow and deeper layers.}
\vspace{-0.3cm}
\subsubsection{Initial Stage: Shallow Layers}
\label{sec:initial-stage}
\vspace{-0.2cm}
\begin{theorem}
\textbf{[Initial Stage]} \yy{Under "non-swapping condition", during} message passing in shallow layers, the nodes with \textbf{low} homophily $h_i \leq \frac{\pi}{1+\pi}$ and the nodes with high homophily $h_i > \frac{\pi}{1+\pi}$ but \textbf{small} degree $d_i$ (w.r.t.\ their neighbors) are prone to be misclassified.
% Denote $M_i$ by $\frac{1}{M_i} \equiv \frac{1}{d_i}\sum_{j \in \gN_i}{\frac{1}{\sqrt{(d_j+1)}}}$.
Defining $r_{ij}\equiv\sqrt{\frac{d_i + 1}{d_j + 1}}$ and $\ratioi \equiv \frac{1}{d_i} \sum_{j \in \gN_i} r_{ij}$, the expectation of feature $\rvf_i^1$ is \yy{(suppose $v_i$ is from target class):}\yaoqing{I don't quite believe this. If the feature vector propagates through a matrix vector multiplication, wouldn't that change the direction of the feature vector? Do you just consider one linear matrix and all the nodes have the same mean vector? It's useful to clarify somewhere.}
% after operation $\tilde{\rmA}\rmF^{0}$ at layer 1 is:
% $\gamma_i^1 \E(\rvf^0_i)$, where $\gamma_i^l$ is a scalar and
\vspace{-0.2cm}
\begin{equation}
% \E(\rvf^1_i) =  \left (\frac{1}{(d_i+1)}+\frac{(2h_i-1)\sum_{j \in \gN_i}{\frac{1}{\sqrt{(d_j+1)}}}}{\sqrt{(d_i+1)}}\right )\E(\rvf^0_i)
% \E(\rvf^1_i) =  \left (\frac{1}{(d_i+1)}+\frac{(2h_i-1)d_i}{M_i\sqrt{(d_i+1)}}\right )\E(\rvf^0_i)
\E(\rvf^1_i) =  \left (\frac{((1+\pi)h_i-\pi) d_i \ratioi + 1}{d_i + 1}\right )\E(\rvf^0_i) \equiv \gamma_i^1 \E(\rvf^0_i), \label{eq:factor}
\end{equation}
where the multiplicative factor $\gamma_i^1$ is: %follows:
\vspace{-0.2cm}
\begin{equation}
\gamma_i^1 \in 
\begin{cases}
  (-\infty, \frac{1}{2}], & \text{if}\ h_i\leq \frac{\pi}{1+\pi} \\
  \yy{(\frac{1}{d_i+1}, 1]}, & \text{if}\ h_i>\frac{\pi}{1+\pi} \ \mathrm{\&}\  \ratioi \leq \frac{1}{(1+\pi)h_i-\pi}\\
  (1, \infty), & \mathrm{otherwise}.
\end{cases}
% \begin{cases}
%   \gamma_i^1 \leq \frac{1}{2}, & \text{if}\ h_i\leq0.5 \\
%   \frac{1}{2} < \gamma_i^1 \leq 1, & \text{if}\ h_i>0.5 \ \mathrm{and}\  \ratioi \leq \frac{1}{2h_i-1}\\
%   \gamma_i^1 > 1, & \mathrm{otherwise}.
% \end{cases}
\label{eq:initial_stage}
\end{equation}
% Whether the mean vector moves towards or away from the origin is decided by as follows:
% \vspace{-0.2cm}
% \begin{equation}
% \begin{cases}
%   \|\E(\rvf^1_i)\| \leq \frac{||\E(\rvf^0_i)||}{2}, & \text{if}\ h_i\leq0.5 \\
%   \|\E(\rvf^1_i)\| \leq ||\E(\rvf^0_i)||, & \text{if}\ h_i>0.5\\ & \mathrm{and} \ \ratioi \leq \frac{1}{2h_i-1}\\
%   \|\E(\rvf^1_i)\| > ||\E(\rvf^0_i)||, & \text{otherwise}
% \end{cases}
% \label{eq: initial_stage}
% \end{equation}
%{For independent features $\rvf^0_i$,} the variance of each node is reduced to $\frac{1}{(d_i+1)} \left ( \frac{1}{(d_i+1)}+\sum_{j \in \gN_i}{\frac{1}{(d_j+1)}} \right )\rvSigma \leq \frac{1}{2}\rvSigma$. %, which is bounded by $\frac{1}{2}\rvSigma$. 
\label{theorem: initial_stage}
\end{theorem}
\vspace{-0.6cm}
\begin{proof}
We provide the proof in App.~\ref{app:proof1}. The nodes from the 'rest' class can be derived similarly.
\end{proof}
\vspace{-0.3cm}
% {\textbf{Effects of multiplying weight matrices.} Theorem~\ref{theorem: initial_stage} shows that after performing $\tilde{\rmA}\rmF^{0}$, $\E(\rvf^1_i)$ will remain linearly dependent and the ratio of $\E(\rvf^1_i)$ to $\E(\rvf^1_j)$ is determined by the ratio of $\gamma_i^1$ to $\gamma_j^1$. Multiplying by the same weight matrices will transform $\rvf^1_i$ and class mean at the same time, but it will not change the ratio, and thus it will not affect the linear separability of $\rvf^1_i$.}

{From Thm.~\ref{theorem: initial_stage}, we identify three types of movements of node representations, which are characterized by relative degree $r_{ij}$ and homophily level $h_i$. In Fig.~\ref{fig:concept}, we illustrate the three cases when we have 1D node representations and perform binary classification. The bars reflect the value change of $v_i$'s node representation.} 
\yy{Intuitively, under heterophily (case 1) or under high homophily but low degrees (case 2), the expected feature vectors will move heavily towards the opposing class.}
% Intuitively, under heterophily (case 1), the expected feature vector will move heavily towards the opposing class.
% % the mean feature vector of the opposing class. 
% For high homophily but low degrees (case 2), it will contract towards the origin. 
Otherwise, they will move away from the opposing class (case 3). {Among the three cases, only nodes with high homophily and high relative degree  benefit from propagation and aggregation.}
% Unlike previous works~\citep{chen2020simple, wang2019improving} that focus more on the analysis of final node representations in the limit of infinite layers, we focus on the dynamic analysis of the node representations that are gradually passed to deeper layers.

\begin{figure*}[t]
\centering
\includegraphics[scale=0.21, bb=1025 0 300 250]{Figs/illustration_4.png}
\vspace{-0.2cm}
\caption{Node representation dynamics during neighborhood aggregation (1D), \yy{MR means misclassification rate}. The expectation of node representations (scalars) from class 1 \& 2 are denoted by $\mu$ and $-\mu$, respectively.
The bars show the expected node representations of node $v_i$ before and after the neighborhood aggregation. 
%We list out whether the change will make the node representations more or less linearly separable (LS) in the left table. Case 1 occurs when the homophily is low and is shown in the first sub-figure; case 2 occurs when the homophily is high but relative degree is low and is shown in the second sub-figure; case 3 occurs when the homophily and relative degree are both high and is shown in the third sub-figure.
\yaoqing{Shouldn't the expectation of node representation be a vector? Why are they scalars?}}
\label{fig:concept}
\vspace{-0.6cm}
\end{figure*}

% In this section we will demonstrate through 
%At a high level, our analysis highlights that both the oversmoothing problem and the heterophily problem result from \textit{less linear separability} of learned representations for nodes in different classes after propagation and aggregation across layers.
%Specifically, our theory demonstrates that---in expectation---the layer-wise transformation of a node's representation depends on two factors: (1) the level of homophily (proportion of neighbors with the same class label), and (2) the relative degree of the node (how many neighbors it has relative to its neighbors). These factors determine if the node representation will tend to move towards the initial mean feature vector of the opposing class (become less linearly separable) or away (become more linearly separable).  
%As shown in the left panel of Fig.~\ref{fig:concept}, in more detail:
{\textbf{Explanation of the heterophily and oversmoothing problems:}}
\begin{itemize*}
\vspace{-0.3cm}
    \item In heterophily graphs, node representations move heavily towards the opposite class. \yy{According to Lemma 2, under "non-swapping" condition, it indicates higher misclassification rate (poorer performance) of SGC.}
    % The severe decrease in the linear separability causes performance drop in shallow layers (case 1).
    \item In homophily graphs, high-degree nodes may initially benefit (case 3), leading to performance gain in shallow layers. However, the low-degree nodes \yy{tend to move towards the opposing class (case 2)
    % reduce the linear separability (case 2) 
    and eventually flip the labels. The misclassification of low-degree nodes causes a pseudo-heterophily situation (case 1) later.}
\end{itemize*}

% in heterophily (low homophily) graphs, the decrease in the linear separability is more severe, causing  performance drop even in shallow layers (Fig.~\ref{fig:concept}, case 1). In homophily graphs, high-degree nodes might initially benefit (Fig.~\ref{fig:concept} case 3), leading to performance gain in shallow layers, but the low-degree nodes will eventually reduce the linear separability (Fig.~\ref{fig:concept} case 2).


% \yy{Through the following theorems, we would like to point out: both oversmoothing and heterophily problems result from less linear separability after neighborhood aggregation. }
% \yy{In the high heterophilic graphs, the decrease in the linear separability is more severe, causing the performance drop even in shallow layers (Figure~\ref{fig:concept}, case 1). In homophily graphs, large-degree nodes might initially benefit (Figure~\ref{fig:concept} case 3), so we may see performance gain in shallow layers, but the low-degree nodes will eventually trigger the decrease in the linear separability (Figure~\ref{fig:concept} case 2).}

%\vspace{-0.3cm}
%\textbf{Theory.} T
%In more detail, the layer-wise message propagation and aggregation in GCNs is done via the $\tilde{\rmA}\rmF^l$ operation. Thus, for simplicity, our dynamic analysis 
%of the exchanged node representations 
%investigates the impact of this operation on the node class and its relation to the level of  homophily. However, the following conclusions still hold after scaling $\tilde{\rmA}\rmF^l$ by the learnable weight matrix $\rmW^l$. 
%Next, we consider two stages: the \textit{initial stage} at shallow layers of propagation and aggregation (\S~\ref{sec:initial-stage}), and the \textit{developing stage} at deeper layers (\S~\ref{sec:developing-stage}). 

% \yy{For clarity, we analyze the impact of $\tilde{\rmA}\rmF^l$, however, the scaling effect as we will point out later still hold after multiplied by the weight matrix $\rmW^l$.}

%\reminder{incorporate here and explain clearly} Recall the GCN formulation in the Section~\ref{section: background}, the main difference between GCN and standard multilayer perceptrons (MLPs) is the ``propagation and aggregation step'' done by multiplying the adjacency matrix $\tilde{\rmA}$ with the feature matrix $\rmF^{l}$. We will thoroughly discuss its effect in node classification and how it is related to the homophily of the nodes. 
% \vspace{-0.1cm}
% \subsubsection{Initial Stage: Shallow Layers}
% \label{sec:initial-stage}
% \vspace{-0.1cm}
% \begin{theorem}
% \textbf{[Initial Stage]} During message passing in shallow layers, the nodes with \textbf{low} homophily $h_i \leq 0.5$ and the nodes with high homophily $h_i > 0.5$ but \textbf{small} degree $d_i$ (w.r.t.\ their neighbors) are prone to be misclassified.
% % Denote $M_i$ by $\frac{1}{M_i} \equiv \frac{1}{d_i}\sum_{j \in \gN_i}{\frac{1}{\sqrt{(d_j+1)}}}$.
% Defining $r_{ij}\equiv\sqrt{\frac{d_i + 1}{d_j + 1}}$ and $\ratioi \equiv \frac{1}{d_i} \sum_{j \in \gN_i} r_{ij}$, the expectation of feature $\rvf_i^1$ after operation $\tilde{\rmA}\rmF^{0}$ at layer 1 is:
% \vspace{-0.2cm}
% \begin{equation}
% % \E(\rvf^1_i) =  \left (\frac{1}{(d_i+1)}+\frac{(2h_i-1)\sum_{j \in \gN_i}{\frac{1}{\sqrt{(d_j+1)}}}}{\sqrt{(d_i+1)}}\right )\E(\rvf^0_i)
% % \E(\rvf^1_i) =  \left (\frac{1}{(d_i+1)}+\frac{(2h_i-1)d_i}{M_i\sqrt{(d_i+1)}}\right )\E(\rvf^0_i)
% \E(\rvf^1_i) =  \left (\frac{(2h_i - 1) d_i \ratioi + 1}{d_i + 1}\right )\E(\rvf^0_i) \equiv \gamma_i^1 \E(\rvf^0_i), \label{eq:factor}
% \end{equation}
% % where the multiplicative factor $\gamma_i^1$ is: %follows:
% \vspace{-0.2cm}
% \begin{equation}
% \text{where } \gamma_i^1 \in 
% \begin{cases}
%   (-\infty, \frac{1}{2}], & \text{if}\ h_i\leq0.5 \\
%   (\frac{1}{2}, 1], & \text{if}\ h_i>0.5 \ \mathrm{\&}\  \ratioi \leq \frac{1}{2h_i-1}\\
%   (1, \infty), & \mathrm{otherwise}.
% \end{cases}
% % \begin{cases}
% %   \gamma_i^1 \leq \frac{1}{2}, & \text{if}\ h_i\leq0.5 \\
% %   \frac{1}{2} < \gamma_i^1 \leq 1, & \text{if}\ h_i>0.5 \ \mathrm{and}\  \ratioi \leq \frac{1}{2h_i-1}\\
% %   \gamma_i^1 > 1, & \mathrm{otherwise}.
% % \end{cases}
% \label{eq:initial_stage}
% \end{equation}
% % Whether the mean vector moves towards or away from the origin is decided by as follows:
% % \vspace{-0.2cm}
% % \begin{equation}
% % \begin{cases}
% %   \|\E(\rvf^1_i)\| \leq \frac{||\E(\rvf^0_i)||}{2}, & \text{if}\ h_i\leq0.5 \\
% %   \|\E(\rvf^1_i)\| \leq ||\E(\rvf^0_i)||, & \text{if}\ h_i>0.5\\ & \mathrm{and} \ \ratioi \leq \frac{1}{2h_i-1}\\
% %   \|\E(\rvf^1_i)\| > ||\E(\rvf^0_i)||, & \text{otherwise}
% % \end{cases}
% % \label{eq: initial_stage}
% % \end{equation}
% {For independent features $\rvf^0_i$,} the variance of each node is reduced to $\frac{1}{(d_i+1)} \left ( \frac{1}{(d_i+1)}+\sum_{j \in \gN_i}{\frac{1}{(d_j+1)}} \right )\rvSigma \leq \frac{1}{2}\rvSigma$. %, which is bounded by $\frac{1}{2}\rvSigma$. 
% \label{theorem: initial_stage}
% \end{theorem}
% \vspace{-0.4cm}
% \begin{proof}
% We provide the proof in App.~\ref{app:proof1}.
% \end{proof}
% % Avid readers can refer to the Appendix~\ref{app:proof1} for the complete proof. 

%\vspace{-0.4cm}
 % vector.

%We note that our analysis shows that the variance of \textit{each node} is reduced in the initial stage regardless of the homophily level. 
%However, this does \textit{not} mean that the variance of the nodes in the same \textit{class} is reduced. 
%The class variance %of the class 
%is decided not only by the node variance %of each node 
%but also how dispersed their mean is. 
%\reminder{mention at the end of 3.1.1?}

\yaoqing{I now understand what you are trying to do. I think the paper should be much clear at the beginning on the several assumptions.}
\vspace{-0.5cm}
\subsubsection{Developing Stage: Deeper Layers}
\label{sec:developing-stage}
\vspace{-0.2cm}
% Based on Eqs.~(\ref{eq:factor})-(\ref{eq:initial_stage}), after propagation in several layers, the features of low-homophily nodes, and those of high-homophily but low-degree nodes may flip their labels. 
\yy{The following theorem analyzes the pseudo-heterophily situation in deeper layers. Based on Thm.~\ref{theorem: initial_stage}, message passing will result in scaling of node features($\gamma_i^1$) and some nodes may cross the origin. To account for those, 
let $\xi^l_i>0$ be an accumulated discount factor at the $l$-th layer and
\vspace{-0.1cm}
$$\rvf_i^{l} = \begin{cases}\xi^l_i\rvf_i^0 & \text{if the nodes do not cross the origin.} \\
-\pi\xi^l_i\rvf_i^0 & \text{if the nodes from the target class move across the origin.} \\
-\frac{1}{\pi}\xi^l_i\rvf_i^0 & \text{if the nodes from the 'rest' class move across the origin.}\end{cases}
$$}
\vspace{-0.2cm}
% Assuming initial features $\rvf^0_i$, propagation through $l$ layers, and accumulated discount factor at the $l$-th layer  $\gamma^l_i > 0$, we denote the sign-flipping features as $\rvf^l_i=-\gamma^l_i \rvf^0_i\rmW^{e}$, and the remaining features as 
% $\rvf^l_i=\gamma^l_i \rvf^0_i\rmW^{e}$, {where $\rmW^{e}$ is a weight matrix that is equivalent to multiplying all of the weight matrices up to the $(l-1)$-th layer}.
% Suppose we have propagated through $l$ layers of the network, starting from initial features $\rvf^0_i$. 
% We denote sign-flipping features as $\rvf^l_i=-\gamma^l_i \rvf^0_i$, where $\gamma^l_i > 0$ is the accumulated discount factor at layer $l$ due to previous propagation. 
% Likewise, for the nodes whose features do not flip their sign, we have: $\rvf^l_i=\gamma^l_i \rvf^0_i$. 
\yy{We further define the \textbf{effective homophily} $\heterophilyil=\E(\frac{|\{v_j|\rvf_i^0\cdot {\rvf_j^l}^T>0, v_j \in \gN_i\}|}{|\gN_i|}).$} 
% of node $v_i$  as the ratio of the neighbors that have the same sign as $v_i$ at the $l$-th layer.
%class and have \textit{not flipped} their sign at the  $l$-th layer. 
% Similar to the analysis in the initial stage, we have:

% For example, from $\rvf^0_i$ to $\rvf^l_i=-\gamma^l_i \rvf^0_i, \gamma^l_i>0$, $\gamma^l_i$ represents the accumulated discount factor at layer $l$ due to the propagation from previous layers. For the nodes whose features do not flip the sign, we have: $\rvf^l_i=\gamma^l_i \rvf^0_i, \gamma^l_i>0$. We denote the effective homophily $\heterophilyil$ as the ratio of the nodes that are of the same class and have \textit{not flipped} the sign at the  $l$-th layer. Then similar to the analysis in the initial stage, we have:


\begin{theorem}
\textbf{[Developing Stage]} \yy{Under "non-swapping condition", during} message passing in deeper layers, when the effective homophily $\heterophilyil$ is sufficiently \textbf{low} ($\heterophilyil \leq \frac{\pi}{1+\pi}$), the \textbf{higher}-degree nodes %$d_i$ 
(w.r.t.\ its neighbors) %nodes 
are prone to misclassification. Specifically, defining $r_{ij}'\equiv r_{ij}\frac{\xi^l_j}{\xi^l_i}$ and $\ratioi' \equiv \frac{1}{d_i} \sum_{j \in \gN_i} r_{ij}'$, the expectation of $\rvf_i^{l+1}$ is 
% after the operation $\tilde{\rmA}\rmF^{l}$ 
\yy{(suppose $v_i$ is from target class and $\rvf_i^{l+1} \cdot {\rvf_i^{0}}^T>0$):}
\vspace{-0.2cm}
\begin{equation}
% \E(\rvf_i^{l+1}) = \left (\frac{1}{(d_i+1)}-(1-\hat{2h_i^l})\cdot \frac{d_i\cdot \gamma^l_j}{M_i \cdot \sqrt{(d_i+1)}}\right )\E(\rvf_i^{l})
% \E(\rvf_i^{l+1}) = \left (\frac{1}{(d_i+1)}+\frac{(\hat{2h_i^l} - 1) d_i \gamma^l_j}{M_i \sqrt{(d_i+1)}}\right )\E(\rvf_i^{l})
\yy{\E(\rvf_i^{l+1}) = \left (\frac{((1+\pi)\heterophilyil-\pi) d_i \ratioi' + 1}{d_i+1}\right )\xi^l_i\E(\rvf_i^{0}) \equiv \gamma_i^{(l+1)}\E(\rvf_i^{0}).}
\label{eq: developing stage}
\end{equation}
\label{theorem: developing stage}
\vspace{-0.2cm}
\end{theorem}
\vspace{-0.6cm}
\begin{proof}
We provide the proof in App.~\ref{app:proof2}. Other nodes can be derived similarly.
%The derivation is similar to that of Theorem~\ref{theorem: initial_stage} except that we replace the ground truth heterophily $h_i$ with the effective heterophily $\heterophilyil$ and $\E(\rvf_i^{l})$ with $\gamma^l_i\E(\rvf_i^{0})$. Since graph $\gG$ is connected, the node degrees $d_i \geq 1$; thus, $\frac{d_i}{d_i+1}$ and $\ratioi$ are increasing functions of $d_i$, while $\frac{1}{d_i+1}$ is a decreasing function of $d_i$. When $\heterophilyil \leq 0.5$, we have $(2\heterophilyil - 1) \leq 0$, and $(2\heterophilyil - 1) \cdot \frac{d_i}{d_i+1} \cdot \ratioi + \frac{1}{d_i+1}$ is a decreasing function of $d_i$ in Eq.~(\ref{eq: developing stage}). This suggests that the higher-degree nodes move towards the opposing class more.
\vspace{-0.2cm}
\end{proof}
\vspace{-0.3cm}
\yy{We note that Eq.~(\ref{eq: developing stage}) holds for layers $l \geq 2$ in general. For layers when $\heterophilyil > \frac{\pi}{1+\pi}$ is held for most nodes, we regard them as
% up to the layer when the effective homophily $\hat{h_i^l}$ becomes smaller or equal to $\frac{\pi}{1+\pi}$ for all the nodes. 
% {We regard these layers 
part of the initial stage, as they have three cases similar to Eq.~(\ref{eq:initial_stage}).}
%In those layers, we have three cases similar to Eq.~(\ref{eq:initial_stage}) and we regard them part of the initial stage.}

%Tracing how $\E(\rvf^l_i)$ and $\sV(\rvf_t^{l})$ will change after the message propagation will help us better understand whether the node features will be easier to separate. In our case where the data is drawn from two Gaussians with opposite means, moving $\E(\rvf_t^{l})$ away from the opposing mean towards the true class mean, along with a reduced $\|\sV(\rvf_t^{l})\|$, is beneficial for the node classification task. In particular, it means that they become more linearly separable. 
\vspace{-0.2cm}
% \subsubsection{Implications from Theoretical Results} 
% \label{sec:summary-theory}
% \vspace{-0.2cm}
% Three conjectures follow from Thm.~\ref{theorem: initial_stage} and~\ref{theorem: developing stage}:
% %\vspace{-0.3cm}
% %\begin{enumerate}
% % \vspace{-0.1cm}  
% \textbf{(1)} After message propagation, the mean vectors $\E(\rvf^1_i)$ will be dispersed. For a high-homophily graph, in the initial stage, the features of \textit{low}-degree nodes (where $\ratioi \ll \frac{1}{(1+\pi)h_i-\pi}$) will first move towards the opposing class mean and have relatively lower accuracy (case 2). Later, when propagating to more layers, if the accuracy of low-degree nodes drops to a level such that the $\hat{h_i^l}$ of higher degree nodes satisfies $\heterophilyil \leq \frac{\pi}{1+\pi}$, then their features begin to move towards the opposing class mean vector (case 1) because $((1+\pi)\heterophilyil-\pi) \leq 0$ in Eq.~(\ref{eq: developing stage}).
%     % Later, when propagating to more layers, the accuracy of low degree nodes drop to a level such that the effective homophily  of higher degree nodes satisfies: $\heterophilyil \leq 0.5$, then the \textit{larger} degree $d_i$ compared to $M_i$, the larger $\frac{d_i\cdot \gamma^l_j}{M_i \cdot (d_i+1)^{\frac{1}{2}}}$ is and the smaller $\|\E(\rvf_i^{l+1})\|$ is (Equation~\ref{eq: developing stage}). We will show this phenomenon in the experiments.
    
% \textbf{(2)} GCNs perform differently on graphs with different degree distributions. For homophily graphs with power-law distribution (with many low-degree nodes), the performance of low-degree nodes will degenerate fast in the initial stage and the model will quickly enter the developing stage. Then, due to few high-degree nodes, the performance will degenerate more slowly. % will be slowed down.

% \textbf{(3)} The normalization scheme of the adjacency matrix of a graph makes a difference. 
% The reason that node degrees appear in Eqs.~(\ref{eq:initial_stage})-(\ref{eq: developing stage}) is the renormalization trick on $\rmA$ in GCN (\S~\ref{section: background}). Another normalization scheme such as row-normalization makes the scenario equivalent to a $d$-regular graph where nodes have the same degree (App.~\ref{app:proof1}). 

% scheme for the graphs also makes a difference. The reason that node degrees are involved in Equations~(\ref{eq:initial_stage})-(\ref{eq: developing stage}) is due to the renormalization scheme (Section~\ref{section: background}). If another normalization scheme is used, e.g. row-normalization, then the scenario is equivalent to a d-regular graph where nodes have the same degree (Appendix~\ref{app:proof1}). 
% \end{enumerate}
% \vspace{-0.3cm}
% Based on the analysis above, we can explain the GCN behavior in various settings: when a shallow GCN model is trained with a high-homophily graph, the increased mean distances between the large-degree nodes of different classes and the reduction in the variance lead to performance gain; when the model becomes deeper or is trained with a low-homophily graph, the reduction in the mean distances between the low-degree nodes becomes dominant and leads to degenerated performances.

% \vspace{-0.3cm}
\subsection{Signed Messages for Heterophily \& Oversmoothing}
\label{subsec: sign_theory}
\vspace{-0.1cm}
Attention-based GCN models~\citep{velivckovic2017graph} typically use \textit{non-negative} attention weights to discount the contribution from dissimilar neighbors. {Though some concurrent works~\citep{chien2021adaptive, bo2021beyond} use negative attention weights, they do not to provide theoretical justifications. We provide the following theorem to show that} 
 signed messages are crucial for enhancing performance in heterophily graphs and  alleviating \yy{oversmoothing.}
%  the oversmoothing problem. 
Due to limited space,
% space limitations, 
we only show the effect of signed messages in the initial stage; similar results can be derived in the developing stage. % can be derived similarly.

\textbf{Setup.} %Consider the following scenario: 
% Consider the scenario where 
\yy{Ideally, we want} the ``messages'' sent by neighbors of a different class \yy{are negated (opposites)}, 
%multiplied by a negative sign 
and those by neighbors of the same class \yy{are} sent as-is. \yy{In reality, ground-truth labels are not accessible for every node, so we use approximations and produce errors.}
% ``messages'' as they are. 
For node $v_i$, we define $m_i^l$ as the \textit{ratio of neighbors that send incorrect ``messages''} at the $l$-th layer (i.e., different-class neighbors that send non-negated messages %without being multiplied by a negative sign 
and same-class neighbors that send negated messages). %multiplied by a negative sign). 
We also define the $l$-th layer \textit{error rate} as $e_i^l=\E(m_i^l)$, where the expectation is over the randomness of the neighbors that send incorrect messages. %We assume the expectation is the same for all the nodes.
We make two  assumptions:
% \vspace{-0.2cm}
% \begin{enumerate}
    % \item 
    (1)~Conditioned on $m_i^l$, whether the neighbor $v_j$ will wrongly send the information is independent of its class $\chi(v_j)$; 
    % \item 
    (2)~The variable $m_i^l$ is independent of the classes that nodes $v_j\in\gN_i$ belong to. 
% \end{enumerate}
\begin{theorem}
With the independence assumptions and \yy{under "non-swapping condition",} by allowing the messages to be optionally multiplied by a negative sign, in the initial stage, the mean distance between the nodes in different classes will {\textbf{be less affected} by the initial homophily level $h_i$, and will be dependent on the \textbf{error rate} $e_i^l$}. Specifically, the multiplicative factor $\gamma_i^1$ at the first layer is \yy{(suppose $v_i$ is from target class)}:
\vspace{-0.1cm}
\begin{equation}
% \E(\rvf^1_i) = (\frac{1}{(d_i+1)} + (1-2e_i^0) \frac{d_i}{M_i\cdot (d_i+1)^{\frac{1}{2}}})\E(\rvf^0_i)
\E(\rvf^1_i) = \left ( \frac{(1 - 2e_i^0)(\pi+(1-\pi)h_i)d_i\ratioi + 1}{d_i+1}\right )\E(\rvf^0_i) \\
\equiv \gamma_i^1 \E(\rvf^0_i),
\label{eq:signed_messages}
\vspace{-0.2cm}
\end{equation}
\begin{equation}
\vspace{-0.1cm}
\text{where } \gamma_i^1 \in 
\begin{cases}
  (-\infty, \frac{1}{2}], & \text{if}\ e_i^0 \geq 0.5 \\
  \yy{(\frac{1}{d_i+1}, 1]}, & \text{if}\ e_i^0 < 0.5 \ \mathrm{\&}\  \ratioi \leq \frac{1}{(1 - 2e_i^0)(\pi+(1-\pi)h_i)}\\
  (1, \infty), & \mathrm{otherwise}.
% \begin{cases}
%   \gamma_i^1 \leq \frac{1}{2}, & \text{if}\ e_i^0 \geq 0.5 \\
%   \frac{1}{2} < \gamma_i^1 \leq 1, & \text{if}\ e_i^0 < 0.5 \ \mathrm{and}\  \ratioi \leq \frac{1}{1 - 2e_i^0}\\
%   \gamma_i^1 > 1, & \mathrm{otherwise}
%   ||\E(\rvf^1_i)|| \leq \frac{||\E(\rvf^0_i)||}{2}, & \text{if}\ e_i^0\geq0.5 \\
%   ||\E(\rvf^1_i)|| \leq ||\E(\rvf^0_i)||, & \text{if}\ (e_i^0<0.5)\\ & \& \ (d_i \leq (\frac{M_i}{1-2e_i^0})^2-1)\\
%   ||\E(\rvf^1_i)|| > ||\E(\rvf^0_i)||, & \text{otherwise}
\end{cases}
\label{eq: signed_message_initial_stage}
\end{equation}
\label{theorem: signed_messages}
\end{theorem}
\vspace{-0.8cm}
\begin{proof}
The proof is provided in App.~\ref{app:proof3}. The nodes from the 'rest' class can be derived similarly.
\end{proof}

\vspace{-0.3cm}
{Given $h_i \leq 1$, we have $\frac{1}{(1+\pi)h_i-\pi} \geq \frac{1}{\pi+(1-\pi)h_i}$. From Eq.~\ref{eq: signed_message_initial_stage}, we see that when using signed messages, to benefit from ($\gamma_i^1>1$), $\ratioi \leq \frac{1}{(1 - 2e_i^0)(\pi+(1-\pi)h_i)}$. If the error rate is low ($e_i^0 \ll 0.5$), $\frac{1}{(1 - 2e_i^0)(\pi+(1-\pi)h_i)} \leq \frac{1}{(1+\pi)h_i-\pi}$, which implies that more nodes can benefit from signed messages.}
% From Eq.~(\ref{eq:signed_messages}), we conclude that:
% % \vspace{-0.3cm}
% % \begin{enumerate}
%     % \item
%     \textbf{(1)} Allowing neighbors of a different class to negate their messages prevents low homophily from degenerating performance.
%     % If we allow the neighbors of a different class to send information but be multiplied with a negative sign, then low homophily will not degenerate the performance. 
%     For a model that achieves low error rate at shallow layers (i.e, $e_i^0 \ll 0.5$), the low-degree nodes ($\ratioi \ll \frac{1}{1 - 2e_i^0}$) trigger oversmoothing. 
%     % \item
%     \textbf{(2)}~If a model does not work well under heterophily (i.e., high error rate $e_i^l$ in identifying neighbors from other classes), 
%     % in the heterophily setting, i.e., they have a higher error rate $e_i^l$ in identifying neighbors from another class, the model will be 
%     it is prone to oversmoothing even  in shallow layers. 
% \end{enumerate}


% \subsection{Additional Considerations \reminder{appendix?}} 
% % \vspace{-0.3cm}
% % \begin{enumerate}

% \textbf{On Batch norm vs.\ Layer norm.} % Whether it is beneficial to use batch norm or whether the trained weights can compensate for the shrinking distances. 
% Batch norm and trained weights cannot compensate for the dispersion of the mean vectors due to different degrees and homophily levels of the nodes. Though to some extent, it reduces the speed of the feature vectors of the susceptible nodes moving towards the other class (good for oversmoothing), it also prevents the feature vectors of the nodes who were supposed to gain from the propagation from increasing the distances (drop in accuracy). We find in our experiments (\S~\ref{section: experiments}) that, in general, adding batch norm significantly decreases the accuracy in heterophily datasets, but helps alleviate oversmoothing. Layer norm is a better option~\citep{zhou2020understanding} for oversmoothing and leads to smaller accuracy drop compared to batch norm in most datasets. However, in our experiments, layer norm has a significant accuracy drop for some datsets when some features are more important than the others.

% suggestion from Google reviewer
% \textbf{Generalization.} So far we have shown theoretical results on a binary classification task. However, this approach is general and can be applied to multi-class classification as well. In the next section we show the experiments on standard multi-class classification datasets.

% \textbf{Variance reduction.} In the analysis, we show that the variance of \textit{each node} is reduced in the initial stage regardless of the homophily level. However, it does not mean that the variance of the nodes in the same \textit{class} is reduced. The variance of the class is decided not only by the variance of each node but also how dispersed their mean is. \reminder{mention at the end of 3.1.1?}
% \end{enumerate}
